Higher category models of the pi-calculus

We present an approach to modeling computational calculi using higher category theory. Specifically we present a fully abstract semantics for the pi-calculus. The interpretation is consistent with Curry-Howard, interpreting terms as typed morphisms, while simultaneously providing an explicit interpretation of the rewrite rules of standard operational presentations as 2-morphisms. One of the key contributions, inspired by catalysis in chemical reactions, is a method of restricting the application of 2-morphisms interpreting rewrites to specific contexts.

==> pst-3d.tex <==
%% $Id: pst-3d.tex 290 2010-02-13 15:24:44Z herbert $
%% This is file `pst-3d.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-3d.tex'
%%
%% Timothy Van Zandt <tvz@nwu.edu> (tvz)
%% Herbert Voss <hvoss _at_ tug.org> (hv)
%% 
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-3d' is a PSTricks package for tilting and other pseudo-3D tricks
%%
%
\csname PSTthreeDLoaded\endcsname
\let\PSTthreeDLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey    \fi % (hv 2005-09-03)
%
\def\fileversion{1.11}
\def\filedate{2010/02/14}
\message{`PST-3d' v\fileversion, \filedate\space (tvz)}
%
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
\pst@addfams{pst-3d}

%% prologue for postcript
%
\pstheader{pst-3d.pro}%
%
\def\tx@SetMatrixThreeD{ tx@3Ddict begin SetMatrixThreeD end }
\def\tx@ProjThreeD{ tx@3Ddict begin ProjThreeD end }
\def\tx@SetMatrixEmbed{ tx@3Ddict begin SetMatrixEmbed end }
\def\tx@TMSave{ tx@3Ddict begin TMSave end }
\def\tx@TMRestore{ tx@3Ddict begin TMRestore end }
\def\tx@TMChange{ tx@3Ddict begin TMChange end }
%
\let\pssetzlength\pssetylength
\define@key[psset]{pst-3d}{viewpoint}[1 -1 1]{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@viewpoint\pst@tempg}
\def\psset@@viewpoint#1 #2 #3 #4\@nil{%
  \begingroup
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetzlength\pst@dimc{#3}%
    \xdef\pst@tempg{%
      \pst@number\pst@dima \pst@number\pst@dimb \pst@number\pst@dimc}%
  \endgroup}
\psset[pst-3d]{viewpoint=1 -1 1}
\define@key[psset]{pst-3d}{viewangle}[0]{\pst@getangle{#1}\psk@viewangle}
\psset[pst-3d]{viewangle=0}
\define@key[psset]{pst-3d}{normal}[0 0 1]{%
  \pst@expandafter\psset@@viewpoint#1 {} {} {} \@nil
  \let\psk@normal\pst@tempg}
\psset[pst-3d]{normal=0 0 1}
\define@key[psset]{pst-3d}{embedangle}[0]{\pst@getangle{#1}\psk@embedangle}
\psset[pst-3d]{embedangle=0}
\define@key[psset]{pst-3d}{Tshadowsize}[1]{\pst@checknum{#1}\psTshadowsize}
\psset[pst-3d]{Tshadowsize=1}
\define@key[psset]{pst-3d}{Tshadowangle}[60]{\pst@getangle{#1}\psk@Tshadowangle}
\psset[pst-3d]{Tshadowangle=60}
\define@key[psset]{pst-3d}{Tshadowcolor}[lightgray]{\pst@getcolor{#1}\psTshadowcolor}
\psset[pst-3d]{Tshadowcolor=lightgray}
%
\def\ThreeDput{\pst@object{ThreeDput}}
\def\ThreeDput@i{\@ifnextchar({\ThreeDput@ii}{\ThreeDput@ii(\z@,\z@,\z@)}}
\def\ThreeDput@ii(#1,#2,#3){%
  \pst@killglue\pst@makebox{\ThreeDput@iii(#1,#2,#3)}}
\def\ThreeDput@iii(#1,#2,#3){%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi
  \pst@makesmall\pst@hbox
  \pssetxlength\pst@dima{#1}%
  \pssetylength\pst@dimb{#2}%
  \pssetzlength\pst@dimc{#3}%
  \leavevmode
  \hbox{%
    \pst@Verb{%
        { \pst@number\pst@dima
          \pst@number\pst@dimb
          \pst@number\pst@dimc
          \psk@normal
          \psk@embedangle
          \psk@viewpoint
          \psk@viewangle
          \tx@SetMatrixEmbed
        } \tx@TMChange}%
    \box\pst@hbox
    \pst@Verb{\tx@TMRestore}}%
  \endgroup
  \ignorespaces}
%
\def\pst@sinandcos#1{%
  \begingroup
    \pst@dima=#1\relax
    \pst@dima=.366022\pst@dima     %Now 1pt=1/32rad
    \pst@dimb=\pst@dima   % dimb->32sin(angle) in pts
    \pst@dimc=32\p@       % dimc->32cos(angle) in pts
    \pst@dimtonum\pst@dima\pst@tempa
    \pst@cntb=\tw@
    \pst@cntc=-\@ne
    \pst@cntg=32
    \loop
    \ifnum\pst@dima>\@cclvi % 256
      \pst@dima=\pst@tempa\pst@dima
      \divide\pst@dima\pst@cntg
      \divide\pst@dima\pst@cntb
      \ifodd\pst@cntb
        \advance\pst@dimb \pst@cntc\pst@dima
        \pst@cntc=-\pst@cntc
      \else
        \advance\pst@dimc by \pst@cntc\pst@dima
      \fi
      \advance\pst@cntb\@ne
    \repeat
    \divide\pst@dimb\pst@cntg
    \divide\pst@dimc\pst@cntg
    \global\pst@dimg\pst@dimb
    \global\pst@dimh\pst@dimc
  \endgroup}
%
\def\pst@getsinandcos#1{%
  \pst@dimg=100000sp
  \pst@dimg=#1\pst@dimg
  \pst@dimh=36000000sp
  \pst@cntg=0
  \loop
  \ifnum\pst@dimg<\z@
    \advance\pst@dimg\pst@dimh
  \repeat
  \loop
  \ifnum\pst@dimg>\pst@dimh
    \advance\pst@dimg-\pst@dimh
  \repeat
  \pst@dimh=9000000sp
  \def\pst@tempg{%
    \ifnum\pst@dimg<\pst@dimh\else
      \advance\pst@dimg-\pst@dimh
      \advance\pst@cntg\@ne
      \ifnum\pst@cntg>\thr@@ \advance\pst@cntg-4 \fi
      \expandafter\pst@tempg
    \fi}%
  \pst@tempg
  \chardef\pst@quadrant\pst@cntg
  \ifdim\pst@dimg=\z@
    \def\pst@sin{0}%
    \def\pst@cos{1}%
  \else
    \pst@sinandcos\pst@dimg
    \pst@dimtonum\pst@dimg\pst@sin
    \pst@dimtonum\pst@dimh\pst@cos
  \fi%
}
%
\def\pstilt#1{\pst@makebox{\pstilt@{#1}}}
\def\pstilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifcase\pst@quadrant
        \kern\pst@cos\dp\pst@hbox
        \pst@dima=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\ht\pst@hbox
        \dp\pst@hbox=\pst@sin\dp\pst@hbox
      \or
        \kern\pst@sin\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \ht\pst@hbox=\pst@cos\ht\pst@hbox
        \dp\pst@hbox=\pst@cos\dp\pst@hbox
      \or
        \kern\pst@cos\ht\pst@hbox
        \pst@dima=\pst@sin\dp\pst@hbox
        \pst@dimg=\pst@sin\ht\pst@hbox
        \ht\pst@hbox=\pst@sin\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \or
        \kern\pst@sin\dp\pst@hbox
        \pst@dima=\pst@sin\ht\pst@hbox
        \pst@dimg=\pst@cos\ht\pst@hbox
        \ht\pst@hbox=\pst@cos\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \ifnum\pst@quadrant>\@ne neg \fi
            \pst@sin\space
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifodd\pst@quadrant exch \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
%
\def\psTilt#1{\pst@makebox{\psTilt@{#1}}}
\def\psTilt@#1{%
  \begingroup
    \leavevmode
    \pst@getsinandcos{#1}%
    \hbox{%
      \ifodd\pst@quadrant
        \pst@@divide{\dp\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\thr@@\kern\else\pst@dima=\fi\pst@sin\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@cos\p@}%
        \ifnum\pst@quadrant=\@ne\kern\else\pst@dima=\fi\pst@sin\pst@dimg
      \else
        \ifdim\pst@sin\p@=\z@
          \@pstrickserr{\string\psTilt\space angle cannot be 0 or 180}\@ehpa
          \def\pst@sin{.7071}%
          \def\pst@cos{.7071}%
        \fi
        \pst@@divide{\dp\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\z@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
        \pst@@divide{\ht\pst@hbox}{\pst@sin\p@}%
        \ifnum\pst@quadrant=\tw@\kern\else\pst@dima=\fi\pst@cos\pst@dimg
      \fi
      \ifnum\pst@quadrant>\@ne
        \pst@dimg=\ht\pst@hbox
        \ht\pst@hbox=\dp\pst@hbox
        \dp\pst@hbox=\pst@dimg
      \fi
      \pst@Verb{%
        { [ 1 0
            \pst@cos\space \pst@sin\space
            \ifodd\pst@quadrant exch \fi
            \tx@Div
            \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
            \ifnum\pst@quadrant>\@ne -1 \else 1 \fi
            0 0
          ] concat
        } \tx@TMChange}%
      \box\pst@hbox
      \pst@Verb{\tx@TMRestore}%
      \kern\pst@dima}%
  \endgroup}
%
\def\psshadow{\pst@object{psshadow}}
\def\psshadow@i{\pst@makebox{\psshadow@ii}}
\def\psshadow@ii{%
  \begingroup
    \use@par
    \leavevmode
    \pst@getsinandcos{\psk@Tshadowangle}%
    \hbox{%
      \lower\dp\pst@hbox\hbox{%
        \pst@Verb{%
          { [ 1 0
              \pst@cos\space \psTshadowsize mul
              \ifnum\pst@quadrant>\@ne neg \fi
              \pst@sin\space \psTshadowsize mul
              \ifnum\pst@quadrant>\z@\ifnum\pst@quadrant<\thr@@ neg \fi\fi
              \ifodd\pst@quadrant exch \fi
              0 0
            ] concat
          } \tx@TMChange}}%
      \hbox to\z@{%   patch 2 (hv), to get it run with xcolor _and_ TeX
       \pst@Verb{ gsave \pst@usecolor\psTshadowcolor}%
       \copy\pst@hbox
       \pst@Verb{ grestore}\hss}%
      \pst@Verb{\tx@TMRestore}%
      \box\pst@hbox}%
  \endgroup}
%
\def\psAffinTransform{\pst@object{psAffinTransform}}
\def\psAffinTransform@i#1{%
  \begin@SpecialObj%
  \pst@makebox{\psAffinTransform@ii{#1}}}%
\def\psAffinTransform@ii#1{%
  \pst@Verb{ { [#1] concat } \tx@TMChange }%
  \box\pst@hbox \pst@Verb{ \tx@TMRestore }%
  \end@SpecialObj}
%
\catcode`\@=\PstAtCode\relax
\endinput
%%
%% End of file `pst-3d.tex'.


==> pst-fill.tex <==
%%
%% This is file `pst-fill.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% pst-fill.dtx  (with options: `pst-fill')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pst-fill.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file pst-fill.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%% Package `pst-fill.dtx'
%%
%% Denis Girou (CNRS/IDRIS - France) <Denis.Girou@idris.fr>
%% Herbert Voss <voss@pstricks.de>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-fill' is a PSTricks package for filling and tiling areas
%%
%%     \pscircle[linestyle=none,fillstyle=solid,fillcolor=yellow,fillsep=0.5,
%%               addfillstyle=boxfill](2,2){2}
\def\fileversion{1.01}
\def\filedate{2007/03/10}
\message{`PST-Fill' v\fileversion, \filedate\space (tvz,dg,hv)}
\csname PSTboxfillLoaded\endcsname
\let\PSTboxfillLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey\fi
\edef\PstAtCode{\the\catcode`\@}\catcode`\@=11\relax

\pst@addfams{pst-fill}
\def\pst@@boxfillsize#1(#2,#3)#4(#5,#6)#7(#8\@nil{%
  \begingroup
    \ifx\@empty#7\relax
      \pst@dima\z@
      \pst@dimb\z@
      \pssetxlength\pst@dimc{#2}%
      \pssetylength\pst@dimd{#3}%
    \else
      \pssetxlength\pst@dima{#2}%
      \pssetylength\pst@dimb{#3}%
      \pssetxlength\pst@dimc{#5}%
      \pssetylength\pst@dimd{#6}%
    \fi
    \xdef\pst@tempg{%
      \pst@dima=\number\pst@dima sp
      \pst@dimb=\number\pst@dimb sp
      \pst@dimc=\number\pst@dimc sp
      \pst@dimd=\number\pst@dimd sp }%
  \endgroup
  \let\psk@boxfillsize\pst@tempg}

\define@key[psset]{pst-fill}{boxfillsize}{%
  \def\pst@tempg{#1}\def\pst@temph{auto}%
  \ifx\pst@tempg\pst@temph
    \let\psk@boxfillsize\relax
  \else
    \pst@@boxfillsize#1(\z@,\z@)\@empty(\z@,\z@)(\@nil
  \fi}
\psset{boxfillsize={(-15cm,-15cm)(15cm,15cm)}}
\define@key[psset]{pst-fill}{boxfillcolor}{\pst@getcolor{#1}\psboxfillcolor}
\psset{boxfillcolor=black}% hv
\define@key[psset]{pst-fill}{boxfillangle}{\pst@getangle{#1}\psk@boxfillangle}
\psset{boxfillangle=0}
\define@key[psset]{pst-fill}{fillsepx}{%
  \pst@getlength{#1}\psk@fillsepx}
\define@key[psset]{pst-fill}{fillsepy}{%
  \pst@getlength{#1}\psk@fillsepy}
\define@key[psset]{pst-fill}{fillsep}{%
  \pst@getlength{#1}\psk@fillsepx%
  \let\psk@fillsepy\psk@fillsepx}
\psset{fillsep=2pt}

\ifx\PstTiling\@undefined
  \define@key[psset]{pst-fill}{fillcycle}{\pst@getint{#1}\psk@fillcycle}
  \psset{fillcycle=0}
\else
  \define@key[psset]{pst-fill}{fillangle}{\pst@getangle{#1}\psk@boxfillangle}
  \define@key[psset]{pst-fill}{fillsize}{%
      \def\pst@tempg{#1}\def\pst@temph{auto}%
      \ifx\pst@tempg\pst@temph\let\psk@boxfillsize\relax
      \else\pst@@boxfillsize#1(\z@,\z@)\@empty(\z@,\z@)(\@nil\fi}
  \psset{fillsep=0,fillsize=auto}
  \define@key[psset]{pst-fill}{fillcyclex}{\pst@getint{#1}\psk@fillcyclex}
  \define@key[psset]{pst-fill}{fillcycley}{\pst@getint{#1}\psk@fillcycley}
  \define@key[psset]{pst-fill}{fillcycle}{%
    \pst@getint{#1}\psk@fillcyclex\let\psk@fillcycley\psk@fillcyclex}
  \psset{fillcycle=0}
  \define@key[psset]{pst-fill}{fillmovex}{\pst@getlength{#1}\psk@fillmovex}
  \define@key[psset]{pst-fill}{fillmovey}{\pst@getlength{#1}\psk@fillmovey}
  \define@key[psset]{pst-fill}{fillmove}{%
      \pst@getlength{#1}\psk@fillmovex\let\psk@fillmovey\psk@fillmovex}
  \psset{fillmove=0pt}
  \define@key[psset]{pst-fill}{fillloopaddx}{\pst@getint{#1}\psk@fillloopaddx}
  \define@key[psset]{pst-fill}{fillloopaddy}{\pst@getint{#1}\psk@fillloopaddy}
  \define@key[psset]{pst-fill}{fillloopadd}{%
    \pst@getint{#1}\psk@fillloopaddx\let\psk@fillloopaddy\psk@fillloopaddx}
  \psset{fillloopadd=0}
%%    \define@key[psset]{pst-fill}{PstDebug}{\pst@getint{#1}\psk@PstDebug}
    \psset{PstDebug=0}
\fi

\newbox\pst@fillbox
\def\psboxfill{\pst@killglue\pst@makebox\psboxfill@i}
\def\psboxfill@i{\setbox\pst@fillbox\box\pst@hbox\ignorespaces}
\def\psfs@boxfill{%
  \ifvoid\pst@fillbox
    \@pstrickserr{Fill box is empty. Use \string\psboxfill\space first.}\@ehpa
  \else
    \ifx\psk@boxfillsize\relax \pst@AutoBoxFill
    \else\pst@ManualBoxFill\fi
  \fi}
\def\pst@ManualBoxFill{%
  \leavevmode
  \begingroup
    \pst@FlushCode
    \begin@psclip
    \pstVerb{clip}%
    \expandafter\pst@AddFillBox\psk@boxfillsize
    \end@psclip
  \endgroup}
\def\pst@FlushCode{%
  \pst@Verb{%
    /mtrxc CM def
    CP CP T
    \tx@STV
    \psk@origin
    \psk@swapaxes
    \pst@newpath
    \pst@code
    mtrxc setmatrix
    moveto
    0 setgray}%
  \gdef\pst@code{}}
\def\pst@AddFillBox#1 #2 #3 #4 {%
  \begingroup
    \setbox\pst@fillbox=\vbox{%
      \hbox{\unhcopy\pst@fillbox\kern\psk@fillsepx\p@}%
      \vskip\psk@fillsepy\p@}%
    \psk@boxfillsize
    \pst@cnta=\pst@dimc
    \advance\pst@cnta-\pst@dima
    \divide\pst@cnta\wd\pst@fillbox
    \pst@cntb=\pst@dimd
    \advance\pst@cntb-\pst@dimb
    \pst@dimd=\ht\pst@fillbox
    \divide\pst@cntb\pst@dimd
    \def\pst@tempa{%
      \pst@tempg
      \copy\pst@fillbox
      \advance\pst@cntc\@ne
      \ifnum\pst@cntc<\pst@cntd\expandafter\pst@tempa\fi}%
    \let\pst@tempg\relax
    \pst@cntc-\tw@
    \pst@cntd\pst@cnta
    \setbox\pst@fillbox=\hbox to \z@{%
      \kern\pst@dima
      \kern-\wd\pst@fillbox
      \pst@tempa
      \hss}%
    \pst@cntd\pst@cntb
%% DG modification begin - Dec. 11, 1997 - Patch 2
    \ifx\PstTiling\@undefined
      \ifnum\psk@fillcycle=\z@\pst@ManualFillCycle\fi
    \else
      \ifnum\psk@fillcyclex=\z@\pst@ManualFillCycle\fi
    \fi
%% DG modification end
    \global\setbox\pst@boxg=\vbox to\z@{%
      \offinterlineskip
      \vss
      \pst@tempa
      \vskip\pst@dimb}%
  \endgroup
  \setbox\pst@fillbox\box\pst@boxg
  \pst@rotate\psk@boxfillangle\pst@fillbox
  \box\pst@fillbox}
\def\pst@ManualFillCycle{%
  \ifx\PstTiling\@undefined
    \pst@cntg=\psk@fillcycle
  \else
    \pst@cntg=\psk@fillcyclex
  \fi
  \pst@dimg=\wd\pst@fillbox
  \ifnum\pst@cntg=\z@
  \else
  \divide\pst@dimg\pst@cntg
  \fi
  \ifnum\pst@cntg<\z@\pst@cntg=-\pst@cntg\fi
  \advance\pst@cntg\m@ne
  \pst@cnth=\pst@cntg
  \def\pst@tempg{%
    \ifnum\pst@cnth<\pst@cntg\advance\pst@cnth\@ne\else\pst@cnth\z@\fi
    \moveright\pst@cnth\pst@dimg}}
%% Auto box fill:        !! Fix dictionary
%% DG addition begin - Apr. 8, 1997 and Dec. 1997 - Patch 2
\ifx\PstTiling\@undefined
\pst@def{AutoFillCycle}<%
  /c ED
  /n 0 def
  /s {
    /x x w c div n mul add def
    /n n c abs 1 sub lt { n 1 add } { 0 } ifelse def
  } def>

\pst@def{BoxFill}<%
  gsave
    gsave \tx@STV CM grestore dtransform CM idtransform
    abs /h ED abs /w ED
    pathbbox
    h div round 2 add cvi /y2 ED
    w div round 2 add cvi /x2 ED
    h div round 2 sub cvi /y1 ED
    w div round 2 sub cvi /x1 ED
    /y2 y2 y1 sub def
    /x2 x2 x1 sub def
    CP
    y1 h mul sub neg /y1 ED
    x1 w mul sub neg /x1 ED
    clip
    y2 {
      /x x1 def
      s
      x2 {
        save CP x y1
%% patch 4   hv --------------
        \ifx\VTeXversion\undefined
        \else
%%============ mv: 09-10-01 ??? this is likely to be a right change
        neg
%%============
        \fi
%% end patch 4
T moveto Box restore
        /x x w add def
      } repeat
      /y1 y1 h add def
    } repeat
    % Next line not useful... To see that, suppress clipping (DG)
    CP x y1 T moveto Box
  currentpoint currentfont grestore setfont moveto>
\else
%% DG modification begin - Apr. 8, 1997 and Nov. / Dec. 1997 - Patch 2
\pst@def{AutoFillCycleX}<%
  /cX ED
  /nX 0 def
  /CycleX {
    /x x w cX div nX mul add def
    /nX nX cX abs 1 sub lt { nX 1 add } { 0 } ifelse def
  } def>
\pst@def{AutoFillCycleY}<%
  /cY ED
  /mY 0 def
  /nY 0 def
  /CycleY {
    /y1 y1 h cY div mY mul sub def
    nY cY abs 1 sub lt { /nY nY 1 add def /mY 1 def }
                       { /nY 0 def        /mY cY abs 1 sub neg def } ifelse
  } def>

\pst@def{BoxFill}<%
  gsave
    gsave \tx@STV CM grestore dtransform CM idtransform
    abs /h ED abs /w ED
    pathbbox
    h div round 2 add cvi /y2 ED
    w div round 2 add cvi /x2 ED
    h div round 2 sub cvi /y1 ED
    w div round 2 sub cvi /x1 ED
    /CoefLoopX 0 def
    /CoefLoopY 0 def
    /CoefMoveX 0 def
    /CoefMoveY 0 def
    \psk@boxfillangle\space 0 ne {/CoefLoopX 8 def /CoefLoopY 8 def} if
    \psk@fillcyclex\space 0 ne {/CoefLoopX CoefLoopX 1 add def} if
    \psk@fillcycley\space 0 ne {/CoefLoopY CoefLoopY 1 add def} if
    \psk@fillmovex\space 0 ne
      {/CoefLoopX CoefLoopX 2 add def
       \psk@fillmovex\space 0 gt {/CoefMoveX CoefLoopX def}
                           {/CoefMoveX CoefLoopX neg def} ifelse} if
    \psk@fillmovey\space 0 ne
      {/CoefLoopY CoefLoopY 2 add def
       \psk@fillmovey\space 0 gt {/CoefMoveY CoefLoopY def}
                           {/CoefMoveY CoefLoopY neg def} ifelse} if
    \psk@fillsepx\space 0 ne {/CoefLoopX CoefLoopX 1 add def} if
    \psk@fillsepy\space 0 ne {/CoefLoopY CoefLoopY 1 add def} if
    /CoefLoopX CoefLoopX \psk@fillloopaddx\space add def
    /CoefLoopY CoefLoopY \psk@fillloopaddy\space add def
    /x2 x2 x1 sub 4 sub CoefLoopX 2 mul add def
    /y2 y2 y1 sub 4 sub CoefLoopY 2 mul add def
%% We must fix the origin of tiling, as it must not vary according other stuff
%% in the page!
    w x1 CoefLoopX add CoefMoveX add mul
      h y1 y2 add 1 sub CoefLoopY sub CoefMoveY sub mul moveto
    CP
    y1 h mul sub neg /y1 ED
    x1 w mul sub neg /x1 ED
%%  hv 2004-06-22   to prevent clash with pst-gr3d
%%    \psk@PstDebug 0 eq {clip} if
    \Pst@Debug 0 eq {clip} if
%% end hv
    \psk@fillmovex\space \psk@fillmovey
    gsave \tx@STV CM grestore dtransform CM idtransform
    /hmove ED /wmove ED
    /row 0 def
   y2 {
       /row row 1 add def
       /column 0 def
       /x x1 def
       CycleX
       save
       x2 {
          /column column 1 add def
          CycleY
          save CP x y1
%% patch 4   hv --------------
          \ifx\VTeXversion\undefined
          \else
%%============ mv: 09-10-01 ??? this is likely to be a right change
          neg
%%============
          \fi
  T moveto Box restore
          /x x w add def
          0 hmove translate
          } repeat
       restore
       /y1 y1 h add def
       wmove 0 translate
       } repeat
  currentpoint currentfont grestore setfont moveto>
\fi

\def\pst@AutoBoxFill{%
  \leavevmode
  \begingroup
    \pst@stroke
    \pst@FlushCode
    \pst@Verb{\psk@boxfillangle\space \tx@RotBegin}%
    \pstVerb{\pst@dict /Box \pslbrace end}%
    \ifx\PstTiling\@undefined
    \else
      \ifx\pst@tempa\@undefined % Undefined for instance for \pscharpath
      \else\ifx\pst@tempa\@empty\else
        \def\pst@temph{0}%
        \ifx\pst@tempa\pst@temph
        \else
          \pstVerb{/TR {pop pop currentpoint translate \pst@tempa\space translate } def}%
        \fi
      \fi\fi
    \fi
    \hbox to \z@{\vbox to\z@{\vss\copy\pst@fillbox\vskip-\dp\pst@fillbox}\hss}%
    \ifx\PstTiling\@undefined
      \pstVerb{%
        tx@Dict begin \psrbrace def
        \ifnum\psk@fillcycle=\z@
          /s {} def
        \else
          \psk@fillcycle \tx@AutoFillCycle
        \fi
        \pst@number{\wd\pst@fillbox}%
        \psk@fillsepx\space add
        \pst@number{\ht\pst@fillbox}%
        \pst@number{\dp\pst@fillbox}%
        \psk@fillsepy\space add add
        \tx@BoxFill
        end}%
      \else
      \pstVerb{%
        tx@Dict begin \psrbrace def
        \ifnum\psk@fillcyclex=\z@
          /CycleX {} def
        \else
          \psk@fillcyclex\space \tx@AutoFillCycleX
        \fi
        \ifnum\psk@fillcycley=\z@
          /CycleY {} def
        \else
          \psk@fillcycley\space \tx@AutoFillCycleY
        \fi
        \pst@number{\wd\pst@fillbox}%
        \psk@fillsepx\space add
        \pst@number{\ht\pst@fillbox}%
        \pst@number{\dp\pst@fillbox}%
        \psk@fillsepy\space add add
        \tx@BoxFill
        end}%
    \fi
    \pst@Verb{\tx@RotEnd}%
  \endgroup}
\catcode`\@=\PstAtCode\relax
\endinput
%%
%% End of file `pst-fill.tex'.


==> pst-fp.tex <==
%% $Id: pst-fp.tex 837 2013-10-22 07:53:07Z herbert $
%%
%%
%% This is file `pst-fp.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-fp.tex'
%%
%% Herbert Voss <hvoss@tug.org>
%% stolen from the fp package by Michael Mehlich
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-fp' is a PSTricks related package for a division, 
%%    multiplication and addition
%%
\csname PSTFPloaded\endcsname
\let\PSTFPloaded\endinput
%
% Requires some packages
\ifx\PSTricksLoaded\endinput\else\input pstricks \fi
%
\def\fileversion{0.05}
\def\filedate{2010/01/17}
\message{`pst-fp' v\fileversion, \filedate\space (hv)}
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax

%fixed point arithmetic with values between (including)
%      -999999999999999999.999999999999999999
% and  +999999999999999999.999999999999999999

\def\pstFPadd#1#2#3{\pstFP@callc\pstFP@add#1{#2}{#3}+\relax} % #1 := #2+#3
\def\pstFPsub#1#2#3{\pstFP@callc\pstFP@add#1{#2}{-#3}-\relax}% #1 := #2-#3
\def\pstFPmul#1#2#3{\pstFP@callc\pstFP@mul#1{#2}{#3}}        % #1 := #2*#3
\def\pstFPdiv#1#2#3{\pstFP@callc\pstFP@div#1{#2}{#3}}        % #1 := #2/#3

\def\pst@int#1{\expandafter\pst@@int#1..\@nil}
\def\pst@@int#1.#2.\@nil{#1}
\def\pst@Int#1{%
  \@tempdima=#1\relax%
  \expandafter\pst@@Int\the\@tempdima\@nil}
\def\pst@@Int#1.#2\@nil{#1}

%
\def\pstFPMul#1#2#3{\pstFP@callc\pstFP@mul#1{#2}{#3}%        % #1 := int(#2*#3)
  \edef#1{\pst@int{#1}}}%
\def\pstFPDiv#1#2#3{\pstFP@callc\pstFP@div#1{#2}{#3}%        % #1 := int(#2/#3)
  \edef#1{\pst@int{#1}}}%
\def\pstFPstripZeros#1#2{\pst@dimm=#1pt\relax \edef#2{\strip@pt\pst@dimm}}
%
\countdef\pstFP@actcounter=10 % register 0 for counter
\ifnum\pstFP@actcounter<60\relax \pstFP@actcounter=60\fi

\newcount\pstFP@xs %sign of 1st value
\newcount\pstFP@xia%integer part of 1st value
\newcount\pstFP@xib%integer part of 1st value
\newcount\pstFP@xfa%fractional part of 1st value
\newcount\pstFP@xfb%fractional part of 1st value

\countdef\pstFP@ys=5 %sign of 2nd value
\countdef\pstFP@yia=6%integer part of 2nd value
\countdef\pstFP@yib=7%integer part of 2nd value
\countdef\pstFP@yfa=8%fractional part of 2nd value
\countdef\pstFP@yfb=9%fractional part of 2nd value

\countdef\pstFP@xk=10  %registers for splitting 1st value
\countdef\pstFP@xl=11
\countdef\pstFP@xm=12
\countdef\pstFP@xn=13
\countdef\pstFP@xo=14
\countdef\pstFP@xp=15
\countdef\pstFP@xq=16
\countdef\pstFP@xr=17
\countdef\pstFP@xz=18
\countdef\pstFP@xt=19
\countdef\pstFP@xu=20
\countdef\pstFP@xv=21

\countdef\pstFP@yk=22 %registers for splitting 2nd value
\countdef\pstFP@yl=23
\countdef\pstFP@ym=24
\countdef\pstFP@yn=25
\countdef\pstFP@yo=26
\countdef\pstFP@yp=27
\countdef\pstFP@yq=28
\countdef\pstFP@yr=29
\countdef\pstFP@yz=30
\countdef\pstFP@yt=31
\countdef\pstFP@yu=32
\countdef\pstFP@yv=33

\newcount\pstFP@rega   %auxiliary registers
\newcount\pstFP@regb
\countdef\pstFP@regc=36
\countdef\pstFP@regd=37
\countdef\pstFP@rege=38

\countdef\pstFP@rs=39 %result registers
\countdef\pstFP@ria=40
\countdef\pstFP@rib=41
\countdef\pstFP@rfa=42
\countdef\pstFP@rfb=43

\newcount\pstFP@regs    %local auxiliary registers
\countdef\pstFP@count=45
\countdef\pstFP@res=46
\countdef\pstFP@shift=47
\newcount\pstFP@times
\countdef\pstFP@prod=49

%auxiliary macros which may be used in all of the following macros
\newif\ifpstFP@test

\def\pstFP@ignorenext#1{}
\def\pstFP@first#1#2\relax{#1}
\def\pstFP@swallow#1\relax{}
%
\def\ifpstFP@zero#1{%
  \ifnum%
    \expandafter\ifnum\csname pstFP@#1ia\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1ib\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1fa\endcsname=0 0\else1\fi%
    \expandafter\ifnum\csname pstFP@#1fb\endcsname=0 0\else1\fi%
    =0\relax%
}
%
%read value
%
\def\pstFP@correctintcounter#1\relax{%
  {\edef\pstFP@tmp{#1}%
   \pstFP@count=0\relax%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa0\relax%
        \advance\pstFP@count1\relax%
        \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \ifnum\pstFP@count>18\relax \typeout{>>>> Overflow}\fi%
   \expandafter\if!\pstFP@tmp!%
     \advance\pstFP@count-18\relax%
     \pstFP@count=-\pstFP@count%
     \loop%
       \ifnum\pstFP@count>0\relax%
          \pstFP@regc=\pstFP@rega%
	  \divide\pstFP@rega10\relax\multiply\pstFP@rega10\relax%
	  \advance\pstFP@regc-\pstFP@rega\multiply\pstFP@regc100000000\relax%
	  \divide\pstFP@rega10\relax%
	  \divide\pstFP@regb10\relax\advance\pstFP@regb\pstFP@regc%
	  \advance\pstFP@count-1\relax%
       \repeat%
     \global\pstFP@rega=\pstFP@rega%
     \global\pstFP@regb=\pstFP@regb%
   \else%
     \typeout{>>>>Number too big}%
   \fi%
  }%
}
\def\pstFP@@setintcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@regb=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@correctintcounter%
}
\def\pstFP@setintcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@rega=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@@setintcounter%
}

\def\pstFP@@setfractcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@regb=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@swallow%
}
\def\pstFP@setfractcounter#1#2#3#4#5#6#7#8#9{%
  \pstFP@rega=#1#2#3#4#5#6#7#8#9\relax%
  \pstFP@@setfractcounter%
}

\def\pstFP@getsign#1\relax{%
  {\pstFP@regs=1\relax%
   \edef\pstFP@tmp{#1}%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa-\relax%
        \multiply\pstFP@regs-1\relax%
     \fi%
     \ifnum\expandafter\ifx\pstFP@tmpa-1\else0\fi\expandafter\ifx\pstFP@tmpa+1\else0\fi>0%
        \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \global\let\pstFP@tmp\pstFP@tmp%
   \global\pstFP@regs=\pstFP@regs%
  }%
}

\def\pstFP@removeleadingzeros#1\relax{%
  {\edef\pstFP@tmp{#1}%
   \loop%
     \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
     \expandafter\ifx\pstFP@tmpa0\relax%
       \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
     \repeat%
   \global\let\pstFP@tmp\pstFP@tmp%
  }%
}

\newif\ifpstFP@nonstop
\def\pstFP@strip#1{%
  {\edef\pstFP@tmp{#1}%
   \edef\pstFP@tmpb{}%
   \ifx\pstFP@tmp\@empty\else%
     \pstFP@nonstoptrue%
     \loop%
       \edef\pstFP@tmpa{\expandafter\pstFP@first\pstFP@tmp\noexpand\relax}%
       \expandafter\ifx\pstFP@tmpa-\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa+\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa0\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa1\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa2\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa3\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa4\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa5\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa6\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa7\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa8\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \expandafter\ifx\pstFP@tmpa9\relax\edef\pstFP@tmpb{\pstFP@tmpb\pstFP@tmpa}\else%
       \ifx\pstFP@tmpa\@empty\pstFP@nonstopfalse\else%
       \ifx\pstFP@tmpa\space\pstFP@nonstopfalse\else%
         \typeout{>>> Illegal character \pstFP@tmpa\space found in float number}%
       \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
       \edef\pstFP@tmp{\expandafter\pstFP@ignorenext\pstFP@tmp}%
       \ifx\pstFP@tmp\@empty\pstFP@nonstopfalse\fi%
       \ifpstFP@nonstop%
       \repeat%
   \fi%
   \global\let\pstFP@tmp\pstFP@tmpb%
  }%
}

\def\pstFP@readvalue#1#2#3{%
  % #1    macro family to catch the value
  % #2.#3 value
  %
  % regular expression [+|-]*[d]_0^18.[d]*
  %
  \pstFP@strip{#2}%
  %sign
  \expandafter\pstFP@getsign\pstFP@tmp\relax%
  \csname pstFP@#1s\endcsname=\pstFP@regs%
  %
  %integer part
  \pstFP@removeleadingzeros\pstFP@tmp\relax%
  \expandafter\pstFP@setintcounter\pstFP@tmp000000000000000000\relax%
  \csname pstFP@#1ia\endcsname=\pstFP@rega%
  \csname pstFP@#1ib\endcsname=\pstFP@regb%
  %
  %fractional part
  \pstFP@strip{#3}%
  \expandafter\pstFP@setfractcounter\pstFP@tmp000000000000000000\relax%
  \csname pstFP@#1fa\endcsname=\pstFP@rega%
  \csname pstFP@#1fb\endcsname=\pstFP@regb%
  %
  %correct sign
  \ifnum\pstFP@rega=0\relax%
    \ifnum\pstFP@regb=0\relax%
      \expandafter\ifnum\csname pstFP@#1ib\endcsname=0\relax%
        \expandafter\ifnum\csname pstFP@#1ia\endcsname=0\relax%
	  \csname pstFP@#1s\endcsname=1\relax%
	\fi%
      \fi%
    \fi%
  \fi%
}
%
%store value in macro
%
\def\pstFP@store#1#2{%
  % #1 macro
  % #2 macro family (value) to store
  %
  \ifpstFP@zero{#2}%
    \csname pstFP@#2s\endcsname=1\relax%
  \fi%
  \expandafter\ifnum\csname pstFP@#2s\endcsname<0\relax%
    \edef#1{-}%
  \else%
    \edef#1{}%
  \fi%
  \expandafter\ifnum\csname pstFP@#2ia\endcsname=0\relax%
     \expandafter\ifnum\csname pstFP@#2ib\endcsname=0\relax%
       \edef#1{#10}%
     \else%
       \edef#1{#1\expandafter\the\csname pstFP@#2ib\endcsname}%
     \fi%
  \else%
    \expandafter\advance\csname pstFP@#2ib\endcsname1000000000\relax%
    \edef#1{#1\expandafter\the\csname pstFP@#2ia\endcsname\expandafter\pstFP@ignorenext\the\csname pstFP@#2ib\endcsname}%
  \fi%
  \expandafter\advance\csname pstFP@#2fa\endcsname1000000000\relax%
  \expandafter\advance\csname pstFP@#2fb\endcsname1000000000\relax%
  \edef#1{#1\noexpand.\expandafter\pstFP@ignorenext\the\csname pstFP@#2fa\endcsname\expandafter\pstFP@ignorenext\the\csname pstFP@#2fb\endcsname}%
}
%macros to expand some arguments
%
\def\pstFP@callc#1#2#3#4{%
  % #1 macro to call
  % #2 macro, which gets the result
  % #3 1st value
  % #4 2nd value
  % expand the values and split them into the integer and the fractional parts
  \edef\next{\noexpand#1\noexpand#2#3..\noexpand\relax#4..\noexpand\relax}%
  \next%
}
%
\def\pstFP@divten#1{%
  \expandafter\pstFP@regc\csname pstFP@#1ia\endcsname%
  \expandafter\divide\csname pstFP@#1ia\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1ia\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@regc-\pstFP@regb%
  \multiply\pstFP@regc100000000\relax%
  %
  \expandafter\pstFP@rega\csname pstFP@#1ib\endcsname%
  \expandafter\divide\csname pstFP@#1ib\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1ib\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@rega-\pstFP@regb%
  \multiply\pstFP@rega100000000\relax%
  \expandafter\advance\csname pstFP@#1ib\endcsname\pstFP@regc%
  %
  \expandafter\pstFP@regc\csname pstFP@#1fa\endcsname%
  \expandafter\divide\csname pstFP@#1fa\endcsname10\relax%
  \expandafter\pstFP@regb\csname pstFP@#1fa\endcsname%
  \multiply\pstFP@regb10\relax%
  \advance\pstFP@regc-\pstFP@regb%
  \multiply\pstFP@regc100000000\relax%
  \expandafter\advance\csname pstFP@#1fa\endcsname\pstFP@rega%
  %
  \expandafter\divide\csname pstFP@#1fb\endcsname10\relax%
  \expandafter\advance\csname pstFP@#1fb\endcsname\pstFP@regc%
}
%
\def\pstFP@multen#1{%
  \expandafter\multiply\csname pstFP@#1ia\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1ib\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1ib\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ia\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ib\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1ib\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1fa\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1fa\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1ib\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fa\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1fa\endcsname10\relax%
  \expandafter\ifnum\csname pstFP@#1fb\endcsname<100000000\relax%
  \else%
    \expandafter\pstFP@regc\csname pstFP@#1fb\endcsname%
    \divide\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fa\endcsname\pstFP@regc%
    \multiply\pstFP@regc100000000%
    \expandafter\advance\csname pstFP@#1fb\endcsname-\pstFP@regc%
  \fi%
  \expandafter\multiply\csname pstFP@#1fb\endcsname10\relax%
}
%
\def\pstFP@counttimes{%
  {\global\pstFP@times=0\relax%
   \loop%
     \ifnum%
        \ifnum\pstFP@xia>\pstFP@yia1%
	\else\ifnum\pstFP@xia<\pstFP@yia0%
	\else%
	  \ifnum\pstFP@xib>\pstFP@yib1%
	  \else\ifnum\pstFP@xib<\pstFP@yib0%
	  \else%
	    \ifnum\pstFP@xfa>\pstFP@yfa1%
	    \else\ifnum\pstFP@xfa<\pstFP@yfa0%
	    \else%
	      \ifnum\pstFP@xfb>\pstFP@yfb1%
	      \else\ifnum\pstFP@xfb<\pstFP@yfb0%
	      \else%
	         1%
	      \fi\fi%
	    \fi\fi%
	  \fi\fi%
	\fi\fi%
	=1\relax%
       \global\advance\pstFP@times1\relax%
       \global\advance\pstFP@xfb-\pstFP@yfb%
       \ifnum\pstFP@xfb<0\relax%
         \global\advance\pstFP@xfb1000000000\relax%
	 \global\advance\pstFP@xfa-1\relax%
       \fi%
       \global\advance\pstFP@xfa-\pstFP@yfa%
       \ifnum\pstFP@xfa<0\relax%
         \global\advance\pstFP@xfa1000000000\relax%
	 \global\advance\pstFP@xib-1\relax%
       \fi%
       \global\advance\pstFP@xib-\pstFP@yib%
       \ifnum\pstFP@xib<0\relax%
         \global\advance\pstFP@xib1000000000\relax%
	 \global\advance\pstFP@xia-1\relax%
       \fi%
       \global\advance\pstFP@xia-\pstFP@yia%
     \repeat%
  }%
}
%
\def\pstFP@add#1#2.#3.#4\relax#5.#6.#7\relax#8\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   \ifnum\pstFP@xs=\pstFP@ys%
     \advance\pstFP@xfb\pstFP@yfb%
     \advance\pstFP@xfa\pstFP@yfa%
     \ifnum\pstFP@xfb<1000000000\relax\else%
       \advance\pstFP@xfb-1000000000\relax%
       \advance\pstFP@xfa1\relax%
     \fi%
     \advance\pstFP@xib\pstFP@yib%
     \ifnum\pstFP@xfa<1000000000\relax\else%
       \advance\pstFP@xfa-1000000000\relax%
       \advance\pstFP@xib1\relax%
     \fi%
     \advance\pstFP@xia\pstFP@yia%
     \ifnum\pstFP@xib<1000000000\relax\else%
       \advance\pstFP@xib-1000000000\relax%
       \advance\pstFP@xia1\relax%
     \fi%
     \ifnum\pstFP@xia<1000000000\relax\else%
       \pstFP@errmessage{Overflow}%
     \fi%
     \pstFP@store\pstFP@tmp{x}%
   \else%
     \advance\pstFP@xfb-\pstFP@yfb%
     \ifnum\pstFP@xfb<0\relax%
       \advance\pstFP@yfa1\relax%
       \advance\pstFP@xfb1000000000\relax%
     \fi%
     \advance\pstFP@xfa-\pstFP@yfa%
     \ifnum\pstFP@xfa<0\relax%
       \advance\pstFP@yib1\relax%
       \advance\pstFP@xfa1000000000\relax%
     \fi%
     \advance\pstFP@xib-\pstFP@yib%
     \ifnum\pstFP@xib<0\relax%
       \advance\pstFP@yia1\relax%
       \advance\pstFP@xib1000000000\relax%
     \fi%
     \advance\pstFP@xia-\pstFP@yia%
     \ifnum\pstFP@xia<0\relax%
       \pstFP@xs=-\pstFP@xs%
       \ifnum\pstFP@xfb=0\relax\else%
         \advance\pstFP@xfb-1000000000\relax\pstFP@xfb=-\pstFP@xfb%
	 \advance\pstFP@xfa1\relax%
       \fi%
       \ifnum\pstFP@xfa=0\relax\else%
         \advance\pstFP@xfa-1000000000\relax\pstFP@xfa=-\pstFP@xfa%
	 \advance\pstFP@xib1\relax%
       \fi%
       \ifnum\pstFP@xib=0\relax\else%
         \advance\pstFP@xib-1000000000\relax\pstFP@xib=-\pstFP@xib%
	 \advance\pstFP@xia1\relax%
       \fi%
       \relax\pstFP@xia=-\pstFP@xia%
     \fi%
     \pstFP@store\pstFP@tmp{x}%
   \fi%
   \global\let\pstFP@tmp\pstFP@tmp%
  }%
  \let#1\pstFP@tmp%
}


\def\pstFP@div#1#2.#3.#4\relax#5.#6.#7\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  % algorithmic idea (for x>0, y>0)
  %   - %determine \pstFP@shift  such that y*10^\pstFP@shift <100000000<=y*10^(\pstFP@shift+1)
  %   - %determine \pstFP@shift' such that x*10^\pstFP@shift'<100000000<=x*10^(\pstFP@shift+1)
  %   - x=x*\pstFP@shift'
  %   - y=y*\pstFP@shift
  %   - \pstFP@shift=\pstFP@shift-\pstFP@shift'
  %   - res=0
  %   - while y>0 %fixed-point representation!
  %   -   \pstFP@times=0
  %   -	  while x>y
  %   -     \pstFP@times=\pstFP@times+1
  %   -     x=x-y
  %   -   end
  %   -   y=y/10
  %   -   res=10*res+\pstFP@times/1000000000
  %   - end
  %   - %shift the result according to \pstFP@shift
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   %sign
   \multiply\pstFP@xs\pstFP@ys%
   \pstFP@rs=\pstFP@xs%
   %
   %compute division
   \ifpstFP@zero{y}%
     \typeout{>>>>Division by zero}%
   \else%
     \ifpstFP@zero{x}\def\next##1{\edef\pstFP@tmp{0}}\else\def\next##1{##1}\fi%
     \next%
       {\pstFP@shift=0\relax%
        \loop%
          \ifnum\pstFP@yia<100000000\relax%
	     \pstFP@multen{y}%
	     \advance\pstFP@shift1\relax%
	   \repeat%
        \loop%
          \ifnum\pstFP@xia<100000000\relax%
	     \pstFP@multen{x}%
	     \advance\pstFP@shift-1\relax%
	  \repeat%
        \pstFP@ria=0\pstFP@rib=0\pstFP@rfa=0\pstFP@rfb=0\relax%
        \loop%
          \ifpstFP@zero{y}\else%
	     \pstFP@counttimes%divides x by \pstFP@times*y
	     \pstFP@divten{y}%
	     \pstFP@multen{r}%
	     \advance\pstFP@rfb\pstFP@times%
	     \ifnum\pstFP@rfb<1000000000\relax\else%
	       \advance\pstFP@rfa1\advance\pstFP@rfb-1000000000\relax%
	       \ifnum\pstFP@rfa<1000000000\relax\else%
	         \advance\pstFP@rib1\advance\pstFP@rfa-1000000000\relax%
		 \ifnum\pstFP@rib<1000000000\relax\else%
		   \advance\pstFP@ria1\advance\pstFP@rib-1000000000\relax%
		 \fi%
	       \fi%
	     \fi%
	  \repeat%
        \loop%
          \ifnum\pstFP@shift>17%
	    \advance\pstFP@shift-1\relax%
	    \ifnum\pstFP@ria<100000000\else\pstFP@ria=-1\fi%
	    \ifnum\pstFP@ria<0\pstFP@ria=-1\fi%
	    \pstFP@multen{r}%
	  \repeat%
        \ifnum\pstFP@ria<1000000000\else\pstFP@ria=-1\fi%
        \loop%
          \ifnum\pstFP@shift<17%
	    \advance\pstFP@shift1\relax%
	    \pstFP@divten{r}%
	  \repeat%
        \ifnum\pstFP@ria<0\relax%
          \typeout{>>>>Overflow}%
        \else%
          \pstFP@store\pstFP@tmp{r}%
        \fi%
       }%
    \fi%
   %
   \global\let\pstFP@tmp=\pstFP@tmp%
   %
  }%
  \let#1\pstFP@tmp%
}
%multiply two values

\def\pstFP@firstnine#1#2#3#4#5#6#7#8#9{%
  \pstFP@res=#1#2#3#4#5#6#7#8#9\relax%
}
\def\pstFP@@ninesplit#1\relax#2\end#3{%
  #1%
  \edef#3{#2}%
}
\def\pstFP@ninesplit#1{%
  \edef#1{\expandafter\pstFP@firstnine\pstFP@rd}%
  \expandafter\pstFP@@ninesplit#1\end#1\relax%
}

\def\pstFP@split#1#2#3#4{%
  % #1 highest three digits
  % #2 medium three digits
  % #3 least three digits
  % #4 counter
  \pstFP@regc=#4%
  \divide\pstFP@regc1000000\relax%
  #1=\pstFP@regc%
  \multiply\pstFP@regc-1000000\relax\advance\pstFP@regc#4%
  #3=\pstFP@regc%
  \divide\pstFP@regc1000\relax%
  #2=\pstFP@regc%
  \multiply\pstFP@regc-1000\relax\advance\pstFP@regc#3%
  #3=\pstFP@regc%
}

\def\pstFP@@mul#1#2#3{%
  \pstFP@regc=\csname pstFP@x#1\endcsname%
  \multiply\pstFP@regc\csname pstFP@y#2\endcsname%
  \advance\pstFP@prod\pstFP@regc%
  %
  \ifx#3\relax%
    \let\next=\relax% 
  \else%
    \let\next=\pstFP@@mul%
  \fi%
  \next#3%
}

\def\pstFP@saveshift{%
  % save rightmost three digits 
  \pstFP@regc=\pstFP@prod%
  \divide\pstFP@prod1000\relax%
  \multiply\pstFP@prod1000\relax%
  \advance\pstFP@regc-\pstFP@prod%
  \advance\pstFP@regc1000\relax%
  \edef\pstFP@rd{\expandafter\pstFP@ignorenext\the\pstFP@regc\pstFP@rd}%
  %
  \divide\pstFP@prod1000\relax%
}

\def\pstFP@mul#1#2.#3.#4\relax#5.#6.#7\relax{%
  % #1 macro, which gets the result
  % #2 integer part of 1st value 
  % #3 fractional part of 1st value
  % #4 dummy to swallow everthing after the 2nd '.'
  % #5 integer part of 2nd value 
  % #6 fractional part of 2nd value
  % #7 dummy to swallow everthing after the 2nd '.'
  %
  % split value in various parts
  % x y = 123 456 789 123 456 789 . 123 456 789 123 456 789
  % ->    xk  xl  xm  xn  xo  xp    xq  xr  xs  xt  xu  xv
  % ->    yk  yl  ym  yn  yo  yp    yq  yr  ys  yt  yu  yv
  % multiply these parts and save the result wrt the necessary shifts
  %
  {\pstFP@readvalue{x}{#2}{#3}%
   \pstFP@readvalue{y}{#5}{#6}%
   %
   %sign
   \multiply\pstFP@xs\pstFP@ys%
   \pstFP@rs=\pstFP@xs%
   %
   % split parts
   \pstFP@split\pstFP@xk\pstFP@xl\pstFP@xm\pstFP@xia\pstFP@split\pstFP@xn\pstFP@xo\pstFP@xp\pstFP@xib%
   \pstFP@split\pstFP@xq\pstFP@xr\pstFP@xz\pstFP@xfa\pstFP@split\pstFP@xt\pstFP@xu\pstFP@xv\pstFP@xfb%
   \pstFP@split\pstFP@yk\pstFP@yl\pstFP@ym\pstFP@yia\pstFP@split\pstFP@yn\pstFP@yo\pstFP@yp\pstFP@yib%
   \pstFP@split\pstFP@yq\pstFP@yr\pstFP@yz\pstFP@yfa\pstFP@split\pstFP@yt\pstFP@yu\pstFP@yv\pstFP@yfb%
   %
   \pstFP@prod=0\relax%
   \edef\pstFP@rd{}%
   %
   %compute result
   \pstFP@@mul vv 				   \relax\pstFP@saveshift%
   \pstFP@@mul vu uv			           \relax\pstFP@saveshift%
   \pstFP@@mul uu vt tv 			   \relax\pstFP@saveshift%
   \pstFP@@mul ut tu vz zv 		           \relax\pstFP@saveshift%
   \pstFP@@mul tt zu uz rv vr		           \relax\pstFP@saveshift%
   \pstFP@@mul zt tz ur ru vq qv 		   \relax\pstFP@saveshift%
   \pstFP@@mul zz rt tr uq qu vp pv  	           \relax\pstFP@saveshift%
   \pstFP@@mul zr rz tq qt up pu vo ov 	           \relax\pstFP@saveshift%
   \pstFP@@mul rr qz zq tp pt uo ou vn nv 	   \relax\pstFP@saveshift%
   \pstFP@@mul rq qr zp pz to ot un nu vm mv       \relax\pstFP@saveshift%
   \pstFP@@mul qq rp pr zo oz tn nt um mu vl lv    \relax\pstFP@saveshift%
   \pstFP@@mul qp pq ro or zn nz tm mt ul lu kv vk \relax\pstFP@saveshift%
   \pstFP@@mul pp oq qo rn nr zm mz tl lt ku uk    \relax\pstFP@saveshift%
   \pstFP@@mul op po nq qn rm mr zl lz tk kt       \relax\pstFP@saveshift%
   \pstFP@@mul oo pn np mq qm rl lr kz zk          \relax\pstFP@saveshift%
   \pstFP@@mul no on mp pm lq ql kr rk 	           \relax\pstFP@saveshift%
   \pstFP@@mul nn mo om pl lp qk kq 	           \relax\pstFP@saveshift%
   \pstFP@@mul mn nm lo ok pk kp 		   \relax\pstFP@saveshift%
   \pstFP@@mul mm ln nl ko ok 		           \relax\pstFP@saveshift%
   \pstFP@@mul lm ml kn nk			   \relax\pstFP@saveshift%
   \pstFP@@mul ll km mk 			   \relax\pstFP@saveshift%
   \pstFP@@mul kl lk 			           \relax\pstFP@saveshift%
   \pstFP@@mul kk 				   \relax\pstFP@saveshift\pstFP@saveshift%
   \pstFP@ninesplit\pstFP@rd%
   \ifnum\pstFP@res=0\relax%
     \pstFP@ninesplit\pstFP@rd%
     \ifnum\pstFP@res=0\relax%
       \pstFP@ninesplit\pstFP@rd\pstFP@ria=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rib=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rfa=\pstFP@res%
       \pstFP@ninesplit\pstFP@rd\pstFP@rfb=\pstFP@res%
       \pstFP@store\pstFP@tmp{r}%
     \else\typeout{pstFPmul: Overflow}\fi%
   \else\typeout{pstFPmul: Overflow}\fi%
   \global\let\pstFP@tmp\pstFP@tmp}%
  \let#1\pstFP@tmp%
}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pst-fp.tex
\endinput


==> pst-grad.tex <==
%% BEGIN pst-grad.tex
%%
%% Gradient fillstyle with PSTricks.
%% See the PSTricks User's Guide for description.
%% This uses the header file `pst-grad.pro'.
%%
%% Based on some EPS files by leeweyr!bill@nuchat.sccsi.com (W. R. Lee).
%%
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%%           2006 Herbert Voss, hvoss@tug.org
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%% This defines a new fill style, "gradient", for use with PSTricks,
%% which has gradiated color. The following parameters are used:
%%
%%    gradbegin=color     : Beginning color.
%%    gradend=color       : Final color.
%%    gradlines=int       : Number of lines to use. The higher the number,
%%                           the slower the rendering.
%%    gradmidpoint=num    : Gradient color goes from gradbegin to gradend,
%%                           and then back to beginning. Midpoint (point
%%                           where "gradend" color appears, is gradmidpoint
%%                           from the top.  (0 <= Gmidpoint <= 1).
%%    gradangle=angle     : Rotate image by angle.
%%    GradientCircle=true : Instead of a linear a circled gradient is build.
%%                          (version 1.04)
%%    GradientPos=(x,y) :   the center of the circled gradient
%%                          (version 1.04)
%%    GradientScale=float : scaling factor of the circled gradient
%%                          (version 1.04)
%%    GradientHSB	  : Use HSB color model
%%    cmyk		  : Use CMYK color model
%%
\csname GradientLoaded\endcsname
\let\GradientLoaded\endinput
\ifx\PSTricksLoaded\endinput\else
  \def\next{\input pstricks.tex }\expandafter\next
\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi

\def\fileversion{1.06}
\def\filedate{2006/11/27}
\message{`pst-grad' v\fileversion, \filedate\space (tvz,dg,hv)}

\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
\pst@addfams{pst-grad}

\pstheader{pst-grad.pro}

\define@boolkey[psset]{pst-grad}[Pst@]{cmyk}[true]{%
  \ifPst@cmyk
    \newcmykcolor{gradbegin}{0 .1 .95 0.1}
    \newcmykcolor{gradend}{0 0.8 0.6 0.5}
  \else
    \newrgbcolor{gradbegin}{0 .1 .95}
    \newrgbcolor{gradend}{0 1 1}
  \fi%
}
\psset[pst-grad]{cmyk=false}
%
\define@key[psset]{pst-grad}{gradbegin}{\pst@getcolor{#1}\psgradbegin}
\define@key[psset]{pst-grad}{gradend}{\pst@getcolor{#1}\psgradend}
\define@key[psset]{pst-grad}{gradlines}{%
  \pst@getint{#1}\psgradlines
  \ifnum\psgradlines<2
    \@pstrickserr{gradlines must be at least 2}\@epha
    \def\psgradlines{2 }%
  \fi}
\define@key[psset]{pst-grad}{gradmidpoint}{\pst@checknum{#1}\psgradmidpoint}
\define@key[psset]{pst-grad}{gradangle}{\pst@getangle{#1}\psk@gradangle}
\psset[pst-grad]{gradangle=0,gradlines=300,gradend=gradend,gradbegin=gradbegin,
    gradmidpoint=0.9}

% Denis Girou - April 1998  ------- patch 2 (hv)
% To define the gradient as linear or as circle
%==================================================================
\define@boolkey[psset]{pst-grad}[Pst@]{GradientCircle}[true]{}
% Position of the center of the gradient
\define@key[psset]{pst-grad}{GradientPos}{\psset@@GradientPos#1}%
\def\psset@@GradientPos(#1){\edef\ps@GradientPos{#1}}
% Scale factor
\define@key[psset]{pst-grad}{GradientScale}{\def\ps@GradientScale{#1}}
\psset[pst-grad]{GradientCircle=false,GradientScale=1,GradientPos={(0,0)}}
%=====================================================================
%
\define@boolkey[psset]{pst-grad}[Pst@]{gradientHSB}[true]{}
\psset[pst-grad]{gradientHSB=false}
%
\def\psfs@gradient{%
  \ifPst@gradientHSB
    \addto@pscode{%
      gsave
      gsave \pst@usecolor\psgradbegin currenthsbcolor grestore
      gsave \pst@usecolor\psgradend currenthsbcolor grestore
      \psgradlines
      \psgradmidpoint
      \psk@gradangle
%  hv 2004-05-05 begin    fixed a spurious blank
      tx@GradientDict begin GradientFillHSB end grestore%
    }%
%    tx@GradientHSBDict begin GradientFillHSB end grestore}
%  hv 2004-05-05 end
  \else%
%    hv 2004-06-25 begin    fixed a spurious blank
    \pst@getcoor{\ps@GradientPos}{\pst@tempa}% <- "%"  hv 2004-06-23 
%    hv end
    \addto@pscode{%
      gsave
      \ifPst@GradientCircle\space true \else false \fi
      \ps@GradientScale\space
      \pst@tempa\space
      gsave \pst@usecolor\psgradbegin 
      \ifPst@cmyk currentcmykcolor \else currentrgbcolor \fi grestore
      gsave \pst@usecolor\psgradend 
      \ifPst@cmyk currentcmykcolor \else currentrgbcolor \fi grestore
      \psgradlines
      \psgradmidpoint
      \psk@gradangle
      \ifPst@cmyk true \else false \fi
      tx@GradientDict begin GradientFill end grestore%
    }%
  \fi%
}
%
\catcode`\@=\TheAtCode\relax
%
\endinput
%%
%% END pst-grad.tex


==> pst-math.tex <==
%%
%% This is file `pst-math.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-math.tex'
%%
%% Christophe Jorssen 
%% Herbert Voss <hvoss@tug.org>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory CTAN:/macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-math' is a PSTricks package to enhance math in PSTricks
%%
%%
%
\csname PSTmathLoaded\endcsname
\let\PSTmathLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\def\fileversion{0.62}
\def\filedate{2010/10/20}
\message{`pst-math' v\fileversion\space, (CJ,hv)}

\pstheader{pst-math.pro}
%
\def\pstPI#1{\ifcase#1\or3.141593\or1.570796\or1.047198\or0.785398\fi}
%
\endinput


==> pst-node.tex <==
% $Id: pst-node.tex 898 2014-03-25 20:52:31Z herbert $
%% BEGIN pst-node.tex
%%
%% Nodes with PSTricks.
%% See the betadoc documentation for usage. 
%% This uses the header file `pst-node.pro'.
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2009-2014 by Herbert Voss, hvoss tug.org.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%
\csname PSTnodesLoaded\endcsname
\let\PSTnodesLoaded\endinput
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex \fi\relax
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey \fi
%
\def\fileversion{1.33}
\def\filedate{2014/03/25}
\message{ v\fileversion, \filedate}
%
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
%
\pstheader{pst-node.pro}
\pst@addfams{pst-node}
%
\SpecialCoor
%
%%%%%%%%%% compatibility stuff
\define@boolkey[psset]{pst-node}[Pst@]{trueAngle}[true]{}
\psset[pst-node]{trueAngle=false}
%%%%%%%%%% compatibility stuff
\define@boolkey[psset]{pst-node}[Pst@]{storeNodeInfo}[true]{}
\psset[pst-node]{storeNodeInfo=false}
%
\def\pst@nodedict{tx@NodeDict begin }
\def\pst@zapspace#1 #2{%
#1%
\ifx#2\@empty\else\expandafter\pst@zapspace\fi
#2}
%
\def\pst@getnode#1#2{\pst@expandafter\pst@@getnode{#1},,\@nil#2}
\def\pst@@getnode#1,#2,#3\@nil#4{%
  \ifx\@empty#3\@empty
    \edef#4{/N@\pst@zapspace#1 \@empty\space}%
  \else
    \pst@cntg=#1\relax
    \pst@cnth=#2\relax
    \edef#4{/N@M-\ifnum\psmatrixcnt=\z@ 1\else\the\psmatrixcnt\fi
    -\the\pst@cntg-\the\pst@cnth\space}%
  \fi}
%
% bug fix for xelatex, dvipdfmx uses the wrong scaling
\def\tx@NewNode{/NodeScale {\ifx\pstnodescale\@undefined  \else\pstnodescale \fi} def NewNode }
%
\define@boolkey[psset]{pst-node}[Pst@]{showNode}[true]{}% write coors into the logfile
\define@boolkey[psset]{pst-node}[Pst@]{markNode}[true]{}% makr the node with its name
\define@boolkey[psset]{pst-node}[Pst@]{saveNodeCoors}[true]{}
\define@key[psset]{pst-node}{NodeCoorPrefix}[]{\def\psk@NodeCoorPrefix{#1}}% if empty it is N-<Name>.x|y
\psset[pst-node]{saveNodeCoors=false,showNode=false,markNode=false,NodeCoorPrefix=}% <NodeCoorPrefix<Name>x|y>
%
\def\psopenNodeFile{\pstVerb{ tx@NodeDict begin %/NodeFile { 
  (\jobname.nodes)(w) file %} def 
  end }}
\def\pscloseNodeFile{\pstVerb{ tx@NodeDict begin currentfile closefile end }}
%
\def\pst@newnode#1#2#3#4{%
\pst@killglue
\leavevmode
\pst@getnode{#1}\pst@thenode
\pst@Verb{
  \ifPst@saveNodeCoors
    \ifx\relax#3\relax 0 0 \else gsave \pst@dict STV CP T end #3 \tx@UserCoor grestore \fi 
    \if$\psk@NodeCoorPrefix$
      /N-#1.y exch def
      /N-#1.x exch def
    \else
      /\psk@NodeCoorPrefix#1y exch def
      /\psk@NodeCoorPrefix#1x exch def
    \fi
  \fi
  \pst@nodedict
  {#3}
  \ifx\psk@name\relax false \else \psk@name true \fi
  \pst@thenode
  #2
  {#4}
  \ifPst@showNode
    5 copy 
    cvlit aload pop 
    20 string cvs (; )   6 2 roll % InitPnode
    20 string cvs (; )   7 2 roll % type
    20 string cvs (; )   8 2 roll %/N@Name
    20 string cvs (; )   9 2 roll % true/false
    cvlit aload pop exch 
    20 string cvs (; ) 11 2 roll 
    20 string cvs (, ) 12 2 roll  % x,y
    12 array astore concatstringarray 
    currentfile exch  writestring
%    NodeFile exch  writestring
  \fi
  \tx@NewNode
  end 
}%
%
\global\let\psk@name\relax%
\pstree@nodehook%
\global\let\pstree@nodehook\relax}
%
\let\pstree@nodehook\relax
\define@boolkey[psset]{pst-node}[Pst@]{nodealign}[true]{}
\psset[pst-node]{nodealign=false}

\def\pst@nodealign{%
\pst@dimg=\ht\pst@hbox
\advance\pst@dimg-\dp\pst@hbox
\divide\pst@dimg2
\lower\pst@dimg}
%
\def\tx@InitPnode{InitPnode }
\def\pnode{\@ifnextchar[{\pnode@i}{\pnode@iii}}
\def\pnode@i[#1]{\@ifnextchar({\pnode@ii[#1]}{\pnode@ii[#1](0,0)}}
\def\pnode@ii[#1](#2)#3{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pst@newnode{#3}{10}{%
    \pst@tempA \pst@tempB 3 -1 roll add 3 1 roll add exch }{\tx@InitPnode}%
  \ifPst@showNode\psdot(#3)\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#3){#3}\fi
  \ignorespaces}
%
\def\pnode@iii{\@ifnextchar({\pnode@}{\pnode@(0,0)}}
\def\pnode@(#1)#2{%
  \pst@@getcoor{#1}%
  \pst@newnode{#2}{10}{\pst@coor}{\tx@InitPnode}%
  \ifPst@showNode\psdot(#2)\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#2){#2}\fi
  \ignorespaces}
%
\def\pnodes{\@ifnextchar[{\pnodes@i}{\pnodes@i[0,0]}}
\def\pnodes@i[#1]{\@ifnextchar({\psnodes@ii[#1]}{\pnodes@ii}}
\def\psnodes@ii[#1](#2)#3{%
  \pnode[#1](#2){#3}%
  \@ifnextchar({\psnodes@ii[#1]}{}%
}
%
\def\tx@InitCnode{InitCnode }
%
\def\cnode{\pst@object{cnode}}
\def\cnode@i{\@ifnextchar({\cnode@ii}{\cnode@ii(0,0)}}
\def\cnode@ii(#1)#2#3{%
  \leavevmode
  \hbox{%
    \use@par
    \pst@@getcoor{#1}%
    \pssetlength\pst@dimc{#2}%
    \pst@dimg=\psk@dimen\pslinewidth
    \advance\pst@dimc-\pst@dimg
    \advance\pst@dimc.5\pslinewidth
    \ifPst@nodealign
      \kern\pst@dimc
      \vrule width\z@ height \pst@dimc depth \pst@dimc
    \fi
    \pscircle@do(#1){#2}%
    \pst@newnode{#3}{11}{\pst@coor \pst@number\pst@dimc}{\tx@InitCnode}%
%%    % DG/SR modification begin - Jul. 30, 1997 - Patch 2
%%    %\ifPst@nodealign \kern\pst@dimc\egroup \fi}%
    \ifPst@nodealign\kern\pst@dimc\fi%
%%    % DG/SR modification end
  }%
  \ignorespaces}
%
\def\Cnode{\pst@object{Cnode}}
\def\Cnode@i{\@ifnextchar({\Cnode@ii}{\Cnode@ii(0,0)}}
\def\Cnode@ii(#1)#2{\cnode@ii(#1){\psk@radius}{#2}}%
%
\def\cnodeput{\pst@object{cnodeput}}
\def\cnodeput@i{\@ifnextchar({\cnodeput@iii}{\cnodeput@ii}}
\def\cnodeput@ii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\cnodeput@iii}{\cnodeput@iii(\z@,\z@)}}
\def\cnodeput@iii(#1)#2{%
  \pst@killglue
  \@fixedradiusfalse
  \def\pst@nodehook{\cnodeput@iv{#2}}%
  \pst@makebox{\cput@v{#1}}}
\def\cnodeput@iv#1{%
  \pst@newnode{#1}{11}{\pscirclebox@iv \pst@number\pslinewidth add}{\tx@InitCnode}%
  \global\let\pst@nodehook\relax}
%  
\def\Cnodeput{\pst@object{Cnodeput}}
\def\Cnodeput@i{\@ifnextchar({\Cnodeput@iii}{\Cnodeput@ii}}
\def\Cnodeput@ii#1{%
\addto@par{rot={#1}}%
\@ifnextchar({\Cnodeput@iii}{\Cnodeput@iii(\z@,\z@)}}
\def\Cnodeput@iii(#1)#2{%
\pst@killglue
\@fixedradiustrue
\def\pst@nodehook{\Cnodeput@iv{#2}}%
\pst@makebox{\cput@v{#1}}}
\def\Cnodeput@iv#1{%
\pst@newnode{#1}{11}{%
\pst@number{\wd\pst@hbox} 2 div \pst@number\pst@dima % x y
\pst@number\pst@dimb \pst@number\pslinewidth \psk@dimen .5 sub mul sub }% r
{\tx@InitCnode}%
\global\let\pst@nodehook\relax}
%
\def\circlenode{\pst@object{circlenode}}
\def\circlenode@i#1{\pst@makebox{\circlenode@ii{#1}}}
\def\circlenode@ii#1{%
  \begingroup
  \pst@useboxpar
  \setbox\pst@hbox=\hbox{%
    \cnodeput@iv{#1}%
    \pscirclebox@iii
    \box\pst@hbox}%
  \ifPst@nodealign \psboxseptrue \fi
  \ifpsboxsep \pscirclebox@sep \fi
  \leavevmode
  \ifPst@nodealign\pst@nodealign\fi
  \box\pst@hbox
  \endgroup}
%
\def\Circlenode{\pst@object{Circlenode}}
\def\Circlenode@i#1{\pst@makebox{\Circlenode@ii{#1}}}
\def\Circlenode@ii#1{%
\begingroup
\pst@useboxpar
\pst@dima=\ht\pst@hbox
\advance\pst@dima\dp\pst@hbox
\divide\pst@dima\tw@
\pssetlength\pst@dimb\psk@radius
\setbox\pst@hbox=\hbox{%
\Cnodeput@iv{#1}%
\pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
\box\pst@hbox}%
\ifPst@nodealign \psboxseptrue \fi
\ifpsboxsep \psCirclebox@sep \fi
\leavevmode
\ifPst@nodealign\pst@nodealign\fi
\box\pst@hbox
\endgroup}
\def\tx@GetRnodePos{GetRnodePos }
\def\tx@InitRnode{InitRnode }
%
\def\psnode{\pst@object{psnode}}
\def\psnode@i{\@ifnextchar(\psnode@ii{\psnode@ii(0,0)}}
\def\psnode@ii(#1)#2#3{%    #1: coordinates, #2: node name,  #3 contents
  \rput(#1){\rnode{#2}{#3}}}
%
\def\rnode{\@ifnextchar[{\rnode@i}{\def\pst@par{}\rnode@ii}}
\def\rnode@i[#1]{\def\pst@par{ref=#1}\rnode@ii}
\def\rnode@ii#1{\pst@makebox{\rnode@iii\rnode@iv{#1}}}
\def\rnode@iii#1#2{%
% DG modification begin - Jan. 1997
\leavevmode
% DG modification end
\begingroup
% DG/SR modification begin - Apr. 28, 1998 - Patch 6
\pst@useboxpar
% DG/SR modification end
#1%
\if@star\pst@starbox\fi
\ifPst@nodealign\lower\pst@dimb\fi
\hbox{%
\pst@newnode{#2}{16}{%
\pst@number{\ht\pst@hbox}%
\pst@number{\dp\pst@hbox}%
\pst@number{\wd\pst@hbox}%
\pst@number\pst@dima%
\pst@number\pst@dimb}%
{\tx@InitRnode}%
\box\pst@hbox}%
\endgroup}
\def\rnode@iv{%
\pst@dima=\psk@xref\wd\pst@hbox
\ifx\psk@yref\relax
\pst@dimb=\z@
\else
\pst@dimb=\ht\pst@hbox
\advance\pst@dimb\dp\pst@hbox
\pst@dimb=\psk@yref\pst@dimb
\advance\pst@dimb-\dp\pst@hbox
\fi}
%
\define@key[psset]{pst-node}{href}[0]{\pst@checknum{#1}\psk@href}
\psset[pst-node]{href=0}
\define@key[psset]{pst-node}{vref}[0.7ex]{\def\psk@vref{#1}}
\psset[pst-node]{vref=0.7ex}
\def\Rnode{\pst@object{Rnode}}
\def\Rnode@i#1{\pst@makebox{\rnode@iii\Rnode@ii{#1}}}
\def\Rnode@ii{%
% DG modification begin - Jan. 1997
%   - \begingroup removed  as it seems to doesn't work any more
%   - \Rnode doesn't process the optional parameter changes
%\begingroup
\use@par
% DG modification end
\pst@dima=\psk@href\wd\pst@hbox
\advance\pst@dima\wd\pst@hbox
\divide\pst@dima 2
\pssetlength\pst@dimb{\psk@vref}}
\def\tx@DiaNodePos{DiaNodePos }
\def\dianode{\pst@object{dianode}}
\def\dianode@i#1{\pst@makebox{\dianode@ii{#1}}}
\def\dianode@ii#1{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc 2 mul def
/h \pst@number\pst@dimd 2 mul def
/NodePos { \tx@DiaNodePos } def}%
\box\pst@hbox}%
\ifPst@nodealign\psboxseptrue\fi
\ifpsboxsep\psdiabox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifPst@nodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
%
\def\tx@TriNodePos{TriNodePos }
\def\tx@InitTriNode{InitTriNode }
%
\def\trinode{\pst@object{trinode}}
\def\trinode@i#1{\pst@makebox{\trinode@ii{#1}}}
\def\trinode@ii#1{%
  \begingroup%
  \pst@useboxpar%
  \pstribox@iii
  \setbox\pst@hbox=\hbox{%
    \pst@newnode{#1}{14}{}{
      \pst@number\pst@dimc
      \pst@number\pst@dimd
      \ifodd\psk@trimode
        exch
        \pst@number\pst@dima
      \else
        \pst@number\pst@dimb
      \fi
      \psk@trimode
      \pst@number{\wd\pst@hbox}
      \pst@number{\ht\pst@hbox}
      \pst@number{\dp\pst@hbox}
      \tx@InitTriNode
    }%
    \box\pst@hbox%
  }%
  \ifPst@nodealign\psboxseptrue\fi
  \ifpsboxsep\pstribox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
  \leavevmode
% DG/SR modification end
  \ifPst@nodealign\lower\pst@tempa\fi
  \box\pst@hbox%
  \endgroup}
%
\def\tx@OvalNodePos{OvalNodePos }
\def\ovalnode{\pst@object{ovalnode}}
\def\ovalnode@i#1{\pst@makebox{\ovalnode@ii{#1}}}
\def\ovalnode@ii#1{%
\begingroup
\pst@useboxpar
\psovalbox@iii
\setbox\pst@hbox=\hbox{%
\pst@newnode{#1}{14}{}{%
/X \pst@number\pst@dima def
/Y \pst@number\pst@dimb def
/w \pst@number\pst@dimc def
/h \pst@number\pst@dimd def
/NodePos { \tx@OvalNodePos } def}%
\unhbox\pst@hbox}%
\ifPst@nodealign\psboxseptrue\fi
\ifpsboxsep\psovalbox@sep\fi
% DG/SR modification begin - Sep. 2, 1997 - Patch 3
\leavevmode
% DG/SR modification end
\ifPst@nodealign\lower\pst@dimb\fi
\box\pst@hbox
\endgroup}
%
\def\dotnode{\pst@object{dotnode}}
\def\dotnode@i{\@ifnextchar({\dotnode@ii}{\dotnode@ii(\z@,\z@)}}
\def\dotnode@ii(#1)#2{%
  \leavevmode
  \hbox{%
    \use@par
    \pst@@getcoor{#1}%
    \pst@getdotsize
    \pstree@nodehook
    \ifPst@nodealign
      \pst@dima=\pst@dimg
      \kern\pst@dima
      \vrule width\z@ height \pst@dimh depth \pst@dimh
    \fi
    \pst@newnode{#2}{14}{}{
      \pst@coor
      /Y exch def /X exch def
      /w \pst@number\pst@dimg def
      /h \pst@number\pst@dimh def
      /NodePos { \tx@OvalNodePos } def}%
    \psdot@ii(#1)%
    \ifPst@nodealign\kern\pst@dima\fi}%
  \ifPst@markNode\uput[\ifx\psk@rot\@empty0\else\psk@rot\fi]{0}(#2){#2}\fi
  \ignorespaces}
%
\def\dotnodes{\pst@object{dotnodes}}
\def\dotnodes@i{\use@par\dotnodes@ii}
\def\dotnodes@ii(#1)#2{%
  \dotnode(#1){#2}%
  \@ifnextchar(\dotnodes@ii{\def\pst@par{}}}
%
\define@key[psset]{pst-node}{framesize}{\pst@expandafter\psset@@framesize{#1} \@nil}
\def\psset@@framesize#1 #2\@nil{%
  \pssetlength\pst@dimg{#1}%
  \divide\pst@dimg2
  \edef\psk@framewidth{\pst@number\pst@dimg}%
  \ifx\@empty#2\@empty
    \let\psk@frameheight\psk@framewidth
  \else
    \pssetlength\pst@dimg{#2}%
    \divide\pst@dimg2
    \edef\psk@frameheight{\pst@number\pst@dimg}%
  \fi}
%
\psset[pst-node]{framesize=10pt}
%
\def\fnode{\pst@object{fnode}}
\def\fnode@i{\@ifnextchar({\fnode@ii}{\fnode@ii(\z@,\z@)}}
\def\fnode@ii(#1)#2{%
  \leavevmode
  \pst@killglue
  \hbox{%
    \use@par%
    \begin@ClosedObj%
    \ifPst@nodealign
      \kern\psk@framewidth\p@
      \vrule width\z@ height \psk@frameheight\p@ depth \psk@frameheight\p@
      \edef\pst@coor{0 0 }%
    \else\pst@@getcoor{#1}\fi
    \pst@newnode{#2}{14}{}{
      \pst@coor
      /Y exch def /X exch def
      /d \psk@dimen .5 sub CLW mul neg def
      /r \psk@framewidth d add def
      /l r neg def
      /u \psk@frameheight d add def
      /d u neg def
      /NodePos { \tx@GetRnodePos } def}%
    \addto@pscode{
      /x2 \psk@framewidth CLW \psk@dimen mul sub def
      /y2 \psk@frameheight CLW \psk@dimen mul sub def
      \pst@coor 2 copy
      y2 sub /y1 ED
      x2 sub /x1 exch def
      y2 add /y2 exch def
      x2 add /x2 exch def
      \psk@cornersize
      1 index 0 eq { pop pop \tx@Rect } { \tx@OvalFrame } ifelse}%
    \def\pst@linetype{2}%
    \showpointsfalse%
    \end@ClosedObj%
    \ifPst@nodealign\kern\psk@framewidth\p@\fi}% end of \hbox
  \ignorespaces}
%
%
% This fixes a bug in pst-node, where the XY-direction is wrong
% the types are changed 1<->2 between X<->Y
%
\define@key[psset]{}{XnodesepA}{\pst@getlength{#1}\psk@nodesepA\def\psk@nodeseptypeA{2 }}
\define@key[psset]{}{XnodesepB}{\pst@getlength{#1}\psk@nodesepB\def\psk@nodeseptypeB{2 }}
\define@key[psset]{}{Xnodesep}{%
    \pst@getlength{#1}\psk@nodesepA
    \let\psk@nodesepB\psk@nodesepA
    \def\psk@nodeseptypeA{2 }%
    \def\psk@nodeseptypeB{2 }}
\define@key[psset]{}{YnodesepA}{\pst@getlength{#1}\psk@nodesepA\def\psk@nodeseptypeA{1 }}
\define@key[psset]{}{YnodesepB}{\pst@getlength{#1}\psk@nodesepB\def\psk@nodeseptypeB{1 }}
\define@key[psset]{}{Ynodesep}{%
    \pst@getlength{#1}\psk@nodesepA
    \let\psk@nodesepB\psk@nodesepA
    \def\psk@nodeseptypeA{1 }%
    \def\psk@nodeseptypeB{1 }}
%%%% end bugfix %%%%%
\define@key[psset]{pst-node}{nodesepA}[0pt]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{0 }}
\define@key[psset]{pst-node}{nodesepB}[0pt]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{0 }}
\define@key[psset]{pst-node}{nodesep}[0pt]{%
  \pst@getlength{#1}\psk@nodesepA
  \let\psk@nodesepB\psk@nodesepA
  \def\psk@nodeseptypeA{0 }%
  \def\psk@nodeseptypeB{0 }}
\psset[pst-node]{nodesep=0pt}
%\define@key[psset]{pst-node}{XnodesepA}[]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{1 }}
%\define@key[psset]{pst-node}{XnodesepB}[]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{1 }}
%\define@key[psset]{pst-node}{Xnodesep}[]{%
%  \pst@getlength{#1}\psk@nodesepA
%  \let\psk@nodesepB\psk@nodesepA
%  \def\psk@nodeseptypeA{1 }%
%  \def\psk@nodeseptypeB{1 }}
%\define@key[psset]{pst-node}{YnodesepA}[]{\pst@getlength{#1}\psk@nodesepA \def\psk@nodeseptypeA{2 }}
%\define@key[psset]{pst-node}{YnodesepB}[]{\pst@getlength{#1}\psk@nodesepB \def\psk@nodeseptypeB{2 }}
%\define@key[psset]{pst-node}{Ynodesep}[]{
%  \pst@getlength{#1}\psk@nodesepA
%  \let\psk@nodesepB\psk@nodesepA
%  \def\psk@nodeseptypeA{2 }%
%  \def\psk@nodeseptypeB{2 }}
\define@key[psset]{pst-node}{armA}[10pt]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{0 }}
\define@key[psset]{pst-node}{armB}[10pt]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{0 }}
\define@key[psset]{pst-node}{arm}[10pt]{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{0 }%
  \def\psk@armtypeB{0 }}
\psset[pst-node]{arm=10pt}
\define@key[psset]{pst-node}{XarmA}[]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{1 }}
\define@key[psset]{pst-node}{XarmB}[]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{1 }}
\define@key[psset]{pst-node}{Xarm}{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{1 }%
  \def\psk@armtypeB{1 }}
\define@key[psset]{pst-node}{YarmA}[]{\pst@getlength{#1}\psk@armA \def\psk@armtypeA{2 }}
\define@key[psset]{pst-node}{YarmB}[]{\pst@getlength{#1}\psk@armB \def\psk@armtypeB{2 }}
\define@key[psset]{pst-node}{Yarm}[]{%
  \pst@getlength{#1}\psk@armA
  \let\psk@armB\psk@armA
  \def\psk@armtypeA{2 }%
  \def\psk@armtypeB{2 }}
\define@key[psset]{pst-node}{offsetA}[0pt]{\pst@getlength{#1}\psk@offsetA}
\define@key[psset]{pst-node}{offsetB}[0pt]{\pst@getlength{#1}\psk@offsetB}
\define@key[psset]{pst-node}{offset}[0pt]{\pst@getlength{#1}\psk@offsetA\let\psk@offsetB\psk@offsetA}
\psset[pst-node]{offset=0pt}
\define@key[psset]{pst-node}{angleA}[0]{\pst@getangle{#1}\psk@angleA}
\define@key[psset]{pst-node}{angleB}[0]{\pst@getangle{#1}\psk@angleB}%
\define@key[psset]{pst-node}{angle}[0]{%
  \pst@getangle{#1}\psk@angleA
  \let\psk@angleB\psk@angleA}
\psset[pst-node]{angle=0}
\define@key[psset]{pst-node}{arcangleA}[8]{\pst@getangle{#1}\psk@arcangleA}
\define@key[psset]{pst-node}{arcangleB}[8]{\pst@getangle{#1}\psk@arcangleB}%
\define@key[psset]{pst-node}{arcangle}[8]{%
  \pst@getangle{#1}\psk@arcangleA
  \let\psk@arcangleB\psk@arcangleA}
\psset[pst-node]{arcangle=8}
\define@key[psset]{pst-node}{ncurvA}[0.67]{\pst@checknum{#1}\psk@ncurvA}
\define@key[psset]{pst-node}{ncurvB}[0.67]{\pst@checknum{#1}\psk@ncurvB}%
\define@key[psset]{pst-node}{ncurv}[0.67]{\pst@checknum{#1}\psk@ncurvA\let\psk@ncurvB\psk@ncurvA}
\psset[pst-node]{ncurv=0.67}
%
\def\tx@GetCenter{GetCenter }
\def\tx@XYPos{XYPos }
\def\tx@GetEdge{GetEdge }
\def\tx@AddOffset{AddOffset }
\def\tx@GetEdgeA{GetEdgeA }
\def\tx@GetEdgeB{GetEdgeB }
\def\tx@GetArmA{GetArmA }
\def\tx@GetArmB{GetArmB }
%
\def\check@arrow#1#2{%
  \check@@arrow#2-\@nil
  \if@pst\addto@par{arrows=#2}\def\next{#1}%
  \else\def\next{#1{#2}}\fi
  \next}
\def\check@@arrow#1-#2\@nil{%
\ifx\@nil#2\@nil\@pstfalse\else\@psttrue\fi}
%
\def\tx@InitNC{InitNC }
\def\nc@object#1#2#3#4#5{%
  \csname begin@#1Obj\endcsname
  \showpointsfalse
  \pst@getnode{#2}\pst@tempa
  \pst@getnode{#3}\pst@tempb
  \gdef\npos@default{#4 }%
  \addto@pscode{%
    /NCLW CLW def
    \pst@nodedict
    \psk@offsetA
    \psk@offsetB neg
    \psk@nodesepA
    \psk@nodesepB
    \psk@nodeseptypeA
    \psk@nodeseptypeB
    \pst@tempa
    \pst@tempb
    \tx@InitNC { #5 } if
    end }%
  \def\use@pscode{%
    \pst@Verb{gsave \tx@STV newpath \pst@code\space grestore}%
    \gdef\pst@code{}}%
  \csname end@#1Obj\endcsname
  \pst@shortput}
%
\def\npos@default{.5 }
%
\def\pc@object#1{%
  \@ifnextchar({\pc@@object#1}{\pst@getarrows{\pc@@object#1}}}
\def\pc@@object#1(#2)(#3){%
  \pnode(#2){@@A}\pnode(#3){@@B}%
  #1{@@A}{@@B}}
%
\def\tx@LPutLine{LPutLine }
\def\tx@LPutLines{LPutLines }
\def\tx@BezierMidpoint{BezierMidpoint }
\def\tx@HPosBegin{HPosBegin }
\def\tx@HPosEnd{HPosEnd }
\def\tx@HPutLine{HPutLine }
\def\tx@HPutLines{HPutLines }
\def\tx@VPosBegin{VPosBegin }
\def\tx@VPosEnd{VPosEnd }
\def\tx@VPutLine{VPutLine }
\def\tx@VPutLines{VPutLines }
\def\tx@HPutCurve{HPutCurve }
\def\tx@NCCoor{NCCoor }
\def\tx@NCLine{NCLine }
%
\def\ncline{\pst@object{ncline}}
\def\ncline@i{\check@arrow{\ncline@ii}}
\def\ncline@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{\tx@NCLine}}
%
\def\pcline{\pst@object{pcline}}
\def\pcline@i{\pc@object\ncline@ii}
%
\def\ncLine{\pst@object{ncLine}}
\def\ncLine@i{\check@arrow{\ncLine@ii}}
\def\ncLine@ii#1#2{\nc@object{Open}{#1}{#2}{.5}%
% DG/SR modification begin - Apr. 14, 1999 - Patch 9
%{\tx@NCLine /LPutPos { xB xA yB yA \tx@LPutLine } def}}
{\tx@NCLine /LPutPos { xB yB xA yA \tx@LPutLine } def}}
% DG/SR modification end
%
\def\tx@NCLines{NCLines }
\def\nclines{\pst@object{nclines}}
\def\nclines@i{\check@arrow\nclines@ii}
\def\nclines@ii#1#2{%
\begingroup
\use@par
\def\pst@aftercoors{\nclines@iii{#1}{#2}}%
\def\pst@coors{}%
\pst@@getcoors}
\def\nclines@iii#1#2{%
\nc@object{Open}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
mark \pst@coors \tx@NCLines}%
\endgroup
\ignorespaces}
\def\tx@NCCurve{NCCurve }
\def\nccurve{\pst@object{nccurve}}
\def\nccurve@i{\check@arrow{\nccurve@ii}}
\def\nccurve@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
  /AngleA \psk@angleA\space def /AngleB \psk@angleB\space def
  \psk@ncurvB\space \psk@ncurvA\space
  \tx@NCCurve}}
\def\pccurve{\pst@object{pccurve}}
\def\pccurve@i{\pc@object\nccurve@ii}
%
\def\ncarc{\pst@object{ncarc}}
\def\ncarc@i{\check@arrow{\ncarc@ii}}
\def\ncarc@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{%
  yB yA sub xB xA sub \tx@Atan dup
  \psk@arcangleA\space add /AngleA exch def
  \psk@arcangleB\space sub 180 add /AngleB exch def
  \psk@ncurvB\space \psk@ncurvA\space
  \tx@NCCurve}}
\def\pcarc{\pst@object{pcarc}}
\def\pcarc@i{\pc@object\ncarc@ii}
%
\def\tx@NCAngles{NCAngles }
%
%border or center as reference point (hv)
\define@boolkey[psset]{pst-node}[Pst@]{pcRef}[true]{}
\psset[pst-node]{pcRef=false}
%
\def\ncangles{\pst@object{ncangles}}
\def\ncangles@i{\check@arrow{\ncangles@ii}}
\def\ncangles@ii#1#2{%
  \nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngles}}
\def\ncangles@iii{
  tx@Dict begin \psline@iii pop end
  /AngleA \psk@angleA def
  /AngleB \psk@angleB def
  /ArmA \psk@armA \ifPst@pcRef 
    GetEdgeA yA yA1 sub dup mul xA xA1 sub dup mul add sqrt sub \fi def
  /ArmB \psk@armB def
  /ArmTypeA \psk@armtypeA def
  /ArmTypeB \psk@armtypeB def }
%
\def\pcangles{\pst@object{pcangles}}
\def\pcangles@i{\pc@object\ncangles@ii}
\def\tx@NCAngle{NCAngle }
\def\ncangle{\pst@object{ncangle}}
\def\ncangle@i{\check@arrow{\ncangle@ii}}
\def\ncangle@ii#1#2{%
\nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \tx@NCAngle}}
\def\pcangle{\pst@object{pcangle}}
\def\pcangle@i{\pc@object\ncangle@ii}
\def\tx@NCBar{NCBar }
\def\ncbar{\pst@object{ncbar}}
\def\ncbar@i{\check@arrow{\ncbar@ii}}
\def\ncbar@ii#1#2{\nc@object{Open}{#1}{#2}{1.5}{%
\ncangles@iii /AngleB \psk@angleA def \tx@NCBar}}
\def\pcbar{\pst@object{pcbar}}
\def\pcbar@i{\pc@object\ncbar@ii}
%
\define@key[psset]{pst-node}{lineAngle}[0]{%
  \ifdim#1pt=\z@\else\psset{armB=0.5}\fi
  \def\psk@lineAngle{#1}}%
\psset[pst-node]{lineAngle=0}%
%
\def\tx@NCDiag{NCDiag }
\def\ncdiag{\pst@object{ncdiag}}
\def\ncdiag@i{\check@arrow{\ncdiag@ii}}
\def\ncdiag@ii#1#2{%
  \nc@object{Open}{#1}{#2}{1.5}{\ncangles@iii \psk@lineAngle\space \tx@NCDiag}}
%
\def\pcdiag{\pst@object{pcdiag}}
\def\pcdiag@i{\pc@object\ncdiag@ii}
%
\def\tx@NCDiagg{NCDiagg }
\def\ncdiagg{\pst@object{ncdiagg}}
\def\ncdiagg@i{\check@arrow{\ncdiagg@ii}}
\def\ncdiagg@ii#1#2{%
  \nc@object{Open}{#1}{#2}{.5}{\ncangles@iii \psk@lineAngle\space \tx@NCDiagg}}
\def\pcdiagg{\pst@object{pcdiagg}}
%
\def\pcdiagg@i{\pc@object\ncdiagg@ii}
\def\tx@NCLoop{NCLoop }
\define@key[psset]{pst-node}{loopsize}{\pst@getlength{#1}\psk@loopsize}
\psset[pst-node]{loopsize=1cm}
\def\ncloop{\pst@object{ncloop}}
\def\ncloop@i{\check@arrow{\ncloop@ii}}
\def\ncloop@ii#1#2{%
\nc@object{Open}{#1}{#2}{2.5}%
{\ncangles@iii /loopsize \psk@loopsize def \tx@NCLoop}}
\def\pcloop{\pst@object{pcloop}}
\def\pcloop@i{\pc@object\ncloop@ii}
\def\tx@NCCircle{NCCircle }
\def\nccircle{\pst@object{nccircle}}
\def\nccircle@i{\check@arrow{\nccircle@ii}}
\def\nccircle@ii#1#2{%
\pssetlength\pst@dima{#2}%
\nc@object{Open}{#1}{#1}{.5}{%
/AngleA \psk@angleA def
/r \pst@number\pst@dima def
\tx@NCCircle \psarc@v end}}
\def\tx@NCBox{NCBox }
\def\ncbox{\pst@object{ncbox}}
\def\ncbox@i{\check@arrow{\ncbox@ii}}
\def\ncbox@ii#1#2{%
\def\pst@linetype{2}%
\nc@object{Closed}{#1}{#2}{.5}{%
tx@Dict begin \psline@iii pop end
\psk@boxheight \psk@boxdepth
\tx@NCBox}}
\def\pcbox{\pst@object{pcbox}}
\def\pcbox@i{\pc@object\ncbox@ii}
\def\tx@NCArcBox{NCArcBox }
\define@key[psset]{pst-node}{boxheight}[0.4cm]{\pst@getlength{#1}\psk@boxheight}
\define@key[psset]{pst-node}{boxdepth}[0.4cm]{\pst@getlength{#1}\psk@boxdepth}
\define@key[psset]{pst-node}{boxsize}[0.4cm]{%
  \pst@getlength{#1}\psk@boxheight%  
  \let\psk@boxdepth\psk@boxheight}
\psset[pst-node]{boxsize=0.4cm}
%
\def\ncarcbox{\pst@object{ncarcbox}}
\def\ncarcbox@i{\check@arrow{\ncarcbox@ii}}
\def\ncarcbox@ii#1#2{%
\def\pst@linetype{1}%
\nc@object{Closed}{#1}{#2}{.5}{%
\psk@arcangleA \psk@boxheight \psk@boxdepth \pst@number\pslinearc
\tx@NCArcBox}}
\def\pcarcbox{\pst@object{pcarcbox}}
\def\pcarcbox@i{\pc@object\ncarcbox@ii}
\def\tx@Tfan{Tfan }
% Changed according pst-beta.bug December 3, 1993
% nrot=:<angle> does not work when : is active.
\begingroup
\catcode`\:=13
\gdef\pst@activerot{\def:{\string:}}
\endgroup
\define@key[psset]{pst-node}{nrot}[0]{%
  \begingroup
  \pst@activerot
  \pst@expandafter{\@ifnextchar:{\psset@@nrot}{\psset@@rot}}{#1}\@nil
  \global\let\pst@tempg\psk@rot
  \endgroup
  \let\psk@nrot\pst@tempg}
%  
\def\psset@@nrot:#1\@nil{%
  \psset@@rot#1\@nil
  \edef\psk@rot{NAngle \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\psset[pst-node]{nrot=0}
%
\def\tx@LPutCoor{LPutCoor }
\def\tx@LPut{LPut }
\define@key[psset]{pst-node}{npos}[{}]{%
  \def\pst@tempa{#1}%
  \ifx\pst@tempa\@empty\def\psk@npos{\npos@default}\else\pst@checknum{#1}\psk@npos\fi}
\psset[pst-node]{npos=}
%
\def\ncput{\pst@object{ncput}}
\def\ncput@i{\pst@killglue\pst@makebox{\ncput@ii}}
\def\ncput@ii{%
  \begingroup%
  \use@par%
  \if@star\pst@starbox\fi%
  \pst@makesmall\pst@hbox%
  \pst@rotate\psk@nrot\pst@hbox%
  \ncput@iii%
  \endgroup%
  \pst@shortput}
\def\ncput@iii{%
  \leavevmode%
  \hbox{%
    \pst@Verb{
      \pst@nodedict
      /t \psk@npos def
      \tx@LPut
      end
      \tx@PutBegin}%
    \box\pst@hbox%
    \pst@Verb{\tx@PutEnd}}}
%
\def\naput{\pst@object{naput}}
\def\naput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 add}}}
\def\naput@ii#1{%
  \begingroup
%  \addto@par{labelsep=15pt}%
  \use@par
  \if@star\pst@starbox\fi
  \def\psk@refangle{#1 }%
  \let\psk@rot\psk@nrot
  \pst@Verb{ 
    gsave  STV CP T /ps@refangle {#1 } def 
    /ps@rot { \psk@rot } def grestore }%ADDED (MJS)
  \uput@vii
  {exch pop add a \tx@PtoC h1 add exch w1 add exch }%
  {tx@Dict /NCLW known { NCLW add } if }%
  \ncput@iii
  \endgroup
  \pst@shortput}
%
\def\nbput{\pst@object{nbput}}
\def\nbput@i{\pst@killglue\pst@makebox{\naput@ii{NAngle 90 sub}}}
\define@key[psset]{pst-node}{tpos}[0.5]{%
  \pst@checknum{#1}\psk@tpos
  \ifdim\psk@tpos \p@<\z@
    \def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
    \@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa
% DG/SR modification end
  \else
    \ifdim\psk@tpos \p@>\p@
      \def\psk@tpos{.5}%
% DG/SR modification begin - Sep. 23, 1998 - Patch 7
%\@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@epha
      \@pstrickserr{Bad `tpos' value: `#1'. Must be 0<tpos<1}\@ehpa%
% DG/SR modification end
    \fi%
  \fi}
\psset[pst-node]{tpos=0.5}
%
\def\nlput{\pst@object{nlput}}
\def\nlput@i(#1)(#2)#3#4{%
  \begin@SpecialObj
  \psLDNode(#1)(#2){#3}{temp@lnput}
  \pcline[linestyle=none](#1)(temp@lnput)%
  \ncput[npos=1]{#4}%
  \end@SpecialObj}
%
\def\tvput{\pst@object{tvput}}
\def\tvput@i{\pst@makebox{\psput@tput{H}{1}}}
\def\tlput{\pst@object{tlput}}
\def\tlput@i{\pst@makebox{\psput@tput{H}{true}}}
\def\trput{\pst@object{trput}}
\def\trput@i{\pst@makebox{\psput@tput{H}{false}}}
\def\thput{\pst@object{thput}}
\def\thput@i{\pst@makebox{\psput@tput{V}{1}}}
\def\taput{\pst@object{taput}}
\def\taput@i{\pst@makebox{\psput@tput{V}{true}}}
\def\tbput{\pst@object{tbput}}
\def\tbput@i{\pst@makebox{\psput@tput{V}{false}}}
\def\tx@HPutAdjust{HPutAdjust }
\def\tx@VPutAdjust{VPutAdjust }
\def\psput@tput#1#2{%
  \begingroup
  \use@par
  \pst@tputmakesmall
  \leavevmode
  \hbox{%
    \pst@Verb{%
      \pst@nodedict
      /t \psk@tpos \pst@tposflip def
      tx@NodeDict /HPutPos known
        { #1PutPos }
        { CP /Y exch def /X exch def /NAngle 0 def /NCLW 0 def }
      ifelse
      /Sin NAngle sin def
      /Cos NAngle cos def
      /s \pst@number\pslabelsep NCLW add def
      /l \pst@number\pst@dima def
      /r \pst@number\pst@dimb def
      /h \pst@number\pst@dimc def
      /d \pst@number\pst@dimd def
% DG/SR modification begin - Sep. 26, 1997 - Patch 4
%\ifnum1=0#2\else
      \ifnum1=0#2 \else
% DG/SR modification end
        /flag #2 def
        \csname tx@#1PutAdjust\endcsname
      \fi
      \tx@LPutCoor
      end
      \tx@PutBegin}%
    \box\pst@hbox
    \pst@Verb{\tx@PutEnd}}%
  \endgroup
  \pst@shortput}
%  
\def\pst@tposflip{}
\def\pst@tputmakesmall{%
%
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimg=\psk@href\pst@dimg
\pst@dimb\pst@dima
\advance\pst@dima\pst@dimg % leftsize
\advance\pst@dimb-\pst@dimg % rightsize
\pst@dimd=\psk@vref\relax
\pst@dimc=\ht\pst@hbox
\advance\pst@dimc-\pst@dimd % height
\advance\pst@dimd\dp\pst@hbox % depth
\setbox\pst@hbox=\hbox to\z@{%
\kern-\pst@dima\vbox to\z@{\vss\box\pst@hbox\vskip-\pst@dimd}\hss}}
\def\MakeShortNab#1#2{%
  \def\pst@shortput@nab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\naput
    \else
      \ifx#2\next
        \let\pst@tempg\nbput
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortNab{^}{_}
\def\MakeShortTablr#1#2#3#4{%
  \def\pst@shortput@tablr{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \let\pst@tempg\taput
    \else
      \ifx#2\next
        \let\pst@tempg\tbput
      \else
        \ifx#3\next
          \let\pst@tempg\tlput
        \else
          \ifx#4\next
            \let\pst@tempg\trput
          \else
            \ifx\@sptoken\next
              \let\pst@tempg\pst@shortput
            \fi
          \fi
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTablr{^}{_}{<}{>}
\def\MakeShortTab#1#2{%
  \def\pst@shortput@tab{%
    \def\pst@tempg{\next}%
    \ifx#1\next
      \def\pst@tempg{%
        \@nameuse{%
          t\ifodd\psk@treemode\ifpstreeflip b\else a\fi
          \else\ifpstreeflip r\else l\fi\fi put}}%
    \else
      \ifx#2\next
        \def\pst@tempg{%
          \@nameuse{%
            t\ifodd\psk@treemode\ifpstreeflip a\else b\fi
            \else\ifpstreeflip l\else r\fi\fi put}}%
      \else
        \ifx\@sptoken\next
          \let\pst@tempg\pst@shortput
        \fi
      \fi
    \fi
    \pst@tempg}}
\MakeShortTab{^}{_}
\define@key[psset]{pst-node}{shortput}[none]{%
  \def\pst@tempg{#1}%
  \ifx\pst@tempg\@none
    \let\pst@shortput\ignorespaces
  \else
    \@ifundefined{pst@shortput@#1}%
     {\@pstrickserr{Bad short put: `#1'}\@ehpa}%
     {\edef\pst@shortput{\noexpand\afterassignment\expandafter\noexpand
      \csname pst@shortput@#1\endcsname\noexpand\let\noexpand\next}}%
  \fi}
\psset[pst-node]{shortput=none}
%
\def\lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\lput@i}{\lput@ii}}}
\def\lput@i[#1]{\addto@par{ref=#1}\lput@ii}
\def\lput@ii{\@ifnextchar({\lput@iv}{\lput@iii}}
\def\lput@iii#1{\addto@par{nrot=#1}\@ifnextchar({\lput@iv}{\ncput@i}}
\def\lput@iv(#1){\addto@par{npos=#1}\ncput@i}
\def\mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\mput@i}{\ncput@i}}}
\def\mput@i[#1]{\addto@par{ref=#1}\ncput@i}
\def\Lput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Lput@ii}{\Lput@i}}}
\def\Lput@i#1{\addto@par{labelsep=#1}\Lput@ii}
\def\Lput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Lput@iv}{\Lput@iii}}
\def\Lput@iii#1{\addto@par{nrot={#1}}\@ifnextchar({\Lput@iv}{\Lput@v}}
\def\Lput@iv(#1){\addto@par{npos=#1}\Lput@v}
\def\Lput@v{\pst@killglue\pst@makebox{\Lput@vi}}
\def\Lput@vi{%
\begingroup
\use@par
\if@star\pst@starbox\fi
\Rput@vi
\pst@makesmall\pst@hbox
\ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%\pst@rotate\psk@nrot\pst@hbox
\ncput@iii
\endgroup
\pst@shortput}
\def\Mput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Mput@ii}{\Mput@i}}}
\def\Mput@i#1{\addto@par{labelsep=#1}\Mput@ii}
\def\Mput@ii[#1]{\addto@par{ref={#1}}\Lput@v}
\def\aput@#1{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\aput@i#1}{\aput@ii#1}}}
\def\aput@i#1[#2]{\addto@par{labelsep=#2}\aput@ii#1}
\def\aput@ii#1{\@ifnextchar({\aput@iv#1}{\aput@iii#1}}
\def\aput@iii#1#2{\addto@par{nrot=#2}\@ifnextchar({\aput@iv#1}{#1}}
\def\aput@iv#1(#2){\addto@par{npos=#2}#1}
\def\aput{\aput@\naput@i}
\def\bput{\aput@\nbput@i}
\def\Aput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Aput@i}{\naput@i}}}
\def\Aput@i[#1]{\addto@par{labelsep=#1}\naput@i}
\def\Bput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Bput@i}{\nbput@i}}}
\def\Bput@i[#1]{\addto@par{labelsep=#1}\nbput@i}
%
\def\node@coor#1;#2\@nil{%  for normal nodes (name)
  \pst@getnode{#1}\pst@tempg
  \edef\pst@coor{%
    \pst@nodedict
    tx@NodeDict \pst@tempg known
    \pslbrace \pst@tempg load \tx@GetCenter \psrbrace
    \pslbrace 0 0 \psrbrace ifelse
    end }}
%
\def\Node@coor[#1]#2;#3\@nil{%  for special nodes ([...]{node}node)
\begingroup
\psset{angle=0,#1}%   angle=0, to prevent problems if angle is set globally
\@ifnextchar\bgroup{\Node@@@coor}% we have an additional node [...]{node}
                   {\Node@@coor}#2\@nil% we have  [...]node
\endgroup
\let\pst@coor\pst@tempg}
%
\def\Node@@coor#1\@nil{%
\pst@getnode{#1}\pst@tempg
\xdef\pst@tempg{%
\pst@nodedict
tx@NodeDict \pst@tempg known
  { \psk@nodesepA \psk@angleA 
    \pst@tempg load \psk@nodeseptypeA \tx@GetEdge
    \psk@offsetA \psk@angleA \tx@AddOffset
    \pst@tempg load \tx@GetCenter
    3 -1 roll add 3 1 roll add exch }
  { CP } ifelse end }}
%
\def\Node@@@coor#1{%   [...]{#1}node
\pst@@getcoor{#1}%
\def\psk@angleA{%
  \pst@tempg load \tx@GetCenter \pst@coor
  3 -1 roll sub 3 1 roll sub neg \tx@Atan \psk@angleB add
  }%
\Node@@coor}
%
\def\nput{\pst@object{nput}}
\def\nput@i#1#2{\pst@killglue\pst@makebox{\nput@ii{#1}{#2}}}
\def\nput@ii#1#2{%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi%
  \psset[pstricks]{refangle=#1}%
  \let\psk@angleA\psk@refangle
  \edef\psk@nodesepA{\pst@number\pslabelsep}%
  \def\psk@nodeseptypeA{0 }%
  \pslabelsep\z@
  \uput@vi
  \Node@@coor#2\@nil
  \let\pst@coor\pst@tempg
  \leavevmode
  \psput@special\pst@hbox
  \endgroup
  \ignorespaces}
%  
\newcount\psrow
\newcount\pscol
\newcount\psmatrixcnt
\newskip\psrowsep
\newskip\pscolsep
%
\define@key[psset]{pst-node}{colsep}[1.5cm]{\pssetlength\pscolsep{#1}}
\define@key[psset]{pst-node}{rowsep}[1.5cm]{\pssetlength\psrowsep{#1}}
\psset[pst-node]{colsep=1.5cm}
\psset[pst-node]{rowsep=1.5cm}
\newif\ifpsmatrix
% DG/SR modification begin - Nov. 27, 1998 - Patch 8
%\let\mscount\@multicnt
\ifx\mscount\@undefined\let\mscount\@multicnt\fi
% DG/SR modification end
\def\psmatrix{\begingroup{\ifnum0=`}\fi % Don't want to expand any &.
  \@ifnextchar[{\psmatrix@i}{\ifnum0=`{\fi}{}\psmatrix@ii}}
\def\psmatrix@i[#1]{%
  \ifnum0=`{\fi}{}%
  \psset{#1}%
  \psmatrix@ii}
\def\psmatrix@ii{%
  \KillGlue
  \edef\psm@beginmath{%
    \ifmmode$\m@th\ifinner\textstyle\else\displaystyle\fi\fi}%
  \edef\psm@endmath{\ifmmode$\fi}%
  \let\\\psm@cr
  \advance\psmatrixcnt by \@ne
  \def\psm@thenode{M-\the\psmatrixcnt-\the\psrow-\the\pscol}%
  \tabskip\z@
  \psrow=\@ne
  \pscol\z@
  \psset{shortput=tablr}%
  \leavevmode
  \vbox\bgroup\halign\bgroup&%
  \begingroup
  \global\advance\pscol by \@ne
  \csname psrowhook\romannumeral\psrow\endcsname
  \csname pscolhook\romannumeral\pscol\endcsname
  \psm@beginnode##\psm@endnode\endgroup
  \cr}
%
\def\endpsmatrix{%
  \crcr\egroup\unskip\egroup
  \endgroup}
%
% hv 2007-10-16  fix bug with \\[name=...]
%\def\psm@cr{{\ifnum0=`}\fi\@ifnextchar[{\psm@@cr}{\psm@@@cr{}}}
\def\psm@cr{{\ifnum0=`}\fi\ps@ifnextchar[{\psm@@cr}{\psm@@@cr{}}}
%
\def\psm@@cr[#1]{\psm@@@cr{\vskip#1\relax}}
\def\psm@@@cr#1{%
  \ifnum0=`{\fi}{}\cr
  \noalign{%
  \global\advance\psrow 1
  \global\pscol\z@
  \vskip\psrowsep
  #1}}
\def\psm@beginnode{%
  \@ifnextchar\psm@endnode
    {\let\psm@endnode@i\relax\setbox\pst@hbox=\hbox{}}%
    {\pst@object{psm@beginnode}}}
\def\psm@beginnode@i{%
  \setbox\pst@hbox=\hbox\bgroup
  \psm@beginmath
  \begingroup
  \ignorespaces}
\def\psm@endnode@i{%
  \unskip
  \endgroup
  \psm@endmath
  \egroup
  \use@par
  \@psttrue}
\def\psm@endnode{%
  \@pstfalse
  \psm@endnode@i
  \ifnum\pscol>1\relax \pshskip\pscolsep \fi
  \psk@mnodesize
  \hfil
  \Pst@nodealigntrue
  \if@pst\csname mnode@\psk@mnode\endcsname
  \else\csname mnode@\psk@emnode\endcsname\fi
  \psk@mcol
  \psk@@mnodesize}
% DG/SR modification begin - Sep. 3, 1999 - Patch 10 - From Michael Sharpe
%\def\psspan#1{\mscount#1\relax\loop\ifnum\mscount>\@ne \sp@n\repeat}
\def\psspan#1{\global\mscount#1\relax\pstloop\ifnum\mscount>\@ne\sp@n\repeat}
\def\pstloop#1\repeat{\gdef\pstiterate{#1\relax\expandafter\pstiterate\fi}%
  \pstiterate
  \let\pstiterate\relax}
% DG/SR modification end
\define@key[psset]{pst-node}{name}[\relax]{\pst@getnode{#1}\psk@name}
\let\psk@name\relax
\define@key[psset]{pst-node}{mcol}[c]{%
  \ifx r#1\relax\let\psk@mcol\relax\else
    \ifx l#1\relax\let\psk@mcol\hfill\else
    \let\psk@mcol\hfil\fi\fi}
\psset[pst-node]{mcol=c}
%
\define@key[psset]{pst-node}{mnodesize}[-1pt]{%
  \pssetlength\pst@dimg{#1}%
  \ifdim\pst@dimg<\z@
    \let\psk@mnodesize\relax
    \let\psk@@mnodesize\relax
  \else
    \edef\psk@mnodesize{\noexpand\hbox to\number\pst@dimg sp\noexpand\bgroup}%
    \let\psk@@mnodesize\egroup
  \fi}
\psset[pst-node]{mnodesize=-1pt}
%
\def\mnode@R{\rnode@iii\Rnode@ii{\psm@thenode}}
\def\mnode@r{\rnode@iii\rnode@iv{\psm@thenode}}
\def\mnode@oval{\ovalnode@ii{\psm@thenode}}
\def\mnode@tri{\trinode@ii{\psm@thenode}}
\def\mnode@dia{\dianode@ii{\psm@thenode}}
\def\mnode@C{{\Pst@nodealigntrue\cnode@ii(\z@,\z@){\psk@radius}{\psm@thenode}}}
\def\mnode@f{{\Pst@nodealigntrue\fnode@ii(\z@,\z@){\psm@thenode}}}
\def\mnode@circle{\circlenode@ii{\psm@thenode}}
% hv modification begin - Aug. 16, 2007
\def\mnode@Circle{\Circlenode@ii{\psm@thenode}}
% hv modification end - Aug. 16, 2007
\def\mnode@p{\pnode(\z@,\z@){\psm@thenode}}
% DG/SR modification begin - Jul. 22, 1997 - Patch 1
\def\mnode@dot{\dotnode@ii(\z@,\z@){\psm@thenode}}
% DG/SR modification end
\def\mnode@none{\box\pst@hbox}
%
\define@key[psset]{pst-node}{mnode}[R]{%
  \@ifundefined{mnode@#1}%
    {\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
    {\edef\psk@mnode{#1}}}
\define@key[psset]{pst-node}{emnode}[none]{%
  \@ifundefined{mnode@#1}%
    {\@pstrickserr{\string\psmatrix\space node `#1' not defined.}\@ehpa}%
    {\edef\psk@emnode{#1}}}
\psset[pst-node]{mnode=R,emnode=none}
%
%%%% FROM pst-coil.tex
\def\nccoil{\pst@object{nccoil}}
\def\nccoil@i{\check@arrow{\nccoil@ii}}
\def\nccoil@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{
  \tx@NCCoor
  tx@Dict begin
  4 2 roll
  \psk@coilwidth \pscoilheight
  \psk@coilarmA \psk@coilarmB
  \psk@coilaspect \psk@coilinc
  \pst@coildict \tx@Coil end
  end}%
}
\def\nczigzag{\pst@object{nczigzag}}
\def\nczigzag@i{\check@arrow{\nczigzag@ii}}
\def\nczigzag@ii#1#2{\nc@object{Open}{#1}{#2}{.5}{
  \tx@NCCoor
  tx@Dict begin
  4 2 roll
  \pscoilheight
  \psk@coilwidth
  \psk@coilarmA
  \psk@coilarmB
  \pst@coildict \tx@ZigZag end
  \psline@iii
  \tx@Line
  end}%
}
% \psGetNodeCenter defines the PS variable #1.x and #1.y, which can then
% be used by the user. #1 must be a valid node name
\def\psGetNodeCenter#1{ tx@NodeDict begin /N@#1 load GetCenter end % x y on stack in system coor
  \pst@number\psyunit div /#1.y exch def 	% /#1.y in user coor
  \pst@number\psxunit div /#1.x exch def }	% /#1.x in user coor
%\def\psGetNodeEdgeA#1#2{ tx@NodeDict begin /N@#2 load #2 GetEdgeA end % x y on stack in system coor
%  \pst@number\psyunit div /#1.y exch def 	% /#1.y in user coor
%  \pst@number\psxunit div /#1.x exch def }	% /#1.x in user coor
\def\psGetEdgeA#1#2{
  tx@NodeDict begin \psk@offsetA \psk@offsetB neg 
    \psk@nodesepA \psk@nodesepB 0 0 
    /N@#1 /N@#2 InitNC { NCCoor } if pop pop \tx@UserCoor end}
\def\psGetEdgeB#1#2{
  tx@NodeDict begin \psk@offsetA \psk@offsetB neg 
    \psk@nodesepA \psk@nodesepB 0 0 
    /N@#1 /N@#2 InitNC { NCCoor } if 4 2 roll pop pop \tx@UserCoor end}
%
%%%%%%%%%%%%%% the pst-node-tools part %%%%%%%%%%%%%%%%%%%%%%%%
%
\def\ncbarr{\pst@object{ncbarr}}
\def\ncbarr@i#1#2{%
  \begingroup
  \use@par%
  \psLNode(#1)(#2){0.5}{barr@tempNode}%
  \pst@dimc=\psk@angleA pt
  \pst@dimd=180pt
  % be sure, that angleA is 0 or 180. if not, we set it to 0
  \ifdim\pst@dimc=\z@\else\ifdim\pst@dimc=\pst@dimd\else\psset{angleA=0}\fi\fi
  \ncbar[arrows=-]{#1}{barr@tempNode}
  \ifdim\psk@angleA pt=\z@\relax
    \ncbar[angleA=180,angleB=180]{barr@tempNode}{#2}
  \else\ncbar[angleA=0,angleB=0]{barr@tempNode}{#2}\fi%
  \endgroup%
}
%   #1-------#4----------------#2
% where #1#4= #3 * #1#2
%
\def\psLNode(#1)(#2)#3#4{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /dx XB XA sub def
    /dy YB YA sub def
    XA dx #3\space mul add YA dy #3\space mul add){#4}}
%
% build the linear combination #2*#1+#4*#3=#5
\def\psLCNode(#1)#2(#3)#4#5{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#3}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    XA #2\space mul XB #4\space mul add
    YA #2\space mul YB #4\space mul add){#5}}
%
\def\psLDNode(#1)(#2)#3#4{%  
% #1: node A  #2: node B  #3: dimen measured from A  #4: node name
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pssetlength\pst@dimb{#3}%
  \pnode(!%
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /dx XB XA sub def
    /dy YB YA sub def
    /angle dy dx Atan def
    /linelength \pst@number\pst@dimb \pst@number\psunit div def
    XA linelength angle cos mul add YA linelength angle sin mul add ){#4}%
}
%
\def\psDefBoxNodes#1#2{\rnode[tl]{#1:tl}{\rnode[Bl]{#1:Bl}{\rnode[tr]{#1:tr}{%
\rnode[bl]{#1:bl}{\rnode[Br]{#1:Br}{\rnode[br]{#1:br}{#2}}}}}}%
\pnode(!\psGetNodeCenter{#1:bl}
          \psGetNodeCenter{#1:tl} 
          #1:bl.x #1:tl.x add 2 div #1:bl.y #1:tl.y add 2 div ){#1:Cl}%
\pnode(!\psGetNodeCenter{#1:tr}
          \psGetNodeCenter{#1:br} 
          #1:tr.x #1:br.x add 2 div #1:tr.y #1:br.y add 2 div ){#1:Cr}%
\pnode(!\psGetNodeCenter{#1:Cl}
          \psGetNodeCenter{#1:Cr} 
          #1:Cl.x #1:Cr.x add 2 div #1:Cl.y #1:Cr.y add 2 div ){#1:C}%
\pnode(!\psGetNodeCenter{#1:Br}
          \psGetNodeCenter{#1:Bl} 
          #1:Br.x #1:Bl.x add 2 div #1:Br.y #1:Bl.y add 2 div ){#1:BC}%
\pnode(!\psGetNodeCenter{#1:tr}
          \psGetNodeCenter{#1:tl} 
          #1:tr.x #1:tl.x add 2 div #1:tr.y #1:tl.y add 2 div ){#1:tC}%
\pnode(!\psGetNodeCenter{#1:br}
          \psGetNodeCenter{#1:bl} 
          #1:br.x #1:bl.x add 2 div #1:br.y #1:bl.y add 2 div ){#1:bC}}%
%
%% Author: Michael Sharpe (msharpe at ucsd.edu)
% Macros defined in this file:
% \defaultvalue{<command>}{<value>} assigns <value> to <command> is command is not defined, or is empty.
% \testAlg---used internally to test whether an parametric expression in t is algebraic
% \trim{<command>} trims white space from ends of expansion of <command>
% \hasparen sets \parentrue if its argument contains a (
% \hasequal sets \equaltrue if its argument starts with =
% \equalwhat returns what follows =
% \parsenodexn parses a node expression recursively. Better to use \nodexn.
% \normalvec(<vec>){<nodename>} returns vector normal to <vec> (same length) in <nodename>
% \curvepnode{<t>}{<expression in t>}{<nodename>} Eg, \curvepnode{1}{sin(t) | cos(t)}{P} sets a pnode named P at (cos(1), sin(1))
% \psparnode{<t>}{<expression> in t>}{<nodename>} is called by \curvename if expression is PostScript, not algebraic
% \algparnode{<t>}{<expression> in t>}{<nodename>} is called by \curvename if expression is algebraic, not PostScript
% \nodexn is like \parsenodexn, slightly different syntax. \nodexn{<exn>}{<name>} evaluates <exn> as a node expression and calls the result <name>. 
% \psxline(P){<nodexn1>}{<nodexn2>} draws line from P+<nodexn1> to P+<nodexn2>. The novelty is that the last two arguments can be node expressions.
% \curvepnodes{<tmin>}{<tmax>}{<expression in t>}{<node root name>} Uses current setting of plotpoints (default 50) to define a sequence of pnodes along the curve. Eg, \curvepnodes[plotpoints=100]{0}{1}{t+t^2 | Ex(-t)}{P} sets pnodes P0..P99 at equally spaced t values along the curve, and defines the macro \Pnodecount to 99, the highest index. The expression in t may be either algebraic or PostScript, and is handled automatically detected.
% \fnpnode{<xval>}{<expression in x>}{<nodename>} sets a single pnode on graph. Eg, \fnpnode{.5}{x 2 mul x 1 add mul}{P} declares the pnode P at the point x=0.5 on the graph. (Same as \pnode(!/x 0.5 def x x 2 mul x 1 add mul}){P}.) If your expression in t is algebraic, you must use the keyword algebraic, as in \fnpnode[algebraic]{0.5}{2*x*(x+1)}{P}.
% \fnpnodes{<xmin}{<xmax>}{<expression in x>}{<node root name>} Is exactly the same as \curvenodes, but for the graph of a function. The keyword algebraic must be specified if your expression is algebraic
% \AtoB(A)(B){C} defines node by name C essentially as B-A
% \AplusB(A)(B){C} defines node by name C essentially as A+B
% \midAB(A)(B){C} defines node by name C essentially as (A+B)/2
% \psnline[linewidth=1pt,arrows=->](3,5){P}, for example, expects that there are pnodes named P3..P7 (total of 5), and effectively gives the same result as \psline[linewidth=1pt,arrows=->](P3)(P4)(P5)(P6)(P7). Note that arrow must be specified with a keyword, not as an argument.
% \shownode(P) displays in the console window the coordinates of node P. This will not appear until the final stage of processing the PostScript file. It is a debugging tool.
% \getnodelist{<node root name>}{<next command>} is useful in writing pstricks macros, where there is a list of parenthesized coordinates to be read and turned into a node sequence, following which <next command> is followed.
% \pnodes{P}(1,2)(2;3)... is effectively \getnodelist{P}{}(1,2)(2;3)..., just a quick way to turn a list of coordinates into pnodes P0 P1 ...
% \psLCNodeVar is similar to \psLCNode, and provides a means of forming a linear combination of two nodes, thought of as vectors. Where \psLCNode(A){a}(B){b}{C} effectively makes C=aA+bB, \psLCNodeVar(A)(B)(a,b){C} does the same, but the third argument (a,b) may be specified in PostScript code or any form recognized by \SpecialCoor. Unlike \psLCNode, the name C may be one of A, B.
% \psRelNodeVar is similar to \psRelNode, and provides a means of rotating and changing the length of a line segment AB about A. The effect of \psRelNodeVar(A)(B)(2;30){C} is the same as \psRelNode[angle=30](A)(B){2}{C}, but the third argument (2;30) may be specified in PostScript code, which is not possible with \psRelNode.
% \psRelLineVar stands to \psRelLine as \psRelNodeVar stands to \psRelNode.
% \rhombus{<edge length>}(A)(B){C}{D} computes the two remaining vertices C, D given two opposing vertices A, B of a rhombus with given edge length. It does not draw the rhombus--- that can be handled easily by \pspolygon(A)(C)(B)(D).
% \psrline(P)(Q)... is like \psline, drawing a line starting at (P), with successive increments (Q)... It has the same options as \psline. Eg, \psrline[linecolor=red]{->}(1,1)(1,0)
% \polyIntersection is the most complicated macro in the collection. It has two forms
% \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B)(1,2)(3;30)(6,5)...
%works with the line starting at A heading toward B, and computes the first point that lies on the polyline (1,2)(3;30)(6,5)..., calling it <Nodename1>. It also computes the first point in the opposite direction (from A) lying on that polyline, naming it <Nodename2>. If one or other of these intersections is empty, the nodes are set to remote points on the line. The two nodes are then joined by a line. The effect depends on the location of A and B relative to the polyline, with two cases worth noting.
% (a) if the polyline is closed and if A, B are interior to one of its components, you get a line segment from one edge to the other, containing AB.
% (b) If the polylne is simple and closed, and one of A, B is inside and the other outside, the resulting line segment will contain A but not B. 
% \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B){P}{n} works exactly the same as \polyIntersection{<Nodename1>}{<Nodename2>}(A)(B)(P0)(P1)...(Pn), assuming P0...Pn are previously defined as pnodes.
% \psStepa is like \psStep (pstricks-add) but for a node sequence rather than equally spaced abscissas. \psStepa[options]{<node root>}{<maxindex>} draws a step function with jumps at the successive nodes in the node sequence. Eg, \psStepa{P}{10} has jumps at P0..P10
%
\newcount\pst@args%used in several macros
\newcount\num@pts
\newcount\pst@argcnt% for use in parsing node expressions
\def\PST@root{}
\let\pst@next\relax
%my scratch variables
\def\my@tempA{}
\def\my@tempB{}
\def\my@tempC{}
\def\my@tempD{}
\def\my@next{}
\newif\if@paren%
\newif\if@equal%
\newif\if@colon%
\newif\ifshow
\def\plussign{+}\def\minussign{-}
%
%
\def\defaultvalue#1#2{%#1 is a command, #2 is a value, possibly a command
  \ifdefined#1\ifx#1\@empty\xdef#1{#2}\fi\else\xdef#1{#2}\fi}%
%
\def\testAlg#1|#2\@nil{%
\ifx\relax#2\relax%
   \let\my@next\psparnode\xdef\my@tempD{}%
\else%
   \let\my@next\algparnode\xdef\my@tempD{A}% algebraic
\fi}%
%
%Jonathan Fine's trim
\def\trim #1{\expandafter\trim@\expandafter{#1 }#1}%
\def\trim@ #1{\trim@@ @#1 @ #1 @ @@}%
\def\trim@@ #1@ #2@ #3@@{\trim@@@\empty #2 @}%
\def\unbrace#1{#1}%
\unbrace{\def\trim@@@ #1 } #2@#3{\expandafter\def%
  \expandafter #3\expandafter {#1}}%
%
\def\hasparen#1(#2\@nil{%check if expression contains a (--call with \hasparen#1(\@nil
  \ifx\relax#2\relax \@parenfalse \else \@parentrue\fi}%
%
\def\hasequal#1=#2\@nil{%check if expression contains a =--call with \hasequal#1=\@nil
  \ifx\relax#2\relax \@equalfalse \else \@equaltrue\fi
  \hascolon#2:\@nil}%
%
\def\hascolon#1:#2\@nil{%check if expression contains a :--call with \hascolon#1:\@nil
\ifx\relax#2\relax \@colonfalse \else \@colontrue\fi}%
%
\def\equalwhat#1=#2:#3\@nil{{#2}{#3}}%
%
\def\parsenodexn#1(#2)#3\@nil{%
  \def\coeffA{#1}\edef\nodeA{#2}%
  \trim\coeffA%
  \ifx\nodeA\@empty\else%
    \pnode(#2){@@TMP}%
    \ifx\coeffA\@empty\def\coeffA{1}\else%
      \ifx\coeffA\plussign\def\coeffA{1}\else\ifx\coeffA\minussign\def\coeffA{-1}\fi\fi\fi% 
  \edef\cmd{\noexpand\psLCNode(@TMP\the\pst@argcnt){1}(@@TMP){\coeffA}{@TMP}}%
  \cmd%
  \advance\pst@argcnt by \@ne%
  \pnode(@TMP){@TMP\the\pst@argcnt}%
  \parsenodexn#3\@nil%
  \fi}%
%
\def\normalvec(#1)#2{%
%pnode | new pnode normal to old, same  length
  \psRelNodeVar(0,0)(#1)(0,1){#2}}%
%
\def\curvepnode#1#2#3{%
% #1=t value, #2=x(t) y(t) in either form,#3=node name,
%must first detect which form of x(t) y(t), looking for |
  \edef\my@tempA{#2}% x(t) y(t) expanded
  \expandafter\testAlg\my@tempA|\@nil\my@next {#1}{#2}{#3}}
%
\def\psparnode#1#2#3{%
% #1=t value, #2=x(t) y(t) in PS form,#3=node name,
  \pnode(!/t #1 def #2){#3}%
  \pnode(!/t #1 .001 sub def #2 
          /t #1 .001 add def 
           #2 3 -1 roll sub 3 1 roll sub neg 
           2 copy Pyth dup 3 1 roll div 3 1 roll div ){#3tang}}%unit tangent vector at t
%
\def\algparnode#1#2#3{%
% #1=t value, #2=x(t) | y(t) in alg form,#3=node name,
%\pstVerb{tx@Dict begin /t #1 def /Func (#2) AlgParser cvx def end}
%\pnode(!Func){#3}}%
  \pstVerb{tx@Dict begin /Func (#2) AlgParser cvx def end }
  \pnode(!/t #1 def Func){#3}
  \pnode(!/t #1 .001 sub def Func 
          /t #1 .001 add def 
          Func 3 -1 roll sub 3 1 roll sub neg 
          2 copy Pyth dup 3 1 roll div 3 1 roll div ){#3tang}%unit tangent vector at t
}%
%
\def\nodex#1{%
%#1=node expression --set nodename to @TMP
\expandafter\hasparen#1(\@nil%
\if@paren%it's an expression
  \pnode(0,0){@TMP0}%
  \pst@argcnt=0%
  \expandafter\parsenodexn#1()\@nil%
\else%
  \def\my@tempC{#1}%
  \ifx\my@tempC\@empty\pnode(0,0){@TMP}\else\pnode(#1){@TMP}\fi%
\fi}%\if@paren
%
\def\nodexn#1#2{%
%#1=node expression | #2=node name
\expandafter\hasparen#1(\@nil%%%      hv 20130917 use \expandafter
\if@paren%it's an expression
  \pnode(0,0){@TMP0}%
  \pst@argcnt=0%
  \parsenodexn#1()\@nil%
  \pnode(@TMP){#2}%
\else%
  \def\my@tempC{#1}%
  \ifx\my@tempC\@empty\pnode(0,0){#2}\else\pnode(#1){#2}\fi%
\fi}%\if@paren
%
\def\psxline{\pst@object{psxline}}%
\def\psxline@i{\@ifnextchar({\psxline@iii}{\psxline@ii}}%
\def\psxline@ii#1{%
\addto@par{arrows=#1}%
\psxline@iii}%
\def\psxline@iii(#1)#2#3{{%#1=basepoint, #2,#3 node expressions
\pst@killglue%
\use@par%
\nodexn{#2}{@TMP@a}%
\AplusB(#1)(@TMP@a){@TMP@A}%
\nodexn{#3}{@TMP@a}%
\AplusB(#1)(@TMP@a){@TMP@B}%
\psline(@TMP@A)(@TMP@B)%
}%
\ignorespaces}%
%
\def\curvepnodes{\pst@object{curvepnodes}}
\def\curvepnodes@i#1#2#3#4{{%optional [plotpoints=xx]
%  #1=tmin,#2=tmax,#3=function (of t),#4=node root name,
  \pst@killglue
  \use@par
  \edef\my@tempA{#3}% x(t) y(t) expanded
  \expandafter\testAlg\my@tempA|\@nil %
  \pstVerb{% 
	tx@Dict begin % so we can use definitions from tx@Dict
	/t0 #1 def
	/t1 #2 def  
	 t1 t0 sub end \psk@plotpoints div /dt exch def }%
  \pst@cntc=\psk@plotpoints\relax%\psk@plotpoints=plotpoints-1
  \advance\pst@cntc by \@ne\relax %=plotpoints
  \ifx\my@tempD\@empty\pstVerb{tx@Dict begin /Func (#3) cvx def end }%add tx@Dict
  \else\pstVerb{tx@Dict begin /Func (#3 ) AlgParser cvx def end }%
  \fi%
    \multido{\i=0+1}{\pst@cntc}{%
      \pnode(! /t #1 dt \i\space mul add def Func ){#4\i}}% remove t before Func
    \expandafter\xdef \csname #4nodecount\endcsname {\psk@plotpoints}%
    \ifnum\Pst@Debug>0 \typeout{Created nodes #40 .. #4\psk@plotpoints}\fi%
}\ignorespaces}%
%
\def\fnpnode{\pst@object{fnpnode}}
\def\fnpnode@i#1#2#3{{%optional [algebraic]
%#1=x value | #2=fn of x | #3=node name
  \pst@killglue
  \use@par
  \ifPst@algebraic\pnode(*#1 {#2}){#3}\else\pnode(! /x #1 def x #2){#3}\fi
}\ignorespaces}%
%
\def\fnpnodes{\pst@object{fnpnodes}}
\def\fnpnodes@i#1#2#3#4{{%optional [algebraic]
%#1=xmin | #2=xmax | #3= fn of x | #4=node name
\pst@killglue
\use@par
\pst@dima=#1pt \pst@dimb=#2pt \advance\pst@dimb -\pst@dima%
\pst@cnta=\psk@plotpoints \relax %=plotpoints-1
\def\PST@root{#4}
\divide\pst@dimb by \pst@cnta%plotpoint-1 intervals
\pst@cntc=\pst@cnta %
\advance\pst@cntc by 1 \relax %=plotpoints
\ifPst@algebraic 
  \multido{\i=0+1}{\pst@cntc}{\pnode(*{\pst@number\pst@dima} {#3}){#4\i}%  hv 20130713
  \advance\pst@dima \pst@dimb}%
\else
    \multido{\i=0+1}{\pst@cntc}{\pnode(!/x \pst@number\pst@dima\space def x #3){#4\i}%
  \advance\pst@dima \pst@dimb}%
\fi%
  \expandafter\xdef \csname \PST@root nodecount\endcsname {\the\pst@cnta}%
  \ifnum\Pst@Debug>0 \typeout{Created nodes #40 .. #4\the\pst@cnta}\fi%
}\ignorespaces}%
%
\def\AtoB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(-1,1){#3}}
\def\AplusB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(1,1){#3}}
\def\midAB(#1)(#2)#3{\psLCNodeVar(#1)(#2)(.5,.5){#3}}
%
\def\psnline{\pst@object{psnline}}%line of nodes
\def\psnline@i{\pst@getarrows{\psnline@ii}}
\def\psnline@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\edef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\psline\@tmp}%
\ignorespaces}%
%
\def\psncurve{\pst@object{psncurve}}%line of nodes
\def\psncurve@i{\pst@getarrows{\psncurve@ii}}
\def\psncurve@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\edef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\pscurve\@tmp}%
\ignorespaces}%
%
\def\psnccurve{\pst@object{psnccurve}}%line of nodes
\def\psnccurve@i{\pst@getarrows{\psnccurve@ii}}
\def\psnccurve@ii(#1,#2)#3{{%
\pst@killglue%
\use@par%
\pst@cnta=#2 \relax\advance\pst@cnta by 1
\xdef\@tmp{}%
\multido{\i=#1+1}{\pst@cnta}{\xdef\@tmp{\@tmp(#3\i)}}%
\expandafter\psccurve\@tmp}%
\ignorespaces}%
%
\def\shownode(#1){%display node user coords in console
  \pst@killglue%
  \pstVerb{% 
    gsave tx@Dict begin %
    tx@NodeDict /N@#1 known { % known node
      /tmpar [(Node #1: ) <28> () (, ) () <29>] def %
      /str 12 string def 
      STV CP T \psGetNodeCenter{#1}\space 
      tmpar 2 #1.x str cvs put 
      /str 12 string def 
      tmpar 4 #1.y str cvs put 
      tmpar concatstringarray = }%
    {% not known
      (Node #1: (NOT KNOWN)) = %
    } ifelse %
    end grestore }%
  \ignorespaces}%
%
% Use to construct a sequence of nodes
% Eg, \pnodes{P}(0,1)(2;5)(3,4) defines nodes P0, P1, P2 with respective locations
% and a macro \Pnodecount containing the highest index created
\def\pnodes@ii#1{\getnodelist{#1}{}}
%
\def\getnodelist#1#2{%
\pst@args=0 \relax%
\def\PST@root{#1}%
\def\pst@next{#2}% command to perform after reading list
\getnext@Node}%
%
\def\getnext@Node{\@ifnextchar({\getnext@Node@i}%
  {\advance\pst@args by \m@ne \expandafter\xdef \csname \PST@root nodecount\endcsname {\the\pst@args}
  \ifnum\Pst@Debug>0 \typeout{Created nodes \PST@root0 .. \PST@root\the\pst@args}\fi% 
  \pst@next}%
}%
%
\def\getnext@Node@i(#1){%
\pnode(#1){\PST@root\the\pst@args}%
\advance\pst@args by \@ne\relax%
\getnext@Node}%
%
\def\psLCNodeVar(#1)(#2)(#3)#4{%
\pst@getcoor{#1}\my@tempA%
\pst@getcoor{#2}\my@tempB%
\pnode(#3){tmpLCn@de}%
\pnode(!%
  \my@tempA /YA exch \pst@number\psyunit div def
  /XA exch \pst@number\psxunit div def
  \my@tempB /YB exch \pst@number\psyunit div def
  /XB exch \pst@number\psxunit div def %stack now empty
  \psGetNodeCenter{tmpLCn@de}\space
  XA tmpLCn@de.x mul XB tmpLCn@de.y mul add
  YA tmpLCn@de.x mul YB tmpLCn@de.y mul add){tmpLCn@deA}%
\pnode(tmpLCn@deA){#4}%
}%
%
\def\psRelNodeVar{\pst@object{psRelNodeVar}}
\def\psRelNodeVar@i(#1)(#2)(#3)#4{{% A - B - factor;angle - node name
  \use@par
  \pst@getcoor{#1}\my@tempA%
  \pst@getcoor{#2}\my@tempB%
   \pnode(#3){tmpn@de}%
\pnode(!
  /unit \pst@number\psyunit \pst@number\psxunit div def % yunit/xunit
    \my@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \my@tempB /YB exch \pst@number\psyunit div YA sub 
    \ifPst@trueAngle\space unit mul \fi\space def
    /XB exch \pst@number\psxunit div XA sub def
    %complex multiply (XB,YB) and (P.x,P.y), then add (XA,YA)
    \psGetNodeCenter{tmpn@de}
    XB tmpn@de.x mul YB tmpn@de.y mul sub
    YB tmpn@de.x mul XB tmpn@de.y mul add
    \ifPst@trueAngle\space unit div \fi\space 
   YA add exch XA add exch %x, y coords on stack
    ){#4}%
}}
%
\def\psRelLineVar{\pst@object{psRelLineVar}}
\def\psRelLineVar@i{\@ifnextchar({\psRelLineVar@iii}{\psRelLineVar@ii}}
\def\psRelLineVar@ii#1{%
  \addto@par{arrows=#1}%
  \psRelLineVar@iii}
\def\psRelLineVar@iii(#1)(#2)(#3)#4{{%
  \pst@killglue
  \use@par
  \psRelNodeVar(#1)(#2)(#3){#4}%
  \psline(#1)(#4)%
}\ignorespaces}
%
\def\rhombus#1(#2)(#3)#4#5{% \rhombus{m}(B)(D){A}{C} 
\AtoB(#2)(#3){node@P}% P=BD
% compute angle between BD and BC, in Postscript
\pnode(! %compute angle and scale in PS
/tmp \psGetNodeCenter{node@P} node@P.x node@P.y 
Pyth 2 div def %tmp=half-length of BD
/ang tmp #1\space div Acos def %ang=angle from BD to BC & BA
#1\space tmp 2 mul div %scale factor s=m/BD
dup ang cos mul exch ang sin mul ){node@A1}% s cos(ang), s sin(ang)
\pnode(! \psGetNodeCenter{node@A1} node@A1.x node@A1.y neg ){node@A2}%reflect in x axis
\psRelNodeVar(#2)(#3)(node@A1){#4}%
\psRelNodeVar(#2)(#3)(node@A2){#5}%
}%
%
\def\psrline{\pst@object{psrline}}% relative lines
\def\psrline@i{\@ifnextchar({\psrline@iii}{\psrline@ii}}%
\def\psrline@ii#1{%
\addto@par{arrows=#1}%
\psrline@iii}%
\def\psrline@iii{%
\getnodelist{@tmpnode}{\psrline@iv}%
}%
\def\psrline@iv{%
   \ifnum\pst@args<0\else%do nothing
      \pnode(@tmpnode0){@tmpnodeB0}%
      \multido{\iA=1+1,\iB=0+1}{\pst@args}{%
      \AplusB(@tmpnodeB\iB)(@tmpnode\iA){@tmpnodeB\iA}}%
      \psrline@v%
   \fi%
}%
\def\psrline@v{{%finish up
  \pst@killglue%
  \use@par%
  \xdef\tmp{(@tmpnodeB0)}%
  \multido{\i=1+1}{\pst@args}%
{\xdef\tmp{\tmp(@tmpnodeB\i)}}%
\expandafter\psline\tmp%
}\ignorespaces}%
%
\def\polyIntersections#1#2(#3)(#4){%
%nodename1 | nodename2 | A | B | % intersections with line from A, B 
\def\nodenameA{#1}\def\nodenameB{#2}%
\pnode(#3){P@A}\pnode(#4){P@B}%
\@ifnextchar({\polyIntersections@next}{\polyIntersections@ii}%
}%
\def\polyIntersections@ii#1#2{%
\def\root@node{#1}\num@pts=#2 \relax%
\polyIntersections@iii}% 
%
\def\polyIntersections@next{%read as many points as exist
\def\root@node{P@}\getnodelist{P@}{\num@pts=\pst@args \relax\polyIntersections@iii}%
}%
\def\polyIntersections@iii{%nodes are now XXX0....XXXn, n=num@pts
\pst@cnta=\num@pts \relax\advance\pst@cnta by 1 \relax%
\pstVerb{%
 /xarray \the\pst@cnta\space array def
 /yarray \the\pst@cnta\space array def  tx@Dict begin }%
\multido{\i=0+1}{\the\pst@cnta}{\pstVerb{ \psGetNodeCenter{\root@node\i} xarray \i\space \root@node\i.x put yarray \i\space \root@node\i.y put }}%
\pstVerb{ /tposmin 100 def /tnegmax -100 def %/argposmin 0 def /argposmax 0 def 
\psGetNodeCenter{P@B} \psGetNodeCenter{P@A} 
/dx P@B.x P@A.x sub def 
/dy P@B.y P@A.y sub def 
/lenAB dx dy Pyth def
/oldx xarray 0 get def /oldy yarray 0 get def 
1 1 \the\num@pts\space {/k exch def /newx xarray k get def /newy yarray k get def 
/ddx newx oldx sub def /ddy newy oldy sub def 
/det ddy dx mul ddx dy mul sub def
det abs lenAB ddx ddy Pyth mul .001 mul gt 
{/ac oldx P@A.x sub def /bd oldy P@A.y sub def 
 /tt  ac ddy mul bd ddx mul sub det div def %solve for t value at intersection
 /ss ac  dy mul bd dx mul sub det div def % solve for s value at intersection
ss 0 ge 
   {ss 1 le 
        {tt 0 lt {tt tnegmax gt {/tnegmax tt def} if } {tt tposmin lt {/tposmin tt def} if } ifelse }
    if } % ss 1 le
if }%ss 0 ge
 if %det>
 /oldx newx def /oldy newy def} for end }%
\pnode(! \psGetNodeCenter{P@A} \psGetNodeCenter{P@B} P@B.x P@A.x sub  tposmin mul P@A.x add  P@B.y P@A.y sub tposmin  mul P@A.y add ){\nodenameA}%
\pnode(! \psGetNodeCenter{P@A} \psGetNodeCenter{P@B} P@B.x P@A.x sub tnegmax mul P@A.x add P@B.y P@A.y sub tnegmax mul P@A.y add){\nodenameB}%
}%
%
\def\actualscale#1 #2 scale{% extract x-scale from, eg,  {2. 2. scale}
#1}
%
\def\psGetCenter#1{ tx@NodeDict begin /N@#1 load GetCenter end }% x y on stack in system coor
%
\def\ArrowNotch{\pst@object{ArrowNotch}}
\def\ArrowNotch@i#1#2#3#4{{%
%noderootname | index | arrowdirection | notchnodename  % 
\pst@killglue%
\use@par%
\def\inc{-1}%
\ifx#3<\def\inc{1}\fi% -1 means notch to left of arrowhead
%get length of pointed arrow under these conditions (types ->, -D> and their reverses)
\pstVerb{ 
    1 \psk@arrowinset\space sub \psk@arrowlength\space \psk@arrowsize\space  
    \pst@number\pslinewidth \space mul add  mul mul 
    \expandafter\actualscale\psk@arrowscale \space  mul 
    /hh exch def /hh1 hh .05 sub def }% PS variable hh contains dist from tip to notch of arrow, in pts
\def\root@node{#1}\num@pts=\csname\root@node nodecount\endcsname %
\pst@cntb=\num@pts \advance\pst@cntb by \@ne%actual node count
\pst@cnta=\num@pts \advance\pst@cnta by \thr@@%size of PS array
\pst@cntc=#2 \relax% index of center of circle
\ifnum\pst@cntc>\num@pts \pnode(0,0){#4}\else
%compute a (screen based) unit vector in directions P1P0 and Pn-1Pn
\pstVerb{%
/PythSq { dup mul exch dup mul add } def
/PtSub {					%  xA yA xB yB
  3 -1 roll 		% xA xB yB yA
  sub neg		% xA xB yA-yB
  3 1 roll 		% yB-yA xA xB
  sub			% yB-yA xA-xB
  exch                     % xB-xA yA-yB
} def
  /xarray \the\pst@cnta\space array def
  /yarray \the\pst@cnta\space array def  
  tx@Dict begin }% end pstVerb
\multido{\i=0+1,\ib=1+1}{\the\pst@cntb}{\pnode(! \psGetCenter{\root@node\i}\space  % center on stack in system coords, not user coords
yarray \ib\space 3 -1 roll put xarray \ib\space 3 -1 roll put 0 0 ){@tmp}}% end multido
%\pstVerb{ \psGetCenter{\root@node6} == == }
\pnode(! xarray 1 get dup yarray 1 get dup 3 1 roll % x1 y1 x1 y1
xarray 2 get yarray 2 get PtSub  % x1 y1 x1-x2 y1-y2
2 copy Pyth hh div 2 div dup % x1 y1 x1-x2 y1-y2 d d ,d->d/2*hh
3 1 roll % x1 y1 x1-x2 d y1-y2 d
div 3 1 roll div %x1 y1  (y1-y2)/d (x1-x2)/d
3 1 roll %x1  (x1-x2)/d y1  (y1-y2)/d
add 3 1 roll add %  y1-(y2-y1)/d x1-(x2-x1)/d
 xarray 0 3 -1 roll put yarray 0 3 -1 roll put %stack empty
 xarray length 2 sub /topnum exch def 
 xarray topnum get dup yarray topnum get dup 3 1 roll %xn yn xn yn
topnum 1 sub /topnum exch def xarray topnum get yarray topnum get % xn yn xn yn x(n-1) y(n-1)
3 -1 roll sub  neg 3 1 roll sub exch % xn yn (xn-x(n-1)) (yn-y(n-1))
2 copy Pyth hh div 2 div dup % xn yn (xn-x(n-1)) (yn-y(n-1)) d d (d->d/(2*h))
3 1 roll div 3 1 roll div %xn yn (xn-x(n-1))/d (yn-y(n-1))/d
3 -1 roll add 3 1 roll % y(n+1) x(n+1)
topnum 2 add /topnum exch def xarray topnum 3 -1 roll put yarray topnum 3 -1 roll put % empty
% next step--find first index outside circle of radius hh 
 /oldcindex \the\pst@cntc\space 1 add def %position in array
 xarray oldcindex get /xc exch def yarray oldcindex get /yc exch def
 %hh .05 sub /hh exch def % that's close enough for a crossing
/inc \inc\space def %+1 for left facing arrow, else -1 
/cindex oldcindex def 
{cindex inc add /cindex exch def xarray cindex get xc sub yarray cindex get yc sub Pyth dup hh1 gt 
{ exit } if } loop % exit from loop with cindex the first index of an external point--dist on stack
 hh1 .1 add lt { xarray cindex get yarray cindex get } %else within segment
{ xarray cindex inc sub get dup yarray cindex inc sub get dup 4 -1 roll exch 
xarray cindex get yarray cindex get PtSub /dy1 exch def /dx1 exch def dx1 dy1 PythSq /Aterm exch def 
% dx1=x(n-1)-x(n), dy1=y(n-1)-y(n) [if inc=1]: dx1=x(n+1)-x(n), dy1=y(n+1)-y(n) [if inc=-1]
% x(n-inc) y(n-inc),  Aterm=dx1^2+dy1^2
 2 copy xc yc PtSub % x(n-inc) y(n-inc) (x(n-inc)-xc) (y(n-inc)-yc)
 2 copy 2 copy 3 -1 roll mul 3 1 roll mul add hh dup mul sub % x(n-inc) y(n-inc) (y(n-inc)-yc) (x(n-inc)-xc) (x(n-inc)-xc)^2+(y(n-inc)-yc)^2-hh^2
 Aterm div /Cterm exch def  % x(n-inc) y(n-inc)  (y(n-inc)-yc) (x(n-inc)-xc) , Cterm=((x(n-inc)-xc)^2+(y(n-inc)-yc)^2-hh^2)/(Aterm) (<0)
 dx1 dy1 %  x(n-inc) y(n-inc) (y(n-inc)-yc)  (x(n-inc)-xc)  dx1 dy1
 4 1 roll mul 3 1 roll mul add Aterm div /Bterm exch def %   x(n-inc) y(n-inc) , Bterm=( (x(n-inc)-xc)*dx1+(y(n-inc)-yc)*dy1)/Aterm
 Bterm abs neg dup dup mul Cterm sub sqrt add dup /tval exch def
% x(n-inc) y(n-inc) tvalue
 dup dx1 dy1 4 1 roll mul 3 1 roll mul  % x(n-inc) y(n-inc) t*dx1 t*dy1
 PtSub } ifelse % x y screen coords of arrow notch now on stack---convert to user x y
 \pst@number\psyunit div exch \pst@number\psxunit div exch  %use coords now on stack
){#4}\fi%
\pstVerb { end } %tx@Dict
}\ignorespaces}%
%
%
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-node.tex


==> pst-plot.tex <==
%% BEGIN pst-plot.tex
%%
%% plotting functions and data with PSTricks.
%% See the betadoc documentation for usage. 
%%
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2009-2014 by Herbert Voss, hvoss@tug.org.
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
%
\csname PSTplotLoaded\endcsname
\let\PSTplotLoaded\endinput
%
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey.tex\fi
\ifx\PSTtoolsloaded\endinput\else\input pst-tools.tex\fi
\ifx\PSTFPloaded\endinput\else   \input pst-fp.tex  \fi
\ifx\MultidoLoaded\endinput\else \input multido.tex \fi
%
\def\fileversion{1.62}
\def\filedate{2014/05/12}
\message{ v\fileversion, \filedate\space (tvz,hv)}
%
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11
%
\pst@addfams{pst-plot}
%
\def\pst@linetype{2}%
\SpecialCoor
%
\def\psPiFour{12.566371}
\def\psPiTwo{6.283185}
\def\psPi{3.14159265}
\def\psPiH{1.570796327}
\newdimen\pstRadUnit
\newdimen\pstRadUnitInv
\pstRadUnit=1.047198cm % this is pi/3
\pstRadUnitInv=0.95493cm % this is 3/pi
%
% Using lists of data is optimized for \dataplot and \fileplot
% Here is the tricky part. As each line is read from file,
% we want to ignore trailing delimiters, and convert arbitrary
% strings of non-trailing delimiters to _D_.
% We end up with
%   D x1 D y1 D x2 D y2 ... D xn D yn
%
\begingroup
\catcode`\{=13
\catcode`\}=13
\catcode`\(=13
\catcode`\)=13
\catcode`\,=13
\catcode`\!=1
\catcode`\*=2
\catcode`\ =13
\catcode`\_=13
\catcode`\^^M=13
\gdef\pst@datadelimiters!% Begin def
\catcode`\{=13%
\catcode`\}=13%
\catcode`\(=13%
\catcode`\)=13%
\catcode`\,=13%
\catcode`\ =13%
\catcode`\^^M=13%
\def,##1!%
\ifcat\noexpand,\noexpand##1%
\expandafter##1%
\else\space%
D\space##1%
\fi*%
\let(,\let),\let{,\let},\let ,\let^^M,\let_\@empty*% End def
\endgroup
\define@key[psset]{pst-plot}{ignoreLines}[0]{\def\psk@ignoreLines{#1}}
\psset[pst-plot]{ignoreLines=0}
%
\newcount\pst@linecnt
\begingroup
\catcode`\,=13
\catcode`\_=13
\gdef\savedata@#1[#2]{%
  \xdef\pst@tempg{#2_}%
  \endgroup
  \let#1\pst@tempg
  \global\let\pst@tempg\relax
  \ignorespaces}
%
\gdef\readdata@{%
  \read1 to \pst@tempA
  \ifnum\pst@linecnt=\psk@nStep
    \global\pst@linecnt=0
    \expandafter\readdata@@\pst@tempA_\@nil
  \fi
  \global\advance\pst@linecnt by 1
  \ifeof1\else\expandafter\readdata@\fi}
\gdef\pst@@readfile#1#2\@nil{\addto@pscode{,#1#2}}%
\gdef\readdata@@#1#2\@nil{\xdef\pst@tempg{\pst@tempg,#1#2}}%
\endgroup
%
\def\readdata{\@ifnextchar[{\readdata@i}{\readdata@i[]}}
\def\readdata@i[#1]#2#3{%
%  \def\pst@tempA{#1}%
  \openin1=#3
  \begingroup
  \ifx#1\relax#1\else\psset{#1}\fi
  \def\pst@tempg{}%
  \ifeof1
    \@pstrickserr{Data file `#3' not found.}\@ehpa
  \else
    \pst@datadelimiters
    \catcode`\[=1
    \catcode`\]=2
    \pst@cnta=0
    \loop \ifnum\the\pst@cnta<\psk@ignoreLines
      \advance\pst@cnta by 1\relax
      \read1 to \pst@tempA
    \repeat
    \psDEBUG[pst-plot]{>>> ignored \the\pst@cnta\space data lines}%
    \global\pst@linecnt=\psk@nStep%
    \readdata@%
  \fi%
  \endgroup%
  \global\let#2\pst@tempg%
  \global\let\pst@tempg\relax%
\ignorespaces}
%
\def\pst@readfile#1{{\let\readdata@@\pst@@readfile\readdata\pst@tempg{#1}}}
\def\pst@altreadfile#1{%
  \openin1=#1
  \ifeof1
    \@pstrickserr{Data file `#1' not found.}\@ehpa
  \else
    \catcode`\{=10
    \catcode`\}=10
    \catcode`\(=10
    \catcode`\)=10
    \catcode`\,=10
    \catcode`\^^M=10
    \catcode`\[=1
    \catcode`\]=2
    \pst@@altreadfile
  \fi}
\def\pst@@altreadfile{%
  \read1 to \pst@tempg
  \expandafter\pst@@@altreadfile\pst@tempg\@empty\@nil
  \ifeof1\else\expandafter\pst@@@altreadfile\fi}
\def\pst@@@altreadfile#1#2\@nil{\addto@pscode{#1#2}}%
%
\def\savedata#1{\begingroup\pst@datadelimiters\savedata@{#1}}
%
\newread\RCD@file
\def\psreadDataColumn#1#2#3#4{%    #1:column #2:delimiter #3:\result #4:data file
  \immediate\openin\RCD@file=#4\relax
  \global\let#3=\@empty
  \loop
    \read\RCD@file to \@tempa
  \ifeof\RCD@file\else
    %%%\typeout{*** \@tempa ***}%
    \edef\@tempa{\@tempa#2}%
    \def\reserved@b{}%
    \@tempswafalse
    \@tempcnta=#1\relax
    \expandafter\@tfor\expandafter\reserved@a
      \expandafter:\expandafter=\@tempa\do{% loop over every token
      \if\reserved@a#2\relax%                delimiter?
        \advance\@tempcnta \m@ne
        \ifnum \@tempcnta=\z@
          \expandafter\g@addto@macro\expandafter#3\expandafter{\reserved@b\space}%
          \@tempswatrue
        \fi
        \def\reserved@b{}% ???
      \else
        \edef\reserved@b{\reserved@b\reserved@a}
      \fi
      \if@tempswa\@break@tfor\fi
    }%
  \repeat
  \immediate\closein\RCD@file
}

%%%%%%%%%%%%%% the plot-styles %%%%%%%%%%%%%%%%%%
%
\def\beginplot@line{\begin@OpenObj}
\def\endplot@line{\psline@ii}
%
\def\beginplot@polygon{\begin@ClosedObj}
\def\endplot@polygon{\pspolygon@ii}
%
\def\beginplot@curve{\begin@OpenObj}
\def\endplot@curve{\pscurve@ii}
%
\def\beginplot@ecurve{\begin@OpenObj}
\def\endplot@ecurve{\psecurve@ii}
%
\def\beginplot@ccurve{\begin@ClosedObj}
\def\endplot@ccurve{\psccurve@ii}
%
\def\beginplot@dots{\begin@SpecialObj}
\def\endplot@dots{\psdots@ii}
%
\define@key[psset]{pst-plot}{Hue}[180]{\pst@getint{#1}\pst@HueAngle}
\psset[pst-plot]{Hue=180}
\def\beginplot@colordots{\begin@SpecialObj}
\def\endplot@colordots{%
  \addto@pscode{%
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    newpath
    /MaxValue 0 def
    /m n 2 mul def
    n { 
      dup MaxValue gt { dup /MaxValue ED } if
      m 2 roll
    } repeat
    n { dup MaxValue div  % y y
      \pst@number\psyunit div abs % to orig y value
      \pst@HueAngle\space 360 div exch dup sethsbcolor % 180 Y Y hsb color
      transform floor .5 add exch floor
      .5 add exch itransform Dot stroke } repeat }%
  \end@SpecialObj%
}
%
\def\beginplot@bubble{\begin@SpecialObj}
\def\endplot@bubble{%
  \addto@pscode{%
    newpath
    n { dup % x y y
      \pst@number\psyunit div abs % to orig y value
      transform floor .5 add exch floor
      .5 add exch itransform 
      0 360 arc \psk@fill 
      stroke } repeat }%
  \end@SpecialObj%
}
%
\def\beginplot@bezier{\begin@OpenObj}
\def\endplot@bezier{\psbezier@ii}
%
\def\beginplot@cbezier{\begin@ClosedObj}
\def\endplot@cbezier{\pscbezier@ii}
%
\def\beginplot@cspline{\begin@OpenObj}%% Christoph Bersch
\def\endplot@cspline{\pscspline@ii}
% 
\let\beginplot@LineToYAxis\beginplot@line  % all from pst-plot added 2007-06-26 (hv)
\def\endplot@LineToYAxis{\psLineToYAxis@ii}
\let\beginqp@LineToYAxis\beginqp@line
\let\doqp@LineToYAxis\doqp@line
\let\endqp@LineToYAxis\endqp@line
\let\testqp@LineToYAxis\testqp@line
\let\beginplot@LineToXAxis\beginplot@line
\def\endplot@LineToXAxis{\psLineToXAxis@ii}
\let\beginqp@LineToXAxis\beginqp@line
\let\doqp@LineToXAxis\doqp@line
\let\endqp@LineToXAxis\endqp@line
\let\testqp@LineToXAxis\testqp@line
%
\newif\ifPst@interrupt \Pst@interruptfalse
\define@key[psset]{pst-plot}{barwidth}[0.25cm]{\pst@getlength{#1}\Add@barwidth}
\psset[pst-plot]{barwidth=0.25cm}
\define@key[psset]{pst-plot}{interrupt}[]{\expandafter\pst@interrupt#1,,,\@nil}
\def\pst@interrupt#1,#2,#3,#4\@nil{%
  \ifx\relax#1\relax \Pst@interruptfalse
  \else
    \Pst@interrupttrue
    \def\pst@interrupt@YMax{#1 }%
    \def\pst@interrupt@YMaxSep{#2 }%
    \def\pst@interrupt@YMaxDiff{#3 }%
  \fi
}
%
\def\psbar@ii{\addto@pscode{false \tx@NArray \psbar@iii}}

\def\psbar@iii{%
  \ifPst@interrupt
    /YMax \pst@interrupt@YMax \strip@pt\psyunit\space mul def
    /YMaxSep \pst@interrupt@YMaxSep \strip@pt\psyunit\space mul def
    /YMaxDiff \pst@interrupt@YMaxDiff \strip@pt\psyunit\space mul def
    /Tilde { % on stack DX
      /Op ED % add or sub
      /DX ED
      currentpoint 2 copy
      /Y ED /X ED   % x y  
      X DX add Y YMaxSep 2 div Op   
      X DX dup add add Y           
      curveto
      currentpoint 2 copy pop /X ED 
      X DX add Y YMaxSep 2 div neg Op  
      X DX dup add add Y    
      curveto      
    } def  
    newpath
    n { 
      /Yval exch def /Xval exch def 
      Xval \number\Add@barwidth 0.5 mul sub 0 moveto 
      Yval YMax le {  
        0 Yval rlineto \number\Add@barwidth 0 rlineto 
        0 Yval neg rlineto \number\Add@barwidth neg 0 rlineto
      }{
        0 YMax rlineto 
        \number\Add@barwidth 4 div 
        { add } Tilde
        0 YMax neg rlineto 
        \number\Add@barwidth neg 0 rlineto
        closepath
        Xval \number\Add@barwidth 0.5 mul sub YMax YMaxSep add moveto 
        0 Yval YMax sub YMaxSep sub YMaxDiff sub rlineto 
        \number\Add@barwidth 0 rlineto 
        0 Yval YMax YMaxSep add sub YMaxDiff sub neg rlineto 
        \number\Add@barwidth 4 div neg 
        { sub } Tilde
      } ifelse
    } repeat
  \else
    newpath
    n { 
      /Yval exch def /Xval exch def 
      Xval \number\Add@barwidth 0.5 mul sub 0 moveto 
      0 Yval rlineto \number\Add@barwidth 0 rlineto 
      0 Yval neg rlineto \number\Add@barwidth neg 0 rlineto
    } repeat
  \fi
}%
\def\beginplot@bar{\begin@SpecialObj}
\def\endplot@bar{%
  \psbar@ii\psk@fillstyle\ifpsshadow\pst@closedshadow\fi%
  \pst@stroke
  \end@SpecialObj}
%
\def\psybar@ii{\addto@pscode{false \tx@NArray \psybar@iii}}
\def\psybar@iii{%
  newpath
  n { 
    /Yval exch def /Xval exch def 
    0 Yval \number\Add@barwidth 0.5 mul sub moveto 
    Xval 0 rlineto 0 \number\Add@barwidth rlineto 
    Xval neg 0 rlineto 0 \number\Add@barwidth neg rlineto
  } repeat
}%
\def\beginplot@ybar{\begin@SpecialObj}
\def\endplot@ybar{%
  \psybar@ii\psk@fillstyle\ifpsshadow\pst@closedshadow\fi%
  \pst@stroke
  \end@SpecialObj}
%
% LSM Least Square Method 2006-03-13 (hv)
\def\psLSM@ii{\addto@pscode{ false \tx@NArray \psLSM@iii }}
\def\psLSM@iii{%
  /xiSquare 0 def				% xi*xi
  /xi 0 def					% xi
  /fi 0 def					% f(xi)
  /xifi 0 def					% xi*f(xi)
  exch dup dup /xEnd ED /xStart ED exch
  n { 						% number of data pairs
    /Yval ED /Xval ED 				% save x y values
    /xi xi Xval add def				% sum xi
    /xiSquare xiSquare Xval dup mul add def	% sum xi*xi
    /xifi xifi Xval Yval mul add def		% sum xi*yi, same as xi*f(xi)
    /fi fi Yval add def				% sum yi, same as f(xi)
    Xval xStart lt { /xStart Xval def } if	% find the lowest xi
    Xval xEnd gt { /xEnd Xval def } if		% find the largest xi
  } repeat
  /u xiSquare fi mul xi xifi mul sub n xiSquare mul xi dup mul sub div def
  /v n xifi mul xi fi mul sub n xiSquare mul xi dup mul sub div def
  \Pst@Debug\space 0 gt { 			% print the equation
    /Helvetica findfont 12 scalefont setfont	
    0 -50 moveto (y=) show 			% print y=
    v \pst@number\psyunit \pst@number\psxunit div div 20 string cvs show ( x+) show		% m*x+
    u \pst@number\psyunit div 20 string cvs show } if
  newpath
  (\psk@xStart) length 0 gt 			% special start value?
    { \psk@xStart\space \pst@number\psxunit mul }
    { xStart } ifelse 
  dup v mul u add 				% xStart f(xStart)  
  moveto		 			% goto first point x1 y(x1)
  (\psk@xEnd) length 0 gt 			% special end value?
    { \psk@xEnd\space \pst@number\psxunit mul }
    { xEnd } ifelse 
  dup v mul u add 				% xEnd f(xEnd)	
  lineto					% line to second point x2 y(x2)
}%
%
\def\beginplot@LSM{\begin@SpecialObj}
\def\endplot@LSM{%
  \psLSM@ii\psk@fillstyle\ifpsshadow\pst@closedshadow\fi%
  \pst@stroke
  \end@SpecialObj}
%
\define@key[psset]{pst-plot}{IQLfactor}{\pst@checknum{#1}\pst@IQLfactor}
\psset[pst-plot]{IQLfactor=1.5}
\define@key[psset]{pst-plot}{postAction}[]{\def\psk@postAction{%
  \ifx\relax#1\relax\else\pst@number\psyunit div #1 \pst@number\psyunit mul \fi }}
\psset[pst-plot]{postAction=}
%
\def\psBoxplot@ii{%
  \addto@pscode{
    /Barwidth \number\Add@barwidth 2 div def  
    /Endwidth Barwidth \psk@arrowlength\space mul def  
   NArray bubblesort
   /NArray ED 				% save sorted array
   [ NArray { yUnit mul } forall ] /NArray ED % multiply with y unit
   NArray 0 get /MinVal ED		% save minimum
   NArray m 1 sub get /MaxVal ED	% maximum
   m 2 div cvi /M ED 			% the middle
   NArray length 2 mod 0 eq {		% even numbers of entries
     M 1 sub NArray exch get 		% even number of values
     NArray M get          		% and the upper one
     add 2 div /Median ED  		% the median
   }{
     NArray M get /Median ED  		% odd numbers of values
   } ifelse
   m 4 mod 0 eq {	  		% get the lower Quartil even/odd
     m 4 div cvi dup 1 sub NArray exch get
     exch NArray exch get
%     M 2 div cvi 1 add dup /M2 ED		% save middle index
%     1 sub NArray exch get 
%     NArray M2 get 
     add 2 div floor /LowerQuartil ED
   }{ 
     NArray M 2 div cvi get /LowerQuartil ED 
   } ifelse				% end even/odd 
   m 0.75 mul dup dup cvi sub 0 eq {	% get the upper Quartil
%    0.75*m is an integer
     cvi dup 1 sub NArray exch get exch NArray exch get
%     M 1.5 mul cvi 1 add dup /M3 ED
%     1 sub NArray exch get 
%     NArray M3 get 
     add 2 div floor /UpperQuartil ED
   }{					% upper quartil
     NArray m 0.75 mul floor cvi get /UpperQuartil ED
   } ifelse 
%
   /IQL UpperQuartil LowerQuartil sub \pst@IQLfactor\space mul def
   0 1 m 1 sub { % Index on stack
     dup /Index ED
     NArray exch get LowerQuartil sub abs IQL sub 0 gt { 
       \psk@dotsize
       \@nameuse{psds@\psk@dotstyle}
       0 NArray Index get \psk@postAction
       Dot
       NArray Index LowerQuartil UpperQuartil LowerQuartil sub \pst@IQLfactor\space mul sub 
       dup /MinVal ED put % replace with 1.5 IQL
       NArray Index 1 add get /MinVal ED 
    } { exit } ifelse
   } for
   m 1 sub -1 0 {	% Index on stack
     dup /Index ED
     NArray exch get UpperQuartil sub abs IQL sub 0 gt { 
%       newpath 
       \psk@dotsize
       \@nameuse{psds@\psk@dotstyle}
       0 NArray Index get \psk@postAction\space
       Dot
       NArray Index UpperQuartil LowerQuartil sub \pst@IQLfactor\space mul UpperQuartil add 
       dup /MaxVal ED put % replace with 1.5 IQL
       NArray Index 1 sub get /MaxVal ED 
     }{ exit } ifelse
   } for
%
   Endwidth neg MaxVal \psk@postAction moveto			% we are on top / lower whisker
   Endwidth dup add 0 rlineto 
   0 MaxVal \psk@postAction moveto 
   0 UpperQuartil \psk@postAction lineto			% upper quartil
%% 
   MinVal \psk@postAction MaxVal \psk@postAction lt {
     0 LowerQuartil \psk@postAction moveto			% line to lower whisker
     0 MinVal \psk@postAction lineto 
     Endwidth neg MinVal \psk@postAction moveto 
     Endwidth dup add 0 rlineto 
   } if
   gsave
   \pst@number\pslinewidth SLW
   \pst@usecolor\pslinecolor
   \tx@setStrokeTransparency 
%   \tx@setStrokeTransparency
   \@nameuse{psls@\pslinestyle}
   stroke
   grestore
   newpath
   Barwidth neg LowerQuartil \psk@postAction moveto	% lower quartil
   Barwidth neg UpperQuartil \psk@postAction lineto
   Barwidth dup add 0 rlineto
   Barwidth LowerQuartil \psk@postAction lineto
   closepath
   gsave \pst@usecolor\psfillcolor \tx@setTransparency fill grestore
   Barwidth neg Median \psk@postAction moveto		% median
   Barwidth dup add 0 rlineto
   \pst@number\pslinewidth SLW
   \pst@usecolor\pslinecolor
   \tx@setStrokeTransparency
%   \tx@setStrokeTransparency
   \@nameuse{psls@solid}
}}%
%
\def\beginplot@Boxplot{\init@pscode}
\def\endplot@Boxplot{%
  \psBoxplot@ii\psk@fillstyle\ifpsshadow\pst@closedshadow\fi%
  \pst@stroke
  \end@SpecialObj}
%
\def\psBoxplot{\def\pst@par{}\pst@object{psBoxplot}}
\def\psBoxplot@i#1{%
  \leavevmode
  \pst@killglue
  \begingroup
  \addbefore@par{barwidth=40pt,arrowlength=0.75}%
  \addto@par{plotstyle=Boxplot}%
  \use@par
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{
    /D {} def
    [ #1 ] /NArray ED 
    NArray aload length /m ED
    /xUnit \pst@number\psxunit def
    /yUnit \pst@number\psyunit def
  }%
  \@nameuse{endplot@\psplotstyle}%
  \ignorespaces%
}
%
\define@key[psset]{pst-plot}{plotstyle}[line]{%
  \@ifundefined{beginplot@#1}%
    {\@pstrickserr{Plot style `#1' not defined}\@eha}%
    {\def\psplotstyle{#1}}}
\psset[pst-plot]{plotstyle=line}
%
\define@key[psset]{pst-plot}{plotpoints}[50]{%
  \pst@cntg=#1\relax
  \ifnum\pst@cntg<2
    \@pstrickserr{plotpoints parameter must be at least 2}\@ehpa
  \else
    \advance\pst@cntg-1
    \edef\psk@plotpoints{\the\pst@cntg\space}%
  \fi}
\psset[pst-plot]{plotpoints=50}
%
%the following works only for plotstyle line, polygon and bezier
\define@key[psset]{pst-plot}{yMaxValue}[1.e30]{\def\psk@yMaxValue{#1 }\def\psk@yMinValue{#1 neg }}
\psset{yMaxValue=1.e30}
\define@key[psset]{pst-plot}{yMinValue}[-1.e30]{\def\psk@yMinValue{#1 }}
\psset{yMinValue=-1.e30}
% can be in PS syntax (eg 1e1.2) and must be positiv! negative values
% will beignored
%
% For quick plots, define:
%   \beginqp@<foo>   : What to do to first point (PS code only).
%   \doqp@<foo>      : What to do to subsequent points (PS code only).
%   \endqp@<foo>     : How to end plot.
%   \testqp@<foo>    : Set \@psttrue if OK to use quick plot.
%
\def\beginqp@line{\pst@oplineto}
\def\doqp@line{ 
  dup
  \psk@yMaxValue \pst@number\psyunit mul gt 
    { moveto }
    { dup \psk@yMinValue \pst@number\psyunit mul lt 
      { moveto }
      { L } ifelse 
    } ifelse
}
\def\endqp@line{%
  \ifPst@variableLW \addto@pscode{ \pst@flattenpath }\fi%
  \end@OpenObj}%

\def\testqp@line{%
  \ifdim\pslinearc>\z@\else
    \ifshowpoints\else
      \ifx\psk@arrowA\@empty
        \ifx\psk@arrowB\@empty
          \@psttrue
        \fi
      \fi
    \fi
  \fi}
%
\def\beginqp@polygon{moveto }
\def\doqp@polygon{ 
      dup
      \psk@yMaxValue \pst@number\psyunit mul gt 
      { moveto }{ 
          dup
          \psk@yMinValue \pst@number\psyunit mul lt 
          { moveto }{ L } ifelse 
      } ifelse
}
\def\endqp@polygon{%
  \addto@pscode{closepath}%
  \end@ClosedObj}
\def\testqp@polygon{%
  \ifdim\pslinearc>\z@\else
    \ifshowpoints\else
      \@psttrue
    \fi
  \fi}
%
\def\beginqp@dots{%
  \psk@dotsize
  \@nameuse{psds@\psk@dotstyle}
% DG/SR modification begin - Dec. 12, 1999 - Patch 2
%  /TheDot { gsave \psk@dotangle \psk@dotscale Dot grestore } def
%  TheDot }
  Dot }
%\def\doqp@dots{TheDot }
\def\doqp@dots{Dot }
% DG/SR modification end
\def\endqp@dots{\end@SpecialObj}
\def\testqp@dots{\@psttrue}
%
\def\beginqp@bezier{/n 0 def \pst@oplineto}
\def\doqp@bezier{/n n 1 add def n 3 mod 0 eq { % we need 3 points   
    dup \psk@yMaxValue\space \pst@number\psyunit mul gt 
    { moveto pop pop pop pop}
    { dup \psk@yMinValue\space \pst@number\psyunit mul lt 
      { moveto pop pop pop pop}{ curveto } ifelse 
    } ifelse 
  } if
}
\def\endqp@bezier{%
  \addto@pscode{n 3 mod { pop pop } repeat}
  \end@OpenObj}%
\def\testqp@bezier{%
  \ifshowpoints\else
    \ifx\psk@arrowA\@empty
      \ifx\psk@arrowB\@empty
        \@psttrue
      \fi
    \fi
  \fi}
%
\def\beginqp@cbezier{/n 0 def moveto }
\def\doqp@cbezier{\doqp@bezier}
\def\endqp@cbezier{%
  \addto@pscode{n 3 mod { pop pop } repeat closepath}
  \end@ClosedObj}%
\def\testqp@cbezier{\ifshowpoints\else\@psttrue\fi}
%
% added 2007-06-26 (hv) -------------------------------------------------
\def\tx@LineToYAxis{LineToYAxis }
\def\psLineToYAxis@ii{%
\addto@pscode{\pst@cp \psline@iii \psk@Ox\space \pst@number\psxunit mul \tx@LineToYAxis}%
\end@OpenObj}
%
\def\tx@LineToXAxis{LineToXAxis }
\def\psLineToXAxis@ii{%
\addto@pscode{\pst@cp \psline@iii \psk@Oy\space \pst@number\psyunit mul \tx@LineToXAxis}%
\end@OpenObj}
%
\define@key[psset]{pst-plot}{PSfont}[Times-Roman]{\def\psk@PSfont{/#1 }}
\define@key[psset]{pst-plot}{valuewidth}[10]{\pst@getint{#1}\psk@valuewidth }
\define@key[psset]{pst-plot}{fontscale}[10]{\pst@checknum{#1}\psk@fontscale }
\define@key[psset]{pst-plot}{decimals}[-1]{\pst@getint{#1}\psk@decimals }
\psset[pst-plot]{PSfont=Times-Roman,fontscale=10,valuewidth=10,decimals=-1}
%
\newdimen\psxlabelsep
\newdimen\psylabelsep
\define@key[psset]{pst-plot}{xlabelsep}[5pt]{\pssetlength\psxlabelsep{#1}}
\define@key[psset]{pst-plot}{ylabelsep}[5pt]{\pssetlength\psylabelsep{#1}}
\psset[pst-plot]{xlabelsep=5pt,ylabelsep=5pt}

%
\newif\ifPst@valuesStar\Pst@valuesStarfalse
\newif\ifPst@xvalues\Pst@xvaluesfalse
%
\def\psvalues@ii{\addto@pscode{ false \tx@NArray \psvalues@iii }}
\def\psvalues@iii{
  \psk@PSfont findfont \psk@fontscale scalefont setfont 
  newpath 
  n { /yO ED /xO ED
      gsave
      \ifPst@xvalues
        xO \pst@number\psxunit div
      \else
        yO \pst@number\psyunit div
      \fi
      \psk@decimals 0 eq { cvi } if
      \psk@decimals 0 gt { 10 \psk@decimals exp dup 3 1 roll mul cvi exch div } if
      \psk@valuewidth string cvs /Str ED
      \ifPst@valuesStar
      Str stringwidth pop /yS \psk@fontscale def /xS ED 
      gsave newpath 
        xO \ifPst@xvalues \pst@number\pslabelsep add \fi
        yO \ifPst@xvalues\else \pst@number\pslabelsep add \fi 
        moveto \ifx\psk@rot\@empty\else\psk@rot rotate \fi
        xS 0 rlineto 0 yS rlineto xS neg 0 rlineto 0 yS neg rlineto 
        closepath  1 setgray fill stroke 
      grestore 
      \fi
      xO \ifPst@xvalues \pst@number\pslabelsep add \fi
      yO \ifPst@xvalues\else \pst@number\pslabelsep add \fi 
      moveto \ifx\psk@rot\@empty\else\psk@rot rotate \fi 
      Str show 
      grestore } repeat 
}%
\def\beginplot@values{\Pst@valuesStarfalse\begin@SpecialObj}
\expandafter\def\csname beginplot@values*\endcsname{\Pst@valuesStartrue\begin@SpecialObj}
\def\beginplot@xvalues{\Pst@valuesStarfalse\begin@SpecialObj}
\expandafter\def\csname beginplot@xvalues*\endcsname{\Pst@valuesStartrue\begin@SpecialObj}
\def\endplot@values{%
  \Pst@xvaluesfalse%  
  \psvalues@ii%
  \pst@stroke
  \end@SpecialObj}
\@namedef{endplot@values*}{\endplot@values}
\def\endplot@xvalues{%
  \Pst@xvaluestrue%  
  \psvalues@ii%
  \pst@stroke
  \end@SpecialObj}
\@namedef{endplot@xvalues*}{\endplot@xvalues}
%
% end (hv) --------------------------------------------------------------
%
%
\def\psdataplot{\def\pst@par{}\pst@object{dataplot}}
\def\dataplot{\def\pst@par{}\pst@object{dataplot}}
\def\dataplot@i#1{%
  \pst@killglue
  \begingroup
    \use@par
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst
      \dataplot@ii{\addto@pscode{#1}}%
    \else
      \listplot@ii{\addto@pscode{#1}}%
    \fi
  \endgroup
  \ignorespaces}
%
\def\dataplot@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      /Dx { \pst@number\psxunit mul /D { Dy } def } def
      /Dy { \pst@number\psyunit mul Do /D { Dx } def } def
      /D { /D { Dx } def } def
      /Do {
        \@nameuse{beginqp@\psplotstyle}%
        /Do { \@nameuse{doqp@\psplotstyle}} def
      } def}%
    #1%			% this is \pst@readfile{#1} for fileplot
    \addto@pscode{ D }%
  \@nameuse{endqp@\psplotstyle}}
%
\def\psfileplot{\def\pst@par{}\pst@object{fileplot}}
\def\fileplot{\def\pst@par{}\pst@object{fileplot}}
\def\fileplot@i#1{%
  \pst@killglue%
  \begingroup%
    \use@par%
    \@pstfalse%
    \@nameuse{testqp@\psplotstyle}%
    \if@pst\dataplot@ii{\pst@readfile{#1}}\else\listplot@ii{\pst@altreadfile{#1}}\fi%
  \endgroup%
  \ignorespaces}
%
\def\pslistplot{\pst@object{listplot}}
\def\listplot{\pst@object{listplot}}
\def\listplot@i#1{\listplot@ii{\addto@pscode{#1}}}
\def\listplot@ii#1{%
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{/D {} def mark}%
  #1%
  \addto@pscode{
    \tx@PreparePoints
    \pst@number\psxunit
    \pst@number\psyunit
    \tx@ScalePoints
  }%
  \@nameuse{endplot@\psplotstyle}%
}
%
\define@boolkey[psset]{pst-plot}[Psk@]{xyValues}[true]{}
\define@boolkey[psset]{pst-plot}[Pst@]{ChangeOrder}[true]{}
\psset[pst-plot]{xyValues,ChangeOrder=false}
%
\pst@def{PreparePoints}<{%
  counttomark /m exch def
  /maxYValues \psk@plotNoMax\space def
  /YValuePos \psk@plotNo\space def
  /XValuePos \psk@plotNoX\space def
  \ifPsk@xyValues\else % we have only y values
    /mm m def
    /M m 1 add def
    m { mm exch M 2 roll /M M 1 add def /mm mm 1 sub def } repeat
    /m m dup add def
  \fi
  \ifPst@ChangeOrder
    /m0 m def
    m maxYValues 1 add div 1 sub cvi {
      m0 maxYValues 1 add roll /m0 m0 maxYValues 1 add sub def
    } repeat
  \fi
  /n m maxYValues 1 add div cvi def
%
% when having multiple x values, we first delete the first X value
% and then put the plotNoX onto the first position  
%
  XValuePos 1 gt {% multiple x values?            x y y xNo y
    n {
      maxYValues 1 add XValuePos neg roll    % y x y y xNo
      dup /XValue ED
      maxYValues 1 add XValuePos 1 sub  roll % y y xNo y x
      pop XValue                             % y y xNo y xNo
      maxYValues 1 add 1 roll                % xNo y y xNo y 
      m maxYValues 1 add  roll               % next values
    } repeat
  } if % no multiple data files
  maxYValues 1 gt {% multiple data files?           x y y yNo y 
    n {
      maxYValues YValuePos 1 sub neg roll % x yNo y y y ...
      maxYValues 1 sub { pop } repeat     % x yNo
      /m m maxYValues 1 sub sub def
      m 2 roll
    } repeat
  } if % no multiple data files
%	counttomark /m exch def
%	/n m 2 div cvi def
  /xMax -99999 def /yMax -99999 def
  /xP 0 def /yP 0 def
  m copy
  n {
    /y exch def /x exch def
    xMax x lt { /xMax x def } if
    yMax y lt {/yMax y def } if
    xP x gt { /xP x def } if
    yP y gt { /yP y def } if
  } repeat
%	m 2 roll
  \psk@xStep\space 0 gt \psk@yStep\space 0 gt or (\psk@xStart) length 0 gt or
  (\psk@yStart) length 0 gt or (\psk@xEnd) length 0 gt or (\psk@yEnd) length 0 gt or {
%
    (\psk@xStart) length 0 gt {\psk@xStart\space }{ xP } ifelse /xStart exch def
    (\psk@yStart) length 0 gt {\psk@yStart\space }{ yP } ifelse /yStart exch def
    (\psk@xEnd) length 0 gt { \psk@xEnd\space }{ xMax } ifelse /xEnd exch def
    (\psk@yEnd) length 0 gt { \psk@yEnd\space }{ yMax } ifelse /yEnd exch def
    n {
      m -2 roll
      2 copy /yVal exch def /xVal exch def
      xVal xP ge
      yVal yP ge and
      xVal xEnd le and
      yVal yEnd le and
      xVal xStart ge and
      yVal yStart ge and {
        /xP xP \psk@xStep\space add def
        /yP yP \psk@yStep\space add def
      }{%
        pop pop
        /m m 2 sub def
      } ifelse
    } repeat
  }{%
    /ncount 1 def
    (\psk@nEnd) length 0 gt { \psk@nEnd\space }{ m } ifelse 
    /nEnd exch def
    n {
      m -2 roll
      \psk@nStep\space 1 gt { ncount \psk@nStart\space sub \psk@nStep\space mod 0 eq }{ true } ifelse
        ncount nEnd le and
        ncount \psk@nStart\space ge and not {
%        ncount nEnd le and
%        ncount \psk@nStart\space ge and not {
          pop pop
          /m m 2 sub def
        } if
        /ncount ncount 1 add def
      } repeat
  } ifelse
}>
%
% \psplot
% D.G. addition - Jun.  9, 1998 - Polar plots using the \psplot macro
% Code added according the way suggested by Ulrich Dirr
% For polar plots
\define@boolkey[psset]{pst-plot}[Pst@]{polarplot}[true]{}
\define@boolkey[psset]{pst-plot}[Pst@]{VarStep}[true]{}
\define@key[psset]{pst-plot}{PlotDerivative}{\def\psk@PlotDerivative{#1}}%
\define@key[psset]{pst-plot}{VarStepEpsilon}{\def\psk@VarStepEpsilon{#1}}%
\define@key[psset]{pst-plot}{method}{\def\psk@method{#1}}%     	   adams - rk4
\def\@rkiv{rk4}%		Runge-Kutta 4  method
\def\@varrkiv{varrkiv}%		Runge-Kutta 4 with an adaptive step method
\def\@adams{adams}%		Adams method
\def\@default{default}%		Adams method
\psset[pst-plot]{VarStep=false,PlotDerivative=none,VarStepEpsilon=default,polarplot=false,method={}}
%
\def\psplotinit#1{\xdef\psplot@init{#1 }}
\def\psplot@init{}
%
\def\psplot{\def\pst@par{}\pst@object{psplot}}
\def\psplot@i#1#2{\@ifnextchar[{\psplot@x{#1}{#2}}{\psplot@x{#1}{#2}[]}}
\def\psplot@x#1#2[#3]#4{%
  \pst@killglue%
  \begingroup%
    \use@par%
    \@nameuse{beginplot@\psplotstyle}%
    \ifPst@polarplot%
      \addto@pscode{
        \psplot@init
        #3 
        /x #1 def
        /x1 #2 def
        /dx x1 x sub \psk@plotpoints div def
        /F@pstplot \ifPst@algebraic (#4)
                    \ifx\psk@PlotDerivative\@none\else
                      \psk@PlotDerivative\space { (x) tx@Derive begin Derive end } repeat
                    \fi\space
                    tx@AlgToPs begin AlgToPs end cvx
                 \else { #4 } \fi  def
        \ifPst@VarStep
          /StillZero 0 def /LastNonZeroStep dx def
          /F2@pstplot tx@Derive begin (#4) (x) Derive (x) Derive end
                     \ifx\psk@PlotDerivative\@none\else
                       \psk@PlotDerivative\space { (x) tx@Derive begin Derive end } repeat
                     \fi\space
                    tx@AlgToPs begin AlgToPs end cvx def
          %% computation of the tolerance defined by plotpoints
          /epsilon12 \ifx\psk@VarStepEpsilon\@default tx@Derive begin F2@pstplot end dx 3 exp abs mul abs
                    \else\psk@VarStepEpsilon\space 12 mul \fi def
          /ComputeStep {
            dup 1e-4 lt
            { pop StillZero 2 ge { LastNonZeroStep 2 mul } { LastNonZeroStep } ifelse /StillZero StillZero 1 add def }
            { epsilon12 exch div 1 3 div exp /StillZero 0 def }
            ifelse } bind def
        \fi
        /xy {% Adapted from \parametricplot@i
          F@pstplot x \ifPst@algebraic RadtoDeg \fi PtoC
%          #4 dup x cos mul exch x sin mul
          \pst@number\psyunit mul exch
          \pst@number\psxunit mul exch
        } def}%
    \else% polarplot
    \addto@pscode{
      \psplot@init
      #3 
      /x #1 def
      /x1 #2 def
      /dx x1 x sub \psk@plotpoints div def
      /F@pstplot \ifPst@algebraic (#4)
                    \ifx\psk@PlotDerivative\@none\else
                      \psk@PlotDerivative\space { (x) tx@Derive begin Derive end } repeat
                    \fi\space
                    tx@AlgToPs begin AlgToPs end cvx
                 \else { #4 } \fi  def
      \ifPst@VarStep
         /StillZero 0 def /LastNonZeroStep dx def
         /F2@pstplot tx@Derive begin (#4) (x) Derive (x) Derive end
                     \ifx\psk@PlotDerivative\@none\else
                       \psk@PlotDerivative\space { (x) tx@Derive begin Derive end } repeat
                     \fi\space
                    tx@AlgToPs begin AlgToPs end cvx def
         %% computation of the tolerance defined by plotpoints
         /epsilon12 \ifx\psk@VarStepEpsilon\@default tx@Derive begin F2@pstplot end dx 3 exp abs mul abs
                    \else\psk@VarStepEpsilon\space 12 mul \fi def
         /ComputeStep {
           dup 1e-4 lt
           { pop StillZero 2 ge { LastNonZeroStep 2 mul } { LastNonZeroStep } ifelse /StillZero StillZero 1 add def }
           { epsilon12 exch div 1 3 div exp /StillZero 0 def }
           ifelse } bind def
      \fi
      /xy { x \pst@number\psxunit mul F@pstplot \pst@number\psyunit mul
%       \ifPst@algebraic F@pstplot \else #4 \fi \pst@number\psyunit mul
      } def}%
    \fi%
    \gdef\psplot@init{}%
    \ifx\pslinestyle\psls@@symbol
      \psplot@iii
    \else
      \@pstfalse%
      \@nameuse{testqp@\psplotstyle}%
      \if@pst\psplot@ii\else\psplot@iii\fi%
    \fi%
  \endgroup%
  \ignorespaces}
%
\def\psplot@ii{%
  \ifPst@VarStep%
    \addto@pscode{%
      mark xy \@nameuse{beginqp@\psplotstyle}
      { F2@pstplot abs ComputeStep
        x 2 copy add dup x1 gt {pop x1} if /x exch def F2@pstplot abs ComputeStep
        /x 3 -1 roll def 2 copy gt { exch } if pop
        /x x 3 -1 roll add dup x1 gt {pop x1} if def
        xy \@nameuse{doqp@\psplotstyle}
        x x1 eq { exit } if} loop}%
  \else
    \pst@killglue%
    \addto@pscode{
      /ps@Exit false def
      xy \@nameuse{beginqp@\psplotstyle}
      \ifx\psk@method\@varrkiv\else\psk@plotpoints 1 sub \fi {
        /x x dx add \ifx\psk@method\@varrkiv  dup x1 gt { pop x1 } if \fi def
        xy \@nameuse{doqp@\psplotstyle}
        \ifx\psk@method\@varrkiv  x x1 eq { exit } if \fi
      } 
      ps@Exit { exit } if
      \ifx\psk@method\@varrkiv loop \else repeat \fi
      ps@Exit not {
        /x x1 def
        xy \@nameuse{doqp@\psplotstyle}
      } if }%
  \fi%
  \@nameuse{endqp@\psplotstyle}}
%
\def\psplot@iii{%
  \ifPst@VarStep%
    \addto@pscode{
      /n 2 def
      mark
      { xy n 2 roll F2@pstplot abs
        ComputeStep x 2 copy add dup x1 gt {pop x1} if
        /x exch def F2@pstplot abs ComputeStep
        /x 3 -1 roll def 2 copy gt { exch } if pop
        /x x 3 -1 roll dup /LastNonZeroStep exch def add dup x1 gt {pop x1} if def /n n 2 add def
        x x1 eq { exit } if } loop
      xy 
      n 2 roll}%
  \else\pst@killglue%
    \addto@pscode{
      mark
      /n 2 def
      \ifx\psk@method\@varrkiv\else\psk@plotpoints\fi {
        xy
        n 2 roll
        /n n 2 add def
        /x x dx add \ifx\psk@method\@varrkiv  dup x1 gt { pop x1 } if \fi def
        \ifx\psk@method\@varrkiv  x x1 eq { exit } if \fi
      } \ifx\psk@method\@varrkiv loop\else repeat \fi \space
      /x x1 def
      xy 
      2 copy \tx@UserCoor 2 array astore /FinalState ED
      n 2 roll}%
  \fi%
  \@nameuse{endplot@\psplotstyle}}
%
\def\psparametricplot{\pst@object{parametricplot}}% 	hv 2008-11-22
\def\parametricplot{\pst@object{parametricplot}}
\def\parametricplot@i#1#2{\@ifnextchar[{\parametricplot@x{#1}{#2}}{\parametricplot@x{#1}{#2}[]}}
\def\parametricplot@x#1#2[#3]{\@ifnextchar[{\parametricplot@xi{#1}{#2}[#3]}{\parametricplot@xi{#1}{#2}[#3][]}}
\def\parametricplot@xi#1#2[#3][#4]#5{%
  \pst@killglue%
  \begingroup%
    \use@par%
    \@nameuse{beginplot@\psplotstyle}%
    \addto@pscode{%
      #3 %prefix PS code
      \psplot@init
      /t #1 def
      /t1 #2 def
      /dt t1 t sub \psk@plotpoints div def
      /F@pstplot \ifPst@algebraic (#5)
                    \ifx\psk@PlotDerivative\@none\else
                      \psk@PlotDerivative\space { (t) tx@Derive begin Derive end } repeat
                    \fi\space
                    tx@AlgToPs begin AlgToPs end cvx
                 \else { #5 } \fi  def
      \ifPst@VarStep
         /StillZero 0 def /LastNonZeroStep dt def
         /F2@pstplot tx@Derive begin (#5) (t) Derive (t) Derive end
                     \ifx\psk@PlotDerivative\@none\else
                       \psk@PlotDerivative\space { (t) tx@Derive begin Derive end } repeat
                     \fi\space
                    tx@AlgToPs begin AlgToPs end cvx def
         %% computation of the tolerance defined by plotpoints
         /epsilon12 \ifx\psk@VarStepEpsilon\@default
                       tx@Derive begin F2@pstplot end Pyth
                       dt 3 exp abs mul
                    \else\psk@VarStepEpsilon\space 12 mul \fi def
         /ComputeStep {
           dup 1e-4 lt
           { pop StillZero 2 ge { LastNonZeroStep 2 mul } { LastNonZeroStep } ifelse /StillZero StillZero 1 add def }
           { epsilon12 exch div 1 3 div exp /StillZero 0 def }
           ifelse } bind def
      \fi
      /xy {
        \ifPst@algebraic F@pstplot \else #5 \fi
        \pst@number\psyunit mul exch
        \pst@number\psxunit mul exch
      } def
      }%
    \gdef\psplot@init{}%
    \@pstfalse
    \@nameuse{testqp@\psplotstyle}%
    \if@pst\parametricplot@ii{#4}\else\parametricplot@iii{#4}\fi
  \endgroup%
  \ignorespaces}
%
\def\parametricplot@ii#1{% para is the post code
  \ifPst@VarStep%
    \addto@pscode{%
      mark xy \@nameuse{beginqp@\psplotstyle}
      { F2@pstplot Pyth ComputeStep
        t 2 copy add dup t1 gt {pop t1} if /t exch def F2@pstplot Pyth ComputeStep
        /t 3 -1 roll def 2 copy gt { exch } if pop
        /t t 3 -1 roll add dup t1 gt {pop t1} if def
        xy \@nameuse{doqp@\psplotstyle}
        t t1 eq { exit } if } loop}%
  \else\pst@killglue%
    \addto@pscode{%
      /ps@Exit false def
      xy \@nameuse{beginqp@\psplotstyle}
      \psk@plotpoints 1 sub {
        /t t dt add def
        xy \@nameuse{doqp@\psplotstyle}
        ps@Exit { exit } if 
      } repeat
      ps@Exit not {
        /t t1 def
        xy \@nameuse{doqp@\psplotstyle}
      } if 
    }%
  \fi%
  \addto@pscode{ #1 }%
  \@nameuse{endqp@\psplotstyle}}
%
\def\parametricplot@iii#1{%
  \ifPst@VarStep%
    \addto@pscode{%
      /n 2 def
      mark
      { xy n 2 roll F2@pstplot Pyth
        ComputeStep t 2 copy add dup t1 gt {pop t1} if
        /t exch def F2@pstplot Pyth ComputeStep
        /t 3 -1 roll def 2 copy gt { exch } if pop
        /t t 3 -1 roll dup /LastNonZeroStep exch def add dup t1 gt {pop t1} if def /n n 2 add def
        t t1 eq { exit } if } loop
      xy 
      2 copy \tx@UserCoor 2 array astore /FinalState ED
      n 2 roll}%
  \else\pst@killglue%
    \addto@pscode{
      mark
      /n 2 def
      \psk@plotpoints {
        xy
        n 2 roll
        /n n 2 add def
        /t t dt add def
      } repeat
      /t t1 def
      xy
      n 2 roll}%
  \fi%
  \addto@pscode{ #1 }%
  \@nameuse{endplot@\psplotstyle}}
%
%
\newdimen\psk@subticksize\psk@subticksize=\z@
\newdimen\pst@xticksizeA
\newdimen\pst@xticksizeB
\newdimen\pst@xticksizeC
\newdimen\pst@yticksizeA
\newdimen\pst@yticksizeB
\newdimen\pst@yticksizeC
%
\define@key[psset]{pst-plot}{ticks}[all]{\pst@expandafter\psset@@ticks{#1}\@nil\psk@ticks}
\def\psset@@ticks#1#2\@nil#3{%
  \ifx#1a\let#3\z@\else%				0=a)ll
    \ifx#1x\let#3\@ne\else%				1=x
      \ifx#1y\let#3\tw@\else%				2=y
        \ifx#1n\let#3\thr@@\else%			3=n)one
          \@pstrickserr{Bad argument: `#1#2'}\@ehpa
  \fi\fi\fi\fi}
\psset[pst-plot]{ticks=all}
%
\define@key[psset]{pst-plot}{labels}[all]{\pst@expandafter\psset@@ticks{#1}\@nil\psk@labels}% same as ticks
\psset[pst-plot]{labels=all}
%
\define@key[psset]{pst-plot}{Ox}[0]{\def\psk@Ox{#1}}
\psset[pst-plot]{Ox=0}
\define@key[psset]{pst-plot}{Dx}[1]{\def\psk@Dx{#1}}
\psset[pst-plot]{Dx=1}
\define@key[psset]{pst-plot}{dx}[0]{%
  \pssetxlength\pst@dimg{#1}%
  \edef\psk@dx{\number\pst@dimg}}
\psset[pst-plot]{dx=0}
%
\define@key[psset]{pst-plot}{Oy}[0]{\def\psk@Oy{#1}}
\psset[pst-plot]{Oy=0}
\define@key[psset]{pst-plot}{Dy}[1]{\def\psk@Dy{#1}}
\psset[pst-plot]{Dy=1}
\define@key[psset]{pst-plot}{dy}[0]{%
  \pssetylength\pst@dimg{#1}%
  \edef\psk@dy{\number\pst@dimg}}
\psset[pst-plot]{dy=0}
%
\define@boolkey[psset]{pst-plot}[]{showorigin}[true]{}
\psset[pst-plot]{showorigin}
%
\define@key[psset]{pst-plot}{labelFontSize}[{}]{\def\psk@labelFontSize{#1}}%
\define@boolkey[psset]{pst-plot}[Pst@]{mathLabel}[true]{%
  \ifPst@mathLabel%
    \def\pshlabel##1{$\psk@labelFontSize##1$}%
    \def\psvlabel##1{$\psk@labelFontSize##1$}%
  \else%
    \def\pshlabel##1{\psk@labelFontSize##1}%
    \def\psvlabel##1{\psk@labelFontSize##1}%
  \fi}
\psset[pst-plot]{labelFontSize={},mathLabel}
%
\define@boolkey[psset]{pst-plot}[Pst@]{xAxis}[true]{}
\define@boolkey[psset]{pst-plot}[Pst@]{yAxis}[true]{}
\define@boolkey[psset]{pst-plot}[Pst@]{xyAxes}[true]{%
    \@nameuse{Pst@xAxis#1}\@nameuse{Pst@yAxis#1}}%
\psset[pst-plot]{xAxis,yAxis}%
%
\define@key[psset]{pst-plot}{xlabelPos}[b]{\pst@expandafter\psset@@xlabelPos{#1}\@nil}
\define@key[psset]{pst-plot}{ylabelPos}[l]{\pst@expandafter\psset@@ylabelPos{#1}\@nil}
\def\psset@@xlabelPos#1#2\@nil{%
  \ifx#1t
    \def\psk@xlabelPos{\tw@}%		2=top
    \pst@xticksizeC=\pst@xticksizeB%
  \else
    \ifx#1a
      \def\psk@xlabelPos{\@ne}%	 	1=axis
      \pst@xticksizeC=\z@%
    \else
      \def\psk@xlabelPos{\z@}%		0=bottom	
      \pst@xticksizeC=\pst@xticksizeA%
  \fi\fi}%
\def\psset@@ylabelPos#1#2\@nil{%
  \ifx#1r
    \def\psk@ylabelPos{\tw@}%		2=right
    \pst@yticksizeC=\pst@yticksizeB%
  \else
    \ifx#1a
      \def\psk@ylabelPos{\@ne}% 	1=axis
      \pst@yticksizeC=\z@%
    \else 
      \def\psk@ylabelPos{\z@}%		0=left	
      \pst@yticksizeC=\pst@yticksizeA%
  \fi\fi}
\psset[pst-plot]{xlabelPos=b, ylabelPos=l}%
%
\define@key[psset]{pst-plot}{xyDecimals}[{}]{\def\psk@xDecimals{#1}\def\psk@yDecimals{#1}}
\define@key[psset]{pst-plot}{xDecimals}[{}]{\def\psk@xDecimals{#1}}
\define@key[psset]{pst-plot}{yDecimals}[{}]{\def\psk@yDecimals{#1}}
\psset[pst-plot]{xyDecimals={}}%
%
\define@key[psset]{pst-plot}{xlogBase}[{}]{\def\psk@xlogBase{#1}}
\define@key[psset]{pst-plot}{ylogBase}[{}]{\def\psk@ylogBase{#1}}
\define@key[psset]{pst-plot}{xylogBase}[{}]{\def\psk@xlogBase{#1}\def\psk@ylogBase{#1}}%
\psset[pst-plot]{xylogBase={}}%
%
\define@key[psset]{pst-plot}{trigLabelBase}[0]{\pst@getint{#1}{\psk@trigLabelBase}}
\psset[pst-plot]{trigLabelBase=0}
%
\define@boolkey[psset]{pst-plot}[Pst@]{xtrigLabels}[true]{%
  \ifPst@xtrigLabels
    \def\pst@@@hlabel##1{\pshlabel{##1}}
    \def\pshlabel##1{%
      \ifnum\psk@trigLabelBase<2
        \def\de@nominator{\@ne}\else\def\de@nominator{\psk@trigLabelBase}\fi
      \def\pst@tempA{##1} 
      \pst@abs{\pst@tempA}\pst@cntm 
      \pst@mod{\pst@cntm}{\de@nominator}\pst@cntp % cntb=##1 modulo trigLabelBase
      \ifnum\@ne>\pst@cntp                  % 1 > modulo -> then we have pi/x
        \pst@cnto=\pst@cntm \divide\pst@cnto by \de@nominator  
	\ifPst@mathLabel%
          $\psk@labelFontSize
  	  \ifnum\pst@tempA<0 -\fi
          \ifnum\pst@cnto=\@ne                % #1 = trigLabelBase
            \pi                 	      % print pi
          \else
            \the\pst@cnto\pi 	              % print \pst@cnto/\de@nominator pi
          \fi$%   
	\else%
          \psk@labelFontSize%
  	  \ifnum\pst@tempA<0 -\fi%
          \ifnum\pst@cnto=\@ne%                % #1 = trigLabelBase
            $\pi$%                             % print pi
          \else%
            \the\pst@cnto$\pi$%                % print \pst@cnto/\de@nominator pi
          \fi%
	\fi%
      \else%
	\ifPst@mathLabel%
          $\psk@labelFontSize%
          \ifnum\pst@cntp=\@ne%                % < 1 pi?
            \if\pst@cntm=\@ne%
              \frac{\pi}{\de@nominator}%   % pi/x
            \else\ifnum\pst@tempA=-1 \frac{-\pi}{\de@nominator}%
              \else \ifnum\pst@tempA=1 \frac{\pi}{\de@nominator}%
                \else\frac{\pst@tempA\pi}{\de@nominator}% (x pi)/y
            \fi\fi\fi%
          \else%
            \ifnum\pst@tempA=1 \frac{\pi}{\de@nominator}%
            \else\ifnum\pst@tempA=\de@nominator \pi%
              \else\frac{\pst@tempA\pi}{\de@nominator}% 
          \fi\fi\fi$%
	\else%
          \psk@labelFontSize%
          \ifnum\pst@cntp=\@ne%                % < 1 pi?
            \if\pst@cntm=\@ne%
              $\frac{\pi}{\de@nominator}$%   % pi/x
            \else\ifnum\pst@tempA=-1 $\frac{-\pi}{\de@nominator}$%
              \else \ifnum\pst@tempA=1 $\frac{\pi}{\de@nominator}$%
                \else$\frac{\pst@tempA\pi}{\de@nominator}$% (x pi)/y
            \fi\fi\fi%
          \else%
            \ifnum\pst@tempA=1 $\frac{\pi}{\de@nominator}$%
            \else\ifnum\pst@tempA=\de@nominator $\pi$%
              \else$\frac{\pst@tempA\pi}{\de@nominator}$% 
          \fi\fi\fi%
	\fi%
      \fi%
    }%
  \else%
    \def\pst@@@hlabel##1{%
      \edef\@xyDecimals{\psk@xDecimals}%
%      \ifnum\psk@ticks<\tw@  % ticks=all|x
      \ifnum\psk@labels<\tw@  % labels=all|x
        \ifx\psk@xlogBase\@empty%
          \pshlabel{\psk@labelFontSize\expandafter\@LabelComma##1..\@nil\psk@xlabelFactor}%
        \else%
          \ifPst@mathLabel%
            \pshlabel{\psk@labelFontSize\psk@xlogBase^{\expandafter\@stripDecimals##1..\@nil}}%
          \else%
            \pshlabel{\psk@labelFontSize\psk@xlogBase\textsuperscript{\expandafter\@stripDecimals##1..\@nil}}%
          \fi
        \fi%
      \fi%
    }%
    \ifPst@mathLabel%
      \def\pshlabel##1{$\psk@labelFontSize##1$}\else\def\pshlabel##1{\psk@labelFontSize##1}\fi%
  \fi%
}%
%
\define@boolkey[psset]{pst-plot}[Pst@]{ytrigLabels}[true]{%
  \ifPst@ytrigLabels
    \def\pst@@@vlabel##1{\psvlabel{##1}}
    \def\psvlabel##1{%
      \ifnum\psk@trigLabelBase<2
        \def\de@nominator{\@ne}\else\def\de@nominator{\psk@trigLabelBase}\fi
      \def\pst@tempA{##1} 
      \pst@abs{\pst@tempA}\pst@cntm 
      \pst@mod{\pst@cntm}{\de@nominator}\pst@cntp % cntb=##1 modulo trigLabelBase
      \ifnum\@ne>\pst@cntp                  % 1 > modulo -> then we have pi/x
        \pst@cnto=\pst@cntm \divide\pst@cnto by \de@nominator  
	\ifPst@mathLabel%
          $\psk@labelFontSize
  	  \ifnum\pst@tempA<0 -\fi
          \ifnum\pst@cnto=\@ne                % #1 = trigLabelBase
            \pi                 	      % print pi
          \else
            \the\pst@cnto\pi 	              % print \pst@cnto/\de@nominator pi
          \fi$%   
	\else%
          \psk@labelFontSize%
  	  \ifnum\pst@tempA<0 -\fi%
          \ifnum\pst@cnto=\@ne%                % #1 = trigLabelBase
            $\pi$%                             % print pi
          \else%
            \the\pst@cnto$\pi$%                % print \pst@cnto/\de@nominator pi
          \fi%
	\fi%
      \else%
	\ifPst@mathLabel%
          $\psk@labelFontSize%
          \ifnum\pst@cntp=\@ne%                % < 1 pi?
            \if\pst@cntm=\@ne%
              \frac{\pi}{\de@nominator}%   % pi/x
            \else\ifnum\pst@tempA=-1 \frac{-\pi}{\de@nominator}%
              \else \ifnum\pst@tempA=1 \frac{\pi}{\de@nominator}%
                \else\frac{\pst@tempA\pi}{\de@nominator}% (x pi)/y
            \fi\fi\fi%
          \else%
            \ifnum\pst@tempA=1 \frac{\pi}{\de@nominator}%
            \else\ifnum\pst@tempA=\de@nominator \pi%
              \else\frac{\pst@tempA\pi}{\de@nominator}% 
          \fi\fi\fi$%
	\else%
          \psk@labelFontSize%
          \ifnum\pst@cntp=\@ne%                % < 1 pi?
            \if\pst@cntm=\@ne%
              $\frac{\pi}{\de@nominator}$%   % pi/x
            \else\ifnum\pst@tempA=-1 $\frac{-\pi}{\de@nominator}$%
              \else \ifnum\pst@tempA=1 $\frac{\pi}{\de@nominator}$%
                \else$\frac{\pst@tempA\pi}{\de@nominator}$% (x pi)/y
            \fi\fi\fi%
          \else%
            \ifnum\pst@tempA=1 $\frac{\pi}{\de@nominator}$%
            \else\ifnum\pst@tempA=\de@nominator $\pi$%
              \else$\frac{\pst@tempA\pi}{\de@nominator}$% 
          \fi\fi\fi%
	\fi%
      \fi%
    }%
  \else
    \def\pst@@@vlabel##1{%
      \edef\@xyDecimals{\psk@yDecimals}%
%      \ifodd\psk@ticks % ticks=all||y (0,2)
      \ifodd\psk@labels % labelss=all||y (0,2)
      \else%
        \ifx\psk@ylogBase\@empty%
          \psvlabel{\expandafter\@LabelComma##1..\@nil\psk@ylabelFactor}%
        \else%
          \ifPst@mathLabel%
            \psvlabel{\psk@ylogBase^{\expandafter\@stripDecimals##1..\@nil }}%
	  \else
            \psvlabel{\psk@ylogBase\textsuperscript{\expandafter\@stripDecimals##1..\@nil }}%
          \fi%
        \fi%
      \fi%
    }%
  \fi}%
\define@boolkey[psset]{pst-plot}[Pst@]{trigLabels}[true]{%
  \ifPst@trigLabels\psset[pst-plot]{xtrigLabels,ytrigLabels=false}
  \else            \psset[pst-plot]{xtrigLabels=false,ytrigLabels=false}%
  \fi}
\psset[pst-plot]{trigLabels=false}
%
%logLines=all|x|y|none  (0,1,2,3)
\def\psk@logLines{3}
\define@key[psset]{pst-plot}{logLines}[none]{\pst@expandafter\psset@@logLines#1\@nil\psk@logLines}
\def\psset@@logLines#1#2\@nil#3{%
  \ifx#1a
    \let#3\z@
    \Pst@maxxTickstrue\Pst@maxyTickstrue
    \set@xticksize{0 4pt}\set@yticksize{0 4pt}%
    \def\psk@xsubticksize{1}\def\psk@ysubticksize{1}%
  \else
    \ifx#1x
      \let#3\@ne
      \Pst@maxxTickstrue\Pst@maxyTicksfalse
      \set@xticksize{0 4pt}\def\psk@xsubticksize{1}%
    \else
      \ifx#1y
        \let#3\tw@
	\Pst@maxyTickstrue\Pst@maxxTicksfalse
	\set@yticksize{0 4pt}\def\psk@ysubticksize{1}%
      \else
        \ifx#1n\let#3\thr@@\else
          \@pstrickserr{Bad argument: `#1#2'}\@ehpa
  \fi\fi\fi\fi}
\psset[pst-plot]{logLines=none}%
%
\define@key[psset]{pst-plot}{ylabelFactor}[\relax]{\def\psk@ylabelFactor{#1}}
\define@key[psset]{pst-plot}{xlabelFactor}[\relax]{\def\psk@xlabelFactor{#1}}
\define@boolkey[psset]{pst-plot}[Pst@]{showOriginTick}[true]{}%
\psset[pst-plot]{xlabelFactor=\relax,ylabelFactor=\relax,showOriginTick}%

%% #1 : optional arguments passed to psline
%% #2 : rotating angle
%% #3 : x value
%% #4 : label
\def\psxTick{\pst@object{psxTick}}% idea by Martin Chicoine
\def\psxTick@i{\@ifnextchar({\psxTick@ii{0}}\psxTick@ii}
\def\psxTick@ii#1(#2)#3{{
  \pst@killglue
  \addbefore@par{arrows=-,linewidth=\psk@xtickwidth\pslinewidth}
  \use@par
  \psline(#2, \pst@xticksizeB)(#2,\pst@xticksizeA)
  \rput[t]{#1}(! \psk@origin 
                 #2 \pst@number\psxlabelsep \pst@number\pst@xticksizeB add
                 \pst@number\psyunit div neg ){\pshlabel{#3\vphantom{1}}}}\ignorespaces}
%
%% #1 : optional arguments passed to psline
%% #2 : rotating angle
%% #3 : y value
%% #4 : label
\def\psyTick{\pst@object{psyTick}}% idea by Martin Chicoine
\def\psyTick@i{\@ifnextchar({\psyTick@ii{0}}\psyTick@ii}
\def\psyTick@ii#1(#2)#3{{
  \pst@killglue
  \addbefore@par{arrows=-,linewidth=\psk@ytickwidth\pslinewidth}
  \use@par
  \psline(\pst@yticksizeB,#2)(\pst@yticksizeA,#2)
  \rput[r]{#1}(! \psk@origin
                \pst@number\pst@yticksizeB \pst@number\psylabelsep add
                \pst@number\psxunit div neg #2){\psvlabel{#3}}}\ignorespaces}
%
\def\psCoordinates{\pst@object{psCoordinates}}
\def\psCoordinates@i(#1){%
  \pst@killglue%
  \begin@OpenObj
  \SpecialCoor%
  \psline(#1|0,0)(#1)\psline(#1)(0,0|#1)\psdot(#1)%
  \end@OpenObj%
  \ignorespaces%
}
%
\def\stripDecimals#1{\expandafter\@stripDecimals#1..\@nil}
%% #1 integer
%% #2 decimals
%% #3 dot
\def\@stripDecimals#1.#2.#3\@nil{%
  \def\pst@dummy{#1}%
  \ifx\pst@dummy\@empty\the\@zero\else#1\fi% the integer part
}
%
\newcount\@digitcounter\@digitcounter=0\relax
\def\@inc@digitcounter{\global\advance\@digitcounter by 1\relax}
\def\@get@digitcounter{\the\@digitcounter\relax}
\def\@Reset@digitcounter{\global\@digitcounter=0\relax}
\def\@zeroFill{%
  \ifnum \@xyDecimals>\@get@digitcounter
    \bgroup
      0\@inc@digitcounter\@zeroFill
    \egroup%
  \fi%
}
% #1 the value, maybe empty
%
\def\@process@digits#1#2;{%
  \ifx *#1\@zeroFill\else#1\@inc@digitcounter 
  \ifnum\@xyDecimals>\@get@digitcounter\expandafter\@process@digits#2;\fi\fi%
}
%
\def\@writeDecimals#1{%
  \ifx\@xyDecimals\@empty% take value as is
    \def\@tempa{#1}% write only if not empty
    \ifx\@tempa\@empty% write nothing
    \else\ifmmode\expandafter\mathord\expandafter{\psk@decimalSeparator}\else\psk@decimalSeparator\fi#1\fi%
%    \else\psk@decimalSeparator\fi%
  \else% write only \xy@decimals
    \ifnum\@xyDecimals>\@zero
      \ifmmode\expandafter\mathord\expandafter{\psk@decimalSeparator}\else\psk@decimalSeparator\fi%
%      \psk@decimalSeparator
        \@Reset@digitcounter
        \expandafter\@process@digits#1*;
      \fi%
  \fi%
}
%% #1 integer
%% #2 decimals
%% #3 dot
\def\@LabelComma#1.#2.#3\@nil{%
  \def\pst@tempA{#1}%
  \ifx\pst@tempA\@empty\the\@zero\else#1\fi% the integer part
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty\@writeDecimals{}\else\@writeDecimals{#2}\fi}
%
%
\def\set@xticksize#1{%
  \pst@expandafter\pst@getydimdim{#1} {} {}\@nil% y-unit!! 
  \ifdim\pst@dimm>\pst@dimn% 		%	first > second value
    \pst@xticksizeA=\the\pst@dimn%
    \pst@xticksizeB=\the\pst@dimm%
  \else%
    \pst@xticksizeA=\the\pst@dimm%
    \pst@xticksizeB=\the\pst@dimn%	first > second value
  \fi%
  \edef\psk@xticksize{\pst@number\pst@xticksizeA \pst@number\pst@xticksizeB}%
  \ifnum\psk@xlabelPos<\z@\relax	% top
    \pst@xticksizeC=\pst@dimn%
  \else%
    \pst@xticksizeC=\pst@dimm%	bottom	
  \fi%
}
\def\set@yticksize#1{%
  \pst@expandafter\pst@getxdimdim{#1} {} {}\@nil% x-unit!
  \ifdim\pst@dimm>\pst@dimn\relax%   		%	first > second value
    \pst@yticksizeA=\the\pst@dimn%
    \pst@yticksizeB=\the\pst@dimm%
  \else%
    \pst@yticksizeA=\the\pst@dimm%
    \pst@yticksizeB=\the\pst@dimn%	first > second value
  \fi%
  \edef\psk@yticksize{\pst@number\pst@yticksizeA \pst@number\pst@yticksizeB}%
  \ifnum\psk@ylabelPos<\z@	% right	
    \pst@yticksizeC=\pst@dimn%
  \else%
      \pst@yticksizeC=\pst@dimo%  left
  \fi%
}
\newif\ifPst@maxxTicks
\newif\ifPst@maxyTicks
\define@key[psset]{pst-plot}{ticksize}[-4pt 4pt]{%
  \def\pst@tempA{max}%
  \def\pst@tempB{#1}%
  \ifx\pst@tempA\pst@tempB%
    \Pst@maxxTickstrue\Pst@maxyTickstrue%
    \set@xticksize{0 4pt}\set@yticksize{0 4pt}%
  \else%
    \Pst@maxxTicksfalse\Pst@maxyTicksfalse%
    \set@xticksize{#1}\set@yticksize{#1}%
  \fi}
\define@key[psset]{pst-plot}{xticksize}{%
  \def\pst@tempA{max}%
  \def\pst@tempB{#1}%
  \ifx\pst@tempA\pst@tempB
    \Pst@maxxTickstrue\set@xticksize{0 4pt}%
  \else\set@xticksize{#1}\Pst@maxxTicksfalse\fi}
\define@key[psset]{pst-plot}{yticksize}{%
  \def\pst@tempA{max}%
  \def\pst@tempB{#1}%
  \ifx\pst@tempA\pst@tempB%
    \Pst@maxyTickstrue\set@yticksize{0 4pt}%
  \else\set@yticksize{#1}\Pst@maxyTicksfalse\fi}%
\psset[pst-plot]{ticksize=-4pt 4pt}
%
% full= 0, top=1, bottom=-1, inner=2  => -1 0 1 2
\define@key[psset]{pst-plot}{tickstyle}[full]{\pst@expandafter\psset@@tickstyle{#1}\@nil}
\def\psset@@tickstyle#1#2\@nil{%
  \ifx#1f\let\psk@tickstyle\z@\else			% 0=f)ull
    \ifx#1t\let\psk@tickstyle\@ne			% 1=t)op
      \edef\psk@xticksize{0 \pst@number\pst@xticksizeB}%
      \edef\psk@yticksize{0 \pst@number\pst@yticksizeB}%
    \else\ifx#1b\let\psk@tickstyle\m@ne			% -1=b)ottom
      \edef\psk@xticksize{\pst@number\pst@xticksizeA 0}%
      \edef\psk@yticksize{\pst@number\pst@yticksizeA 0}%
      \else\ifx#1i\let\psk@tickstyle\tw@%		% 2=i)nner (for frame)
        \else\@pstrickserr{Bad tick style: `#1#2'}\@ehpa
  \fi\fi\fi\fi}
\psset[pst-plot]{tickstyle=full}
%
\define@key[psset]{pst-plot}{subticks}[1]{\def\psk@xsubticks{#1}\def\psk@ysubticks{#1}}
\define@key[psset]{pst-plot}{xsubticks}[1]{\def\psk@xsubticks{#1}}
\define@key[psset]{pst-plot}{ysubticks}[1]{\def\psk@ysubticks{#1}}
%
\define@key[psset]{pst-plot}{subticksize}[0.75]{\def\psk@xsubticksize{#1}\def\psk@ysubticksize{#1}}
\define@key[psset]{pst-plot}{xsubticksize}[0.75]{\def\psk@xsubticksize{#1}}
\define@key[psset]{pst-plot}{ysubticksize}[0.75]{\def\psk@ysubticksize{#1}}
%
\define@key[psset]{pst-plot}{tickwidth}[0.5\pslinewidth]{%
  \pst@getlength{#1}\psk@xtickwidth%
  \pst@getlength{#1}\psk@ytickwidth}
\define@key[psset]{pst-plot}{xtickwidth}[0.5\pslinewidth]{\pst@getlength{#1}\psk@xtickwidth}
\define@key[psset]{pst-plot}{ytickwidth}[0.5\pslinewidth]{\pst@getlength{#1}\psk@ytickwidth}
\define@key[psset]{pst-plot}{subtickwidth}[0.25\pslinewidth]{%
  \pst@getlength{#1}\psk@xsubtickwidth%
  \pst@getlength{#1}\psk@ysubtickwidth}
\define@key[psset]{pst-plot}{xsubtickwidth}[0.25\pslinewidth]{\pst@getlength{#1}\psk@xsubtickwidth}
\define@key[psset]{pst-plot}{ysubtickwidth}[0.25\pslinewidth]{\pst@getlength{#1}\psk@ysubtickwidth}
%
\define@key[psset]{pst-plot}{labelOffset}[0pt]{%
  \pst@getlength{#1}\psk@xlabelOffset%
  \pst@getlength{#1}\psk@ylabelOffset}
\define@key[psset]{pst-plot}{xlabelOffset}[0pt]{\pst@getlength{#1}\psk@xlabelOffset}
\define@key[psset]{pst-plot}{ylabelOffset}[0pt]{\pst@getlength{#1}\psk@ylabelOffset}
%
\define@key[psset]{pst-plot}{frameOffset}[0pt]{\pst@getlength{#1}\psk@frameOffset}
%
\define@key[psset]{pst-plot}{tickcolor}[black]{%
    \pst@getcolor{#1}\psk@xtickcolor%
    \pst@getcolor{#1}\psk@ytickcolor}
\define@key[psset]{pst-plot}{xtickcolor}[black]{\pst@getcolor{#1}\psk@xtickcolor}
\define@key[psset]{pst-plot}{ytickcolor}[black]{\pst@getcolor{#1}\psk@ytickcolor}
\define@key[psset]{pst-plot}{subtickcolor}[gray]{%
  \pst@getcolor{#1}\psk@xsubtickcolor%
  \pst@getcolor{#1}\psk@ysubtickcolor}
\define@key[psset]{pst-plot}{xsubtickcolor}[gray]{\pst@getcolor{#1}\psk@xsubtickcolor}
\define@key[psset]{pst-plot}{ysubtickcolor}[gray]{\pst@getcolor{#1}\psk@ysubtickcolor}
%
\define@key[psset]{pst-plot}{xticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psxticklinestyle{#1}}}
\define@key[psset]{pst-plot}{xsubticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psxsubticklinestyle{#1}}}
\define@key[psset]{pst-plot}{yticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psyticklinestyle{#1}}}
\define@key[psset]{pst-plot}{ysubticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psysubticklinestyle{#1}}}
\define@key[psset]{pst-plot}{ticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psxticklinestyle{#1}\def\psyticklinestyle{#1}}}
\define@key[psset]{pst-plot}{subticklinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psxsubticklinestyle{#1}\def\psysubticklinestyle{#1}}}
%
\psset[pst-plot]{subticksize=0.75,subticks=1,tickcolor=black,ticklinestyle=solid,
  subticklinestyle=solid,subtickcolor=gray,tickwidth=0.5\pslinewidth,
  subtickwidth=0.25\pslinewidth,labelOffset=0pt,frameOffset=0pt}
%
\define@key[psset]{pst-plot}{nStep}[1]{\def\psk@nStep{#1}}
\define@key[psset]{pst-plot}{nStart}[0]{\def\psk@nStart{#1}}
\define@key[psset]{pst-plot}{nEnd}[{}]{\def\psk@nEnd{#1}}
\define@key[psset]{pst-plot}{xStep}[0]{\def\psk@xStep{#1}}
\define@key[psset]{pst-plot}{yStep}[0]{\def\psk@yStep{#1}}
%
\define@key[psset]{pst-plot}{xStart}[{}]{\def\psk@xStart{#1}}
\define@key[psset]{pst-plot}{xEnd}[{}]{\def\psk@xEnd{#1}}
\define@key[psset]{pst-plot}{yStart}[{}]{\def\psk@yStart{#1}}
\define@key[psset]{pst-plot}{yEnd}[{}]{\def\psk@yEnd{#1}}
%
\define@key[psset]{pst-plot}{plotNoX}[1]{\def\psk@plotNoX{#1}}
\define@key[psset]{pst-plot}{plotNo}[1]{\def\psk@plotNo{#1}}
\define@key[psset]{pst-plot}{plotNoMax}[1]{\def\psk@plotNoMax{#1}}
%
\psset[pst-plot]{nStep=1, nStart=0, nEnd={},%
  xStep=0, yStep=0, xStart={}, xEnd={},  yStart={}, yEnd={}, 
  plotNo=1,plotNoMax=1,plotNoX=1}%
%
\def\pstScalePoints(#1,#2)#3#4{%
%  xScale | yScale | xOperator | yOperator  
% the operators can be any Postscript code
  \def\pstXScale{#1 }%
  \def\pstYScale{#2 }%
  \def\pstXPSScale{#3 }%
  \def\pstYPSScale{#4 }%
  \pst@def{ScalePoints}<%
    /yVal ED /xVal ED
    /yPSOp { #4 yVal mul #2 mul } def
    /xPSOp { #3 xVal mul #1 mul } def
    counttomark dup dup cvi eq not { exch pop } if
    /m exch def /n m 2 div cvi def
    n {
      \ifPst@polarplot exch cvi 360 mod PtoC \fi  % x cvi 360 mod PtoC
      yPSOp m 1 roll xPSOp m 1 roll 
      /m m 2 sub
      def } repeat>%
}
\pstScalePoints(1,1){}{}% the default -> no special operators
%
\def\psxs@none{\let\psk@arrowA\@empty\let\psk@arrowB\@empty\psxs@axes}
%
\def\psxs@axes{{%
  \ifPst@xAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{}{x}\fi%
  \ifPst@yAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{exch}{y}\fi%
}}
%
\def\psaxes{\pst@object{psaxes}}
\def\psaxes@i{\pst@getarrows\psaxes@ii}
\def\psaxes@ii(#1){\@ifnextchar({\psaxes@iii(#1)}{\psaxes@iv(0,0)(0,0)(#1)}}
\def\psaxes@iii(#1)(#2){\@ifnextchar({\psaxes@iv(#1)(#2)}{\psaxes@iv(#1)(#1)(#2)}}
\def\psaxes@iv(#1)(#2)(#3){\@ifnextchar[{\psaxes@v(#1)(#2)(#3)}{\psaxes@vii(#1)(#2)(#3)}}%
\def\psaxes@v(#1)(#2)(#3)[#4]{\@ifnextchar[{\psaxes@vi(#1)(#2)(#3)[#4]}{\psaxes@vi(#1)(#2)(#3)[#4][]}}%
\def\psaxes@vi(#1)(#2)(#3)[#4,#5][#6,#7]{%
  \psaxes@vii(#1)(#2)(#3)%
  \begingroup%
  \SpecialCoor
  \use@par
  \uput{\psxlabelsep}[#5](#3|#1){#4}\uput{\psylabelsep}[#7](#1|#3){#6}%
  \endgroup%
  \ignorespaces}
%
\def\psaxes@vii(#1,#2)(#3,#4)(#5,#6){%
  \pst@killglue%
  \begingroup%
  \pssetxlength\pst@dimc{#5}% ur-x
  \pssetylength\pst@dimd{#6}% ur-y
  \ifdim\pst@dimc<\z@\ifdim\pst@dimd<\z@\relax% axes show to left and down
    \addbefore@par{xlabelPos=top,ylabelPos=right}\fi\fi%
  \setbox\pst@hbox=\hbox\bgroup%
  \use@par%	now the same with an optional unit=... in par
  \pssetxlength\pst@dimg{#1}% o-x
  \pssetylength\pst@dimh{#2}% o-y
  \pssetxlength\pst@dima{#3}% ll-x
  \pssetylength\pst@dimb{#4}% ll-y
  \pssetxlength\pst@dimc{#5}% ur-x
  \pssetylength\pst@dimd{#6}% ur-y
% If minimum values are negative in log mode, we modify Ox
% (respectively Oy) if this was not done by the user
% X axis labels (\psk@log = 0 or 1)
%
% Whole thing will be translated to origin:
  \advance\pst@dima by -\pst@dimg% Dist. from ll-x to o-x
  \advance\pst@dimb by -\pst@dimh% Dist. from ll-y to o-y
  \advance\pst@dimc by -\pst@dimg% Dist. from ur-x to o-x
  \advance\pst@dimd by -\pst@dimh% Dist. from ur-y to o-y
% Make lines/arrows or frame:
  \@nameuse{psxs@\psk@axesstyle}%  \psxs@axes or \psxs@frame or \psxs@polar
  \ifPst@yAxis%
  \begingroup%
    \ifdim\pst@dima=\z@\else\showoriginfalse\fi%
    \ifnum\psk@dy=\z@%
      \pst@dimg=\psk@Dy\psyunit%
      \ifdim\pst@dimg<\p@\pst@cnta=\psk@Dy\edef\psk@Dy{-\the\pst@cnta}\fi% v.1.21
      \edef\psk@dy{\number\pst@dimg}%
    \fi%
%    \ifPst@xAxis\else\showorigintrue\fi%		2009-10-21
    \pst@vlabels{\pst@dimd}{\psk@arrowB}{#3}{#5}%
    \ifPst@xAxis\ifdim\pst@dima<\z@\showoriginfalse\fi\fi% no 0 when x- axis is crossing
    \pst@vlabels{\pst@dimb}{\psk@arrowA}{#3}{#5}%
  \endgroup%
  \fi%
  \ifPst@xAxis%
  \begingroup%
    \ifdim\pst@dimb=\z@\else\showoriginfalse\fi%
    \ifnum\psk@dx=\z@%
      \pst@dimg=\psk@Dx\psxunit%
      \ifdim\pst@dimg<\p@\pst@cnta=\psk@Dx\edef\psk@Dx{-\the\pst@cnta}% v.1.21
      \fi% v.1.21
      \edef\psk@dx{\number\pst@dimg}%
    \fi%
%    \ifPst@yAxis\else\showorigintrue\fi%		2009-10-21
    \pst@hlabels{\pst@dimc}{\psk@arrowB}{#4}{#6}%
    \ifPst@yAxis\showoriginfalse\fi%
    \pst@hlabels{\pst@dima}{\psk@arrowA}{#4}{#6}%
  \endgroup%
  \fi%
% Now close "\pst@hbox" (which is 0-dimensional), and put it at the origin.
  \egroup% 
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \leavevmode\psput@cartesian\pst@hbox%
  \endgroup%
  \ignorespaces%
}
%
\newif\ifis@yAxis%
%
\def\psxs@@axes#1#2#3#4#5#6{% llx,lly,urx,ury,exch,x|y,arrowA,arrowB
  \pst@killglue%
  \begin@SpecialObj%
    \ifx#6x\relax%				% x-axis?
      \is@yAxisfalse%
      \ifnum\psk@dx=\z@%
        \pst@dimg=\psk@Dx\psxunit%
        \def\psk@dx{\number\pst@dimg}%
      \fi%
    \else%
      \is@yAxistrue%
      \ifnum\psk@dy=\z@%
        \pst@dimg=\psk@Dy\psyunit%
        \def\psk@dy{\number\pst@dimg}%
      \fi%
    \fi% 
    \let\pst@linetype\pst@arrowtype%
    \def\pst@axes{axes}%
    \pst@addarrowdef%
    \addto@pscode{
      /showOrigin \ifPst@showOriginTick true \else false \fi def 	% ticks for 0/0 ?
      \ifis@yAxis 0 \pst@number#4 \else \pst@number#3 0 \fi
      \ifis@yAxis 0 \pst@number#2 \else \pst@number#1 0 \fi
      ArrowA
      CP 4 2 roll
      ArrowB 
      2 copy
      /yEnd exch def /xEnd exch def
      \ifx\psk@axesstyle\@none   
        pop pop % axesstyle = none (only ticks) or frame (already drawn)
      \else
        gsave                              		% save current state
        L                                  		% the line with arrows 
        \@nameuse{psls@\pslinestyle}                 	% linestyle for the axes
        stroke                                       	% draw the main line
        grestore
      \fi
      /yStart exch def
      /xStart exch def
%     \psk@ticks: all=0; x=1; y=2; none=3
      \number\psk@ticks\space dup 2 mod 0 eq \ifis@yAxis true \else false \fi and 
      exch 2 lt \ifis@yAxis false \else true \fi and or {
      /viceversa 
        \ifis@yAxis\pst@number#2 \pst@number#4 \else\pst@number#1 \pst@number#3 \fi
         gt { true }{ false } ifelse def           % other way round
      /epsilon 0.01 def                            % rounding errors
      /minTickline \ifis@yAxis \pst@number#1 \else \pst@number#2 \fi def
      /maxTickline \ifis@yAxis \pst@number#3 \else \pst@number#4 \fi def
      /dT \ifis@yAxis \psk@dy \else \psk@dx \fi\space abs  % added abs 2006-07-07
        65536 div viceversa { neg } if def                 % div to get pt instead of sp
      /DT \ifis@yAxis \psk@Dy \else \psk@Dx \fi\space abs viceversa { neg } if def  
      /subTNo \ifis@yAxis\psk@ysubticks\else\psk@xsubticks\fi \space def
      subTNo 0 gt { /dsubT dT subTNo div def}{ /dsubT 0 def } ifelse  % deltaSubTick
      \ifis@yAxis \psk@yticksize \else \psk@xticksize \fi
      /tickend exch def /tickstart exch def
      /Twidth \ifis@yAxis \psk@ytickwidth \else \psk@xtickwidth \fi\space def
      /subTwidth \ifis@yAxis \psk@ysubtickwidth \else \psk@xsubtickwidth \fi\space def
      /STsize \ifis@yAxis \psk@ysubticksize \else \psk@xsubticksize \fi\space def
      /TColor {
        \ifis@yAxis\pst@usecolor\psk@ytickcolor
        \else\pst@usecolor\psk@xtickcolor\fi\space } def
      /subTColor {
        \ifis@yAxis\pst@usecolor\psk@ysubtickcolor
        \else\pst@usecolor\psk@xsubtickcolor\fi\space } def
      /MinValue { \ifis@yAxis yStart \else xStart \fi
        \ifx\psk@arrowA\@empty\else 
          \psk@arrowsize\space CLW mul add \psk@arrowlength\space mul 
           viceversa { sub epsilon add }{ add epsilon sub } ifelse \fi } def
      /MaxValue { \ifis@yAxis yEnd \else xEnd \fi 
        \ifx\psk@arrowB\@empty\else
          \psk@arrowsize\space CLW mul add \psk@arrowlength\space mul 
           viceversa { add epsilon sub }{ sub epsilon add } ifelse \fi } def
      /logLines {
        \ifnum\psk@logLines=\z@ true \else         % all axes
          \ifnum\psk@logLines<\tw@                 % x axis
            \ifis@yAxis false \else true \fi       % do we have x or y axis
          \else
            \ifnum\psk@logLines<\thr@@             % y axis
              \ifis@yAxis true \else false \fi     % do we have x or y axis
            \else 
              false                                % no one
            \fi
          \fi
        \fi
      } def
      /LSstroke {                                  % set linestyle and stroke
        \ifis@yAxis \@nameuse{psls@\psyticklinestyle}
        \else       \@nameuse{psls@\psxticklinestyle}\fi 
        stroke} def
      /subLSstroke {                               % set sublinestyle and stroke
        \ifis@yAxis \@nameuse{psls@\psysubticklinestyle}
        \else       \@nameuse{psls@\psxsubticklinestyle}\fi 
        stroke} def
%\iffalse
% start ticks ---------------------------------------------------------
%      showOrigin { 0 }{ dT } ifelse
      0 dT MaxValue 1 add {                        % the positive part of the axes, step unit is pt
        /cntTick exch def                          % the index
        logLines {                                 % log lines?
          gsave
          1 1 DT {
           1 sub /OffSet exch def
%          1 10 subTNo div 9.99 {                   % do not write a line for 1
%         10 subTNo 1 add div dup 10 {                   % do not write a line for 1
          -10 subTNo 1 add div dup 10 add exch dup -0.1 mul 1 add {                   % do not write a line for 10 and 1, trace lines between 10 and 1 by steps of 10/subTno
            /dx exch def                           % save index
%            /x cntTick dT dx log mul add def       %
            /x dx log OffSet add \ifis@yAxis\pst@number\psyunit\else\pst@number\psxunit\fi\space mul cntTick add def       %
            x abs MaxValue abs le {                % out of range?
	      \ifis@yAxis
	        \ifPst@maxyTicks true \else false \fi
	      \else
	        \ifPst@maxxTicks true \else false \fi
	      \fi
                { x minTickline #5 moveto
                  x maxTickline #5 lineto }
                { x tickstart STsize mul #5 moveto
                  x tickend STsize mul #5 lineto } ifelse
            } if
          } for } for
          subTwidth SLW subTColor                  % set line width and subtick color
          subLSstroke
          grestore                                 % restore main tick status
          stroke
          /dsubT 0 def                             % no other subticks
        } if 					   % end logLines
        dsubT abs 0 gt {                           % du we have subticks?
          gsave                                    % save graphic state
% start subticks ----------------------------------------------------------
          /cntsubTick cntTick dsubT add def
          subTNo 1 sub {
            cntsubTick abs MaxValue abs le {       % out of range?
    	    \ifis@yAxis
              \ifPst@maxyTicks true \else false \fi
    	    \else
              \ifPst@maxxTicks true \else false \fi
    	    \fi
              { cntsubTick minTickline STsize mul #5 moveto
                cntsubTick maxTickline STsize mul #5 lineto }
              { cntsubTick tickstart STsize mul #5 moveto
                cntsubTick tickend STsize mul #5 lineto } ifelse
            }{ exit }  ifelse
            /cntsubTick cntsubTick dsubT add def
          } repeat 
          subTwidth SLW subTColor               % set line width and subtick color
          subLSstroke
% end subticks ----------------------------------------------------------
          grestore                              % restore tick status
        } if
        showOrigin {
          gsave
          \ifis@yAxis
            \ifPst@maxyTicks true \else false \fi
          \else
            \ifPst@maxxTicks true \else false \fi
          \fi
            { cntTick minTickline #5 moveto
              cntTick maxTickline #5 lineto }
            { cntTick tickstart #5 moveto        % line begin main Tick
              cntTick tickend #5 lineto } ifelse % lineto tick end
          Twidth SLW TColor                      % set line width and tick color
          LSstroke
          grestore
        }{ /showOrigin true def } ifelse         % only for the very first tick valid
      } for
% end ticks ----------------------------------------------------------
%\fi
%\iffalse
% ================================================ % the other side 
      /showOrigin \ifPst@showOriginTick true \else false \fi def % ticks for 0/0 ?
      /dT dT neg def                               % the other side of the axis
      /dsubT dsubT neg def
% start ticks ----------------------------------------------------------
%      showOrigin { 0 }{ dT } ifelse
      0 dT MinValue epsilon viceversa { add }{ sub } ifelse {
        /cntTick exch def
        logLines {                                 % log lines?
          gsave
          1 1 DT cvi {
            1 sub /OffSet exch def
          -10 subTNo 1 add div dup 10 add exch dup -0.1 mul 1 add {                   % do not write a line for 10 and 1, trace lines between 10 and 1 by steps of 10/subTno
%			10 subTNo 1 add div dup 10 {           % do not write a line for 1
%          1 10 subTNo div 9.99 {                   % do not write a line for 1
            /dx exch def                           % save index
%            /x cntTick dT dx log mul add def       %
            /x dx log OffSet add \ifis@yAxis\pst@number\psyunit\else\pst@number\psxunit\fi\space mul cntTick add def
            x abs MinValue abs le {                % out of range?
	      \ifis@yAxis
	        \ifPst@maxyTicks true \else false \fi
	      \else
	        \ifPst@maxxTicks true \else false \fi
	      \fi
                { x minTickline #5 moveto
                  x maxTickline #5 lineto }
                { x tickstart STsize mul #5 moveto
                  x tickend STsize mul #5 lineto } ifelse
            } if
          } for } for
          /dsubT 0 def 
          subTwidth SLW subTColor                  % set line width and subtick color
          subLSstroke
          grestore
        }                                          % end loglines
        dsubT abs 0 gt {                           % do we have subticks?
          gsave                                    % save main state
% start subticks ----------------------------------------------------------
          /cntsubTick cntTick dsubT add def
          subTNo 1 sub {
            cntsubTick abs MinValue abs le {       % out of range?
              cntsubTick tickstart STsize mul #5 moveto
              cntsubTick tickend STsize mul #5 lineto
            }{ exit } ifelse
            /cntsubTick cntsubTick dsubT add def
          } repeat % for
% end subticks ----------------------------------------------------------
          subTwidth SLW subTColor                  % set line width and subtick color
          subLSstroke
          grestore                                 % restore main state
        } if
        showOrigin {
          gsave
          cntTick tickstart #5 moveto         	% line begin main Tick
          cntTick tickend #5 lineto    	       	% lineto tick end
          Twidth SLW TColor                         % set line width and tick color
          LSstroke
          grestore
        }{ /showOrigin true def } ifelse         % only for the very first tick valid
      } for
% end ticks ----------------------------------------------------------
%\fi    
    } if
   }%	end of \pscode
  \end@SpecialObj%
  % now draw the axes again with the correct linecolor
  \ifx\psk@axesstyle\@none\else
    \ifPst@yAxis\psline[linecolor=\pslinecolor](0,#2)(0,#4)\fi%
    \ifPst@xAxis\psline[linecolor=\pslinecolor](#1,0)(#3,0)\fi%
  \fi%
  \ignorespaces%
}%
%
\def\psxs@frame{%
  \psset{axesstyle=none}%
  \begin@SpecialObj%
    \addto@pscode{					% the frame
      \pst@number\pst@dima \psk@frameOffset sub \pst@number\pst@dimb \psk@frameOffset sub moveto 	% lower left
      \pst@number\pst@dimc \psk@frameOffset add \pst@number\pst@dimb \psk@frameOffset sub L	% upper left
      \pst@number\pst@dimc \psk@frameOffset add \pst@number\pst@dimd \psk@frameOffset add L 	% upper right
      \pst@number\pst@dima \psk@frameOffset sub \pst@number\pst@dimd \psk@frameOffset add L 	% lower right
      closepath 
      }%
    \pst@stroke%
    \psk@fillstyle%
  \end@SpecialObj%
  \let\psk@arrowA\@empty%
  \let\psk@arrowB\@empty%
  \pst@xticksizeC=\z@\pst@yticksizeC=\z@  
  \ifPst@xAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{}{x}\fi%		x axis
  \ifPst@yAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{ exch }{y}\fi%	y axis
  \ifnum\psk@tickstyle=\tw@	% llx,lly,urx,ury,exch,x|y,arrowA,arrowB	
    \psDEBUG[psxs@frame]{psk@tickstyle=2 (inner)}%
    \psDEBUG[psxs@frame]{pst@dima=\pst@number\pst@dima}%
    \psDEBUG[psxs@frame]{pst@dimb=\pst@number\pst@dimb}%
    \psDEBUG[psxs@frame]{pst@dimc=\pst@number\pst@dimc}%
    \psDEBUG[psxs@frame]{pst@dimd=\pst@number\pst@dimd}%
    \ifPst@xAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{ neg \pst@number\pst@dimd add }{x}\fi%	% upper x axis
    \ifPst@yAxis\psxs@@axes\pst@dima\pst@dimb\pst@dimc\pst@dimd{ neg \pst@number\pst@dimc add exch }{y}\fi%  right y axis
  \fi%
}
%
%\def\psk@EndAngle{360}% be sure that it isn't undefined
%\define@key[psset]{pst-plot}{quadrant}[4]{%
%  \ifcase#1 \or
%    \def\psk@EndAngle{90}\or
%    \def\psk@EndAngle{180}\or
%    \def\psk@EndAngle{270}\else
%    \def\psk@EndAngle{360}%
%  \fi}
%\psset[pst-plot]{quadrant=4}

\def\psxs@polar{% (rx,ry) % all other values are ignored
  \pst@killglue
  \begingroup
  \edef\pst@dimC{\strip@pt\pst@dimc}% 			RadiusX
  \pstFPDiv\pstR@dius{\pst@dimC}{\strip@pt\psxunit}%	in cm and as integer
  \edef\pst@dimD{\strip@pt\pst@dimd}% 			RadiusX
  \pstFPDiv\psk@EndAngle{\pst@dimD}{\strip@pt\psyunit}%	in cm and as integer
  \ifnum\psk@EndAngle=0 \def\psk@EndAngle{360}\fi
  \use@keep@par
  \pstFPDiv\pstN@lpha{\psk@EndAngle}{\psk@Dy}% 			No. of (int) main lines
  \pstFPdiv\pstd@lpha{\psk@Dy}{\psk@ysubticks}% 	sub dAlpha
  \pstFPdiv\pstdR@dius{1}{\psk@xsubticks}%		sub dRadius
  \pst@cntm=\psk@xsubticks\advance\pst@cntm by \m@ne
  \multido{\iA=\psk@Dx+\psk@Dx,\rB=\pstdR@dius+\psk@Dx,\iB=0+1}{\pstR@dius}{%
    \multido{\rA=\rB+\pstdR@dius}{\the\pst@cntm}{%
      \psarc[linestyle=\psxsubticklinestyle,
         linecolor=\psk@xsubtickcolor,linewidth=\psk@xsubtickwidth pt](0,0){\rA}{0}{\psk@EndAngle}}    
    \psarc[linestyle=\psxticklinestyle,linecolor=\psk@xtickcolor,
		linewidth=\psk@xtickwidth pt](0,0){\iA}{0}{\psk@EndAngle}%
    \ifnum\psk@labels<2\relax% is all or x (0,1)
      \uput[-45](\iB,0){\pshlabel{\iB}}\uput[45](0,\iB){\pshlabel{\iB}}%
    \fi%
  }%
%  \uput[-45](\pstR@dius,0){\pstR@dius}\uput[45](0,\pstR@dius){\pstR@dius}%
  \pst@cntm=\psk@ysubticks\advance\pst@cntm by \m@ne
  \multido{\iA=\psk@Dy+\psk@Dy,\rB=\pstd@lpha+\psk@Dy}{\pstN@lpha}{%
    \multido{\rA=\rB+\pstd@lpha}{\the\pst@cntm}{\psline[linestyle=\psysubticklinestyle,
      linecolor=\psk@ysubtickcolor,linewidth=\psk@ysubtickwidth pt](\pstR@dius;\rA)} 
    \psline[linestyle=\psyticklinestyle,
      linecolor=\psk@ytickcolor,linewidth=\psk@ytickwidth pt](\pstR@dius;\iA)%
    \ifodd\psk@labels\else% is all or y (0,3)
      \uput[\iA](\pstR@dius;\iA){\psvlabel{\iA}}%
    \fi%
  }%
  \ifnum\psk@EndAngle<360 \psline[linestyle=\psyticklinestyle,
      linecolor=\psk@ytickcolor,linewidth=\psk@ytickwidth pt](\pstR@dius;0)\fi
  \endgroup\ignorespaces%
  \Pst@xAxisfalse\Pst@yAxisfalse%
}
%
\def\@polar{polar}
\define@key[psset]{pst-plot}{axesstyle}[axes]{%
  \@ifundefined{psxs@#1}%
    {\@pstrickserr{Axes style `#1' not defined}\@eha}%
    {\def\psk@axesstyle{#1}%
     \ifx\psk@axesstyle\@polar\psset{Dy=30}\fi}}
\psset[pst-plot]{axesstyle=axes}
\define@key[psset]{pst-plot}{xLabels}[]{\def\psk@xLabels{#1}}
\define@key[psset]{pst-plot}{xLabelsRot}[0]{\pst@getangle{#1}\pst@xLabelsRot}
\psset[pst-plot]{xLabels=,xLabelsRot=0}
\define@key[psset]{pst-plot}{yLabels}[]{\def\psk@yLabels{#1}}
\define@key[psset]{pst-plot}{yLabelsRot}[0]{\pst@getangle{#1}\pst@yLabelsRot}
\psset[pst-plot]{yLabels=,yLabelsRot=0}
%
% #1:Max/Min in pt from origin; #2:arrow; #3:min; #4:max
\def\pst@hlabels#1#2#3#4{%
 \kern\psk@xlabelOffset pt%            % set the x offset?
 \ifx\empty\psk@xLabels
  \ifdim#1=\z@\else%                   % start from 0 ?
    \ifx#2\empty\else\advance#1\ifdim#1>\z@-\fi7\pslinewidth\fi%
    \pst@cnta=#1\relax%                % Distance (in sp) to end.
    \divide\pst@cnta\psk@dx\relax%     % Number of ticks/labels
    \ifnum\pst@cnta=\z@\else%
      \pst@dimb=\psk@dx sp%            % Space between ticks.
        \ifPst@yAxis\else\showorigintrue\fi%
        \ifnum\psk@labels<\tw@\ifPst@xAxis\pst@@hlabels\fi\fi%
        \showoriginfalse%
    \fi%
  \fi%
 \else
  \pst@cnta=#1\relax%                % Distance (in sp) to end.
  \pstFPdiv\pst@tempA{\the\pst@cnta}{\psk@dx}
  \pstFPadd\pst@tempA{1.55}{\pst@tempA}   % to prevent rounding errors
  \edef\pst@tempB{\pst@int{\pst@tempA}}
%  \divide\pst@cnta\psk@dx\relax%     % Number of ticks/labels
  \edef\pst@tempA{\psk@Dx}
  \multido{\iB=#3+1,\rB=#3+\pst@tempA}{\pst@tempB}%
    {\uput{\psxlabelsep}[-90]{\pst@xLabelsRot}(\rB,0)%\psxlabelsep)
    {\strut\pshlabel{\psPutXLabel{\iB}}}}%
 \fi%
}
% Knows \pst@dimb and \pst@cnta
\def\pst@@hlabels{%
  \psDEBUG[pst@@hlabels]{xticksizeC=\the\pst@xticksizeC}%
  \setbox\z@=\vbox{%			save all in a box
    \ifcase\psk@xlabelPos% 0
      \vskip-\pst@xticksizeA\vskip\psxlabelsep\or % 1
      \vskip-1ex\vskip-\pslabelsep\or % 2
      \vskip-\pst@xticksizeB\vskip-\psxlabelsep\vskip-1ex % 3
    \fi
    \ifnum\pst@cnta<\z@ \pst@dimb=-\pst@dimb\fi
    \hbox to\z@{%
      \ifshoworigin\hbox to \z@{\hss\pst@@@hlabel{\psk@Ox}\hss}\fi%
      \mmultido{\nA=\psk@Ox+\psk@Dx}{\pst@cnta}{%
        \hskip\pst@dimb\hbox to \z@{\hss%
          \ifdim\nA pt=\z@ \pst@@@hlabel{0}%
          \else\expandafter\pst@@@hlabel{\nA}%
          \fi% prevent -0, doesn't work with \ifnum
        \hss}%
      }\hss%
    }%
  }\ht\z@\z@ \dp\z@\z@ \box\z@}% set all values to zero
%
% #1:Max/Min in pt from origin; #2:arrow; #3:min; #4:max
% \psk@labels 0:all; 1:x; 2:y; 3:none
\def\pst@vlabels#1#2#3#4{%
 \ifx\empty\psk@yLabels
   \ifdim#1=\z@\else%
    \ifx#2\empty\else\advance#1\ifdim#1>\z@-\fi7\pslinewidth\fi%
    \pst@cnta=#1\relax%          %      % Distance (in sp) to end.
    \divide\pst@cnta\psk@dy\relax%   % Number of ticks/labels
    \ifnum\pst@cnta=\z@\else%
      \pst@dima=\psk@dy sp%            % Space between ticks.
      \ifodd\number\psk@labels\else\ifPst@yAxis\pst@@vlabels\fi\fi%
      \showoriginfalse%
    \fi%
  \fi%
 \else%
  \pst@cnta=#1\relax%          %      % Distance (in sp) to end.
  \pstFPdiv\pst@tempA{\the\pst@cnta}{\psk@dy}
  \pstFPadd\pst@tempA{1.55}{\pst@tempA}   % to prevent rounding errors
  \edef\pst@tempB{\pst@int{\pst@tempA}}
%  \divide\pst@cnta\psk@dy\relax%   % Number of ticks/labels
  \edef\pst@tempA{\psk@Dy}
  \multido{\nA=#3+1,\rA=#3+\pst@tempA}{\pst@tempB}{\uput{\psylabelsep}[180]{\pst@yLabelsRot}(0,\rA){%
    \strut\expandafter\psvlabel\expandafter{\psPutYLabel{\nA}}}}%
 \fi%
}
% \pst@dima: the width between two labels in pt
% \pst@dimc: the coordinate of the origin in pt
% \pst@cnta: the lowest label
% \pst@ticksizeC the lowest or highest value
\def\pst@@vlabels{%
  \psDEBUG[pst@@vlabels]{yticksizeC=\the\pst@yticksizeC}% for left labels we use \def\llap#1{\hb@xt@\z@{\hss#1}}
  \vbox to\z@{%
  \vbox to -\psk@ylabelOffset pt{}% the y label offset
    \ifnum\pst@cnta>\z@ \pst@dima=-\pst@dima\fi%  up or down label positions
    \offinterlineskip%
    \ifshoworigin%
      \vbox to \z@{\vss\hbox to\z@{%
        \ifcase\psk@ylabelPos%
	  \hss\pst@@@vlabel{\psk@Oy}\hskip\psylabelsep\hskip-\pst@yticksizeA\or%
	  \hskip\pslabelsep\hss\pst@@@vlabel{\psk@Oy}\hss\or		% right labels
	  \hskip\pst@yticksizeB\hskip\psylabelsep\pst@@@vlabel{\psk@Oy}%
	\fi}\vss}%
    \fi%
    \mmultido{\nA=\psk@Oy+\psk@Dy}{\pst@cnta}{%
      \vbox to\pst@dima{\vss}%
      \vbox to \z@{%
        \vss\hbox to\z@{%
        \ifcase\psk@ylabelPos% and also check for -0
	  \hss\ifdim\nA pt=\z@ \pst@@@vlabel{0}\else\pst@@@vlabel{\nA}\fi%
	    \hskip\psylabelsep\hskip-\pst@yticksizeA\or% top
	  \hss\ifdim\nA pt=\z@\pst@@@vlabel{0}\else\pst@@@vlabel{\nA}\fi%
	  \ifdim\psylabelsep=\z@\hss\else\kern-\psylabelsep\fi\or%   axis
	  \hskip\pst@yticksizeB\hskip\psylabelsep%
	  \ifdim\nA pt=\z@\pst@@@vlabel{0}\else\pst@@@vlabel{\nA}\fi% bottom
	\fi}\vss}%
    }\vss}%
}
%
\define@key[psset]{pst-plot}{xAxisLabel}[x]{\def\psk@xAxisLabel{#1}}
\define@key[psset]{pst-plot}{yAxisLabel}[y]{\def\psk@yAxisLabel{#1}}
\psset[pst-plot]{xAxisLabel=x,yAxisLabel=y}
\define@key[psset]{pst-plot}{xAxisLabelPos}[{}]{\def\psk@xAxisLabelPos{#1}}
\define@key[psset]{pst-plot}{yAxisLabelPos}[{}]{\def\psk@yAxisLabelPos{#1}}
\psset[pst-plot]{yAxisLabelPos={},xAxisLabelPos={}}
%
\newdimen\psk@llx
\newdimen\psk@lly
\newdimen\psk@urx
\newdimen\psk@ury
\define@key[psset]{pst-plot}{llx}[\z@]{\pssetxlength\psk@llx{#1}}
\define@key[psset]{pst-plot}{lly}[\z@]{\pssetylength\psk@lly{#1}}
\define@key[psset]{pst-plot}{urx}[\z@]{\pssetxlength\psk@urx{#1}}
\define@key[psset]{pst-plot}{ury}[\z@]{\pssetylength\psk@ury{#1}}
\psset[pst-plot]{llx=\z@, lly=\z@, urx=\z@, ury=\z@}% prevents rounding errors 
%
\define@boolkey[psset]{pst-plot}[Pst@]{psgrid}[true]{}
\define@key[psset]{pst-plot}{gridpara}[{}]{\def\psk@gridpara{#1}}
\define@key[psset]{pst-plot}{gridcoor}[\relax]{\def\psk@gridcoor{#1}}
\psset[pst-plot]{psgrid=false,gridpara={},gridcoor=\relax}
%
\newdimen\pst@xunit
\newdimen\pst@yunit
%
\def\pslegend{\@ifnextchar[\pslegend@i{\pslegend@i[rt]}}
\def\pslegend@i[#1]{\@ifnextchar({\pslegend@ii[#1]}{\pslegend@ii[#1](\pst@number\pslabelsep,\pst@number\pslabelsep)}}
\def\pslegend@ii[#1](#2,#3)#4{%
  \gdef\pslegend@ref{#1}%
  \xdef\pslegend@sepx{#2 }%
  \xdef\pslegend@sepy{#3 }%
  \gdef\pslegend@text{#4}}
%
\newpsstyle{legendstyle}{fillstyle=solid,fillcolor=white,linewidth=0.5pt}
%
\def\pslegend@iii[#1](#2){\rput[#1](#2){\psframebox[style=legendstyle]{%
  \footnotesize\tabcolsep=2pt%
  \tabular[t]{@{}ll@{}}\pslegend@text\endtabular}}\global\let\pslegend@text\relax}
\let\pslegend@text\relax% define it as empty
%
\def\psgraph{\pst@object{psgraph}}
\def\psgraph@i{\pst@getarrows\psgraph@ii}
\def\psgraph@ii(#1,#2){\catcode`\!=12\relax
  \@ifnextchar({\psgraph@iii(#1,#2)}{\psgraph@iv(0,0)(#1,#2)}}
\def\psgraph@iii(#1,#2)(#3,#4){\@ifnextchar({\psgraph@v(#1,#2)(#3,#4)}{\psgraph@iv(#1,#2)(#3,#4)}}
%
\def\psgraph@iv(#1,#2)(#3,#4)#5#6{%  no special origin defined
% minX | minY | maxX | maxY | Length x-axis | length y-axis%  
  \pst@killglue%
  \begingroup%
  \bgroup%
  \use@keep@par%
  \ifPst@psgrid%
     \expandafter\psset\expandafter{\psk@gridpara}%
      \rput(0,0){\expandafter\psgrid\psk@gridcoor}  
  \fi%
  \egroup%
  \pstFPsub\pst@tempA{#3}{#1}%
  \pst@dimm=#5%
  \pst@dimo=\pst@tempA pt%
  \pstFPdiv\pst@@dx{\strip@pt\pst@dimm}{\pst@tempA}%
  \pst@xunit=\pst@@dx\p@%
%
  \ifx!#6\let\pst@yunit=\pst@xunit\else%
    \pst@dimm=#6%
%  \pst@dimm=\pst@@dx\pst@dimo\else\pst@dimm=#6\fi%
    \pstFPsub\pst@tempA{#4}{#2}%
    \pstFPdiv\pst@@dy{\strip@pt\pst@dimm}{\pst@tempA}%
    \pst@yunit=\pst@@dy\p@%
  \fi%
  %
  \pst@dimm=#1\pst@xunit\advance\pst@dimm by \psk@llx%
  \pst@dimn=#2\pst@yunit\advance\pst@dimn by \psk@lly%
  \pst@dimo=#3\pst@xunit\advance\pst@dimo by \psk@urx%
  \pst@dimp=#4\pst@yunit\advance\pst@dimp by \psk@ury%
  \if@star\pspicture*(\pst@dimm,\pst@dimn)(\pst@dimo,\pst@dimp)\else%
  \pspicture(\pst@dimm,\pst@dimn)(\pst@dimo,\pst@dimp)\fi%
  \let\psxunit\pst@xunit \let\psyunit\pst@yunit%
  \ifdim\pst@xunit=\pst@yunit\relax\psset[pstricks]{runit=\pst@xunit}\fi%
  \bgroup%
  \use@par%
  \psaxes(#1,#2)(#3,#4)%
  \egroup%
  \psgraph@vi(#1,#2)(#1,#2)(#3,#4)%
}
\def\psgraph@v(#1,#2)(#3,#4)(#5,#6)#7#8{%  with special origin
% Xorig | yorig | minX | minY | maxX | maxY | Length x-axis | length y-axis%  
  \pst@killglue%
  \begingroup%
  \bgroup%
  \use@keep@par%
  \ifPst@psgrid%
     \expandafter\psset\expandafter{\psk@gridpara}%
      \rput(0,0){\expandafter\psgrid\psk@gridcoor}
  \fi%
  \egroup%
  \pstFPsub\pst@tempA{#5}{#3}%
  \pst@dimm=#7%
  \pst@dimo=\pst@tempA pt%
  \pstFPdiv\pst@@dx{\strip@pt\pst@dimm}\pst@tempA%
  \pst@xunit=\pst@@dx\p@%
%
  \ifx!#8\let\pst@yunit=\pst@xunit\else
    \pst@dimm=#8%
    \pstFPsub\pst@tempA{#6}{#4}%
    \pstFPdiv\pst@@dy{\strip@pt\pst@dimm}\pst@tempA%
    \pst@yunit=\pst@@dy\p@%
  \fi%
  %
  \pst@dima=#3\pst@xunit \advance\pst@dima by \psk@llx%
  \pst@dimb=#4\pst@yunit \advance\pst@dimb by \psk@lly%
  \pst@dimc=#5\pst@xunit \advance\pst@dimc by \psk@urx%
  \pst@dimd=#6\pst@yunit \advance\pst@dimd by \psk@ury%
  \if@star\pspicture*(\pst@dima,\pst@dimb)(\pst@dimc,\pst@dimd)\else%
          \pspicture(\pst@dima,\pst@dimb)(\pst@dimc,\pst@dimd)\fi%
  \psset[pstricks]{xunit=\pst@xunit,yunit=\pst@yunit}
  \ifdim\pst@xunit=\pst@yunit \psset[pstricks]{runit=\pst@xunit}\fi%
  \bgroup%
  \use@par%
  \psaxes(#1,#2)(#3,#4)(#5,#6)%
  \egroup%
  \psgraph@vi(#1,#2)(#3,#4)(#5,#6)%
}
%
\def\setxLabelC@@r#1,#2(#3,#4)(#5){%
  \pst@getcoor{#5}\pst@tempB%
  \ifx c#1 
    \pssetylength\pst@dimm{#2}%
    \rput(! #4 #3 add 2 div \pst@number\pst@dimm \pst@tempB\space exch pop add 
      \pst@number\psyunit div ){\psk@xAxisLabel}%
  \else%
    \pst@getcoor{\psk@xAxisLabelPos}\pst@tempA%
    \rput(! \pst@tempA\space \pst@tempB\space exch pop add \tx@UserCoor ){\psk@xAxisLabel}%
  \fi}
\def\setyLabelC@@r#1,#2(#3,#4)(#5){%
  \pst@getcoor{#5}\pst@tempB%
  \ifx c#2
    \pssetxlength\pst@dimm{#1}%
    \rput{90}(! \pst@number\pst@dimm \pst@tempB\space pop add \pst@number\psxunit div #4 #3 add 2 div ){\psk@yAxisLabel}%
  \else%
    \pst@getcoor{\psk@yAxisLabelPos}\pst@tempA%
    \rput{90}(! \pst@tempB\space pop \pst@tempA\space 3 1 roll add exch \tx@UserCoor ){\psk@yAxisLabel}%
  \fi}
%  
\def\psgraph@vi(#1,#2)(#3,#4)(#5,#6){%
  \ifx\psk@xAxisLabel\@empty\else%
    \ifx\psk@xAxisLabelPos\@empty\uput[0](#5,#2){\psk@xAxisLabel}%
    \else\expandafter\setxLabelC@@r\psk@xAxisLabelPos(#3,#5)(#1,#2)\fi%
  \fi%
  \ifx\psk@yAxisLabel\@empty\else%
    \ifx\psk@yAxisLabelPos\@empty\uput[90](#1,#6){\psk@yAxisLabel}%
    \else\expandafter\setyLabelC@@r\psk@yAxisLabelPos(#4,#6)(#1,#2)\fi%
  \fi%
  \def\lt@@{lt}\def\lb@@{lb}\def\rb@@{rb}%
  \ifx\pslegend@ref\lb@@    \gdef\pslegend@coor{#3 \pslegend@sepx \pst@number\psxunit div add 
                                                   \pslegend@sepy \pst@number\psyunit div}%
  \else%
    \ifx\pslegend@ref\lt@@  \gdef\pslegend@coor{#3 \pslegend@sepx \pst@number\psxunit div add 
                                                #6 \pslegend@sepy \pst@number\psyunit div sub}%
    \else%
      \ifx\pslegend@ref\rb@@\gdef\pslegend@coor{#5 \pslegend@sepx \pst@number\psxunit div sub 
                                                   \pslegend@sepy \pst@number\psyunit div}%
      \else                 \gdef\pslegend@coor{#5 \pslegend@sepx \pst@number\psxunit div sub 
                                                #6 \pslegend@sepy \pst@number\psyunit div sub}%
      \fi%
    \fi%
  \fi%
  \xdef\psgraphLLx{#3}\xdef\psgraphLLy{#4}\xdef\psgraphURx{#5}\xdef\psgraphURy{#6}%
  \ignorespaces
}
%
\def\endpsgraph{%
%  \pst@killglue%
  \ifx\relax\pslegend@text\relax \else\pslegend@iii[\pslegend@ref](!\pslegend@coor)\fi%
  \endpspicture%
  \endgroup\ignorespaces}
%
\@namedef{psgraph*}{\psgraph*}
\@namedef{endpsgraph*}{\endpsgraph}
%
\def\psPutXLabel#1{%
  \global\pst@cnto=0\relax
  \global\pst@cntp=#1\relax
  \expandafter\get@Label\psk@xLabels,,\@nil%
}
\def\psPutYLabel#1{%        
  \global\pst@cnto=0\relax
  \global\pst@cntp=#1\relax
  \expandafter\get@Label\psk@yLabels,,\@nil%
}
\def\get@Label#1,#2,#3\@nil{%
    \ifnum\the\pst@cnto<\the\pst@cntp
      \global\advance\pst@cnto by \@ne 
      \ifx\relax#3\relax\else\expandafter\get@Label#2,#3\@nil\fi%
    \else #1\fi%
}
%
\def\psVectorfield{\pst@object{psVectorfield}}
\def\psVectorfield@i(#1,#2)(#3,#4)#5{{%
  \addbefore@par{Dx=0.1,Dy=0.1,Ox=3,arrows=->,linewidth=0.2pt}%
  \begin@SpecialObj
  \SpecialCoor
  \pstFPsub\pst@tempA{#3}{#1}%
  \pstFPsub\pst@tempB{#4}{#2}%
  \pstFPDiv{\pst@tempC}{\pst@tempA}{\psk@Dx}%
  \pstFPDiv{\pst@tempD}{\pst@tempB}{\psk@Dy}%
  \pstVerb{ /yStrich \ifPst@algebraic (#5) tx@AlgToPs begin AlgToPs end cvx
                \else { #5 } \fi def }%
  \multido{\rX=#1+\psk@Dx}{\numexpr\pst@tempC+1}{%
    \multido{\rY=#2+\psk@Dy}{\numexpr\pst@tempD+1}{%
       \psline%
         (! /x \rX\space def 
%           /ocount 0 def  %%%%%%%%%%%%%%%%%%%% WARUM???? %%%%%%%%
            /y \rY\space def 
            /yTemp yStrich \psk@Dx\space \psk@Ox\space div mul def 
            \rX\space \psk@Dx\space \psk@Ox\space div sub \rY\space yTemp sub)%
         (! /x \rX\space def 
%           /ocount 0 def  %%%%%%%%%%%%%%%%%%%% WARUM???? %%%%%%%%
            /y \rY\space def 
            /yTemp yStrich \psk@Dx\space \psk@Ox\space div mul def 
            \rX\space \psk@Dx\space \psk@Ox\space div add \rY\space yTemp add)%
   }}%
  \end@SpecialObj
}\ignorespaces}  
%
\def\psFixpoint{\pst@object{psFixpoint}}
\def\psFixpoint@i#1#2#3{% #1: xStart #2: f(x) #3: number of iterations
  \pst@killglue%
  \begingroup%
  \use@par%
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{
    \psplot@init
      /x #1 def
      /F@pstplot \ifPst@algebraic (#2) tx@AlgToPs begin AlgToPs end cvx
                 \else { #2 } \fi  def
      /xy { x \pst@number\psxunit mul F@pstplot dup /x ED \pst@number\psyunit mul } def 
  }%
  \gdef\psplot@init{}%
  \@pstfalse%
  \@nameuse{testqp@\psplotstyle}%
  \addto@pscode{
      mark
      x \pst@number\psxunit mul 0
      /n 2 def
      #3 {
        xy 
        dup dup 
        /n n 4 add def
      } repeat 
  }%
  \@nameuse{endplot@\psplotstyle}%
  \endgroup%
  \ignorespaces}
%
\define@boolkey[psset]{pst-plot}[Pst@]{showDerivation}[true]{}
\psset{showDerivation}
%
\def\psNewton{\pst@object{psNewton}}
\def\psNewton@i#1#2{\@ifnextchar[{\psNewton@ii{#1}{#2}}{\psNewton@iii{#1}{#2}}}
\def\psNewton@ii#1#2[#3]#4{% #1:xStart #2:f(x) #3:f'(x) #4:number of iterations
  \pst@killglue%
  \begingroup%
  \addbefore@par{showDerivation}%
  \use@par%
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{
    \psplot@init
      /x #1 def
      /F@pstplot \ifPst@algebraic (#2) tx@AlgToPs begin AlgToPs end cvx \else { #2 } \fi  def
      /F@pstplotDerive \ifPst@algebraic (#3) tx@AlgToPs begin AlgToPs end cvx \else { #3 } \fi  def
      /newxVal { % y on stack
        F@pstplotDerive % we have m
        div neg %\pst@number\psxunit div % new x val = -y0/m
      } def
  }%
  \gdef\psplot@init{}%
  \@pstfalse%
  \@nameuse{testqp@\psplotstyle}%
  \addto@pscode{
      mark
      x 0 \tx@ScreenCoor % start point
      /n 2 def
      #4 {
        F@pstplot /yVal ED
        x yVal \tx@ScreenCoor
        /n n 2 add def
        yVal newxVal x add /x ED
        x 0 \tx@ScreenCoor 
        \ifPst@showDerivation /n n 4 add def \else moveto /n n 2 add def\fi
      } repeat 
      pstack
  }%
  \@nameuse{endplot@\psplotstyle}%
  \endgroup%
  \ignorespaces}
\def\psNewton@iii#1#2#3{% #1:xStart #2:f(x) #3:number of iterations
  \pst@killglue%
  \begingroup%
  \addbefore@par{VarStepEpsilon=0.01,showDerivation}%
  \use@par%
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{
    \psplot@init
      /epsilon \psk@VarStepEpsilon\space def
      /x #1 def
      /F@pstplot \ifPst@algebraic (#2) tx@AlgToPs begin AlgToPs end cvx \else { #2 } \fi  def
      /newxVal { % y on stack
        /saveX x def
        saveX epsilon add /x ED F@pstplot saveX epsilon sub /x ED F@pstplot sub epsilon dup add div % we have m
        div neg % new x val = -y0/m
        /x saveX def
      } def
  }%
  \gdef\psplot@init{}%
  \@pstfalse%
  \@nameuse{testqp@\psplotstyle}%
  \addto@pscode{
      mark
      x 0 \tx@ScreenCoor % start point
      /n 2 def
      #3 {
        F@pstplot /yVal ED
        x yVal \tx@ScreenCoor
        yVal newxVal x add /x ED
        x 0 \tx@ScreenCoor 
        \ifPst@showDerivation /n n 4 add def \else moveto /n n 2 add def\fi
      } repeat 
  }%
  \@nameuse{endplot@\psplotstyle}%
  \endgroup%
  \ignorespaces}
%
\def\psResetPlotValues{%
  \psset{method={}}%
}%
\catcode`\@=\TheAtCode\relax
\endinput
%%
%% END pst-plot.tex


==> pst-tools.tex <==
%% $Id: pst-tools.tex 599 2011-11-03 19:38:28Z herbert $
%%
%% This is file `pst-tools.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pst-tools.tex'
%%
%% Herbert Voss <hvoss@tug.org>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-tools' is a PSTricks package for helper functions
%%
%%
\csname PSTtoolsLoaded\endcsname
\let\PSTtoolsLoaded\endinput

\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey.tex \fi
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
% interface to the `xkeyval' package
\pst@addfams{pst-tools}
%
\def\fileversion{0.05}
\def\filedate{2014/05/12}
\message{`PST-tools' v\fileversion, \filedate\space (hv)}
%
\define@key[psset]{pst-tools}{decimalSeparator}[.]{\def\psk@decimalSeparator{#1}}%
\define@boolkey[psset]{pst-tools}[Pst@]{comma}[true]{%
  \ifPst@comma\def\psk@decimalSeparator{,}\else\def\psk@decimalSeparator{.}\fi}
\define@boolkey[psset]{pst-tools}[Pst@]{trimSpaces}[true]{}
\define@key[psset]{pst-tools}{xShift}[0]{\def\psk@xShift{#1}}
\define@key[psset]{pst-tools}{yShift}[0]{\def\psk@yShift{#1}}
\define@key[psset]{pst-tools}{postString}[]{\def\psk@postString{#1}}
\define@key[psset]{pst-tools}{VarName}[]{\def\psk@VarName{#1 }}
\define@key[psset]{pst-tools}{PSfont}[Times-Roman]{\def\psk@PSfont{/#1 }}
\define@key[psset]{pst-tools}{valuewidth}[10]{\pst@getint{#1}\psk@valuewidth }
\define@key[psset]{pst-tools}{fontscale}[10]{\pst@checknum{#1}\psk@fontscale }
\define@key[psset]{pst-tools}{decimals}[-1]{\pst@getint{#1}\psk@decimals }
\psset[pst-tools]{PSfont=Times-Roman,fontscale=10,valuewidth=10,decimals=-1,
                  xShift=0,yShift=0,trimSpaces=false,postString={},VarName={},
                  comma=false,decimalSeparator=.}
%
\def\txG{ true setglobal globaldict begin }
\def\etxG{ end false setglobal }
%
\def\psPrintValue{\pst@object{psPrintValue}}
\def\psPrintValue@i#1{\expandafter\psPrintValue@ii#1,,\@nil}
\def\psPrintValue@ii#1,#2,#3\@nil{%  #1,#2 only for algebraic code
  \begin@SpecialObj
  \addto@pscode{  
     gsave \psk@PSfont findfont \psk@fontscale scalefont setfont 
     \ifPst@algebraic 
       /x #1 def 
       /Func (#2) tx@AlgToPs begin AlgToPs end cvx def 
       Func 
     \else #1 \fi
     \ifx\relax\psk@VarName\relax\else dup \txG 10 string cvs /\psk@VarName\space exch def \etxG \fi
     \psk@decimals -1 gt { 10 \psk@decimals exp dup 3 1 roll mul cvi exch div } if
     \psk@valuewidth string cvs %/Output exch def % save output
%/concatstringarray{  %  [(a) (b) ... (z)] --> (ab...z)  20100422
     \ifx\relax\psk@postString\relax\else [ exch (\psk@postString) ] concatstringarray \fi
     \ifPst@trimSpaces rightTrim \fi
     \ifPst@comma dot2comma \fi        % do we have to change dot to comma
     \psk@xShift\space \psk@yShift\space moveto  %Output 
     show grestore
  }%
  \end@SpecialObj%
}

\define@boolkey[psset]{pst-tools}[Pst@]{round}[true]{}%
\define@boolkey[psset]{pst-tools}[Pst@]{science}[true]{%
  \ifPst@science\def\psk@Scin{true }\else\def\psk@Scin{false }\fi}
\psset[pst-tools]{science=false,round=false}
\def\psPrintValueNew{\pst@object{psPrintValueNew}}
\def\psPrintValueNew@i#1{\expandafter\psPrintValueNew@ii#1,,\@nil}
\def\psPrintValueNew@ii#1,#2,#3\@nil{%  #1,#2 only for algebraic code
  \begin@SpecialObj
  \addto@pscode{  %		thanks to Buddy Ledger
     /mfont { \psk@PSfont findfont \psk@fontscale scalefont setfont } bind def
     /mfontexp { \psk@PSfont findfont \psk@fontscale 1.2 div scalefont setfont } bind def
     /s1 { /Symbol findfont \psk@fontscale scalefont setfont } bind def
     \ifPst@algebraic 
        /x #1 def
        /Func (#2) tx@AlgToPs begin AlgToPs end cvx def 
        Func  
     \else #1 \fi
     /value ED
     \psk@Scin {
       value 0 ne { value log floor cvi /expon ED }{ /expon 0 def } ifelse
       value 10 expon exp div 
       \psk@decimals -1 gt { 10  \psk@decimals exp dup 3 1 roll mul 
         \ifPst@round round \else cvi \fi  exch div } if
       \psk@decimals 0 eq { cvi } if /numb ED
       expon \psk@valuewidth string cvs /expon exch def
       numb \psk@valuewidth string cvs 
       \ifPst@comma dot2comma \fi  % do we have to change dot to comma
       /Output exch def
       /txspc \psk@fontscale 4 div def
       \psk@xShift\space 0 moveto mfont Output show
       txspc 0 rmoveto s1 (\string\264) show
       txspc 0 rmoveto mfont (10) show
       txspc 2 div txspc 1.5 mul rmoveto mfontexp expon show }
     { value
       \psk@decimals -1 gt { 10 \psk@decimals exp dup 3 1 roll mul 
         \ifPst@round round \else cvi \fi exch div } if
       \psk@decimals 0 eq { cvi } if %inserted to handle decimals=0
       \psk@valuewidth string cvs 
       \ifPst@comma dot2comma \fi         % do we have to change dot to comma
       \psk@xShift\space 0 moveto mfont %Output 
       show
     } ifelse
  }%
  \end@SpecialObj%
}
%
\catcode`\@=\PstAtCode\relax
%
%% END: pst-tools.tex
\endinput
%


==> pst-xkey.tex <==
%%
%% This is file `pst-xkey.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `pxktex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, pst-xkey.tex, pst-xkey.sty, xkveca.cls, xkvecb.cls,
%% xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex, xkvex2.tex,
%% xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname PSTXKeyLoaded\endcsname
\let\PSTXKeyLoaded\endinput
\edef\PSTXKeyCatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \let\noexpand\PSTXKeyCatcodes\relax
}
\catcode`\@=11\relax
\ifx\ProvidesFile\@undefined
  \message{2005/11/25 v1.6 PSTricks specialization of xkeyval (HA)}
  \ifx\XKeyValLoaded\endinput\else\input xkeyval \fi
\else
  \ProvidesFile{pst-xkey.tex}
    [2005/11/25 v1.6 PSTricks specialization of xkeyval (HA)]
  \@addtofilelist{pst-xkey.tex}
  \RequirePackage{xkeyval}
\fi
\def\pst@famlist{}
\def\pst@addfams#1{%
  \XKV@for@n{#1}\XKV@tempa{%
    \@expandtwoargs\in@{,\XKV@tempa,}{,\pst@famlist,}%
    \ifin@\else\edef\pst@famlist{\pst@famlist,\XKV@tempa}\fi
  }%
}
\def\psset{%
  \expandafter\@testopt\expandafter\pss@t\expandafter{\pst@famlist}%
}
\def\pss@t[#1]#2{\setkeys+[psset]{#1}{#2}\ignorespaces}
\def\@psset#1,\@nil{%
  \edef\XKV@tempa{\noexpand\setkeys+[psset]{\pst@famlist}}%
  \XKV@tempa{#1}%
}
\PSTXKeyCatcodes
\endinput
%%
%% End of file `pst-xkey.tex'.


==> pstricks-add.tex <==
%% $Id: pstricks-add.tex 914 2014-05-17 20:02:53Z herbert $
%%
%% This is file `pstricks-add.tex',
%%
%% IMPORTANT NOTICE:
%%
%% Package `pstricks-add.tex'
%%
%% Dominique Rodriguez 
%% Herbert Voss <hvoss@tug.org>
%% Michael Sharpe <msharpe@ucsd.edu>
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pstricks-add' is a PSTricks package for additionals to the standard
%%         pstricks package
%%
\csname PSTricksAddLoaded\endcsname
\let\PSTricksAddLoaded\endinput
%
% Requires some packages
\ifx\PSTricksLoaded\endinput\else \input pstricks \fi
\ifx\PSTplotLoaded\endinput\else  \input pst-plot \fi
\ifx\PSTnodesLoaded\endinput\else \input pst-node \fi
\ifx\PSTthreeDLoaded\endinput\else\input pst-3d   \fi
\ifx\MultidoLoaded\endinput\else  \input multido  \fi
\ifx\PSTXKeyLoaded\endinput\else  \input pst-xkey \fi
\ifx\PSTmathLoaded\endinput\else  \input pst-math \fi
%
\def\fileversion{3.68}
\def\filedate{2014/05/17}
\message{`pstricks-add' v\fileversion, \filedate\space (dr,hv)}
%
\edef\PstAtCode{\the\catcode`\@} \catcode`\@=11\relax
\SpecialCoor
\pst@addfams{pstricks-add}
%
%% prologue for postcript
\pstheader{pstricks-add.pro}%
%
\def\psGetSlope(#1,#2)(#3,#4)#5{% 4 values without a dimen! #5 is a macro
  \pst@dimm=#1pt%
  \advance\pst@dimm by -#3pt%
  \pst@dimn=#2pt%
  \advance\pst@dimn by -#4pt
  \pst@divide{\pst@dimn}{\pst@dimm}#5}
%
\def\psGetDistance(#1,#2)(#3,#4)#5{% 4 values without a dimen! #5 is a macro
  \pst@dimm=#1pt%
  \advance\pst@dimm by -#3pt%
  \pst@dimn=#2pt%
  \advance\pst@dimn by -#4pt
  \pst@pyth\pst@dimm\pst@dimn\pst@dimo
  \edef#5{\strip@pt\pst@dimo}
}%
%--------------------------------------- small stuff -------------------------------
\define@boolkey[psset]{pstricks-add}[Pst@]{CMYK}[true]{}
\psset[pstricks-add]{CMYK=true}
%
\def\defineTColor{\@ifnextchar[{\defineTColor@i}{\defineTColor@i[]}}
\def\defineTColor@i[#1]#2#3{%     "semi transparency colors"
  \def\pst@tempA{#1}%
  \newpsstyle{#2}{%
     fillstyle=vlines,hatchwidth=0.1\pslinewidth,
     hatchsep=1\pslinewidth,hatchcolor=#3}%
  \ifx\pst@tempA\@empty\else\psset{#1}\fi%
}
\defineTColor{TRed}{red}
\defineTColor{TGreen}{green}
\defineTColor{TBlue}{blue}
%
\def\rmultiput{\pst@object{rmultiput}}
\def\rmultiput@i#1{%
  \pst@killglue%
  \begingroup%
  \use@par%
  \@ifnextchar({\rmultiput@ii{#1}}{\rmultiput@ii{#1}(\z@,\z@)}}
\def\rmultiput@ii#1(#2){%
  \if@star\rput*(#2){#1}\else\rput(#2){#1}\fi
  \@ifnextchar({\rmultiput@ii{#1}}{\endgroup}}

% #1: (x,y)  #2: rotAngle   #3: object
\def\psrotate{\pst@object{psrotate}}
\def\psrotate@i(#1)#2{%
  \pst@killglue
  \begingroup%
  \use@par\pst@makebox{\psrotate@ii(#1){#2}}}
\def\psrotate@ii(#1)#2{%
  \pst@getcoor{#1}\pst@tempA%
  \pst@getangle{#2}\pst@tempB%
  \leavevmode%
  \pst@Verb{% 
     { \pst@tempA /yRot ED /xRot ED 
       \pst@tempB dup cos /cosA ED sin /sinA ED
       /ax cosA def
       /by sinA def
       /cx sinA neg def
       /dy cosA def
       /ex xRot cosA mul neg xRot add yRot sinA mul add def
       /fy xRot sinA mul neg yRot add yRot cosA mul sub def
       [ax by cx dy ex fy] concat } \tx@TMChange }%
    \box\pst@hbox%
  \pst@Verb{ \tx@TMRestore }\endgroup}
%
% [#1]: obtargs; (#2,#3): center; {#4}: factor; {#5}: object
\def\psHomothetie{\def\pst@par{}\pst@object{psHomothetie}}
\def\psHomothetie@i(#1)#2{%
  \begin@SpecialObj%
  \pst@getcoor{#1}\pst@tempA% converts the coordinates without a unit into pt
  \pst@makebox{\psHomothetie@ii{#2}}}% put the contents into a box
\def\psHomothetie@ii#1{%
  \pst@Verb{%
    { \pst@tempA  /yH ED /xH ED  
      [#1 0 0 #1 #1 xH mul neg xH add #1 yH mul neg yH add] concat }
      \tx@TMChange }%
  \box\pst@hbox%
  \pst@Verb{ \tx@TMRestore }%
  \end@SpecialObj}
%
\define@key[psset]{pstricks-add}{intSeparator}{\def\psk@intSeparator{#1}}
\psset{intSeparator={,}}
%
\def\psFormatInt{\def\pst@par{}\pst@object{psFormatInt}}
\def\psFormatInt@i#1{{%
  \pst@killglue
  \use@par
  \count1=#1\count2=\count1
  \ifnum\count1=0 0\else
    \ifnum\count1>999999
    \count3=\count1
    \divide\count3 by 1000000
    \the\count3\psk@intSeparator\relax
    \multiply\count3 by 1000000
    \advance\count1 by -\count3 % modulo 1000000
  \fi%
  \ifnum\count2>999
    \count3=\count1
    \divide\count3 by 1000
    \ifnum\count2>99999
	\ifnum\count3<100 0\fi
	\ifnum\count3<10 0\fi
    \fi%
    \the\count3\psk@intSeparator\relax
    \multiply\count3 by 1000
    \advance\count1 by -\count3 %modulo 1000
  \fi%
  \ifnum\count2>999
    \ifnum\count1<100 0\fi
    \ifnum\count1<10 0\fi
  \fi%
  \the\count1
  \fi%
}\ignorespaces}
%
\define@key[psset]{pstricks-add}{braceWidth}{\pst@getlength{#1}\psk@braceWidth}
\define@key[psset]{pstricks-add}{bracePos}{\pst@checknum{#1}\psk@bracePos}
\define@key[psset]{pstricks-add}{braceWidthInner}{\pst@getlength{#1}\psk@braceWidthInner}
\define@key[psset]{pstricks-add}{braceWidthOuter}{\pst@getlength{#1}\psk@braceWidthOuter}
%
\def\psbrace{\def\pst@par{}\pst@object{psbrace}}
\def\psbrace@i(#1)(#2)#3{%
  \addbefore@par{ref=lb,linewidth=0.01pt,fillstyle=solid,fillcolor=black}% default setting
  \begin@SpecialObj
  \if@star\def\pst@tempC{true }\else\def\pst@tempC{false }\fi
  \ifx\psk@rot\empty\def\psk@@rot{0}\else\let\psk@@rot\psk@rot\fi
  \def\psk@rot{Alpha \psk@@rot\space add 90 sub}%
  \pst@getcoor{#1}\pst@tempA
  \pst@getcoor{#2}\pst@tempB
  \rput(!
    /ifStar \pst@tempC def
    /radius1 \psk@braceWidthOuter def
    /radius2 \psk@braceWidthInner def
    /Alpha \pst@tempA \pst@tempB 3 -1 roll sub 3 1 roll exch sub atan def 
    gsave  STV CP T /ps@rot \psk@rot\space def grestore 
    /Length \pst@tempA \pst@tempB Pyth2 def
    /Left { Length \psk@bracePos\space mul } bind def
    /Right { Length Left sub } bind def
    /Width \psk@braceWidth def
    /pop4 { pop pop pop pop } def
    gsave
    [ Alpha cos Alpha sin Alpha sin neg Alpha cos \pst@tempA ] concat 
    0 0 moveto
    0 radius2 neg radius2 radius2 neg radius2 arcto pop4
    Left radius2 sub radius1 sub 0 rlineto 
    Left radius2 neg Left radius2 radius1 add neg radius1 arcto pop4
    currentpoint /y@Label ED /x@Label ED
    Left radius2 neg Left radius1 add radius2 neg radius1 arcto pop4
    Right radius2 sub radius1 sub 0 rlineto
    Length radius2 neg Length 0 radius2 arcto pop4
%    0 Width neg rlineto
    Length radius2 Width add neg Length radius2 sub radius2 Width add neg radius2 arcto pop4
    Right radius2 sub radius1 sub neg 0 rlineto
    Left radius1 add Width radius1 add radius2 add neg radius1 90 180 arc
    Left radius1 sub Width radius1 add radius2 add neg radius1 0 90 arc
    Left radius2 sub radius1 sub neg 0 rlineto 
    radius2 Width neg radius2 270 180 arcn
    0 0 lineto 
    \ifx\psk@fillstyle\relax\else
      gsave
      ifStar { \pst@usecolor\pslinecolor }{ \pst@usecolor\psfillcolor } ifelse 
      fill
    grestore
    \fi 
    \pst@number\pslinewidth setlinewidth \pst@usecolor\pslinecolor stroke
    0 0 moveto
    grestore
%   now calculate the label pos
    /Dh radius1 radius2 add Width add def
    \pst@tempA \pst@tempB 3 -1 roll sub 3 1 roll exch sub % dy dx 
    \psk@bracePos\space mul exch \psk@bracePos\space mul  % d'x d'y
    \pst@tempA 3 -1 roll add Dh Alpha cos mul sub	  % d'x x yA
    \psk@nodesepB sub					  % use minus sign to shidt right
    3 1 roll add Dh Alpha sin mul add \psk@nodesepA add 
    exch \tx@UserCoor ){#3}
  \end@SpecialObj}
%
\def\psBrace{\def\pst@par{}\pst@object{psBrace}}
\def\psBrace@i(#1)(#2){%
  \begin@ClosedObj
  \if@star\def\pst@tempC{true }\else\def\pst@tempC{false }\fi
%  \ifx\psk@rot\empty\def\psk@@rot{0}\else\let\psk@@rot\psk@rot\fi
%  \def\psk@rot{Alpha \psk@@rot\space add 90 sub}%
  \pst@getcoor{#1}\pst@tempA
  \pst@getcoor{#2}\pst@tempB
  \addto@pscode{
    /ifStar \pst@tempC def
    /radius1 \psk@braceWidthOuter def
    /radius2 \psk@braceWidthInner def
    /Alpha \pst@tempA \pst@tempB 3 -1 roll sub 3 1 roll exch sub atan def 
%    gsave  STV CP T /ps@rot \psk@rot\space def grestore 
    /Length \pst@tempA \pst@tempB Pyth2 def
    /Left { Length \psk@bracePos\space mul } bind def
    /Right { Length Left sub } bind def
    /Width \psk@braceWidth def
    /pop4 { pop pop pop pop } def
    [ Alpha cos Alpha sin Alpha sin neg Alpha cos \pst@tempA ] concat 
    0 0 moveto
    0 radius2 neg radius2 radius2 neg radius2 arcto pop4
    Left radius2 sub radius1 sub 0 rlineto 
    Left radius2 neg Left radius2 radius1 add neg radius1 arcto pop4
    currentpoint /y@Label ED /x@Label ED
    Left radius2 neg Left radius1 add radius2 neg radius1 arcto pop4
    Right radius2 sub radius1 sub 0 rlineto
    Length radius2 neg Length 0 radius2 arcto pop4
%    0 Width neg rlineto
    Length radius2 Width add neg Length radius2 sub radius2 Width add neg radius2 arcto pop4
    Right radius2 sub radius1 sub neg 0 rlineto
    Left radius1 add Width radius1 add radius2 add neg radius1 90 180 arc
    Left radius1 sub Width radius1 add radius2 add neg radius1 0 90 arc
    Left radius2 sub radius1 sub neg 0 rlineto 
    radius2 Width neg radius2 270 180 arcn
    0 0 lineto }
  \end@ClosedObj
  \ignorespaces}
%  
\newdimen\psparallelogramsep
\define@key[psset]{pstricks-add}{parallelogramsep}[3mm]{\pssetlength\psparallelogramsep{#1}}
\psset[pstricks-add]{parallelogramsep=3mm}
%
\def\psparallelogrambox{\pst@object{psparallelogrambox}}
\def\psparallelogrambox@i{\pst@makebox\psparallelogrambox@ii}
\def\psparallelogrambox@ii{%
	\begingroup
	\pst@useboxpar
	\pst@dima=\pslinewidth
	\advance\pst@dima by \psframesep
	\pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
	\pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
	\pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
% Dirk Osburg modification begin - Jul. 16, 2011
	\divide\psparallelogramsep by 2
	\advance\pst@dima by \psparallelogramsep 
	\advance\pst@dimc by \psparallelogramsep 
% Dirk Osburg modification end
	\setbox\pst@hbox=\hbox{%
		\ifpsboxsep\kern\pst@dima\fi
		\begin@ClosedObj
		\addto@pscode{%
			\psk@cornersize
			\pst@number\pst@dima neg % left
			\pst@number\pst@dimb neg % lower
			\pst@number\pst@dimc % right
			\pst@number\pst@dimd % upper
			.5
% D.G. modification begin - Nov. 28, 2001
%\tx@Frame}%
			\pst@number\psparallelogramsep
			\tx@Parallelogram}%
% D.G. modification end

			\def\pst@linetype{2}%
			\showpointsfalse
		\end@ClosedObj
		\box\pst@hbox
		\ifpsboxsep\kern\pst@dima\fi%
	}%
	\ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
	\leavevmode\box\pst@hbox
	\endgroup%
}

% From the Frame and Rect PostScript macros
\pst@def{Parallelogram}<{%
  /ParallelogramA {
% Dirk Osburg modification begin - Jul. 16, 2011
%%%% old stuff: %%%
%x1 pgs sub y1 moveto
%x1 y2 lineto
%x2 pgs add y2 lineto
%x2 y1 lineto
%x1 pgs sub y1 lineto
%%%% replaced by: %%%
  x1 pgs sub y1 moveto
  x1 pgs add y2 lineto
  x2 pgs add y2 lineto
  x2 pgs sub y1 lineto
  x1 pgs sub y1 lineto
% Dirk Osburg modification end
  closepath} def
%
/pgs ED
CLW mul
/a ED
3 -1 roll
2 copy gt { exch } if
a sub
/y2 ED
a add
/y1 ED
2 copy gt { exch } if
a sub
/x2 ED
a add
/x1 ED
1 index 0 eq {pop pop ParallelogramA } { OvalFrame } ifelse}>
%
%
% -------------- the arrow part -------------
%
\def\psBigArrow{\pst@object{psBigArrow}}
\def\psBigArrow@i(#1)(#2){%
  \addbefore@par{doublesep=1cm}
  \begin@ClosedObj
  \pssetlength\pst@dimm{\psdoublesep}
  \pst@getcoor{#1}\pst@tempA 
  \pst@getcoor{#2}\pst@tempB  
  \addto@pscode{
    /Width \pst@number\pst@dimm def
    \pst@tempA % x y 
    \pst@tempB % x y
    exch       % x y y x
    4 -1 roll   % y y x x
    sub        % y y dx
    3 1 roll   % dx y y
    sub        % dx dy
    exch       % dy dx
    atan neg      % alpha
    \pst@tempA
    translate
    rotate     
    0 0 moveto
    0 Width 2 div rlineto % |
    \pst@tempB \pst@tempA Pyth2 Width 1.5 mul sub 0 rlineto
    0 Width 1.5 div rlineto
    Width 1.5 mul dup neg rlineto
    Width 1.5 mul neg dup rlineto
    0 Width 1.5 div rlineto
    \pst@tempB \pst@tempA Pyth2 neg Width 1.5 mul add 0 rlineto
    closepath 
  }%
  \end@ClosedObj
}
%  the original table
% \def\pst@arrowtable{,<->,<<->>,>-<,>>-<<,(-),[-],)-(,]-[,|>-<|}
%
% v : Vee arrow (inside)                 v,V,f and F by Christophe FOUREY
% V : Vee arrow (outside)
% f : Filled vee arrow (inside)
% F : Filled vee arrow (outside)
\edef\pst@arrowtable{\pst@arrowtable,v-v,V-V,f-f,F-F,t-t,T-T}

% Vee arrow
\define@key[psset]{pstricks-add}{veearrowlength}[3mm]{\pst@getlength{#1}\psk@veearrowlength}
\psset[pstricks-add]{veearrowlength=3mm} % default projected length
\define@key[psset]{pstricks-add}{veearrowangle}[30]{\pst@getangle{#1}\psk@veearrowangle}
\psset[pstricks-add]{veearrowangle=30} % default angle
\define@key[psset]{pstricks-add}{veearrowlinewidth}[0.35mm]{\pst@getlength{#1}\psk@veearrowlinewidth}
\psset[pstricks-add]{veearrowlinewidth=0.35mm} % default vee arrow line width

% Filled vee arrow
\define@key[psset]{pstricks-add}{filledveearrowlength}[3mm]{\pst@getlength{#1}\psk@filledveearrowlength}
\psset[pstricks-add]{filledveearrowlength=3mm} % default projected length
\define@key[psset]{pstricks-add}{filledveearrowangle}[15]{\pst@getangle{#1}\psk@filledveearrowangle}
\psset[pstricks-add]{filledveearrowangle=15} % default angle
\define@key[psset]{pstricks-add}{filledveearrowlinewidth}[0.35mm]{\pst@getlength{#1}\psk@filledveearrowlinewidth}
\psset[pstricks-add]{filledveearrowlinewidth=0.35mm} % default vee arrow line width
\define@key[psset]{pstricks-add}{arrowlinestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\psarrowlinestyle{#1}}}
\psset[pstricks-add]{arrowlinestyle=solid} % default
\pst@def{VeeArrow}<%
    1 setlinecap            % round caps
    1 setlinejoin            % round join
    setlinewidth            % vee arrow line width
    /y ED                % projected length
    2 div /a ED                % angle (divide by 2)
    /t ED                % false = inside, true = outside
    a sin a cos div y mul /x ED        % perpendicular length : x=tan(a).y
    t { 1 -1 scale } if            % if outside : symmetry
    x neg y moveto            % point #1
    0 0 L                % point #2
    x y L                % point #3
    { closepath gsave fill grestore } if    % if filled : close and fill
    \@nameuse{psls@\psarrowlinestyle}
    stroke                % draw line
    0 t { y 2 mul } { 0 } ifelse moveto>    % if outside : twice longer line

% VeeArrow : filled?   outside?   (total) angle   (projected) length   (arrow) line width

\@namedef{psas@v}{%
  false false \psk@veearrowangle \psk@veearrowlength \psk@veearrowlinewidth \tx@VeeArrow}
\@namedef{psas@V}{%
  false true \psk@veearrowangle \psk@veearrowlength \psk@veearrowlinewidth \tx@VeeArrow}
\@namedef{psas@f}{%
  true false \psk@filledveearrowangle \psk@filledveearrowlength \psk@filledveearrowlinewidth \tx@VeeArrow}
\@namedef{psas@F}{%
  true true \psk@filledveearrowangle \psk@filledveearrowlength \psk@filledveearrowlinewidth \tx@VeeArrow}

% And An another arrowhead
% architectural tick / oblique arrow

% Tick arrow
\define@key[psset]{pstricks-add}{tickarrowlength}[1.5mm]{\pst@getlength{#1}\psk@tickarrowlength}
\psset[pstricks-add]{tickarrowlength=1.5mm} % default projected length
\define@key[psset]{pstricks-add}{tickarrowlinewidth}[0.35mm]{\pst@getlength{#1}\psk@tickarrowlinewidth}
\psset[pstricks-add]{tickarrowlinewidth=0.35mm} % default tick arrow line width

\pst@def{TickArrow}<%
    1 setlinecap            % round caps
    1 setlinejoin            % round join
    setlinewidth            % tick line width
    /y ED                % projected length
    /t ED                % false = normal, true = reversed
    t { 1 -1 scale } if            % if reversed : symmetry
    y neg y moveto            % point #1
    y y neg L                % point #2
    \@nameuse{psls@\psarrowlinestyle}
    stroke                % draw line
    0 0 moveto>                % origin

\@namedef{psas@t}{ false \psk@tickarrowlength \psk@tickarrowlinewidth \tx@TickArrow }
\@namedef{psas@T}{ true \psk@tickarrowlength \psk@tickarrowlinewidth \tx@TickArrow }
%
% HookLeft/RightArrow
\newdimen\pshooklength
\newdimen\pshookwidth
\define@key[psset]{pstricks-add}{hooklength}[3mm]{\pssetlength\pshooklength{#1}}
\define@key[psset]{pstricks-add}{hookwidth}[1mm]{\pssetlength\pshookwidth{#1}}
%\psset{hooklength=3mm,hookwidth=1mm}
%
\edef\pst@arrowtable{\pst@arrowtable,H-H,h-h} % add new arrow
\def\tx@RHook{RHook }         % PostScript name
\def\tx@Rhook{Rhook }         % PostScript name
\@namedef{psas@H}{%
  /RHook {
    /x ED                     % hook width
    /y ED                     % hook length 
    /z CLW 2 div def          % save it
    x y moveto                % goto first point
    x 0 0 0 0 y 
    curveto                   % draw Bezier
    stroke 
    0 y moveto                % define current point
  } def
  \pst@number\pshooklength
  \pst@number\pshookwidth
  \tx@RHook 
}
\@namedef{psas@h}{%
  /Rhook {
    CLW mul 			% size * CLW
    add dup 			% +length  size*CLW+length size*CLW+length 
    2 div /w ED	 		% (size*CLW+length)/2  -> w 
    mul dup /h ED mul 		% (size*CLW+length)
    /a ED  
    w neg h abs moveto 0 0 L 
    gsave 
    stroke grestore 
  } def
  0 \psk@arrowlength \psk@arrowsize \tx@Rhook 
}
% New parameter "arrowfill", with default as "true"
\define@boolkey[psset]{pstricks-add}[ps]{ArrowFill}[true]{}
%
% Modification of the PostScript macro Arrow to choose to fill or not the arrow
% (it require to restore the current linewidth, despite of the scaling)
\pst@def{Arrow}<{%
    CLW mul add dup 2 div
    /w ED mul dup
    /h ED mul
    /a ED { 0 h T 1 -1 scale } if
    gsave
    \ifpsArrowFill\else\pst@number\pslinewidth \pst@arrowscale\space div SLW \fi
    w neg h moveto
    0 0 L w h L w neg a neg rlineto
    \ifpsArrowFill gsave fill grestore \else gsave closepath stroke grestore \fi
    grestore
    0 h a sub moveto
}>
%
\define@key[psset]{pstricks-add}{nArrowsA}[2]{\def\psk@nArrowsA{#1}}
\define@key[psset]{pstricks-add}{nArrowsB}[2]{\def\psk@nArrowsB{#1}}
\define@key[psset]{pstricks-add}{nArrows}[2]{\def\psk@nArrowsA{#1}\def\psk@nArrowsB{#1}}
\psset{nArrows=2}
%
\@namedef{psas@>>}{%
    \psk@nArrowsA\space 1 sub {
      false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
      0 h a sub T
    } repeat
    gsave
    newpath
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    CP
    grestore
    moveto
}
%
\@namedef{psas@<<}{%
    true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h neg a add T
  \psk@nArrowsB\space 2 sub {
    false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
    0 h neg a add T
  } repeat
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  0 h a 5 mul 2 div sub moveto
}
%
% DG addition begin - Dec. 18/19, 1997 and Oct. 11, 2002
% Adapted from \psset@arrows
\define@key[psset]{pstricks-add}{ArrowInside}{%
  \def\pst@tempArrow{#1}%
  \ifx\pst@tempArrow\@empty \def\psk@ArrowInside{} %
  \else%
    \begingroup%
      \pst@activearrows%
      \xdef\pst@tempg{<#1}%
    \endgroup%
    \expandafter\psset@@ArrowInside\pst@tempg\@empty-\@empty\@nil%
    \if@pst\else\@pstrickserr{Bad intermediate arrow specification: #1}\@ehpa\fi%
  \fi%
}
% Adapted from \psset@@arrows
\def\psset@@ArrowInside#1-#2\@empty#3\@nil{%
  \@psttrue
  \def\next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
  \expandafter\next\pst@arrowtable,#1-#1,\@nil
  \@ifundefined{psas@#2}%
    {\@pstfalse\def\psk@ArrowInside{}}%
    {\def\psk@ArrowInside{#2}}%
}
% Default value empty
\psset{ArrowInside={}}
% Modified version of \pst@addarrowdef
\def\pst@addarrowdef{%
  \addto@pscode{%
    /ArrowA {
      \ifx\psk@arrowA\@empty
        \pst@oplineto
      \else
	\pst@arrowdef{A}
	moveto
      \fi
    } def
    /ArrowB { \ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi } def
% DG addition
    /ArrowInside { 
      \ifx\psk@ArrowInside\@empty \else \pst@arrowdefA{Inside} \fi 
    } def
  }%
}
% Adapted from \pst@arrowdef
\def\pst@arrowdefA#1{%
  \ifnum\pst@repeatarrowsflag>\z@ /Arrow#1c [ 6 2 roll ] cvx def Arrow#1c\fi 
  \tx@BeginArrow
  \psk@arrowscale
  \@nameuse{psas@\@nameuse{psk@Arrow#1}}
  \tx@EndArrow%
}
% ArrowInsidePos parameter (default value 0.5)
\define@key[psset]{pstricks-add}{ArrowInsidePos}[0.5]{\pst@checknum{#1}\psk@ArrowInsidePos}%
%\psset{ArrowInsidePos=0.5}
%
%
% Redefinition of the PostScript /Line macro to print the intermediate
% arrow on each segment of the line
%
\define@key[psset]{pstricks-add}{ArrowInsideNo}[1]{\pst@checknum{#1}\psk@ArrowInsideNo}% hv 20031001
\define@key[psset]{pstricks-add}{ArrowInsideOffset}[0]{\pst@checknum{#1}\psk@ArrowInsideOffset}% hv 20031001
%\psset{ArrowInsideNo=1,ArrowInsideOffset=0}
%
\def\arrowType@H{H}
\pst@def{Line}<
  NArray n 0 eq not { n 1 eq { 0 0 /n 2 def } if
  (\psk@ArrowInside) length 0 gt { 
    \ifx\psk@arrowA\arrowType@H   % do we have a Hook arrow at the beginning?
      \pst@number\pshooklength  % yes 
    \else
      \psk@arrowsize\space CLW mul add dup \psk@arrowlength\space mul exch \psk@arrowinset mul neg add  
    \fi
    /arrowlength exch def 
    4 copy 				% copy all four values for the arrow line
    /y1 ED /x1 ED /y2 ED /x2 ED 	% save them
    /Alpha y2 y1 sub x2 x1 sub Atan def % the gradient of the line
%    2 copy /y1 ED /x1 ED ArrowA x1 y1  
    ArrowA 				% draw arrowA
    x1 Alpha cos arrowlength mul add	% dx add
    y1 Alpha sin arrowlength mul add	% dy add, to get the current point at the end of the arrow tip
    /n n 1 sub def
    n {
      4 copy
      /y1 ED /x1 ED /y2 ED /x2 ED
      x1 y1
      \psk@ArrowInsidePos\space 1 gt {
        /Alpha y2 y1 sub x2 x1 sub Atan def
        /ArrowPos \psk@ArrowInsideOffset\space def
        /dArrowPos \psk@ArrowInsidePos\space abs def
%        /Length x2 x1 sub y2 y1 sub Pyth def
        \psk@ArrowInsideNo\space cvi {
          /ArrowPos ArrowPos dArrowPos add def
%          ArrowPos Length gt { exit } if
          x1 Alpha cos ArrowPos mul add
          y1 Alpha sin ArrowPos mul add
          ArrowInside
          pop pop
        } repeat
      }{
        /ArrowPos \psk@ArrowInsideOffset\space def
        /dArrowPos \psk@ArrowInsideNo 1 gt {%
          1.0 \psk@ArrowInsideNo 1.0 add div
        }{\psk@ArrowInsidePos } ifelse def
          \psk@ArrowInsideNo\space cvi {
            /ArrowPos ArrowPos dArrowPos add def
            x2 x1 sub ArrowPos mul x1 add
            y2 y1 sub ArrowPos mul y1 add
            ArrowInside
            pop pop
          } repeat
      } ifelse
      pop pop Lineto
    } repeat
  }{ ArrowA /n n 2 sub def n { Lineto } repeat } ifelse
  CP 4 2 roll ArrowB L pop pop } if >
%
% Redefinition of the PostScript /Polygon macro to print the intermediate
% arrow on each segment of the line
\pst@def{Polygon}<{%
    NArray n 2 eq { 0 0 /n 3 def } if
    n 3 lt {
	n { pop pop } repeat
    }{
	n 3 gt { CheckClosed } if
	n 2 mul	-2 roll
	/y0 ED
	/x0 ED
    	/y1 ED
    	/x1 ED
    	/xx1 x1 def
    	/yy1 y1 def
    	x1 y1
    	/x1 x0 x1 add 2 div def
    	/y1 y0 y1 add 2 div def
    	x1 y1 moveto
    	/n n 2 sub def
	/drawArrows {
	    x11 y11
	    \psk@ArrowInsidePos\space 1 gt {
		/Alpha y12 y11 sub x12 x11 sub atan def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/Length x12 x11 sub y12 y11 sub Pyth def
		/dArrowPos \psk@ArrowInsidePos\space abs def
		{
		    /ArrowPos ArrowPos dArrowPos add def
		    ArrowPos Length gt { exit } if
		    x11 Alpha cos ArrowPos mul add
		    y11 Alpha sin ArrowPos mul add
		    currentdict /ArrowInside known { ArrowInside } if
		    pop pop
		} loop
	    }{
		/ArrowPos \psk@ArrowInsideOffset\space def
		/dArrowPos \psk@ArrowInsideNo\space 1 gt {%
	    	    1.0 \psk@ArrowInsideNo\space 1.0 add div
		}{ \psk@ArrowInsidePos } ifelse def
		\psk@ArrowInsideNo\space cvi {
		    /ArrowPos ArrowPos dArrowPos add def
		    x12 x11 sub ArrowPos mul x11 add
		    y12 y11 sub ArrowPos mul y11 add
		    currentdict /ArrowInside known { ArrowInside } if
		    pop pop
		} repeat
	    } ifelse
	    pop pop Lineto
	} def
	n {
	    4 copy
	    /y11 ED /x11 ED /y12 ED /x12 ED
	    drawArrows
	} repeat
	x1 y1 x0 y0
	6 4 roll
	2 copy
	/y11 ED /x11 ED /y12 y0 def /x12 x0 def
	drawArrows
	/y11 y0 def /x11 x0 def /y12 yy1 def /x12 xx1 def
	drawArrows
	pop pop
    	closepath
    } ifelse %
}>
%
%
% Redefinition of the PostScript /OpenBezier macro to print the intermediate
% arrow
\pst@def{OpenBezier}<{%
  /dArrowPos \psk@ArrowInsideNo 1 gt {%
    1.0 \psk@ArrowInsideNo 1.0 add div
    }{ \psk@ArrowInsidePos } ifelse def
      BezierNArray
      n 1 eq { pop pop
      }{ 2 copy
        /y0 ED /x0 ED
        ArrowA
        n 4 sub 3 idiv { 6 2 roll 4 2 roll curveto } repeat
        6 2 roll
        4 2 roll
        ArrowB
        /y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
        /cx x1 x0 sub 3 mul def
        /cy y1 y0 sub 3 mul def
        /bx x2 x1 sub 3 mul cx sub def
        /by y2 y1 sub 3 mul cy sub def
        /ax x3 x0 sub cx sub bx sub def
        /ay y3 y0 sub cy sub by sub def
        /getValues {
          ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
          ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
          ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
          ay t 3 exp mul by t t mul mul add cy t mul add y0 add
        } def
        /getdL {
          getValues
          3 -1 roll sub 3 1 roll sub Pyth
        } def
        /CurveLength {
          /u 0 def
          /du 0.01 def
          0 100 {
            /t0 u def
            /u u du add def
            /t u def
            getdL add
          } repeat } def
          /GetArrowPos {
            /ende \psk@ArrowInsidePos\space 1 gt
              {ArrowPos}
              {ArrowPos CurveLength mul} ifelse def
            /u 0 def
            /du 0.01 def
            /sum 0 def
            { /t0 u def
              /u u du add def
              /t u def
              /sum getdL sum add def
              sum ende gt {exit} if
            } loop u
          } def
          /ArrowPos \psk@ArrowInsideOffset\space def
          /loopNo \psk@ArrowInsidePos\space 1 gt {%
            CurveLength \psk@ArrowInsidePos\space div cvi
          }{ \psk@ArrowInsideNo } ifelse def
            loopNo cvi {
              /ArrowPos ArrowPos dArrowPos add def
              /t GetArrowPos def
              /t0 t 0.95 mul def
              getValues
              ArrowInside pop pop pop pop
            } repeat
            x1 y1 x2 y2 x3 y3 curveto
  } ifelse
}>
%
% Redefinition of the PostScript /NCLine macro to print the intermediate
% arrow of the line
\pst@def{NCLine}<{%
	NCCoor
	tx@Dict begin
	ArrowA CP 4 2 roll ArrowB
	4 copy
	/y2 ED /x2 ED /y1 ED /x1 ED
	x1 y1
	\psk@ArrowInsidePos\space 1 gt {
		/Alpha y2 y1 sub x2 x1 sub atan def
		/ArrowPos \psk@ArrowInsideOffset\space def
		/Length x2 x1 sub y2 y1 sub Pyth def
		/dArrowPos \psk@ArrowInsidePos\space abs def
		{%
			/ArrowPos ArrowPos dArrowPos add def
			ArrowPos Length gt { exit } if
			x1 Alpha cos ArrowPos mul add
			y1 Alpha sin ArrowPos mul add
			ArrowInside
			pop pop
		} loop
	}{%
		/ArrowPos \psk@ArrowInsideOffset\space def
		/dArrowPos \psk@ArrowInsideNo 1 gt {%
			1.0 \psk@ArrowInsideNo 1.0 add div
		}{ \psk@ArrowInsidePos } ifelse def
		\psk@ArrowInsideNo\space cvi {
			/ArrowPos ArrowPos dArrowPos add def
			x2 x1 sub ArrowPos mul x1 add
			y2 y1 sub ArrowPos mul y1 add
			ArrowInside
			pop pop
		} repeat
	} ifelse
	pop pop lineto pop pop
	end%
}>
%
\pst@def{NCCurve}<{%
	GetEdgeA GetEdgeB
	xA1 xB1 sub yA1 yB1 sub
	Pyth 2 div dup 3 -1 roll mul
	/ArmA ED
	mul
	/ArmB ED
	/ArmTypeA 0 def
	/ArmTypeB 0 def
	GetArmA GetArmB
	xA2 yA2 xA1 yA1
	2 copy
	/y0 ED /x0 ED
	tx@Dict begin
		ArrowA
	end
	xB2 yB2 xB1 yB1
	tx@Dict begin
		ArrowB
	end
	/y3 ED /x3 ED /y2 ED /x2 ED /y1 ED /x1 ED
	/cx x1 x0 sub 3 mul def
	/cy y1 y0 sub 3 mul def
	/bx x2 x1 sub 3 mul cx sub def
	/by y2 y1 sub 3 mul cy sub def
	/ax x3 x0 sub cx sub bx sub def
	/ay y3 y0 sub cy sub by sub def
	/getValues {
		ax t0 3 exp mul bx t0 t0 mul mul add cx t0 mul add x0 add
		ay t0 3 exp mul by t0 t0 mul mul add cy t0 mul add y0 add
		ax t 3 exp mul bx t t mul mul add cx t mul add x0 add
	ay t 3 exp mul by t t mul mul add cy t mul add y0 add
	} def
	/getdL {
		getValues
		3 -1 roll sub 3 1 roll sub Pyth
	} def
	/CurveLength {
		/u 0 def
		/du 0.01 def
		0 100 {
			/t0 u def
			/u u du add def
			/t u def
			getdL add
		} repeat } def
	/GetArrowPos {
		/ende \psk@ArrowInsidePos\space 1 gt {ArrowPos}{ArrowPos CurveLength mul} ifelse def
		/u 0 def
		/du 0.01 def
		/sum 0 def
		{
			/t0 u def
			/u u du add def
			/t u def
			/sum getdL sum add def
			sum ende gt {exit} if
		} loop u
	} def
	/dArrowPos \psk@ArrowInsideNo 1 gt {%
		1.0 \psk@ArrowInsideNo 1.0 add div
	}{ \psk@ArrowInsidePos } ifelse def
	/ArrowPos \psk@ArrowInsideOffset\space def
	/loopNo \psk@ArrowInsidePos\space 1 gt {%
		CurveLength \psk@ArrowInsidePos\space div cvi
		}{ \psk@ArrowInsideNo } ifelse def
	loopNo cvi {
		/ArrowPos ArrowPos dArrowPos add def
		/t GetArrowPos def
		/t0 t 0.95 mul def
		getValues
		ArrowInside pop pop pop pop
	} repeat
	x1 y1 x2 y2 x3 y3 curveto
	/LPutVar [ xA1 yA1 xA2 yA2 xB2 yB2 xB1 yB1 ] cvx def
	/LPutPos { t LPutVar BezierMidpoint } def
	/HPutPos { { HPutLines } HPutCurve } def
	/VPutPos { { VPutLines } HPutCurve } def
}>
%
\def\parseRP#1;#2;#3\@nil{%check whether arg of refpt contains ;
  \def\arg@A{#1}\def\arg@B{#2}}
%
\def\Put{\pst@object{Put}}%
\def\Put@i{\@ifnextchar({\Put@ii{}}{\Put@ii}}%  
\def\Put@ii#1(#2)#3{{%
  \pst@killglue%
  \use@par%
  \expandafter\parseRP#1;;\@nil%sets \arg@A, \arg@B
  \ifx\arg@B\@empty% use \rput
    \edef\arg@A{\if@star*\fi\ifx\arg@A\@empty\else[\arg@A]\fi}%
    \expandafter\rput\arg@A(>#2){#3}
  \else% use \uput
    \edef\arg@A{\if@star*\fi%
      \ifx\arg@A\@empty\else{\arg@A}\fi%
      \ifx\arg@B\@empty[0]\else[\arg@B]\fi}%
    \expandafter\uput\arg@A(>#2){#3}
  \fi}\ignorespaces}%

% Modify pst@rot so that a rotation may be specified with a node or ps code
%
\define@key[psset]{pstricks-add}{Os}[0]{\def\PST@Os{#1}}
\psset{Os=0}%
\define@key[psset]{pstricks-add}{Ds}[1]{\def\PST@Ds{#1}}
\psset{Ds=1}%
\define@key[psset]{pstricks-add}{metricInitValue}[0]{\def\PST@metricInitValue{#1}}
\psset{metricInitValue=0}%
\define@boolkey[psset]{pstricks-add}[PST@]{metricFunction}[true]{}%use \ifPST@metricFunction
\psset{metricFunction=false}%
\def\pscurvepoints{\pst@object{pscurvepoints}}%
\def\pscurvepoints@i#1#2#3#4{{%optional [plotpoints=xx]
%  #1=tmin,#2=tmax,#3=function (of t),#4=array root name,
  \pst@killglue%
  \use@par%
  \edef\my@tempA{#3}% x(t) y(t) expanded
  \expandafter\testAlg\my@tempA|\@nil%
  \pst@Verb{                   % so we can use definitions from tx@Dict
	/unitratio \pst@number\psyunit \pst@number\psxunit div def 
	/unitratiosq unitratio dup mul def
	/t0 #1 def
	/t1 #2 def  
	 t1 t0 sub \psk@plotpoints\space div /dt exch def }%
  \pst@cntc=\psk@plotpoints\relax%\psk@plotpoints=plotpoints-1
  \pst@cntb=\pst@cntc\relax%\psk@plotpoints=plotpoints-1
  \advance\pst@cntc by \@ne\relax%=plotpoints
  \ifx\my@tempD\@empty\pst@Verb{ /Func (#3) cvx def }%
  \else\pst@Verb{ /Func (#3 ) AlgParser cvx def }%
  \fi%
  \pst@Verb{ 
    /#4.X \the\pst@cntc\space array def
    /#4.Y \the\pst@cntc\space array def %
    /#4Delta.X \the\pst@cntc\space array def %
    /#4Delta.Y \the\pst@cntc\space array def %
    /#4Normal.X \the\pst@cntc\space array def %
    /#4Normal.Y \the\pst@cntc\space array def %
    /t #1 def Func 2 copy /priory ED /priorx ED #4.Y  0 3 -1 roll put #4.X 0 3 -1 roll put %
    1 1 \the\pst@cntb\space { dup /j ED dt mul #1 add /t ED Func %x y on stack
    2 copy priory sub dup #4Delta.Y j 3 -1 roll put % x y x y-priory
    unitratiosq mul neg #4Normal.X j 3 -1 roll put % x y x
    priorx sub dup #4Delta.X j 3 -1 roll put % x y x-priorx
    #4Normal.Y j 3 -1 roll put % x y
    2 copy /priory ED /priorx ED % x y
    #4.Y j 3 -1 roll put #4.X j 3 -1 roll put } for %
     }%
  \expandafter\xdef \csname #4pointcount\endcsname {\psk@plotpoints}%
%  \typeout{Created points #40 .. #4\psk@plotpoints}%
}\ignorespaces}%
%
%code to place ticks along polyline
\def\pspolylineticks{\pst@object{pspolylineticks}}%
\def\pspolylineticks@i#1{\@ifnextchar[{\pspolylineticks@ii{#1}}{\pspolylineticks@ii{#1}[]}}%  
\newcount\pst@cntC%
\def\pspolylineticks@ii#1[#2]#3#4#5{{%
%#1= root name,#2=pscode (optional),#3=metric function,#4=first tick,#5=tick count
% Metric function may be a function of x, y (keyword metricFunction)
% or a function of x, y, dx, dy, ds  requiring incremental build
  \addbefore@par{arrows=-,linewidth=\psk@ytickwidth\pslinewidth}%
  \use@par%
  \pst@killglue%there's a leak that can occur here with ticksize--fixed in recent pstricks.tex
  \pst@cntC=\expandafter\csname #1pointcount\endcsname\relax%
  \pst@cntb=\pst@cntC\advance\pst@cntb\m@ne\relax%
  \pst@cntd=\pst@cntC\advance\pst@cntd\@ne\relax%
  \pst@Verb{ % so we can use definitions from tx@Dict in pstricks.pro
    /TDict 20 dict def TDict begin %
    /Func (#3) cvx def /sarray \the\pst@cntd\space array def %
    #2 
    \ifPST@metricFunction 
      0 1 #1.X length 1 sub { 
        /j ED sarray j %
        #1.X j get /x ED #1.Y j get /y ED Func put 
      } for %
    \else %build by increments
      sarray 0 \PST@metricInitValue\space put %
      1 1 #1.X length 1 sub { 
        /j ED sarray j %
        #1.X j 1 sub get 
        /x ED #1.Y j 1 sub get 
        /y ED #1Delta.X j get 
        /dx ED #1Delta.Y j get 
        /dy ED /ds dx dup mul dy dup mul add sqrt def %
        Func sarray j 1 sub get add put 
      } for %
    \fi %\ifPSTfunctionMetric
    \ifnum\Pst@Debug>0
      /str 10 string def 
      /tmpar [(Metric range: [) () (, ) () (])] def %
      tmpar 1 sarray 0 get str cvs put 
      /str 10 string def 
      tmpar 3 sarray \the\pst@cntC\space get str cvs put tmpar 
      tx@NodeDict begin concatstringarray = end %
    \fi % end debug
%compute ticks
  /nl 0 def /nu \the\pst@cntC\space def 
  /smin sarray 0 get def 
  /smax sarray nu get def 
  /Os \ifx\PST@Os\@empty smin \else \PST@Os\space \fi def %
  /Ds \ifx\PST@Ds\@empty smax Os sub 10 div \else \PST@Ds\space \fi def %
  /scount smax Os sub Ds div cvi def %
  /tarray scount 1 add array def %
  /#1Tick.X scount 1 add array def %
  /#1Tick.Y scount 1 add array def %
  /#1TickN.X scount 1 add array def %
  /#1TickN.Y scount 1 add array def %
  0 1 scount { dup Ds mul Os add tarray 3 1 roll put } for %tick positions in tarray
  % find the corresponding s values using binary search
  0 1 scount { 
    dup tarray exch get /s exch def /j exch def %sought metric value,index
    /m nl def /n nu def /k nl nu add 2 div cvi def 20 { s sarray k get lt { %
    /n k def /k k m add 2 div cvi def }{ /m k def /nl k def /k k n add 2 div cvi def } ifelse %
    n 1 sub m le { /nl m def exit } if } repeat %
    sarray n get sarray m get dup 3 1 roll % sm sn sm
    sub dup 0 le { pop pop 0 }{%sm sn-sm 
    exch %sn-sm sm
    s sub neg exch div } ifelse % s->(s-sm)/(sn-sm)
    dup #1Delta.X m 1 add get mul #1.X m get add #1Tick.X j 3 -1 roll put % s on stack
    #1Delta.Y m 1 add get mul #1.Y m get add #1Tick.Y j 3 -1 roll put % 
    #1TickN.X j #1Normal.X m 1 add get put #1TickN.Y j #1Normal.Y m 1 add get put %
  } for %
  \ifnum\Pst@Debug>0
    /tmpar 2 array def 
    /str 4 string def tmpar 0 (Created data for points #1Tick0..#1Tick) put 
    tmpar 1 scount str cvs put tmpar tx@NodeDict begin concatstringarray = end 
  \fi%
  end }% end pst@Verb
%Draw ticks
\multido{\iA=#4+1}{#5}{%
  \pnode(! TDict begin \iA\space scount gt 
    { 1 0 /VV ED /UU ED 0 0 }
    { #1TickN.X \iA\space get #1TickN.Y \iA\space get /VV ED /UU ED #1Tick.X \iA\space get #1Tick.Y \iA\space get } ifelse 
    2 copy /YY ED /XX ED end){#1Tick\iA}%
  \pnode(! TDict begin UU VV end ){#1Normal\iA}%
  \pnode(! TDict begin VV UU neg unitratiosq div end ){#1Tangent\iA}%
  \edef\cmd{\noexpand\psline(\the\pst@yticksizeA;{(! TDict begin UU VV end )})(\the\pst@yticksizeB;{(! TDict begin UU VV end )})}%
  \pscustom{\translate(! TDict begin XX YY end)\cmd}}%
}\ignorespaces}%
%
\define@key[psset]{pstricks-add}{randomPoints}[1000]{\def\psk@randomPoints{#1}}
\define@boolkey[psset]{pstricks-add}[Pst@]{color}[true]{}
\psset{randomPoints=1000,color=false}
%
\def\psRandom{\def\pst@par{}\pst@object{psRandom}}%  hv  2004-11-12
\def\psRandom@i{\@ifnextchar({\psRandom@ii}{\psRandom@iii(0,0)(1,1)}}
\def\psRandom@ii(#1){\@ifnextchar({\psRandom@iii(#1)}{\psRandom@iii(0,0)(#1)}}
\def\psRandom@iii(#1)(#2)#3{%
  \def\pst@tempA{#3}%
  \ifx\pst@tempA\pst@empty\psclip{\psframe(#2)}\else\psclip{#3}\fi
  \pst@getcoor{#1}\pst@tempA 
  \pst@getcoor{#2}\pst@tempB 
  \begin@SpecialObj
  \addto@pscode{
    \pst@tempA\space /yMin exch def 
    /xMin exch def
    \pst@tempB\space /yMax exch def 
    /xMax exch def 
    /dy yMax yMin sub def
    /dx xMax xMin sub def
    rrand srand                 % initializes the random generator
    /getRandReal { rand 2147483647 div } def
    \psk@dotsize % defines /DS ... def
    \@nameuse{psds@\psk@dotstyle}
    \psk@randomPoints {
     \ifPst@color getRandReal getRandReal getRandReal setrgbcolor \fi
     getRandReal dx mul xMin add
     getRandReal dy mul yMin add
     Dot
     \ifx\psk@fillstyle\psfs@solid fill \fi stroke
    } repeat
  }%
  \end@SpecialObj
  \endpsclip
  \ignorespaces
}
%
\def\psComment{\def\pst@par{}\pst@object{psComment}}
\def\psComment@i{\pst@getarrows\psComment@ii}
\def\psComment@ii(#1)(#2)#3{\@ifnextchar[
  {\psComment@iii(#1)(#2){#3}}
  {\psComment@iii(#1)(#2){#3}[\ncline]}}
\def\psComment@iii(#1)(#2)#3[#4]{\@ifnextchar[
  {\psComment@iv(#1)(#2){#3}[#4]}
  {\psComment@iv(#1)(#2){#3}[#4][\rput]}}
\def\psComment@iv(#1)(#2)#3[#4][#5]{%
  \pnode(#1){comment@1}
  \pnode(#2){comment@2}
  \ifx\relax#4\relax\let\pst@ConnectionCommand\ncline
  \else\let\pst@ConnectionCommand#4\fi
  \ifx\relax#5\relax\let\pst@PutCommand\rput
  \else\let\pst@PutCommand#5\fi
  \addbefore@par{npos=0}%
  \begin@SpecialObj%
  \pst@ConnectionCommand{comment@1}{comment@2}
  \if@star\pst@PutCommand*(#1){#3}\else\pst@PutCommand(#1){#3}\fi
  \end@SpecialObj%
  \ignorespaces%
}
%
\def\tx@MovetoByHand{ tx@addDict begin MovetoByHand end }
\def\tx@LinetoByHand{ tx@addDict begin LinetoByHand end }
%/amplHand {.8} def 
%/dtHand 2 def

\def\pslineByHand{\def\pst@par{}\pst@object{pslineByHand}}
\def\pslineByHand@i{%
  \addbefore@par{VarStepEpsilon=2,varsteptol=0.8}
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\pslineByHand@ii}}
\def\pslineByHand@ii{%
  \addto@pscode{
    tx@addDict begin 
    /dtHand \psk@VarStepEpsilon\space def
    /amplHand \psk@varsteptol\space def
%    \pst@cp 		% current point
    \tx@setlinejoin 	% hv 2007-10-13
    MovetoByHand
    counttomark 2 div /maxLines ED
    1 1 maxLines { pop LinetoByHand } for
    end
  }%
  \end@OpenObj%
}
%
\def\psRelNode{\pst@object{psRelNode}}
\def\psRelNode@i(#1)(#2)#3#4{{% A - B - factor - node name
  \use@par
%  \pst@killglue
  \pst@getcoor{#1}\pst@tempA%
  \pst@getcoor{#2}\pst@tempB%
  \pnode(!
    \pst@tempA /YA exch \pst@number\psyunit div def
    /XA exch \pst@number\psxunit div def
    \pst@tempB /YB exch \pst@number\psyunit div def
    /XB exch \pst@number\psxunit div def
    /AlphaStrich \psk@angleA\space def
    /unit \pst@number\psyunit \pst@number\psxunit div def % yunit/xunit
%            
    /dx XB XA sub  def
    /dy YB YA sub \ifPst@trueAngle\space unit mul \fi\space def
    /laenge dy dup mul dx dup mul add sqrt #3 mul def
    /Alpha dy dx atan def 
    /beta Alpha AlphaStrich add def
    laenge beta cos mul XA add
    laenge beta sin mul \ifPst@trueAngle\space unit div \fi\space YA add ){#4}%
}\ignorespaces}
%
\def\psRelLine{\def\pst@par{}\pst@object{psRelLine}}
\def\psRelLine@i{\@ifnextchar({\psRelLine@iii}{\psRelLine@ii}}
\def\psRelLine@ii#1{%
  \addto@par{arrows=#1}%
  \psRelLine@iii%
}
\def\psRelLine@iii(#1)(#2)#3#4{{
  \pst@killglue
  \use@par
  \psRelNode(#1)(#2){#3}{#4}
  \psline(#1)(#4)%
}\ignorespaces}
%
% #1 options
% draw a parallel line to #2 #3
%     #2---------#3
%         #4----------#5(new node)
% #5 length of the line
% #6 node name
\def\psParallelLine{\def\pst@par{}\pst@object{psParallelLine}}
\def\psParallelLine@i{\@ifnextchar({\psParallelLine@iii}{\psParallelLine@ii}}
\def\psParallelLine@ii#1{\addto@par{arrows=#1}\psParallelLine@iii}
\def\psParallelLine@iii(#1)(#2)(#3)#4#5{{
  \pst@killglue
  \use@par
  \pst@getcoor{#1}\pst@tempA
  \pst@getcoor{#2}\pst@tempB
  \pst@getcoor{#3}\pst@tempC
%  \pst@getlength{#4}\pst@dima
  \pnode(!%
     \pst@tempA /YA exch \pst@number\psyunit div def
     /XA exch \pst@number\psxunit div def
     \pst@tempB /YB exch \pst@number\psyunit div def
     /XB exch \pst@number\psxunit div def
     \pst@tempC /YC exch \pst@number\psyunit div def
     /XC exch \pst@number\psxunit div def
%            
    /dx XB XA sub  def
    /dy YB YA sub  def
    /laenge dy dup mul dx dup mul add sqrt #4 mul def
    /Alpha dy dx atan def 
    laenge Alpha cos mul XC add
    laenge Alpha sin mul YC add ){#5}%
  \psline(#3)(#5)
}\ignorespaces}
%
\def\psIntersectionPoint(#1)(#2)(#3)(#4)#5{%
    \pst@getcoor{#1}\pst@tempA
    \pst@getcoor{#2}\pst@tempB
    \pst@getcoor{#3}\pst@tempC
    \pst@getcoor{#4}\pst@tempd
\pnode(!%
     \pst@tempA /YA exch \pst@number\psyunit div def
     /XA exch \pst@number\psxunit div def
     \pst@tempB /YB exch \pst@number\psyunit div def
     /XB exch \pst@number\psxunit div def
     \pst@tempC /YC exch \pst@number\psyunit div def
     /XC exch \pst@number\psxunit div def
     \pst@tempd /YD exch \pst@number\psyunit div def
     /XD exch \pst@number\psxunit div def
    /dY1 YB YA sub def
    /dX1 XB XA sub def
    /dY2 YD YC sub def
    /dX2 XD XC sub def
    dX1 abs 0.01 lt {
        /m2 dY2 dX2 div def
        XA dup XC sub m2 mul YC add
    }{
        dX2 abs 0.01 lt {
            /m1 dY1 dX1 div def
            XC dup XA sub m1 mul YA add
        }{%
            /m1 dY1 dX1 div def
            /m2 dY2 dX2 div def
            m1 XA mul m2 XC mul sub YA sub YC add m1 m2 sub div dup
            XA sub m1 mul YA add
        } ifelse
    } ifelse ){#5}%
}
%
\define@cmdkeys[psset]{pstricks-add}[PSTPSPNk@]{% Christophe Jorssen 2007
  blName,bcName,brName,
  clName,ccName,crName,
  tlName,tcName,trName}[]{}%
\psset[pstricks-add]{%
  blName=PSPbl,bcName=PSPbc,brName=PSPbr,
  clName=PSPcl,ccName=PSPcc,crName=PSPcr,
  tlName=PSPtl,tcName=PSPtc,trName=PSPtr}
\def\psDefPSPNodes{\def\pst@par{}\pst@object{psDefPSPNodes}}
\def\psDefPSPNodes@i{%
  \pst@killglue
  \begingroup
  \use@par
  \expandafter\psDefPSPNodes@ii\pic@coor}
%
\def\psDefPSPNodes@ii(#1)(#2)(#3){%
%    \pnode(#1){PSPN@temp}\pnode([nodesep=.75,angle=45]PSPN@temp){\PSTPSPNk@blName}
%    \pnode(#3){PSPN@temp}\pnode([nodesep=.75,angle=-135]PSPN@temp){\PSTPSPNk@trName}
    \pnode(#1){PSPN@temp}\pnode([angle=45]PSPN@temp){\PSTPSPNk@blName}
    \pnode(#3){PSPN@temp}\pnode([angle=-135]PSPN@temp){\PSTPSPNk@trName}
    \pnode(\PSTPSPNk@blName|\PSTPSPNk@trName){\PSTPSPNk@tlName}
    \pnode(\PSTPSPNk@trName|\PSTPSPNk@blName){\PSTPSPNk@brName}
    \ncline[linestyle=none]{\PSTPSPNk@blName}{\PSTPSPNk@tlName}
    \ncput[npos=.5]{\pnode{\PSTPSPNk@clName}}
    \ncline[linestyle=none]{\PSTPSPNk@blName}{\PSTPSPNk@brName}
    \ncput[npos=.5]{\pnode{\PSTPSPNk@bcName}}
    \pnode(\PSTPSPNk@brName|\PSTPSPNk@clName){\PSTPSPNk@crName}
    \pnode(\PSTPSPNk@bcName|\PSTPSPNk@trName){\PSTPSPNk@tcName}
    \pnode(\PSTPSPNk@bcName|\PSTPSPNk@clName){\PSTPSPNk@ccName}
  \endgroup
  \ignorespaces}
%
%\define@key[psset]{pstricks-add}{method}{\def\psk@method{#1}}%     	   defined in pst-plot
\define@key[psset]{pstricks-add}{whichabs}{\def\psk@whichabs{#1}}%
\define@key[psset]{pstricks-add}{whichord}{\def\psk@whichord{#1}}%
\define@key[psset]{pstricks-add}{plotfuncx}{\def\psk@plotfuncx{#1}}%
\define@key[psset]{pstricks-add}{plotfuncy}{\def\psk@plotfuncy{#1}}%
\define@key[psset]{pstricks-add}{expression}{\def\psk@expression{#1}}%
\define@boolkey[psset]{pstricks-add}[Pst@]{buildvector}[true]{}%
%
\define@key[psset]{pstricks-add}{varsteptol}{\def\psk@varsteptol{#1}}%  
\define@key[psset]{pstricks-add}{adamsorder}{\def\psk@adamsorder{#1}}% 
%\define@key[psset]{pstricks-add}{varstepincrease}{\def\psk@varstepincrease{#1}}% varrk4
%
\define@key[psset]{pstricks-add}{StepType}{\pst@expandafter\psset@@StepType{#1}\@nil}%
\def\psset@@StepType#1#2\@nil{%
  \ifx#1u\let\psk@StepType\@ne
  \else\ifx#1l\let\psk@StepType\z@
  \else\ifx#1i\let\psk@StepType\thr@@
  \else\ifx#1s\let\psk@StepType\f@ur
  \else\let\psk@StepType\tw@\fi\fi\fi\fi}
\psset{StepType=lower} %               alternative StepType=upper/inf/sup/Riemann
\define@boolkey[psset]{pstricks-add}[Pst@]{noVerticalLines}[true]{}%
\psset{noVerticalLines=false}
%
\def\psStep{\def\pst@par{}\pst@object{psStep}}
\def\psStep@i(#1,#2)#3#4{%
  \begin@ClosedObj%
  \addto@pscode{
    \ifPst@algebraic /Func (#4) tx@addDict begin AlgParser end cvx def \fi 
    /x #1  def
    /dx #2 #1 sub #3 div def
    /scx { \pst@number\psxunit mul } def 
    /scy { \pst@number\psyunit mul } def
    \ifcase\psk@StepType % 0->lower, height is always f(x)
      x scx 0 moveto 
      #3 {
        \ifPst@algebraic Func \else #4 \fi 
        scy dup x scx exch \ifPst@noVerticalLines  moveto \else lineto \fi
        /x x dx add def
        x scx exch lineto 
        x scx 0 \ifPst@noVerticalLines  moveto \else lineto \fi
      } repeat
    \or % 1-> upper, height is always f(x+dx)
      x scx 0 moveto 
      #3 {
        /x x dx add def
        \ifPst@algebraic Func \else #4 \fi scy dup x dx sub scx exch 
        \ifPst@noVerticalLines  moveto \else lineto \fi
        x scx exch lineto
        x scx 0 \ifPst@noVerticalLines  moveto \else lineto \fi
      } repeat
    \or % 2-> Riemann
      /eps3 500 def   %% increased  from 100 to 500 20140507
      /xMinMax [] def
      /AMax [] def
      /AMin [] def
      /dt dx eps3 div def
      #3 {
        /Max \ifPst@algebraic Func \else #4 \fi def 
        /Min Max def 
	/t x def % save x value
	eps3 {
	  \ifPst@algebraic Func \else #4 \fi 
	  dup
	  Max lt { /Max exch def } { dup Min gt { /Min exch def }{ pop } ifelse } ifelse
	  /x x dt add def
	} repeat 
	/x t def  % restore
	x scx Min scy Max scy xMinMax aload length 3 add array astore /xMinMax exch def
        /x x dx add def
	closepath
      } repeat
      /dx dx scx def
      xMinMax aload length 3 div cvi { 
        /yMax ED /yMin ED /x ED 
	x yMin moveto 
	dx 0 \ifPst@noVerticalLines rmoveto \else rlineto \fi
	x dx add yMax lineto 
	dx neg 0 \ifPst@noVerticalLines rmoveto \else rlineto \fi
	x yMin \ifPst@noVerticalLines moveto \else lineto \fi 
	closepath 
      } repeat
    \or % 3->inf(imum)
      #3 {
        x scx 0 moveto 
        \ifPst@algebraic Func \else #4 \fi /y0 ED % left value f(x)
	/xOld x def
        /x x dx add def
        \ifPst@algebraic Func \else #4 \fi /y1 ED % right value f(x+dx)
        y0 y1 lt { y0 }{ y1 } ifelse 		  % use infimum
	scy dup xOld scx exch \ifPst@noVerticalLines moveto \else lineto \fi 
        x scx exch lineto 
        x scx 0 \ifPst@noVerticalLines moveto \else lineto \fi
	closepath 
      } repeat
    \or % 4-> sup(remum)
      #3 {
        x scx 0 moveto 
        \ifPst@algebraic Func \else #4 \fi /y0 ED % left value f(x)
        /x x dx add def
        \ifPst@algebraic Func \else #4 \fi /y1 ED % right value f(x+dx)
        y0 y1 gt { y0 }{ y1 } ifelse 		  % use supremum
	scy dup x dx sub scx exch \ifPst@noVerticalLines  moveto \else lineto \fi 
        x scx exch lineto 
        x scx 0 \ifPst@noVerticalLines  moveto \else lineto \fi
	closepath 
      } repeat
    \fi
  }%
  \psk@fillstyle
  \pst@stroke
  \end@ClosedObj%
}
%
\define@key[psset]{pstricks-add}{Derive}{\def\psk@Derive{#1}}%
\define@boolkey[psset]{pstricks-add}[PST@]{Tnormal}[true]{}

\psset[pstricks-add]{CMYK=true}
\def\@NOTEMPTY{NOT@EMPTY}%%dr 0606
%
\def\psTangentLine{\def\pst@par{}\pst@object{psTangentLine}}
\def\psTangentLine@i(#1,#2)(#3,#4)(#5,#6)#7#8{%
  \begin@OpenObj%
  \addto@pscode{
    [[#1 dup dup mul exch 1 #2]
     [#3 dup dup mul exch 1 #4]
     [#5 dup dup mul exch 1 #6]]
    SolveLinEqSystem
    /abc ED
    abc aload pop    % a b c on stack
    exch #7          % a c b x
    mul add exch     % c+b*x a
    #7 dup mul mul add 	    % a*x^2+b*x+c
    /y0 ED 		    % save value
    abc aload pop pop exch  % b a
    #7 mul 2 mul add        % b+2*a*x0=mTan
    \ifPST@Tnormal
      neg 1 exch div         % -1/mTan=mOrth
      #8 mul /dy ED          % mOrth*dx=dy
      [
       #7 #8 add y0 dy add \tx@ScreenCoor % x0+dx y0 +dy
       #7 y0 \tx@ScreenCoor   % x0 y0
    \else
      dup                     % mTan mTan
      #8 mul /dy1 ED          % mTan*dx
      #8 neg mul /dy2 ED      % mTan*-dx
      [
       #7 #8 add y0 dy1 add \tx@ScreenCoor % x0+dx y0 +dy1
       #7 #8 sub y0 dy2 add \tx@ScreenCoor % x0-dx y0 +dy2
    \fi
    /Lineto /lineto load def
    \ifshowpoints true \else false \fi
    \tx@setlinejoin 		       %
    \tx@Line 
    }%
  \end@OpenObj%
    \pnode(!
     [[#1 dup dup mul exch 1 #2][#3 dup dup mul exch 1 #4][#5 dup dup mul exch 1 #6]]
     SolveLinEqSystem /abc ED
    abc aload pop    % a b c on stack
    exch #7          % a c b x
    mul add exch     % c+b*x a
    #7 dup mul mul add 	    % a*x^2+b*x+c
    /y0 ED 		    % save value
      #7 y0 ){OCurve}%
    \pnode(!
     [[#1 dup dup mul exch 1 #2][#3 dup dup mul exch 1 #4][#5 dup dup mul exch 1 #6]]
     SolveLinEqSystem /abc ED
    abc aload pop    % a b c on stack
    exch #7          % a c b x
    mul add exch     % c+b*x a
    #7 dup mul mul add 	    % a*x^2+b*x+c
    /y0 ED 		    % save value
    abc aload pop pop exch  % b a
    #7 mul 2 mul add        % b+2*a*x0=mTan
    neg 1 exch div         % -1/mTan=mOrth
      #8 mul /dy ED          % mOrth*dx=dy
      #7 #8 add y0 dy add % x0+dx y0 +dy
     ){ENormal}%
    \pnode(!
      [[#1 dup dup mul exch 1 #2][#3 dup dup mul exch 1 #4][#5 dup dup mul exch 1 #6]]
      SolveLinEqSystem
      /abc ED
      abc aload pop    % a b c on stack
      exch #7          % a c b x
      mul add exch     % c+b*x a
      #7 dup mul mul add 	    % a*x^2+b*x+c
      /y0 ED 		    % save value
      abc aload pop pop exch  % b a
      #7 mul 2 mul add        % b+2*a*x0=mTan
      #8 mul /dy1 ED          % mTan*dx
      #7 #8 add y0 dy1 add ){ETangent}%
\ignorespaces}

\def\psplotTangent@x#1,#2,#3\@nil{%
  \def\pst@tempLeft{#1}%
  \def\pst@tempRight{#2}}
%% #1 : x value
%% #2 : delta x or x0,x1
%% #3 : function
\def\psplotTangent{\@ifnextchar*{\@startrue\psplotTangent@i}{\@starfalse\psplotTangent@i*}}
\def\psplotTangent@i*{\@ifnextchar[{\psplotTangent@ii}{\psplotTangent@ii[]}}
\def\psplotTangent@ii[#1]#2#3#4{%
  \pst@killglue
  \expandafter\psplotTangent@x#3,,\@nil\relax
  \begingroup
  \ifx\relax#1\relax\else\psset{linestyle=solid,#1}\fi%
  \ifx\psk@Derive\@empty\ifPst@algebraic\def\psk@Derive{NOT@EMPTY}\fi\fi              %%dr 0606 hv 1003
  \pst@addarrowdef
  \addto@pscode{
    /F@pstplot \ifPst@algebraic (#4) tx@addDict begin AlgParser end cvx \else { #4 } \fi def % define function
    \ifx\psk@Derive\@empty\else
      \ifx\psk@Derive\@NOTEMPTY\else                                                  %%dr 0606
        /FDer@pstplot                                                                 % do we have a derivation defined?
        \ifPst@algebraic (\psk@Derive) tx@addDict begin AlgParser end cvx \else { \psk@Derive } \fi def % define derivation
      \fi                                                                             %%dr 0606
    \fi%
    /@parametric false def                                                            %%dr 0606
    % first we calculate the origin
    #2 dup /x ED /t ED tx@addDict begin mark F@pstplot end counttomark 1 gt           % test, if we have parametricplot 
      { /y ED /x ED /@parametric true def }                                           % if yes, then we have 2 values %%dr 0606
      { \ifPst@polarplot x \ifPst@algebraic RadtoDeg \fi PtoC /y ED /x ED \else /y ED \fi } ifelse 
    cleartomark 
    \ifx\psk@Derive\@NOTEMPTY                                                         %%begin dr 0606
                                                                                      %% algebraic we can use the derivative machine
        /FDer@pstplot (#4) @parametric { (t) } { (x) } ifelse
        tx@Derive begin Derive end tx@addDict begin AlgParser end cvx def
    \fi                                                                               %%end dr 0606
    x \pst@number\psxunit mul y \pst@number\psyunit mul 
    translate % define the temporary origin
    % now we calculate the slope of the tangent 
    \ifx\psk@Derive\@empty                                                            % de we have a derivation defined?
      #2 abs 1.0e-6 lt                                                                % no, we choose secant for the tangent 
      { #2 0.0005 add dup /x ED /t ED tx@addDict begin mark F@pstplot end counttomark 1 gt % test, if we have parametricplot
        { /y2 ED /x2 ED }                                                             % we have 2 values
        { \ifPst@polarplot dup x \ifPst@algebraic RadtoDeg \fi 
	  cos mul /x2 ED x \ifPst@algebraic RadtoDeg \fi sin mul \else /x2 x def \fi /y2 ED } ifelse
        cleartomark                                                                   % delete the mark
        #2 0.0005 sub dup /x ED /t ED tx@addDict begin mark F@pstplot end counttomark 1 gt % test, if we have parametricplot
          { /y1 ED /x1 ED }
	  { \ifPst@polarplot dup x \ifPst@algebraic RadtoDeg \fi 
	    cos mul /x1 ED x \ifPst@algebraic RadtoDeg \fi sin mul \else /x1 x def \fi /y1 ED } ifelse
         cleartomark 
        y2 y1 sub x2 x1 sub } % dy dx
      {  % > 1.0e-06
        #2 1.0005 mul dup /x ED /t ED tx@addDict begin mark F@pstplot end counttomark 1 gt % test, if we have parametricplot 
          { /y2 ED /x2 ED } % we have 2 values
          { \ifPst@polarplot dup x \ifPst@algebraic RadtoDeg \fi 
	    cos mul /x2 ED x \ifPst@algebraic RadtoDeg \fi sin mul \else /x2 x def \fi /y2 ED } ifelse
	cleartomark 
        #2 .9995 mul dup /x ED /t ED tx@addDict begin mark F@pstplot end counttomark 1 gt % test, if we have parametricplot 
          { /y1 ED /x1 ED } % we have 2 values 
          { \ifPst@polarplot dup x \ifPst@algebraic RadtoDeg \fi 
	    cos mul /x1 ED x \ifPst@algebraic RadtoDeg \fi sin mul \else /x1 x def \fi /y1 ED } ifelse
	cleartomark 
        y2 y1 sub \pst@number\psyunit mul x2 x1 sub \pst@number\psxunit mul } ifelse 
      atan %  atan(dy dx), we have the slope angle of the secant
      \ifPST@Tnormal 90 add \fi
    \else % there is a derivation defined
      #2 dup /x ED /t ED tx@addDict begin mark FDer@pstplot end counttomark 1 gt % test, if we have parametricplot 
        { /y ED /x ED }
        { \ifPst@polarplot /Fphi ED % the value F'(phi) 
            tx@addDict begin F@pstplot end x \ifPst@algebraic RadtoDeg \fi PtoC /y0 ED /x0 ED % the x y values
            x \ifPst@algebraic RadtoDeg \fi sin Fphi mul x0 add /y ED 
            x \ifPst@algebraic RadtoDeg \fi cos Fphi mul y0 sub /x ED 
          \else /y ED /x 1 def \fi } ifelse
      cleartomark 
      y \pst@number\psyunit mul x \pst@number\psxunit mul Atan \ifPST@Tnormal 90 add \fi
  %    y ATAN1  % we have the slope angle of the tangent. ATAN is defined int the pstricks.pro, patch 6
    \fi
    dup  					% to prevent rounding errors use original value
    cvi 180 mod 90 gt { 180 sub } if            % -90 <= angle <= 90
    rotate                                      % rotate, depending to the origin
    /Lineto /lineto load def                    % the pro file needs /Lineto 
    \pst@cp                                     % kill the currentpoint, if any
    [                                           % start array of points
    \ifPST@Tnormal
      0 0 % moveto
      #3 
      y \pst@number\psyunit mul x \pst@number\psxunit mul Atan cos div \pst@number\psxunit mul 0  % lineto
    \else % points are in reverse order ...
      \ifx\pst@tempRight\@empty #3 \else \pst@tempRight\space \fi \pst@number\psxunit mul 0            % moveto
      \if@star 0 
      \else 
          \ifx\pst@tempRight\@empty #3 neg \else \pst@tempLeft\space \fi 
          \pst@number\psxunit mul
        \fi 0     % lineto
    \fi
    \pst@usecolor\pslinecolor
    false                                       % don't show the points
    \tx@Line
    \ifx\pslinestyle\@none\else
      \pst@number\pslinewidth SLW
      \tx@setStrokeTransparency 
      \@nameuse{psls@\pslinestyle}
    \fi
    \ifshowpoints                               % show the points?
      gsave
      \psk@dotsize
      \@nameuse{psds@\psk@dotstyle}
      0 0 Dot
      grestore
    \fi
   }%
  \use@pscode%
  \endgroup%
  \@starfalse%
  \ignorespaces}
%
%% #1-#2 x range
%% #3 initial value of y (which is a vector) y(0) y'(0) y''(0) ...
%% #4 value of the derivative (y and t can be used)
%
\define@boolkey[psset]{pstricks-add}[Pst@]{GetFinalState}[true]{}
\define@key[psset]{pstricks-add}{filename}{\def\psk@filename{#1}}%
\define@boolkey[psset]{pstricks-add}[Pst@]{saveData}[true]{} % \ifPst@saveData
\psset[pstricks-add]{GetFinalState=false,saveData=false,filename=PSTdata}
%
\def\Begin@SaveFinalState{ end 
  /PST@beginspecial /@beginspecial load def 
  /PST@endspecial /@endspecial load def 
  /PST@setspecial /@setspecial load def 
  /@beginspecial {} def /@endspecial{} def /@setspecial {} def
  tx@Dict begin
}
\newif\ifPst@BeginSaveFinalState \Pst@BeginSaveFinalStatefalse
\def\BeginSaveFinalState{\Pst@BeginSaveFinalStatetrue}
\def\End@SaveFinalState{
  /@beginspecial /PST@beginspecial load def 
  /@endspecial /PST@endspecial load def 
  /@setspecial /PST@setspecial load def
}
\def\EndSaveFinalState{\pstverb{\End@SaveFinalState}}

\def\psplotDiffEqn{\def\pst@par{}\pst@object{psplotDiffEqn}}% initial code by Dominique 2005-05-21
\def\psplotDiffEqn@i#1#2#3#4{%
  \addbefore@par{xStart=#1}% 
  \pst@killglue%
  \begingroup%
  \use@par%
  \@nameuse{beginplot@\psplotstyle}%
  \addto@pscode{%
    \ifPst@BeginSaveFinalState \Begin@SaveFinalState \fi
    \ifPst@saveData /Pst@data (\psk@filename) (w) file def \fi
    /x #1 def				% first value
    /x1 #2 def				% last value
    \ifPst@GetFinalState \Begin@SaveFinalState  /y FinalState def
    \else /y [ #3 ] def \fi			% values for t=0
    /ylength y length def		% number of elements in #3
    /addvect {
      1 1 ylength {
        /i exch def
	ylength i sub 2 add -1 roll add ylength 2 mul i sub 1 roll
      } for
    } def
    /dx x1 x sub \psk@plotpoints\space div def
    /mulvect {
      ylength exch
      1 index {
        dup 4 -1 roll mul 2 index 2 add 1 roll
      } repeat
      pop pop } def
    /divvect { ylength exch 1 index { dup 4 -1 roll exch div 2 index 2 add 1 roll } repeat pop pop } def
    /k0 0 def /k1 0 def /k2 0 def /k3 0 def
    \ifPst@algebraic /F@pstplot (#4) tx@addDict begin AlgParser end cvx def \fi
    /Func {
      \ifPst@algebraic F@pstplot ylength array astore
      \else
        \ifPst@buildvector\else y aload pop \fi #4 
        \ifPst@buildvector\else ylength array astore \fi
      \fi
    } def
    \ifx\psk@method\@adams /F1 0 def /F2 0 def /F3 0 def /F4 0 def /F5 0 def /F6 0 def /INIT 1 def \fi
    \ifx\psk@method\@empty\else
      \ifx\psk@method\@varrkiv            %% RUNGE-KUTTA method with var step algorithm
        /VarStep false def /VarStepRatio 1 def
        /RK {
           /k0 Func { dx mul } forall ylength array astore def 				%% y
           dup aload pop k0 { 2 div } forall addvect ylength array astore /y exch def %
           x dup dx 2 div add /x exch def 						%% y x
           /k1 Func { dx mul } forall ylength array astore def 				%% y x
           exch dup aload pop k1 { 2 div } forall addvect y astore pop 			%% x y
           /k2 Func { dx mul } forall ylength array astore def 				%% x y
           dup aload pop k2 aload pop addvect y astore pop exch dup dx add /x exch def 	%% y x
           /k3 Func { dx mul } forall ylength array astore def %% y x
           /x exch def 									%% y
           dup aload pop k0 aload pop k1 aload pop k2 aload pop addvect
           2 mulvect addvect k3 aload pop addvect
           6 divvect addvect y astore
        } def
        /VARRK {
          VarStep
          %{ /dx dx \psk@varstepincrease\space mul def /VarStep false def } if
          { /dx dx VarStepRatio mul def /VarStep false def } if
          x dx add x1 gt { /dx x1 x sub def } if
          %{ /dx dx \psk@varstepdecrease\space div def } ifelse
          %% we compute y(x+dx) from y(x) using RK4
          RK %% y(x) y(x+dx)
          exch /y exch def /dx dx 2 div def
          { %% we compute y(x+dx/2) from y(x) using RK4
            y RK %% y(x+dx) y(x+dx/2)
            %% then y(x+dx) from y(x+dx/2) using RK4
            /y exch def y RK %% y(x+dx) y(x) y(x+dx/2) y(x+dx)
            dup aload pop 4 ylength add -1 roll
            { -1 mul } forall addvect 0 ylength { exch abs 2 copy lt { exch } if pop } repeat
            0 3 -1 roll {abs 2 copy lt { exch } if pop } forall
            dup 1e-6 lt { pop } { div } ifelse
            /dx dx 2 mul def
            dup \psk@varsteptol\space lt
            %{ \psk@varsteptol\space div .1 lt { /VarStep true def } if pop exit } if
            %pop /dx dx 4 div def exch /y exch def } loop
            { .001 div dup .1 lt
              { dup 1e-6 lt { pop 3 } { log neg } ifelse /VarStepRatio exch def /VarStep true def }
              { pop } ifelse pop exit } if
            pop /dx dx 4 div def exch /y exch def } loop
        } def
      \else			%% RUNGE-KUTTA & ADAMS  methods
        /RK {
           /k0 Func { dx mul } forall ylength array astore def 				%% y
           dup aload pop k0 { 2 div } forall addvect ylength array astore /y exch def %
           x dup dx 2 div add /x exch def 						%% y x
           /k1 Func { dx mul } forall ylength array astore def 				%% y x
           exch dup aload pop k1 { 2 div } forall addvect y astore pop 			%% x y
           /k2 Func { dx mul } forall ylength array astore def 				%% x y
           dup aload pop k2 aload pop addvect y astore pop exch dup dx add /x exch def 	%% y x
           /k3 Func { dx mul } forall ylength array astore def %% y x
           /x exch def 									%% y
           dup aload pop k0 aload pop k1 aload pop k2 aload pop addvect
           2 mulvect addvect k3 aload pop addvect
           6 divvect addvect y astore pop
        } def
        \ifx\psk@method\@adams
           /ADAMS {
             \ifcase\psk@adamsorder
                \errmessage{pstricks-add error: no order 0th for adams method (see user's manual)}
             \or\errmessage{pstricks-add error: no order 1st for adams method (see user's manual)}
             \or\errmessage{pstricks-add error: no order 2nd for adams method (see user's manual)}
             \or\errmessage{pstricks-add error: no order 3rd for adams method (see user's manual)}
             \or
             %% ORDRE 4
               F4 aload pop  55 mulvect
               F3 aload pop -59 mulvect addvect
               F2 aload pop  37 mulvect addvect
               F1 aload pop  -9 mulvect addvect
               dx mulvect 24 divvect
             \or
             %% ORDRE 5
               F5 aload pop  1901 mulvect
               F4 aload pop -2774 mulvect addvect
               F3 aload pop  2616 mulvect addvect
               F2 aload pop -1274 mulvect addvect
               F1 aload pop   251 mulvect addvect
               dx mulvect 720 divvect
             \or
             %% ORDRE 6
               F6 aload pop  4277 mulvect
               F5 aload pop -7923 mulvect addvect
               F4 aload pop  9982 mulvect addvect
               F3 aload pop -7298 mulvect addvect
               F2 aload pop  2877 mulvect addvect
               F1 aload pop  -475 mulvect addvect
               dx mulvect 1440 divvect
             \fi
             y aload pop addvect ylength array astore /y exch def } def
        \fi
      \fi
    \fi
    /xy {
      \ifx\psk@plotfuncx\@empty
        \ifx\psk@whichabs\@empty x \else y \psk@whichabs\space get \fi
      \else \psk@plotfuncx\space \fi
      \pst@number\psxunit mul y 
      \ifx\psk@method\@empty							%% EULER method
        /y Func { dx mul } forall y aload pop addvect ylength array astore def
      \else%
        \ifx\psk@method\@varrkiv						%% RUNGE-KUTTA method
	  VARRK
        \else\ifx\psk@method\@rkiv						%% RUNGE-KUTTA method
	  RK
        \else
          /F1 F2 def /F2 F3 def /F3 F4 def /F4 				        %% ADAMS method
          \ifcase\psk@adamsorder\or\or\or\or
           %% ORDRE 4
           Func def
           \or
           %% ORDRE 5
           F5 def /F5 Func def
           \or
           %% ORDRE 6
           F5 def /F5 F6 def /F6 Func def
          \fi
           INIT \psk@adamsorder\space lt
           { RK /INIT INIT 1 add def }
           { ADAMS } ifelse
        \fi\fi
      \fi
      \ifx\psk@plotfuncy\@empty
        \ifx\psk@whichord\@empty 0 \else \psk@whichord\space \fi  get %
      \else \psk@plotfuncy\space \fi
      \pst@number\psyunit mul  
%        Pst@data (\string\[) writestring
      \ifPst@saveData 
        2 copy
        \pst@number\psyunit div exch  \pst@number\psxunit div 
        20 string cvs Pst@data exch writestring 
        Pst@data (\space) writestring 
        20 string cvs Pst@data exch writestring 
        Pst@data (\string\n) writestring 
      \fi
    } def
  }%
  \gdef\psplot@init{}%
  \@pstfalse
  \@nameuse{testqp@\psplotstyle}%
  \if@pst\psplot@ii\else\psplot@iii\fi
%  \addto@pscode{\ifPst@saveData Pst@data closefile \fi}
  \endgroup%
  \ignorespaces%
}
%
%
\def\psGTriangle{\def\pst@par{}\pst@object{psGTriangle}}
\def\psGTriangle@i(#1)(#2)(#3)#4#5#6{{%
  \def\solid@star{}%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempA	%   A: "rgb xr xg xb" or "gray xg"
  \pst@getcoor{#2}\pst@tempB	%   B
  \pst@getcoor{#3}\pst@tempC	%   C
  \pst@getcolor{#4}\pst@colorA
  \pst@getcolor{#5}\pst@colorB
  \pst@getcolor{#6}\pst@colorC
  \addto@pscode{%
    \pst@tempC		    % C
    \pst@tempB		    % B
    \psk@gangle             %   rotating angle
    \pst@tempA 		    % A, temporary origin
    /rgb {} def
    /gray {} def
    [ \pst@colorC ] aload length 1 eq { dup dup } if 3 array astore % gray -> rgb
    [ \pst@colorB ] aload length 1 eq { dup dup } if 3 array astore
    [ \pst@colorA ] aload length 1 eq { dup dup } if 3 array astore
    tx@addDict begin GTriangle end % PS part
  }%
  \if@star\pspolygon[fillstyle=none](#1)(#2)(#3)\fi%	draw borderline
  \def\pst@linetype{2}%
  \end@ClosedObj%
}\ignorespaces}
%
\def\psdice{\def\pst@par{}\pst@object{psdice}}
\def\psdice@i#1{{%
  \pst@killglue%
  \addbefore@par{framearc=0.3,linewidth=1pt}%
  \use@par%
  \psframe(-0.5,-0.5)(0.5,0.5)%
  \ifodd#1 \qdisk(0,0){0.1\psunit}\else\qdisk(-0.3,-0.3){0.1\psunit}\qdisk(0.3,0.3){0.1\psunit}\fi
  \ifcase#1%
    \or\or\or\qdisk(-0.3,-0.3){0.1\psunit}\qdisk(0.3,0.3){0.1\psunit}% 3
    \or\qdisk(-0.3,0.3){0.1\psunit}\qdisk(0.3,-0.3){0.1\psunit}%      4
    \or\qdisk(-0.3,-0.3){0.1\psunit}\qdisk(0.3,0.3){0.1\psunit}%      5
       \qdisk(-0.3,0.3){0.1\psunit}\qdisk(0.3,-0.3){0.1\psunit}
    \or\qdisk(-0.3,0.3){0.1\psunit}\qdisk(0.3,-0.3){0.1\psunit}%      6
       \qdisk(-0.3,0){0.1\psunit}\qdisk(0.3,0){0.1\psunit}%
  \fi%
  \ignorespaces%
}}
%
% the datafile must be a matrix with
% /dotmatrix [
%   .....
%   .....
% ] def
%
\def\pswavelengthToGRAY{ tx@addDict begin wavelengthToGRAY end }
\def\pswavelengthToRGB{ tx@addDict begin wavelengthToRGB Red Green Blue end }
%
\define@key[psset]{pstricks-add}{Xoffset}[0pt]{\pst@getlength{#1}\psk@Xoffset}
\define@key[psset]{pstricks-add}{Yoffset}[0pt]{\pst@getlength{#1}\psk@Yoffset}
\define@key[psset]{pstricks-add}{XYoffset}[0pt]{\pst@getlength{#1}\psk@Xoffset\let\psk@Yoffset\psk@Xoffset}
\psset[pstricks-add]{XYoffset=0pt}
\define@key[psset]{pstricks-add}{colorType}[0]{\def\psk@colorType{#1}}
\define@key[psset]{pstricks-add}{colorTypeDef}[{}]{\def\psk@colorTypeDef{#1\space}}
\psset[pstricks-add]{colorType=0,colorTypeDef={}} % 0-> two color mode 1->wavelength mode (400..700nm)
% 0-> two color mode 
% 1-> wavelength mode (400..700nm)
% 2-> wavelength mode inverse
% 3-> gray color mode
% 4-> gray color mode invers
% 5-> own color definition
\def\psMatrixPlot{\def\pst@par{}\pst@object{psMatrixPlot}}
\def\psMatrixPlot@i#1#2#3{%
  \pst@killglue%
  \addbefore@par{xStep=1,yStep=1}%
  \begin@SpecialObj%
  \addto@pscode{
    (#3) run   		% load the data file
    /Min 0 def /Max 0 def
    dotmatrix { dup Min lt { /Min ED } { dup Max gt { /Max ED } { pop } ifelse } ifelse } forall
    /dMaxMin Max Min sub def
    \psk@dotsize
    \psk@Xoffset\space \psk@Yoffset\space translate
    \@nameuse{psds@\psk@dotstyle} % 
    /n 0 def   		% index for element
    1 1 #1 {		% the y loop (outer one)
      /y exch def	% save y
      1 1 #2 {		% the x loop (inner one)
        /x exch def	% save x
	dotmatrix n get % get value from matrix 
        \ifcase\psk@colorType
  	  dup 0 gt { 	% test if > 0
  	\or
          Min sub dMaxMin div 300 mul 400 add
          \pswavelengthToRGB setrgbcolor
        \or
          Min sub dMaxMin div neg 1 add 300 mul 400 add
          \pswavelengthToRGB setrgbcolor
        \or        
          Min sub dMaxMin div neg 1 add 300 mul 400 add
          \pswavelengthToGRAY setgray
        \or        
          Min sub dMaxMin div neg 1 add 300 mul 400 add
          \pswavelengthToGRAY neg 1 add setgray
        \or
          currentdict /colorTypeDef known { colorTypeDef } { \psk@colorTypeDef } ifelse
        \fi
	  x \psk@xStep\space mul \pst@number\psxunit mul 
	  \ifPst@ChangeOrder #1 y sub 1 add \else y \fi \psk@yStep\space mul \pst@number\psyunit mul Dot%
        \ifcase\psk@colorType
 	  } { pop } ifelse
 	\fi
	/n n 1 add def
      } for 
    } for
  }%
  \end@SpecialObj%
  \ignorespaces%
}
%
\newdimen\chart@ColorIndex
\newdimen\chart@ColorStep
\newdimen\pst@chartHeight
\newdimen\pst@chartStackDepth
\newdimen\pst@chartStackWidth
\newcount\chart@Toggle
\newif\if@chartSep
\newif\if@chartUserColor
%
\define@key[psset]{pstricks-add}{chartStyle}{\def\psk@chartStyle{#1}}
\psset[pstricks-add]{chartStyle=pie}% p)ie P)ie-3d-view h)istogram H)istogram-3dview
%
\define@key[psset]{pstricks-add}{chartColor}{\pst@expandafter\psk@@chartColor{#1}\@nil}
\def\psk@@chartColor#1#2\@nil{%
  \ifx#1r\def\psk@chartColor{2}\else%
    \ifx#1c\def\psk@chartColor{380}\else\def\psk@chartColor{0}\fi\fi}
\psset[pstricks-add]{chartColor=gray}% gray, color, randomColor
%
\define@key[psset]{pstricks-add}{chartSep}{\pst@getlength{#1}\psk@chartSep}
\define@key[psset]{pstricks-add}{chartStack}{\pst@getint{#1}\psk@chartStack}
\define@key[psset]{pstricks-add}{chartStackDepth}{\pssetylength\pst@chartStackDepth{#1}}
\define@key[psset]{pstricks-add}{chartStackWidth}{\pssetxlength\pst@chartStackWidth{#1}}
\define@key[psset]{pstricks-add}{chartHeight}{\pssetylength\pst@chartHeight{#1}}
\psset[pstricks-add]{chartSep=10pt,chartStack=0,chartStackDepth=2cm,chartStackWidth=2cm,%
    chartHeight=5mm}
%
\define@boolkey[psset]{pstricks-add}[Pst@]{uselinecolor}[true]{}
\psset[pstricks-add]{uselinecolor=false}
%
\define@key[psset]{pstricks-add}{userColor}{%
  \chart@Toggle=0\relax%
  \def\chart@option{#1}%
  \ifx\chart@option\@empty\@chartUserColorfalse%
  \else%
    \@chartUserColortrue%
    \expandafter\psk@@chartUserColor#1,,\@nil%
  \fi}
\def\psk@@chartUserColor#1,#2,#3\@nil{%
  \advance\chart@Toggle by \@ne%
  \xglobal\colorlet{chartFillColor\the\chart@Toggle}{#1}%
  \def\chart@option{#2}%
  \ifx\chart@option\@empty\else\psk@@chartUserColor#2,#3,\@nil\fi}%
\psset[pstricks-add]{userColor={}}

\define@key[psset]{pstricks-add}{chartNodeI}{\def\psk@chartNodeI{#1}}
\define@key[psset]{pstricks-add}{chartNodeO}{\def\psk@chartNodeO{#1}}
\psset[pstricks-add]{chartNodeI=0.75,chartNodeO=1.5}
%
\def\psChart{\pst@object{psChart}}
\def\psChart@i#1#2#3{%
% #1:values  #2:separated charts
% #3 radius->pie; max height->histogram
  \pst@killglue%
  \global\pssetylength\pst@chartHeight{#3}%
  \global\let\pst@chartRadius\pst@chartHeight%
  \begingroup%
  \def\psk@chartValues{#1}%
  \def\psk@chartSepValues{#2}% only valid for a pie chart
  \pst@dimm=\z@% sum of all entries (for a pie)
  \pst@cnta=1\relax% number of entries
  \pst@dimn=\z@% greatest entry
  \psforeach{\chart@tempA}{#1}{%
    \global\advance\pst@cnta by \@ne%			% no of entries
    \global\advance\pst@dimm by \chart@tempA\p@%	% sum of all entries
    \pst@dima=\chart@tempA\p@% 
    \ifdim\pst@dima>\pst@dimn\global\pst@dimn=\pst@dima\fi%
  }%
  \addbefore@par{dimen=outer}%
  \begin@SpecialObj%
  \ifnum\psk@chartColor>0\relax%
    \chart@ColorStep=400\p@\else\chart@ColorStep=\p@\fi	% the "numerical color"
  \divide\chart@ColorStep by \pst@cnta%			% step =1/no or 400/no
  \chart@ColorIndex=\psk@chartColor\p@%			% the start color (gray or wave)
  \@nameuse{pscs@\psk@chartStyle}%
  \end@SpecialObj%
  \endgroup%
  \ignorespaces%
}
%
\def\pscs@pie{%
  \degrees[\pst@number\pst@dimm]%			% instead of 360 degrees
  \def\chart@alpha{0}%
  \pst@dimm=\z@\pst@dimn=\z@\pst@dimo=\z@\pst@cnta=0\relax%
  \global\chart@Toggle=1\relax%
  \ifpsshadow%						create shadow first
    \psforeach{\chart@tempA}{\psk@chartValues}{%
      \global\advance\pst@dimm by \chart@tempA\p@%
      \global\advance\pst@dimn by \chart@alpha\p@%
      \global\advance\pst@cnta by \@ne%
      \pst@dimo=0.5\pst@dimn\advance\pst@dimo by 0.5\pst@dimm%	half angle of the chart
      \global\@chartSepfalse%
      \if$\psk@chartSepValues$\else%
        \psforeach{\chart@tempC}{\psk@chartSepValues}{\ifnum\chart@tempC=\the\pst@cnta\relax\global\@chartSeptrue\fi}%
      \fi%
      \if@chartSep% 
        \pswedge(\psk@chartSep\p@;\pst@number\pst@dimo){\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \else%
        \pswedge(0,0){\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \fi%
      \global\let\chart@alpha\chart@tempA%
    }%
    \psshadowfalse%
  \fi%
  \def\chart@alpha{0}%
  \pst@dimm=0pt\pst@dimn=0pt\pst@dimo=0pt\pst@cnta=0\relax%
  \psForeach{\chart@tempA}{\psk@chartValues}{%
    \global\advance\pst@dimm by \chart@tempA\p@%
    \global\advance\pst@dimn by \chart@alpha\p@%
    \def\pst@tempB{\pst@number\chart@ColorIndex}%
%    \psDEBUG[psChart:wave:color]{\pst@tempB}%
    \global\advance\pst@cnta by \@ne%
    \if@chartUserColor\else%
      \def\chart@FillColor{chartFillColor\the\pst@cnta}%
      \ifnum\psk@chartColor>0\relax%
        \xglobal\definecolor{\chart@FillColor}{wave}{\pst@tempB}%
      \else\xglobal\definecolor{\chart@FillColor}{gray}{\pst@tempB}\fi%
    \fi%
    \pst@dimo=0.5\pst@dimn\advance\pst@dimo by 0.5\pst@dimm%	half angle of the chart
    \global\@chartSepfalse%
    \if$\psk@chartSepValues$\else%
      \psForeach{\chart@tempC}{\psk@chartSepValues}{\ifnum\chart@tempC=\the\pst@cnta\relax\global\@chartSeptrue\fi}%
    \fi%
    \if@chartSep
      \ifPst@uselinecolor
        \pswedge[linecolor=\pslinecolor,fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}]%
          (\psk@chartSep\p@;\pst@number\pst@dimo){\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \else
        \pswedge[linecolor={chartFillColor\the\pst@cnta},fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}]%
          (\psk@chartSep\p@;\pst@number\pst@dimo){\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \fi
      \pst@dima=\pst@chartRadius\advance\pst@dima by \psk@chartSep\p@%
      \pnode(\pst@dima;\pst@number\pst@dimo){psChart\the\pst@cnta}%
      \pst@dimb=\psk@chartNodeI\pst@dima%
      \pst@dimc=\psk@chartNodeO\pst@dima%
      \pnode(\pst@dimb;\pst@number\pst@dimo){psChartI\the\pst@cnta}%
      \pnode(\pst@dimc;\pst@number\pst@dimo){psChartO\the\pst@cnta}%
    \else%
      \ifPst@uselinecolor
        \pswedge[linecolor=\pslinecolor,fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}](0,0)%
          {\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \else
        \pswedge[linecolor={chartFillColor\the\pst@cnta},fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}](0,0)%
          {\pst@chartRadius}{\pst@number\pst@dimn}{\pst@number\pst@dimm}%
      \fi
      \pnode(\pst@chartRadius;\pst@number\pst@dimo){psChart\the\pst@cnta}%
      \pst@dima=\pst@chartRadius%
      \pst@dimb=\psk@chartNodeI\pst@dima%
      \pst@dimc=\psk@chartNodeO\pst@dima%
      \pnode(\pst@dimb;\pst@number\pst@dimo){psChartI\the\pst@cnta}%
      \pnode(\pst@dimc;\pst@number\pst@dimo){psChartO\the\pst@cnta}%
    \fi%
    \global\let\chart@alpha\chart@tempA%
    \global\advance\chart@Toggle by \@ne%
    \ifnum\chart@Toggle<3\relax%
      \global\advance\chart@ColorIndex by 2\chart@ColorStep%
    \else%
      \global\chart@Toggle=0%
      \global\advance\chart@ColorIndex by -\chart@ColorStep%
    \fi%
  }% end foreach
  \ignorespaces%
}
%
\def\pscs@histogram{%
  \def\chart@maxValue{\pst@number\pst@dimn}%		max of the data
  \pst@@divide\pst@dimn\pst@chartHeight%		maxValue/maxHeight
  \psDEBUG[pscs@histogram]{chart@maxValue=\chart@maxValue}
  \psDEBUG[pscs@histogram]{(maxValue/maxHeight)pst@dimg=\pst@number\pst@dimg}
  \psDEBUG[pscs@histogram]{pst@chartHeight=\the\pst@chartHeight}
  \pst@dimo=28.46\pst@dimg
  \edef\pst@chartUnit{\pst@number\pst@dimo}
%  \psaxes[axesstyle=frame,
%    dy=1cm,Dy=\pst@number\pst@dimo](\the\pst@cnta,\the\pst@chartHeight)
  \pst@dimm=0pt\pst@dimn=0pt\pst@dimo=0pt\pst@cnta=0%
  \global\chart@Toggle=1
  \psforeach{\chart@tempA}{\psk@chartValues}{%
    \global\advance\pst@dimm by \chart@tempA pt%
    \def\pst@tempB{\pst@number\chart@ColorIndex}%
    \psDEBUG[psChart:wave:color]{\pst@tempB}%
    \global\advance\pst@cnta by \@ne%
    \if@chartUserColor\else
      \def\chart@FillColor{chartFillColor\the\pst@cnta}
      \ifnum\psk@chartColor>0 \xglobal\definecolor{\chart@FillColor}{wave}{\pst@tempB}%
      \else\xglobal\definecolor{\chart@FillColor}{gray}{\pst@tempB}\fi%
    \fi
    \psframe[linecolor={chartFillColor\the\pst@cnta},fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}]%
        (!\the\pst@cnta\space \psk@chartSep\space 28.46 div sub 0)
        (!\the\pst@cnta\space \psk@chartSep\space 28.46 div add \chart@tempA\space \pst@chartUnit\space div)
    \pnode(!\the\pst@cnta\space 0){psChart\the\pst@cnta}%
    \pnode(!\the\pst@cnta\space  \chart@tempA\space 2 div \pst@chartUnit\space div){psChartM\the\pst@cnta}%
    \pnode(!\the\pst@cnta\space  \chart@tempA\space \pst@chartUnit\space div){psChartT\the\pst@cnta}%
    \global\advance\chart@Toggle by \@ne
    \ifnum\chart@Toggle<3
      \global\advance\chart@ColorIndex by 2\chart@ColorStep
    \else
      \global\chart@Toggle=0
      \global\advance\chart@ColorIndex by -\chart@ColorStep%
    \fi%
  }% end foreach
}
%
\def\pst@stackList{}
\def\addbefore@stackList#1{%
  \ifx\pst@stackList\@empty
    \xdef\pst@stackList{#1}%
  \else
    \toks@{#1}%
    \pst@toks\expandafter{\pst@stackList}%
    \xdef\pst@stackList{\the\toks@,\the\pst@toks}%
  \fi%
}
%
\def\pscs@Histogram{%
  \psDEBUG[pscs@Histogram]{psk@chartStack=\psk@chartStack}%
  \def\chart@maxValue{\pst@number\pst@dimn}%		max of the data
  \pst@@divide\pst@dimn\pst@chartHeight%		maxValue/maxHeight
  \psDEBUG[pscs@Histogram]{chart@maxValue=\chart@maxValue}%
  \psDEBUG[pscs@Histogram]{(maxValue/maxHeight)pst@dimg=\pst@number\pst@dimg}%
  \psDEBUG[pscs@Histogram]{pst@chartHeight=\the\pst@chartHeight}%
  \pst@dimo=28.46\pst@dimg%
  \edef\pst@chartUnit{\pst@number\pst@dimo}%
%  \psaxes[axesstyle=frame,
%    dy=1cm,Dy=\pst@number\pst@dimo](\the\pst@cnta,\the\pst@chartHeight)
  \pst@dimm=0pt\pst@dimn=0pt\pst@dimo=0pt\pst@cnta=0%
  \global\chart@Toggle=1			% for color toggling
  \pst@cntn=0					% stacked step
  \pst@cnto=0					% for a stacked view
  \pst@cntp=\psk@chartStack			% for a stacked view
  \def\pst@stackList{}
  \psDEBUG[pscs@Histogram]{psk@chartStack=\the\pst@cntp}%
  \psforeach{\chart@tempA}{\psk@chartValues}{%	  the loop
    \ifnum\pst@cntp>0 				% stacked version?
      \advance\pst@cnto by \@ne 		% increase
      \psDEBUG[pscs@Histogram]{chart@tempA=\chart@tempA}%
      \expandafter\addbefore@stackList\expandafter{\chart@tempA}%
      \psDEBUG[pscs@Histogram]{stack list=\pst@stackList}%
      \ifnum\pst@cnto=\pst@cntp			% draw?
        \pst@cnto=\psk@chartStack\advance\pst@cnto by \m@ne
        \psforeach{\chart@tempB}{\pst@stackList}{%	  the stack loop
          \global\pst@cnta=\pst@cntn				% we do not need the value
          \psDEBUG[pscs@Histogram]{pst@cnto=\the\pst@cnto}%
          \psDEBUG[pscs@Histogram]{pst@chartStackDepth=\the\pst@chartStackDepth}%
          \psDEBUG[pscs@Histogram]{pst@chartStackWidth=\the\pst@chartStackWidth}%
          \edef\pst@tempA{\the\pst@cnto}%
          \psDEBUG[pscs@Histogram]{pst@tempA=\pst@tempA}%
          \ifnum\pst@cnto>0 
            \pst@dima=\pst@chartStackDepth%
            \pst@dimb=\pst@chartStackWidth%
            \divide \pst@dima by \pst@tempA%
            \divide \pst@dimb by \pst@tempA% 
          \else\pst@dima=\z@ \pst@dimb=\z@%
          \fi%
          \rput(\the\pst@dima, \the\pst@dimb){\pscs@Histogram@i{\chart@tempB}}
          \advance\pst@cnto by \m@ne		% decrease stack counter
        }%
        \advance\pst@cntn by \tw@ 		% increase
        \def\pst@stackList{}%			  reset stack list
        \pst@cnto=0				% reset stack counter
      \fi%
    \else%
      \pscs@Histogram@i{\chart@tempA}% non stacked version
    \fi%
  }% end foreach
}
%
\def\pscs@Histogram@i#1{% draw the 3d-like bar
    \def\pst@tempB{\pst@number\chart@ColorIndex}%
    \global\advance\pst@cnta by \@ne%
    \if@chartUserColor\else
      \def\chart@FillColor{chartFillColor\the\pst@cnta}
      \ifnum\psk@chartColor>0 \xglobal\definecolor{\chart@FillColor}{wave}{\pst@tempB}%
      \else\xglobal\definecolor{\chart@FillColor}{gray}{\pst@tempB}\fi%
    \fi
    \pspolygon[fillstyle=solid,fillcolor={chartFillColor\the\pst@cnta}]%
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div sub 0)% ll
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div add 0)% lr
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div 1.5 mul add \psk@chartSep\space 56.92 div)% 'lr 
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div 1.5 mul add 
    	    \psk@chartSep\space 56.92 div #1 \pst@chartUnit\space div add )% 'ur 
      (!\the\pst@cnta\space \psk@chartSep\space 56.92 div sub 
    	    \psk@chartSep\space 56.92 div #1 \pst@chartUnit\space div add )% 'ul 
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div sub #1 \pst@chartUnit\space div)%ul
    \psline%
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div add 0)% lr
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div add #1 \pst@chartUnit\space div)
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div sub #1 \pst@chartUnit\space div)%ul
    \psline%
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div add #1 \pst@chartUnit\space div)
      (!\the\pst@cnta\space \psk@chartSep\space 28.46 div 1.5 mul add 
    	    \psk@chartSep\space 56.92 div #1 \pst@chartUnit\space div add )% 'ur 
     \pnode(!\the\pst@cnta\space 0){psChart\the\pst@cnta}%
     \pnode(!\the\pst@cnta\space  #1 2 div \pst@chartUnit\space div){psChartM\the\pst@cnta}%
     \pnode(!\the\pst@cnta\space  #1 \pst@chartUnit\space div){psChartT\the\pst@cnta}%
    \global\advance\chart@Toggle by \@ne
    \ifnum\chart@Toggle<3
      \global\advance\chart@ColorIndex by 2\chart@ColorStep
    \else
      \global\chart@Toggle=0
      \global\advance\chart@ColorIndex by -\chart@ColorStep%
    \fi%
     \global\advance\chart@ColorIndex by 1pt
}
%
\define@key[psset]{pstricks-add}{cancelType}{\pst@expandafter\psk@@cancelType{#1xx}\@nil}
\def\psk@@cancelType#1#2\@nil{%
  \ifx\relax#1\relax\def\psk@cancelType{2}\else% x
    \ifx#1b\def\psk@cancelType{2}\else%          \
      \ifx#1s\def\psk@cancelType{1}\else%        /
        \def\psk@cancelType{0}\fi\fi\fi}%        x every other

\psset[pstricks-add]{cancelType=}% x, crossing 
\def\psCancel{\def\pst@par{}\pst@object{psCancel}}% by Stefano Baroni 2008-06-21
\def\psCancel@i{\pst@makebox\psCancel@iii}
\def\psCancel@iii{%
  \begingroup
  \solid@star
  \use@par
  \pst@dima=\pslinewidth
  \advance\pst@dima by \psframesep
  \pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
  \pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
  \setbox\pst@hbox=\hbox{%
    \ifpsboxsep\kern\pst@dima\fi
    \begin@ClosedObj
    \addto@pscode{
      \psk@cornersize % arcradius boolean
      \pst@number\pst@dima neg
      \pst@number\pst@dimb neg
      \pst@number\pst@dimc
      \pst@number\pst@dimd
       .5 
      \if@star \tx@Frame \else
         CLW mul /a ED			% the middle of the line
         3 -1 roll 2 copy gt { exch } if
         a sub /y2 ED 
         a add /y1 ED 
         2 copy gt { exch } if
         a sub /x2 ED 
         a add /x1 ED 
         pop pop 			% delete arc values
         \ifnum\psk@cancelType<\tw@ % / or x
           x1 y1 moveto 
           x2 y2 lineto 
         \fi%
         \ifnum\psk@cancelType=\@ne\else % \ or x
           x2 y1 moveto 
           x1 y2 lineto
         \fi
       \fi
     }%
     \def\pst@linetype{2}%
     \showpointsfalse
     \end@ClosedObj
     \box\pst@hbox
     \ifpsboxsep\kern\pst@dima\fi%
   }%
   \ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
   \leavevmode\box\pst@hbox
   \endgroup%
}
%
\newcount\psVectorCtr
\define@boolkey[psset]{pstricks-add}[Pst@]{markAngle}[true]{}
\psset[pstricks-add]{markAngle=false}
%
\newpsstyle{psMarkAngleStyle}{arrows=->,arrowsize=4pt}
\newpsstyle{psMarkAngleLineStyle}{linestyle=dotted,arrows=-}
%
\def\psStartPoint{\@ifnextchar[{\psStartPoint@i}{\psStartPoint@i[Vector]}}
\def\psStartPoint@i[#1](#2){%
  \global\psVectorCtr=\@ne
  \gdef\psVectorName{#1}
  \pnode(#2){#10}
  \pst@getcoor{#2}\pst@tempA% 
  \pstVerb{tx@Dict begin 
           \pst@tempA 
           \pst@number\psyunit div /cp.Y exch def 
           \pst@number\psxunit div /cp.X exch def end }\ignorespaces}
%
\def\psVector{\pst@object{psVector}}
\def\psVector@i(#1){%
  \pst@killglue%
  \addbefore@par{arrows=->,arrowsize=6pt}%
%  \addto@par{showpoints=false}%
  \pst@getcoor{#1}\pst@tempCoor%
  \begingroup
  \use@par%
  \rput(! cp.X cp.Y ){%
    \psline(0,0)(#1)%
    \ifPst@markAngle
      \psarc[style=psMarkAngleStyle](0,0){1}{0}{!\pst@tempCoor exch atan}%
      \psline[style=psMarkAngleLineStyle](1.5,0)%
    \fi}%
  \pnode(! \pst@tempCoor \pst@number\psyunit div cp.Y add exch
                         \pst@number\psxunit div cp.X add exch ){\psVectorName\the\psVectorCtr}%
  \global\advance\psVectorCtr by \@ne%
  \endgroup%
  \pst@Verb{%tx@Dict begin 
    \pst@tempCoor 
    \pst@number\psyunit div cp.Y add /cp.Y exch def 
    \pst@number\psxunit div cp.X add /cp.X exch def %end
  }%  
  \ignorespaces}
%
\define@key[psset]{pstricks-add}{basename}{\def\psk@basename{#1}}%
\psset[pstricks-add]{basename=}%
%
\def\psCircleTangents{\pst@object{psCircleTangents}}
\def\psCircleTangents@i(#1){\@ifnextchar({\psCircleTangents@ii(#1)}{\psCircleTangents@iii(#1)}}%
\def\psCircleTangents@ii(#1)(#2)#3{%  (viewpoint) (circle) {radius}
    \pst@killglue%
    \begingroup%
       \pst@getlength{#3}\pst@LengthA%
       \addbefore@par{basename=CircleT}%
       \use@par%
       \edef\@cmd{\noexpand\psEllipseTangentsN(#2)(! \pst@LengthA dup %
       \pst@number\psxunit div exch \pst@number\psyunit div )(#1){\psk@basename}}%
       \@cmd%
    \endgroup%
  \ignorespaces%  
}%
\def\psCircleTangents@iii(#1)#2(#3)#4{%  two circles--- (Cntr1){radius1}(Cntr2){radius2}
  \pst@killglue%
  \begingroup%
     \pst@getlength{#2}\pst@LengthA% radius1
     \pst@getlength{#4}\pst@LengthB% radius2
     \addbefore@par{basename=CircleT}%
     \use@par%
     \psLCNodeVar(#1)(#3)(! \pst@LengthA \pst@number\psrunit div dup \pst@LengthB %
     \pst@number\psrunit div % r1 r1 r2 on stack
     3 copy add div /tti ED sub dup 0 eq % r1 r1-r2 on stack
     { pop pop /ttx 1000 def }{ div dup abs 1000 gt % r1/(r1-r2) on stack
     { 0 gt { ttx 1000 def }{ ttx -1000 def } ifelse}{ /ttx ED } ifelse } ifelse %
     1 tti sub tti )% 1-tti tti on stack
     {\psk@basename C1}%
     % tti=r1/(r1+r2), ttx=r1/(r1-r2)
     \psLCNodeVar(#1)(#3)(! 1 ttx sub ttx ){\psk@basename C2}% outside crossing pt
     \expandafter\psCircleTangents@ii\expandafter(\psk@basename C1)(#1){#2}%
     \pnode(CircleT1){\psk@basename I1}\pnode(CircleT2){\psk@basename I3}%
     \expandafter\psCircleTangents@ii\expandafter(\psk@basename C1)(#3){#4}%
     \pnode(CircleT1){\psk@basename I2}\pnode(CircleT2){\psk@basename I4}%
     % external tangents
     \expandafter\psCircleTangents@ii\expandafter(\psk@basename C2)(#1){#2}%
     \pnode(CircleT1){\psk@basename O2}\pnode(CircleT2){\psk@basename O4}%
     \expandafter\psCircleTangents@ii\expandafter(\psk@basename C2)(#3){#4}%
     \pnode(CircleT1){\psk@basename O1}\pnode(CircleT2){\psk@basename O3}%
  \endgroup%
  \ignorespaces%  
}%
%
\def\psEllipseTangents{\pst@object{psEllipseTangents}}
\def\psEllipseTangents@i(#1)(#2)(#3){% (Center)(axes)(viewpoint)
   \pst@killglue{%
   \use@par% only one parameter matters---psk@basename
   \ifx\psk@basename\@empty \def\psk@basename{EllipseT}\fi %
   \edef\@cmd{\noexpand\psEllipseTangentsN(#1)(#2)(#3){\psk@basename}}%
   \@cmd}\ignorespaces}%
%
\def\psEllipseTangentsN(#1)(#2)(#3)#4{%  (xe,ye)(a,b)(xP,yP){basename} % no optional arguments
  \pst@killglue
%  \pst@getcoor{#1}\pst@tempA
  \pnodes(#1){E@Cntr}(#2){@@TMP}(#3){@@@TMP}% (center)(semimajor, semiminor)(viewpt)
  \pst@getcoor{#3}\my@tempC% external viewpoint
  \AtoB(E@Cntr)(@@@TMP){@TMP}% center to viewpoint
  \ifnum\Pst@Debug>0
    \shownode(E@Cntr)%
    \shownode(@TMP)%
    \shownode(@@@TMP)%
  \fi%
  \pnode(! 
     \psGetNodeCenter{E@Cntr}\space
     /Xc E@Cntr.x def /Yc E@Cntr.y def
     \psGetNodeCenter{@@TMP}\space
     /B @@TMP.y def % semiminor
     /A @@TMP.x def % semimajor
     \psGetNodeCenter{@TMP}\space
     /Xp @TMP.x def /Yp @TMP.y def % center to viewpoint
%
     /A2 A dup mul def /B2 B dup mul def 
     /C2 B A div dup mul def 
     /Xp2 Xp dup mul def /Yp2 Yp dup mul def
     /R Xp2 A2 sub C2 mul Yp2 add Sqrt def % R=Sqrt{(Xp2-A2) C2 + Yp2}
     /Q C2 Xp2 mul Yp2 add def % C2 Xp2 + Yp2
     /Xta B2 Xp mul A Yp R mul mul sub Q div def
     /Yta Yp Xp R mul A div add B2 mul Q div def
     /Xtb B2 Xp mul A Yp R mul mul add Q div def
     /Ytb Yp Xp R mul A div sub B2 mul Q div def
     0 Xta Yp mul Yta Xp mul sub gt % swap a, b
       { /A Xta def /B Yta def /Xta Xtb def /Yta Ytb def /Xtb A def /Ytb B def } if
          Xta Xc add %/xTemp ED 
          Yta Yc add %/yTemp ED
%     xTemp Xc yTemp Yc Pyth2 /Length ED
%     xTemp Xc sub yTemp Yc sub exch atan 0 add Length exch PtoC 
%     Yc add exch Xc add exch 
          ) {#42}%
  \pnode(! Xtb Xc add Ytb Yc add ) {#41}%
 \ignorespaces}% 
%
\define@key[psset]{pstricks-add}{rotate}{\def\psk@rotate{#1 }}
\psset[pstricks-add]{rotate=0}

\def\pst@saveDegrees{}

\def\psKiviat{\pst@object{psKiviat}}
\def\psKiviat@i#1#2{%  #1: number of edges #2 radius
  \gdef\pst@saveDegrees{#1}
  \begingroup%
  \degrees[#1]%
  \SpecialCoor%
  \addbefore@par{rotate=0}
  \use@par%
  \global\let\psk@@rotate\psk@rotate
  \def\pst@Coordinates{}
  \psLoop{#1}{\xdef\pst@Coordinates{\pst@Coordinates(#2;\the\psLoopIndex)}}
  \rput{\psk@rotate}(0,0){\expandafter\pspolygon\pst@Coordinates
    \multido{\nA=0+1}{#1}{\uput{\pslabelsep}[\nA]{*0}(#2;\nA){\psPutYLabel{\nA}}}}
  \endgroup%
  \ignorespaces}
%
\def\psKiviatLine{\pst@object{psKiviatLine}}
\def\psKiviatLine@i#1{{%
  \addbefore@par{showpoints}%
  \use@par%
  \degrees[\pst@saveDegrees]%
  \psKiviatLine@ii#1\@nil}}%
\def\psKiviatLine@ii#1,#2\@nil{%
  \global\pst@cntm=0
  \global\pst@cntn=1
  \begingroup
  \xdef\pst@saveCoors{}
  \psKiviatLine@iii#1,#2,#1,,\@nil
  \rput{\psk@@rotate}(0,0){\expandafter\pspolygon\pst@saveCoors}
}
\def\psKiviatLine@iii#1,#2,#3\@nil{%
  \ifx\relax#2\relax\else%\psline(#1;\the\pst@cntm)(#2;\the\pst@cntn)
      \xdef\pst@saveCoors{\pst@saveCoors(#1;\the\pst@cntm)}\fi
  \advance\pst@cntm\@ne
  \advance\pst@cntn\@ne
  \ifx\relax#3\relax\endgroup\else\psKiviatLine@iii#2,#3\@nil\fi}
%
\def\psKiviatTicklines{\pst@object{psKiviatTicklines}}
\def\psKiviatTicklines@i#1#2{{%  n, radius
  \degrees[#1]%
  \use@par%
  \pstFPDiv\pst@tempN{#2}{\psk@Dx}% 
  \pst@cntm=\pst@tempN \advance\pst@cntm by \m@ne
  \multido{\rA=\psk@Dx+\psk@Dx}{\the\pst@cntm}{%
    \def\pst@Coordinates{}%
    \psLoop{#1}{\xdef\pst@Coordinates{\pst@Coordinates(\rA;\the\psLoopIndex)}}%
    \rput{\psk@@rotate}(0,0){\expandafter\pspolygon\pst@Coordinates}%
  }%
}\ignorespaces}%
%
\def\psKiviatAxes{\pst@object{psKiviatAxes}}
\def\psKiviatAxes@i#1#2{{%
  \degrees[#1]
  \use@par%
  \multido{\iA=0+1}{#1}{\rput{\psk@@rotate}(0,0){\psline(0,0)(#2;\iA)}}%
  }\ignorespaces}%
%
\define@key[psset]{pstricks-add}{colSteps}{\def\psk@colSteps{#1 }}
\define@boolkey[psset]{pstricks-add}[Pst@]{colored}[true]{}
\psset[pstricks-add]{colSteps=0,colored=false}% continuing colors and grayscale
%
\def\pstContour{\pst@object{pstContour}}
\def\pstContour@i#1{%
\begin@SpecialObj%
  \addto@pscode{
    (#1) run
    /zMax 0 def /zMin 0 def 			% lowest and highest value
    contourdata aload length /N ED 		% get the no of arrays
    N{						% inside contourdata
      /data ED 					% save first inner array
      data aload length 3 div round cvi {		% get the records
        dup zMin lt 				% z<zMin?
	  { /zMin ED }				% yes, save it
	  { dup zMax gt { /zMax ED }{ pop } ifelse } ifelse
        pop pop					% delete x y 
      } repeat
    } repeat
    clear					% clear stack
    /dz zMax zMin sub def			% value range
    /steps \psk@colSteps\space 0 gt { true }{ false } ifelse def
    0 1 N 1 sub { 				% for i=0 to N-1
      contourdata exch get /data ED		% get first array
      data aload length 3 div round cvi {	
        /z ED /y ED /x ED
        z zMin sub dz div 			% relative z (0..1)
        \ifPst@colored 400 mul 380 add tx@addDict begin wavelengthToRGB 
           Red Green Blue end setrgbcolor 	% set color	
        \else
          steps {\psk@colSteps\space mul round \psk@colSteps\space div} if
          setgray 
	\fi
        x \pst@number\psxunit mul y \pst@number\psyunit mul 
        1 0 360 arc fill
      } repeat
    } for
  }%
\end@SpecialObj%
}

\def\resetOptions{%
  \def\pst@linetype{0}%
  \pstScalePoints(1,1){}{}%
  \psset[pstricks-add]{%
    hooklength=3mm, hookwidth=1mm,
    ArrowFill=true,
    ArrowInside={}, ArrowInsidePos=0.5,
    ArrowInsideNo=1, ArrowInsideOffset=0,
    randomPoints=1000,color=false,
    whichabs={},whichord={},
    plotfuncx={},plotfuncy={},buildvector=false,
    Derive={},adamsorder=4,
    Tnormal=false,
    braceWidth=2\pslinewidth,
    bracePos=0.5,
    braceWidthInner=10\pslinewidth,
    braceWidthOuter=10\pslinewidth,
    chartNodeI=0.75,
    chartNodeO=1.5,
    markAngle=false,
    colSteps=0,
    colored=false,
}}
%
\resetOptions
%
\catcode`\@=\PstAtCode\relax
%
%% END: pstricks-add.tex
\endinput



==> pstricks.tex <==
%% pstricks.tex
%% COPYRIGHT 1993, 1994, 1999 by Timothy Van Zandt, tvz@nwu.edu.
%% COPYRIGHT 2000-2003 by Denis Girou.
%% Copyright 2004-2014 Herbert Voss
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2003/12/01 or later.
%
% This work has the LPPL maintenance status "maintained".
% 
% This Current Maintainer of this work is Herbert Voss
%
\csname PSTricksLoaded\endcsname
\let\PSTricksLoaded\endinput  
%
%% !! loading additional TeX packages see line 108 !!
%% !! loading config file pstricks.con    line 473 !!
%% !! loading pro files                   line 486 !!
%% !! fileversion and date see            line 113 !!
%
\edef\PstAtCode{\the\catcode`\@}
\catcode`\@=11\relax
%
\expandafter\ifx\csname @latexerr\endcsname\relax%	do we have LaTeX?
  \def\typeout#1{\immediate\write\@unused{#1}}%
  \alloc@7\write\chardef\sixt@@n\@unused
  \typeout{we are running tex and have to define some LaTeX commands ...}%
  \long\def\@ifundefined#1#2#3{\expandafter\ifx\csname
    #1\endcsname\relax#2\else#3\fi}
  \def\@namedef#1{\expandafter\def\csname #1\endcsname}
  \def\@nameuse#1{\csname #1\endcsname}
  \def\@eha{%
    Your command was ignored.^^J
    Type \space I <command> <return> \space to replace
    it with another command,^^J
    or \space <return> \space to continue without it.}
  \def\@spaces{\space\space\space\space}
  \def\@empty{}
  \def\@gobble#1{}
  \def\@nnil{\@nil}
%
  \def\@ifnextchar#1#2#3{%
    \let\@tempe#1\def\@tempa{#2}\def\@tempb{#3}\futurelet\@tempc\@ifnch}
%
  \def\@ifnch{%
    \ifx\@tempc\@sptoken \let\@tempd\@xifnch
    \else\ifx\@tempc\@tempe \let\@tempd\@tempa \else \let\@tempd\@tempb \fi
    \fi
    \@tempd%
  }
  \begingroup
  \def\:{\global\let\@sptoken= } \:
  \def\:{\@xifnch} \expandafter\gdef\: {\futurelet\@tempc\@ifnch}
  \endgroup
  \def\endtabular{\crcr\egroup\egroup $\egroup}
  \def\@width{width}% needed by pst-node
  \def\@tfor#1:={\@tf@r#1 }
  \long\def\@tf@r#1#2\do#3{\def\@fortmp{#2}\ifx\@fortmp\space\else
     \@tforloop#2\@nil\@nil\@@#1{#3}\fi}%
  \long\def\@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\@nnil
       \expandafter\@fornoop \else
      #4\relax\expandafter\@tforloop\fi#2\@@#3{#4}}
  \long\def\@break@tfor#1\@@#2#3{\csname fi\endcsname\csname fi\endcsname}
\fi%
\catcode`\@=\PstAtCode\relax
%
% now we have all commands defined, for TeX and LaTeX
%
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey.tex \fi
\catcode`\@=11\relax
\def\XKV@ch@ckch@ice#1#2#3{%  bugfix for xkeyval
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
%  \in@{,#2,}{,#3,}%
\begingroup\edef\x{\endgroup\noexpand\in@{,#2,}}\x{,#3,}%
%\expandafter\in@\expandafter{\expandafter,#2,}{,#3,}% --- hv 2012-04-27
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}

\def\ProvidesPackageRCS{\@ifnextchar[\ProvidesPackageRCS@i{\ProvidesPackageRCS@i[] }}  %$
\def\ProvidesPackageRCS@i[#1] $#2${} %$
\catcode`\@=\PstAtCode\relax
\ifx\PSTFPloaded\endinput\else   \input pst-fp.tex\fi

\input pgfutil-common.tex
\input pgfkeys.code.tex
\input pgffor.code.tex
\let\pgfforeach\foreach
%
\def\fileversion{2.54a}
\def\filedate{2014/05/19}
\catcode`\@=11\relax
\pst@addfams{pstricks}
%
% stolen from latex.ltx to make it TeX compatible
\newcount\psLoopIndex
\def\@fornoop#1\@@#2#3{}
\long\def\@for#1:=#2\do#3{%
  \pst@cntm=0%
  \expandafter\def\expandafter\@fortmp\expandafter{#2}%
  \ifx\@fortmp\@empty \else
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}\fi}
\long\def\@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\@nnil \else
       #5\def#4{#2}\ifx #4\@nnil \else\global\advance\psLoopIndex by \@ne\relax%
       #5\@iforloop #3\@@#4{#5}\fi\fi}
\long\def\@iforloop#1,#2\@@#3#4{\global\advance\psLoopIndex by \@ne\relax%
   \def#3{#1}\ifx #3\@nnil
     \expandafter\@fornoop \else
     #4\relax\expandafter\@iforloop\fi#2\@@#3{#4}}
%
\long\def\psforeach#1#2#3{%
  \global\psLoopIndex=0\relax%
  \if$\ifnum9<1#2$\else\fi\psforeach@ii{#1}{#2}{#3}%
  \else                      \expandafter\psforeach@i#2,..,,..,\@nil{#1}{#3}\fi}
\long\def\psforeach@i#1,#2,..,#3,..,#4\@nil#5#6{% 
  \ifx\relax#3\relax\psforeach@ii{#5}{#1,#2}{#6}%
  \else\psforeach@iii{#5}{#1}{#2}{#3}{#6}\fi}
\long\def\psforeach@ii#1#2#3{%
  \begingroup%
  \edef\reserved@a{#2}%
  \@for#1:=\reserved@a\do{#3}%
  \endgroup}
\long\def\psforeach@iii#1#2#3#4#5{%
  \pstFPsub\pst@tempA{#3}{#2}%
  \pst@dimm=\pst@tempA pt
  \pstFPstripZeros{\pst@tempA}\pst@tempB%
  \def\pst@tempA{#2}%
  \def\pst@tempa{#2}%
  \pst@dimn=#4pt%
  \loop%
    \pst@dimm=\pst@tempA pt%
    \ifdim\pst@dimm<\pst@dimn%
      \pstFPadd\pst@tempA{\pst@tempA}{\pst@tempB}%
      \pstFPstripZeros{\pst@tempA}\pst@tempA%
      \edef\pst@tempa{\pst@tempa,\pst@tempA}%
  \repeat%
  \psforeach@ii{#1}{\pst@tempa}{#5}}
%
\long\def\psForeach#1#2#3{%  without grouping the contents
  \global\psLoopIndex=0\relax%
  \if$\ifnum9<1#2$\else\fi\psforeach@ii{#1}{#2}{#3}%
  \else                   \expandafter\psForeach@i#2,..,,..,\@nil{#1}{#3}\fi}
\long\def\psForeach@i#1,#2,..,#3,..,#4\@nil#5#6{% 
  \ifx\relax#3\relax\psForeach@ii{#5}{#1,#2}{#6}%
  \else\psForeach@iii{#5}{#1}{#2}{#3}{#6}\fi%
}
\long\def\psForeach@ii#1#2#3{%
  \edef\reserved@a{#2}%
  \@for#1:=\reserved@a\do{#3}}
\long\def\psForeach@iii#1#2#3#4#5{%
  \pstFPsub\pst@tempA{#3}{#2}%
  \pst@dimm=\pst@tempA pt%
  \pstFPstripZeros{\pst@tempA}\pst@tempB%
  \def\pst@tempA{#2}%
  \def\pst@tempa{#2}%
  \pst@dimn=#4pt%
  \loop%
    \pst@dimm=\pst@tempA pt%
    \ifdim\pst@dimm<\pst@dimn%
      \pstFPadd\pst@tempA{\pst@tempA}{\pst@tempB}%
      \pstFPstripZeros{\pst@tempA}\pst@tempA
      \edef\pst@tempa{\pst@tempa,\pst@tempA}%
  \repeat%
  \psForeach@ii{#1}{\pst@tempa}{#5}
}
  
\def\psrecur@i#1{\csname ps@rn#1\psrecur@i} 
\long\def\ps@rnm#1{\endcsname{#1}#1\global\advance\psLoopIndex by \@ne}
\long\def\ps@rn#1{}
\def\psLoop#1{\global\psLoopIndex=0\relax%
  \csname ps@rn\expandafter\psrecur@i
  \romannumeral\number\number#1 000\endcsname\endcsname}

%
% hv 2007-10-16 to fix the bug in pst-node with \\[name=...]
% hv fix bug with empty fnodes in psmatrix
\def\ps@ifnextchar#1#2#3{%
  \let\reserved@d= #1%
  \def\reserved@a{#2}\def\reserved@b{#3}%
  \futurelet\@let@token\ps@ifnch}
\def\ps@ifnch{%
  \ifx\@let@token\reserved@d \let\reserved@b\reserved@a \fi
  \reserved@b
}
\def\pshskip#1{\vrule \@width\z@\nobreak \hskip #1\hskip \z@skip}
% end bugfix
\typeout{`PSTricks' v\fileversion\space\space <\filedate> (tvz)}
\def\@pstrickserr#1#2{%
  \begingroup
  \newlinechar`\^^J
  \edef\pst@tempc{#2}%
  \expandafter\errhelp\expandafter{\pst@tempc}%
  \typeout{%
    PSTricks error. \space See User's Guide for further information.^^J
    \@spaces\@spaces\@spaces\@spaces
    Type \space H <return> \space for immediate help.}%
  \errmessage{#1}%
  \endgroup}
\def\@ehpa{%
  Your command was ignored. Default value substituted.^^J
  Type \space <return> \space to procede.}
\def\@ehpb{%
  Your command was ignored. Will recover best I can.^^J
  Type \space <return> \space to procede.}
\def\@ehpc{%
  You better fix this before proceding.^^J
  See the PSTricks User's Guide or ask your system administrator for help.^^J
  Type \space X <return> \space to quit.}
\def\@ehpd{%
  Not allowed optional argument.^^J
  Will proceed with the default setting.^^J
  Type \space X <return> \space to quit.}
\def\pst@misplaced#1{\@pstrickserr{Misplaced \string#1 command}\@ehpb}
\newdimen\pst@dima
\newdimen\pst@dimb
\newdimen\pst@dimc
\newdimen\pst@dimd
\newdimen\pst@dimg
\newdimen\pst@dimh
\newdimen\pst@dimm
\newdimen\pst@dimn
\newdimen\pst@dimo
\newdimen\pst@dimp
\chardef\f@ur=4
%
\newbox\pst@hbox
\newbox\pst@ibox
\newbox\pst@boxg
\newcount\pst@cnta
\newcount\pst@cntb
\newcount\pst@cntc
\newcount\pst@cntd
\newcount\pst@cntg
\newcount\pst@cnth
\newcount\pst@cntm
\newcount\pst@cntn
\newcount\pst@cnto
\newcount\pst@cntp
\newcount\@zero\@zero=0\relax
%
\newif\ifPst@SpecialLength
\Pst@SpecialLengthfalse
%
\newif\if@pst
\newtoks\pst@toks
\newif\if@star
\def\pst@ifstar#1{%
  \@ifnextchar*{\@startrue\def\ps@next*{#1}\ps@next}{\@starfalse#1}}
%
\def\pst@expandafter#1#2{%
  \def\ps@next{#1}%
  \edef\@tempa{#2}%
  \ifx\@tempa\@empty
    \@pstrickserr{Unexpected empty argument!}\@ehpb
    \def\@tempa{\@empty}%
  \fi
  \expandafter\ps@next\@tempa}
%
\def\pst@dimtonum#1#2{\edef#2{\pst@@dimtonum#1}}
\def\pst@@dimtonum#1{\expandafter\pst@@@dimtonum\the#1}
{\catcode`\p=12 \catcode`\t=12 \global\@namedef{pst@@@dimtonum}#1pt{#1}}
%
\def\pst@getdimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetlength\pst@dimn{#1}%
    \pst@dimm=\z@%
  \else%
    \pssetlength\pst@dimm{#1}%
    \pssetlength\pst@dimn{#2}%
  \fi%
}
\def\pst@getxdimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetxlength\pst@dimn{#1}%
    \pst@dimm=\z@
  \else%
    \pssetxlength\pst@dimm{#1}%
    \pssetxlength\pst@dimn{#2}%
  \fi%
}
\def\pst@getydimdim#1 #2 #3\@nil{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty
    \pssetylength\pst@dimn{#1}%
    \pst@dimm=\z@%
  \else
    \pssetylength\pst@dimm{#1}%
    \pssetylength\pst@dimn{#2}%
  \fi}
%
% A modulo macro for integer values
% \pst@mod{34}{6}\value ==> \value is 4
%
\def\pst@mod#1#2#3{%
  \begingroup%
  \pst@cntm=#1\pst@cntn=#2\relax%
  \pst@cnto=\pst@cntm%
  \divide\pst@cntm by \pst@cntn%
  \multiply\pst@cntn by \pst@cntm%
  \advance\pst@cnto by -\pst@cntn%
  \edef\value{\endgroup\def\noexpand#3{\number\pst@cnto}}\value%
}
\def\pst@max#1#2#3{%
  \begingroup%
  \pst@cntm=#1\pst@cntn=#2\relax%
  \ifnum\pst@cntm<\pst@cntn\pst@cntm=\pst@cntn\fi
  \global#3=\the\pst@cntm%
  \endgroup%
}
\def\pst@maxdim#1#2#3{%
  \begingroup%
  \pst@dimm=#1\pst@dimn=#2\relax%
  \ifdim\pst@dimm<\pst@dimn\pst@dimm=\pst@dimn\fi
  \global#3=\the\pst@dimm%
  \endgroup%
}
\def\pst@mindim#1#2#3{%
  \begingroup%
  \pst@dimm=#1\pst@dimn=#2\relax%
  \ifdim\pst@dimm>\pst@dimn\pst@dimm=\pst@dimn\fi
  \global#3=\the\pst@dimm%
  \endgroup%
}
\def\pst@abs#1#2{%
  \begingroup%
  \pst@cntm=#1\relax%
  \ifnum\pst@cntm<\z@\pst@cntm=-\pst@cntm\fi%
  \global#2=\the\pst@cntm
  \endgroup%
}
\def\pst@absdim#1#2{%
  \begingroup%
  \pst@dimm=#1\relax%
  \ifdim\pst@dimm<\z@\pst@dimm=-\pst@dimm\fi%
  \global#2=\the\pst@dimm%
  \endgroup%
}
%
\def\pst@pyth#1#2#3{% from pst-3d
  \begingroup%
    \pst@dima=#1\relax%
    \ifnum\pst@dima<\z@\pst@dima=-\pst@dima\fi% dima=abs(x)
    \pst@dimb=#2\relax%
    \ifnum\pst@dimb<\z@\pst@dimb=-\pst@dimb\fi% dimb=abs(y)
    \advance\pst@dimb\pst@dima         % dimb=s=abs(x)+abs(y)
    \ifnum\pst@dimb=\z@
      \global\pst@dimg=\z@             % dimg=z=sqrt(x^2+y^2)
    \else
      \multiply\pst@dima 8\relax              % dima= 8abs(x)
      \pst@@divide\pst@dima\pst@dimb     % dimg =8t=8abs(x)/s
      \advance\pst@dimg -4pt            % dimg = 4tau = (8t-4)
      \multiply\pst@dimg 2
      \pst@dimtonum\pst@dimg\pst@tempa
      \pst@dima=\pst@tempa\pst@dimg           % dima=(8tau)^2
      \advance\pst@dima 64pt         % dima=u=[64+(8tau)^2]/2
      \divide\pst@dima 2\relax                      % =(8f)^2
      \pst@dimd=7pt                % initial guess at sqrt(u)
      \pst@@pyth\pst@@pyth\pst@@pyth            % dimd=sqrt(u)
      \pst@dimtonum\pst@dimd\pst@tempa
      \pst@dimg=\pst@tempa\pst@dimb
      \global\divide\pst@dimg 8             % dimg=z=(8f)*s/8
    \fi
  \endgroup
  #3=\pst@dimg}
%
\def\pst@@pyth{%                      dimd = g <-- (g + u/g)/2
  \pst@@divide\pst@dima\pst@dimd
  \advance\pst@dimd\pst@dimg
  \divide\pst@dimd 2\relax}
%
% ----- the old pst@pyth begin -----  did not use dimens
\def\pst@Pyth#1#2#3{\ifdim#1>#2\pst@@Pyth#1#2#3\else\pst@@Pyth#2#1#3\fi}
\def\pst@@Pyth#1#2#3{%
  \ifdim4#1>9#2\relax
    #3=#1\advance#3 .2122#2%
  \else
    #3=.8384#1\advance#3 .5758#2%
  \fi%
}
% ----- the old pst@pyth end -----
%
%------ new version \pst@divide ̣-------- by Michael Sharpe
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \advance\pst@dimg \pst@cnta pt%
  \pst@dimtonum\pst@dimg{#3}%
}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax%
  \pst@dimh=#2\relax%
  \pst@cnth=\pst@dimh%
  \pst@cntg=\pst@dimg%
  \pst@cnta=\pst@cntg%
  \divide\pst@cnta\pst@cnth%
  \advance\pst@dimg -\pst@cnta\pst@dimh%
  \pst@cntm=67108863\relax %2^26 -1
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide%
  \divide\pst@dimg\pst@cnth%
}%
\def\pst@@@divide{%
  \ifnum%
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cntm%
      \multiply\pst@dimg\sixt@@n%
  \else%
    \divide\pst@cnth\sixt@@n%
  \fi%
}%
%
%-------------- the old version ----------
\iffalse
\def\pst@divide#1#2#3{%
  \pst@@divide{#1}{#2}%
  \pst@dimtonum\pst@dimg{#3}%
}
\def\pst@@divide#1#2{%
  \pst@dimg=#1\relax
  \pst@dimh=#2\relax
  \pst@cntg=\pst@dimh
  \pst@cnth=67108863
  \pst@@@divide\pst@@@divide\pst@@@divide\pst@@@divide
  \divide\pst@dimg\pst@cntg%
}
\def\pst@@@divide{%
  \ifnum
    \ifnum\pst@dimg<\z@-\fi\pst@dimg<\pst@cnth
      \multiply\pst@dimg\sixt@@n
    \else
      \divide\pst@cntg\sixt@@n
    \fi%
}
\fi
%-------------- end old vesrion ---------------
%
\def\pst@configerr#1{%
  \@pstrickserr{\string#1 not defined in pstricks.con}\@ehpc}
%
\def\pstVerb#1{\pst@configerr\pstVerb}
\def\pstverb#1{\pst@configerr\pstverb}
\def\pstverbscale{\pst@configerr\pstverbscale}
\def\pstrotate{\pst@configerr\pstrotate}
\def\pstheader#1{\pst@configerr\pstheader}
\def\pstdriver{\pst@configerr\pstdriver}
\@ifundefined{pstcustomize}%
  {\def\pstcustomize{\endinput\let\pstcustomize\relax}}{}
%
\input pstricks.con		% local config file
%
\newif\ifPSTricks
\PSTrickstrue
\def\PSTricksOff{%
  \def\pstheader##1{}%
  \def\pstverb##1{}%
  \def\pstVerb##1{}%
  \PSTricksfalse%
}
\@ifundefined{pst@def}{\def\pst@def#1<#2>{\@namedef{tx@#1}{#2 }}}{}
\@ifundefined{pst@ATH}{\def\pst@ATH<#1>{}}{}
%
\pstheader{pstricks.pro}
\pstheader{pst-algparser.pro}
\pstheader{pst-tools.pro}
%
\def\pst@dict{tx@Dict begin }
\def\pst@theheaders{pstricks.pro, pst-algparser.pro}
\def\pst@Verb#1{\pstVerb{\pst@dict #1 end}}
\def\tx@Atan{Atan }
\def\tx@Div{Div }
\def\tx@NET{NET }
\def\tx@Pyth{Pyth }
\def\tx@PtoC{PtoC }
\def\tx@PathLength@{PathLength@ }
\def\tx@PathLength{PathLength }
\pst@dimg=\pstunit\relax
\ifdim\pst@dimg=1bp
\def\pst@stp{.996264 dup scale}
\else
\edef\pst@stp{1 \pst@@dimtonum\pst@dimg\space div dup scale}
\fi
\def\tx@STP{STP }
\def\tx@STV{STV }
%
%--------------------------------------- PS stuff ---------------------------------
% on stack x y 
\pst@def{UserCoor}< \pst@number\psyunit div exch \pst@number\psxunit div exch >
\pst@def{ScreenCoor}< \pst@number\psyunit mul exch \pst@number\psxunit mul exch >
%--------------------------------------- PS stuff end -----------------------------
%
\def\pst@number#1{\pst@@dimtonum#1\space}
%
%-----------------------% hv 20100413
\def\pst@strip@dot#1{\expandafter\pst@strip@dot@i#1..\@nil}
\def\pst@strip@dot@i#1.#2.#3\@nil{%
  \ifnum1#2>10\relax #1.#2\else#1\fi}
%-----------------------% hv 20100413
\def\pst@checknum#1#2{%
  \edef\ps@next{#1}%
  \ifx\ps@next\@empty\let\pst@num\z@%
  \else\expandafter\pst@@checknum\ps@next..\@nil%
  \fi%
  \ifcase\pst@num%  0
    \@pstrickserr{Bad number: `#1'. 0 substituted.}\@ehpa%
    \def#2{0 }%
  \or%              1
    \edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
      \expandafter\@gobble\the\pst@cnth\space}%
  \or%              2
    \edef#2{\ifnum\pst@num=\tw@-\fi\the\pst@cntg.%
      \expandafter\@gobble\the\pst@cnth\space}%
  \or%              3
    \edef#2{\pst@tempA\space}%
  \fi}
\def\pst@@checknum{%
  \@ifnextchar-%
  {\let\pst@num\tw@\expandafter\pst@@@checknum\@gobble}%
  {\@ifnextchar !%
    {\def\pst@num{3}\pst@@@@@checknum}
    {\let\pst@num\@ne\pst@@@checknum}}%
}
\def\pst@@@checknum#1.#2.#3\@nil{%
\afterassignment\pst@@@@checknum\pst@cntg=0#1\relax\@nil%
\afterassignment\pst@@@@checknum\pst@cnth=1#2\relax\@nil}
\def\pst@@@@checknum#1\relax\@nil{\ifx\@nil#1\@nil\else\let\pst@num\z@\fi}
%
\def\pst@@@@@checknum#1#2.#3\@nil{\def\pst@tempA{#2}}% PostScript Notation with !<code>
%
\def\pst@getnumii#1 #2 #3\@nil{%
  \pst@checknum{#1}\pst@tempg%
  \ifx\relax#2\relax\let\pst@temph\pst@tempg\else\pst@checknum{#2}\pst@temph\fi}
\def\pst@getnumiii#1 #2 #3 #4\@nil{%
\pst@checknum{#1}\pst@tempg%
\pst@checknum{#2}\pst@temph%
\pst@checknum{#3}\pst@tempi}
\def\pst@getnumiv#1 #2 #3 #4 #5\@nil{%
\pst@checknum{#1}\pst@tempg%
\pst@checknum{#2}\pst@temph%
\pst@checknum{#3}\pst@tempi%
\pst@checknum{#4}\pst@tempj}
%
\def\pst@getdimnum#1 #2 #3\@nil{%
  \pssetlength\pst@dimg{#1}%
  \pst@checknum{#2}\pst@tempg%
}
\def\pst@getscale#1#2{%	read and check a scale input x [y]
  \edef\pst@tempg{#1}%
  \ifx\pst@tempg\@none
    \def#2{}%
  \else
    \pst@expandafter\pst@getnumii{#1 #1} {} {} {}\@nil
    \ifdim\pst@tempg\p@=\z@
      \@pstrickserr{Bad scaling argument `#1'}\@ehpa
      \def#2{}%
    \else
      \ifdim\pst@temph\p@=\z@
        \@pstrickserr{Bad scaling argument `#1'}\@ehpa
        \def#2{}%
      \else
        \edef#2{\pst@tempg\space \pst@temph\space scale }%
      \fi
    \fi
  \fi%
}
\def\pst@getint#1#2{%	read and check an integer
  \pst@cntg=#1\relax
  \edef#2{\the\pst@cntg\space}%
}
\begingroup
\catcode`\{=12
\catcode`\}=12
\catcode`\[=1
\catcode`\]=2
\gdef\pslbrace[{ ]
\gdef\psrbrace[} ]
\endgroup

\pstVerb{
  /pssetRGBcolor  /setrgbcolor  load def
  /pssetCMYKcolor /setcmykcolor load def
  /pssetGraycolor /setgray      load def
}
\def\@newcolor#1#2{%
  \expandafter\edef\csname #1\endcsname{\noexpand\pst@color{#2}}%
  %\expandafter\edef\csname color@#1\endcsname{#2}%
  \expandafter\edef\csname\string\color@#1\endcsname{#2}%    hv 1.14 2005-12-17
  \ignorespaces}
\def\pst@color#1{%
  \def\pst@currentcolor{#1}\pstVerb{#1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@currentcolor}}
\def\pst@currentcolor{0 setgray}
\def\altcolormode{%
\def\pst@color##1{%
  \pstVerb{gsave ##1}\aftergroup\pst@endcolor}%
\def\pst@endcolor{\pstVerb{\pst@grestore}}}
\def\pssetMonochrome{%
  \pstVerb{
    /setrgbcolor { add add 0 gt {0}{1} ifelse setgray } def 
    /setcmykcolor{ 4 dict begin
      /k ED /y ED /m ED /c ED 
      1 1 k sub c mul k add sub 0.29 mul 
      1 1 k sub m mul k add sub 0.587 mul add 
      1 1 k sub y mul k add sub 0.114 mul add
      end 0 gt {0}{1} ifelse setgray } def }}
\def\pssetGrayscale{%
  \pstVerb{
    /setrgbcolor { 0.07 mul exch 0.71 mul add exch 0.21 mul add setgray } def 
    /setcmykcolor{ 4 dict begin
      /k ED /y ED /m ED /c ED 
      1 1 k sub c mul k add sub 0.29 mul 
      1 1 k sub m mul k add sub 0.587 mul add 
      1 1 k sub y mul k add sub 0.114 mul add
      end setgray } def }}
\def\psresetColor{\pstVerb{
    /setrgbcolor  tx@Dict begin /pssetRGBcolor  load end def 
    /setcmykcolor tx@Dict begin /pssetCMYKcolor load end def }}

\def\pst@grestore{
  currentpoint
  matrix currentmatrix
  currentfont
  grestore
  setfont
  setmatrix
  moveto
}
%\def\pst@usecolor#1{\csname color@#1\endcsname\space}%    hv 1.14  2005--12-17
\def\pst@usecolor#1{\csname\string\color@#1\endcsname\space}
%
\def\newgray#1#2{%
  \pst@checknum{#2}\pst@tempg
  \@newcolor{#1}{\pst@tempg setgray}}
\def\newrgbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi setrgbcolor}}
\def\newhsbcolor#1#2{%
  \pst@expandafter\pst@getnumiii{#2} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi sethsbcolor}}
\def\newcmykcolor#1#2{%
  \pst@expandafter\pst@getnumiv{#2} {} {} {} {} {}\@nil
  \@newcolor{#1}{\pst@tempg \pst@temph \pst@tempi \pst@tempj setcmykcolor}}
\newgray{black}{0}
\newgray{darkgray}{.25}
\newgray{gray}{.5}
\newgray{lightgray}{.75}
\newgray{white}{1}
\newrgbcolor{red}{1 0 0}
\newrgbcolor{green}{0 1 0}
\newrgbcolor{blue}{0 0 1}
\newrgbcolor{yellow}{1 1 0}
\newrgbcolor{cyan}{0 1 1}
\newrgbcolor{magenta}{1 0 1}
%
\define@key[psset]{pstricks}{style}{%
  \@ifundefined{pscs@#1}%
    {\@pstrickserr{Custom style `#1' undefined}\@ehpa}%
    {\@nameuse{pscs@#1}}%
}
\def\newpsstyle#1#2{\@namedef{pscs@#1}{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty\else\psset{#2}\fi}%
}
\def\addto@psstyle#1#2{%
    \pst@toks=\expandafter{#1#2}%
    \edef#1{\the\pst@toks}}
\def\addtopsstyle#1#2{%
  \def\pst@tempA{#2}%
  \ifx\pst@tempA\@empty\else
    \@ifundefined{pscs@#1}%
      {\newpsstyle{#1}{#2}}%
      {\expandafter\addto@psstyle\csname pscs@#1\endcsname{\psset{#2}}}%
  \fi}
%------------ hv 1.16 end -------------------
%
\def\@none{none}
\def\pst@getcolor#1#2{%
%  \@ifundefined{color@#1}%	hv 1.14  2005-12-17
  \@ifundefined{\string\color@#1}%
    {\@pstrickserr{Color `#1' not defined}\@eha}%
    {\edef#2{#1}}%
}
\newdimen\psunit \psunit 1cm
\newdimen\psxunit \psxunit 1cm
\newdimen\psyunit \psyunit 1cm
\let\psrunit\psunit
%
\def\pstunit@off{\let\@psunit\ignorespaces\ignorespaces}
%
\def\pssetlength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\psaddtolength#1#2{%
  \let\@psunit\psunit
  \afterassignment\pstunit@off
  \advance#1 #2\@psunit%
}
\def\pssetxlength#1#2{%
  \let\@psunit\psxunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\def\pssetylength#1#2{%
  \let\@psunit\psyunit
  \afterassignment\pstunit@off
  #1 #2\@psunit%
}
\define@key[psset]{pstricks}{unit}[1cm]{%
  \pssetlength\psunit{#1}%
  \psxunit=\psunit%
  \psyunit=\psunit%
}
\define@key[psset]{pstricks}{runit}[1cm]{\pssetlength\psrunit{#1}}
\define@key[psset]{pstricks}{xunit}[1cm]{\pssetxlength\psxunit{#1}}
\define@key[psset]{pstricks}{yunit}[1cm]{\pssetylength\psyunit{#1}}
%
\define@key[psset]{pstricks}{PstDebug}[0]{\pst@getint{#1}\Pst@Debug}% hv 2004-06-22
\psset[pstricks]{PstDebug=0}
\def\psDEBUG{\@ifnextchar[\psDEBUG@i{\psDEBUG@i[PSTricks]}}%
\def\psDEBUG@i[#1]#2{\ifnum\Pst@Debug>0 \expandafter\typeout{<#1>: #2}\fi}%
%
\def\pst@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\pst@number\pst@dimg}%
}
\def\pst@@getlength#1#2{%
  \pssetlength\pst@dimg{#1}%
  \edef#2{\number\pst@dimg sp}%
}
\def\pst@getcoor#1#2{\pst@@getcoor{#1}\let#2\pst@coor}
\def\pst@coor{0 0 }
%
\def\pst@getcoors#1#2{%
  \def\pst@aftercoors{\addto@pscode{#1 \pst@coors }#2}%
  \def\pst@coors{}%
  \pst@@getcoors%
}
\def\pst@@getcoors(#1){%
  \pst@@getcoor{#1}%
  \edef\pst@coors{\pst@coor\pst@coors}%
  \@ifnextchar({\pst@@getcoors}{\pst@aftercoors}%
}
%
\newcount\pst@C@@rType% 0: default cartesian coordinates and angles
%
\def\pst@getangle#1#2{\pst@@getangle{#1}\let#2\pst@angle}
\def\pst@angle{0 }
%
\def\cartesian@coor#1,#2,#3\@nil{%
  \pssetxlength\pst@dimg{#1}%
  \pssetylength\pst@dimh{#2}%
  \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
}
\def\NormalCoor{%
  \def\pst@@getcoor##1{\pst@expandafter\cartesian@coor{##1},\relax,\@nil}%
  \def\pstCheckCoorType##1{\global\pst@C@@rType=0}%
  \Pst@SpecialLengthfalse
  \def\pssetlength##1##2{%
    \let\@psunit\psunit
    \afterassignment\pstunit@off
    ##1 ##2\@psunit%
  }%
  \def\pst@@getangle##1{%
    \pst@checknum{##1}\pst@angle%
    \edef\pst@angle{\pst@angle \pst@angleunit}%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@cartesian}%
}
%\NormalCoor% set to normal read of coors, angles and lengths
%
\def\degrees{\@ifnextchar[{\@degrees}{\def\pst@angleunit{}}}
\def\@degrees[#1]{%
  \pst@checknum{#1}\pst@tempg
  \edef\pst@angleunit{360 \pst@tempg div mul }%
  \ignorespaces}
%
\def\radians{\def\pst@angleunit{57.2956 mul }}
\def\pst@angleunit{}
%
\def\SpecialCoor{%
  \def\pst@@getcoor##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup%
    \expandafter\special@coor\pst@tempg||\@nil}%
  \def\pstCheckCoorType##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup
    \psDEBUG[pstCheckCoorType]{:Checking coor \pst@tempg:}%
    \expandafter\pst@CheckCoorType\pst@tempg||\@nil%
    \psDEBUG[pstCheckCoorType]{::Coor type=\the\pst@C@@rType::}%
  }%
  \def\pssetlength##1##2{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##2}%
    \endgroup%
    \expandafter\special@length\pst@tempg\@nil{##1}%
  \ignorespaces}%
  \def\pst@@getangle##1{%
    \begingroup%
      \pst@activecoor%
      \xdef\pst@tempg{##1}%
    \endgroup%
    \expandafter\special@angle\pst@tempg\@empty)\@nil%
  }%
  \def\psput@##1{\pst@@getcoor{##1}\leavevmode\psput@special}%
}
\SpecialCoor% set to special read of coors, angles and lengths
%
\begingroup
\catcode`\|=13
\catcode`\;=13
\catcode`\!=13
\catcode`\*=13
\catcode`\>=13
\catcode`\+=13
\gdef\pst@activecoor{%
  \def|{\string|}%
  \def;{\string;}%
  \def!{\string!}%
  \def*{\string*}%			algebraic expression hv 2007-11-17
  \def>{\string>}%
  \def+{\string+}%			pure algebaric 2013-04-23
}
\endgroup
% \pst@C@@rType = 0 cartesian (x,y)
%               = 1 polar     (r;phi)
%               = 2 PS        (! x y)
%               = 3 mixed     ((x,y)|(x,y))
%               = 4 algebraic (*x f(x))   x in PostScript notation
%               = 5 node      (A)
%               = 6 special node ([...]A)
%               = 7 node      (>A)
%               = 8 algebraic (+x,f(x))   _both_ algebraic
\def\pst@CheckCoorType#1|#2|#3\@nil{%
  \ifx#3|\relax 
    \global\pst@C@@rType=3\relax
  \else 
    \expandafter\pst@@CheckCoorType#1;;\@nil%
  \fi}
%
\def\pst@@CheckCoorType#1#2;#3;#4\@nil{%
%\typeout{====1:#1}%
%\typeout{====2:#2}%
%\typeout{====3:#3}%
%\typeout{====4:#4}%
  \ifx#1>\relax%			node with special rotation for \uput
    \global\pst@C@@rType=7\relax%
  \else
    \ifcat#1a\relax%			node names should start with a letter
      \global\pst@C@@rType=5\relax%
    \else
      \ifx#1[\relax%			special node coor: [..]A
        \global\pst@C@@rType=6\relax%
      \else
        \ifx#1!\relax%			PostScript code: x y
          \global\pst@C@@rType=2\relax%
        \else
          \ifx#1*\relax%			algebraic PostScript code: x f(x)
            \global\pst@C@@rType=4\relax%
          \else
            \ifx#1+\relax%			algebraic algebraic: x, f(x)
              \global\pst@C@@rType=8\relax%
  	    \else
              \ifx#4;\relax%		polar coordinates
                \global\pst@C@@rType=1\relax%
              \else
                \global\pst@C@@rType=0\relax%
              \fi
            \fi
          \fi
	\fi
      \fi
    \fi
  \fi
  \psDEBUG[pstCheckCoorType]{::\the\pst@C@@rType::}%
  }%
%
%
\def\special@coor#1|#2|#3\@nil{%
  \ifx#3|\relax
    \mixed@coor{#1}{#2}%
  \else
    \special@@coor#1;;\@nil%
  \fi}
%
\def\special@@coor#1{%
  \ifcat#1a\relax%			node names should start with a letter
    \def\ps@next{\node@coor#1}%
  \else
    \ifx#1[\relax%			special node coor: [..]A
      \def\ps@next{\Node@coor[}%
    \else
      \ifx#1>\relax%			PostScript code: x y
        \def\ps@next{\special@@@@coor}%
    \else
      \ifx#1!\relax%			PostScript code: x y
        \def\ps@next{\raw@coor}%
      \else
        \ifx#1*\relax%			PostScript/algebraic code: x f(x)
          \def\ps@next{\alg@coor}%
        \else
          \ifx#1+\relax%		algebraic code: x,f(x)
            \def\ps@next{\algalg@coor}%
	  \else%
            \def\ps@next{\special@@@coor#1}%
          \fi%
	\fi%
      \fi%
    \fi\fi%
  \fi%
  \ps@next%
}
\def\special@@@coor#1;#2;#3\@nil{%
  \ifx#3;\relax
    \polar@coor{#1}{#2}%
  \else
    \cartesian@coor#1,\relax,\@nil
  \fi%
}
\def\special@@@@coor#1#2;#3;#4\@nil{%
  \def\ps@A{A}\def\ps@B{#1}%
  \ifcat\ps@A\ps@B\relax%
    \node@coor#1#2;;\@nil%
  \else%
    \cartesian@coor#1#2,\relax,\@nil
  \fi%
}
\def\mixed@coor#1#2{%
  \begingroup%
% DG/SR modification begin - Oct. 27, 1997 - Patch 6
%\specialcoor@ii#1;;\@nil
%\let\pst@tempa\pst@coor
%\specialcoor@ii#2;;\@nil
    \special@@coor#1;;\@nil%
    \let\pst@tempa\pst@coor%
    \special@@coor#2;;\@nil%
% DG/SR modification end
    \xdef\pst@tempg{\pst@tempa pop \pst@coor exch pop }%
  \endgroup%
  \let\pst@coor\pst@tempg%
}
%
\def\polar@coor#1#2{%
%  \pssetlength\pst@dimg{#1}%
  \pssetlength\pst@dimb{#1}%	hv 2007-10-16  g is already used in get@@angle
  \pst@@getangle{#2}%
%  \edef\pst@coor{\pst@number\pst@dimg \pst@angle \tx@PtoC}%  dito
  \edef\pst@coor{\pst@number\pst@dimb \pst@angle \tx@PtoC }%
}
%
\def\raw@coor{\@ifnextchar !\raw@@coor\raw@@@coor}
\def\raw@@coor!#1;#2\@nil{%		PostScript code without using \tx@ScreenCoor 
  \edef\pst@coor{#1 }}
\def\raw@@@coor#1;#2\@nil{%		PostScript code 
  \edef\pst@coor{ #1 \tx@ScreenCoor }}
%
\def\alg@coor{\@ifnextchar*{\alg@@coor}{\alg@@@@coor}}
\def\alg@@coor*#1;#2\@nil{\expandafter\alg@@@coor#1\@nil}
\def\alg@@@coor#1 #2\@nil{%			algebraic PostScript code 
%\typeout{Nummer1: #1}%
%\typeout{Nummer2: #2}%
  \edef\pst@coor{%
    /Func (#1) AlgParser cvx def    
    /y #2 def
    y Func exch \tx@ScreenCoor }}
%
\def\alg@@@@coor#1;#2\@nil{\expandafter\alg@@@@@coor#1\@nil}
\def\alg@@@@@coor#1 #2\@nil{%			algebraic PostScript code 
  \edef\pst@coor{%
    /x #1 def
    /Func (#2) AlgParser cvx def 
    x Func \tx@ScreenCoor }}
%
\define@boolkey[psset]{}[Pst@]{exchange}[true]{}
\psset{exchange=false}
%
\def\algalg@coor#1;#2\@nil{\expandafter\algalg@@@coor#1\@nil}
\def\algalg@@@coor#1,#2\@nil{%			algebraic algebraic code 
  \edef\pst@coor{%
    /x (#1) AlgParser cvx def    
    /Func (#2) AlgParser cvx def    
    x Func \tx@ScreenCoor  }}
%
\def\node@coor#1\@nil{%
  \@pstrickserr{You must load `pst-node.tex' to use node coordinates.}\@ehps
  \def\pst@coor{0 0 }%
}
\def\Node@coor{\node@coor}
%
\def\special@angle#1#2)#3\@nil{%
  \ifx !#1\relax
    \edef\pst@angle{#2\space \pst@angleunit}%
  \else\ifx(#1\relax
    \pst@@getcoor{#2}%
    \edef\pst@angle{\pst@coor exch \tx@Atan}%
  \else
    \pst@checknum{#1#2}\pst@angle
    \edef\pst@angle{\pst@angle \pst@angleunit}%
  \fi\fi}
%
\def\special@length#1#2\@nil#3{%
  \psDEBUG[special@length]{ #1|#2|#3 }%
  \ifx !#1\relax
    \edef\pst@SpecialLength{ #2 \pst@number\psunit mul }%
    \Pst@SpecialLengthtrue%
    \psDEBUG[special@length]{ Special length: \pst@SpecialLength}%
  \else
    \let\@psunit\psunit
    \afterassignment\pstunit@off
    #3 #1#2\@psunit%
    \Pst@SpecialLengthfalse%
  \psDEBUG[special@length]{ Normal length: \the#3 }%
  \fi}
%
\def\Cartesian{%
  \def\cartesian@coor##1,##2,##3\@nil{%
    \pssetxlength\pst@dimg{##1}%
    \pssetylength\pst@dimh{##2}%
    \edef\pst@coor{\pst@number\pst@dimg \pst@number\pst@dimh}%
  }%
  \@ifnextchar({\Cartesian@}{}%
}
\def\Cartesian@(#1,#2){%
  \pssetxlength\psxunit{#1}%
  \pssetylength\psyunit{#2}%
  \ignorespaces%
}
\def\Polar{%
  \def\psput@cartesian{\psput@special}%
  \def\cartesian@coor##1,##2,##3\@nil{\polar@coor{##1}{##2}}%
}%
\define@key[psset]{pstricks}{origin}[]{%
  \pst@@getcoor{#1}%
  \edef\psk@origin{\pst@coor T }}
\def\psk@origin{}
%
\define@boolkey[psset]{pstricks}[Pst@]{algebraic}[true]{}
\psset%[pstricks]
{algebraic=false}
%
\define@boolkey[psset]{pstricks}[]{swapaxes}[true]{%			\if@pst
  \@nameuse{@pst#1}%
  \if@pst\def\psk@swapaxes{-90 rotate -1 1 scale }%
  \else\def\psk@swapaxes{}%
  \fi}
\psset[pstricks]{swapaxes=false}
%
\define@boolkey[psset]{pstricks}[]{showpoints}[true]{}
\psset[pstricks]{showpoints=false}
%
\let\pst@setrepeatarrowsflag\relax
%
\define@key[psset]{pstricks}{border}[0pt]{\pst@getlength{#1}\psk@border \pst@setrepeatarrowsflag}
\psset[pstricks]{border=0pt}
\define@key[psset]{pstricks}{bordercolor}[white]{\pst@getcolor{#1}\psbordercolor}
\psset[pstricks]{bordercolor=white}
\define@boolkey[psset]{pstricks}[ps]{doubleline}[true]{\pst@setrepeatarrowsflag}
\psset[pstricks]{doubleline=false}
\define@key[psset]{pstricks}{doublesep}[1.25\pslinewidth]{\def\psdoublesep{#1}}
\psset[pstricks]{doublesep=1.25\pslinewidth}
\define@key[psset]{pstricks}{doublecolor}[white]{\pst@getcolor{#1}\psdoublecolor}
\psset[pstricks]{doublecolor=white}
%
\define@boolkey[psset]{pstricks}[ps]{shadow}[true]{\pst@setrepeatarrowsflag}
\psset[pstricks]{shadow=false}
\define@key[psset]{pstricks}{shadowsize}[3pt]{\pst@getlength{#1}\psk@shadowsize}
\psset[pstricks]{shadowsize=3pt}
\define@key[psset]{pstricks}{shadowangle}[-45]{\pst@getangle{#1}\psk@shadowangle}
\psset[pstricks]{shadowangle=-45}
\define@key[psset]{pstricks}{shadowcolor}[darkgrey]{\pst@getcolor{#1}\psshadowcolor}
\psset[pstricks]{shadowcolor=darkgray}
%
\def\pst@repeatarrowsflag{\z@}
\def\pst@setrepeatarrowsflag{%
  \edef\pst@repeatarrowsflag{%
    \ifdim\psk@border\p@>\z@ 1\else\ifpsdoubleline 1\else
      \ifpsshadow 1\else \z@\fi\fi\fi}}
%
\def\psls@none{}
\def\psls@solid{ \psk@linejoin\space setlinejoin \psk@linecap\space setlinecap stroke }
\def\psls@coloreddashed{ \psls@solid grestore gsave \pst@usecolor\psdashcolor \tx@setlinejoin \psls@dashed }
%
\newdimen\pslinewidth
\define@key[psset]{pstricks}{linewidth}[0.8pt]{\pssetlength\pslinewidth{#1}}
\psset[pstricks]{linewidth=.8pt}
\define@key[psset]{pstricks}{linecolor}[black]{\pst@getcolor{#1}\pslinecolor}
\psset[pstricks]{linecolor=black}
\define@key[psset]{pstricks}{kitecolor}[red]{\pst@getcolor{#1}\ps@kitecolor}
\define@key[psset]{pstricks}{dartcolor}[blue]{\pst@getcolor{#1}\ps@dartcolor}
\psset[pstricks]{kitecolor,dartcolor}
%
\newif\ifPst@coloreddashed
\define@key[psset]{pstricks}{dashcolor}[white]{%
  \ifx\relax#1\relax\Pst@coloreddashedfalse%
  \else\Pst@coloreddashedtrue\pst@getcolor{#1}\psdashcolor
  \fi}
\psset{dashcolor=\relax}
%\define@key[psset]{pstricks}{linecap}[0]{\pst@getint{#1}\psk@linecap}%	hv 2007-12-01
%\psset[pstricks]{linecap=0}  >>>>>>>>>>>>> siehe unten
\define@key[psset]{pstricks}{linejoin}[0]{\pst@getint{#1}\psk@linejoin}%	hv 2007-10-13
\psset[pstricks]{linejoin=0}
\def\tx@setlinejoin{\psk@linejoin\space setlinejoin }%	hv 2007-10-13
%
\def\pst@missing{%
  \z@
  \@pstrickserr{Missing number or dimension. 0 substituted}\@ehpa}
%
%%------------------- begin patch 15 HV 2004-05-15 -------------
\def\pst@empty{\z@}

\define@key[psset]{pstricks}{dash}[5pt 3pt 0pt 0pt]{%	defined in pstricks.tex
  \pst@expandafter\psset@@dash{#1}\@nil}% Error handling for empty argument.
\define@key[psset]{pstricks}{maxdashes}[11]{\def\psk@maxdashes{#1}}
\psset[pstricks]{maxdashes=11}
%
\def\psset@@dash#1\@nil{%
 \def\psk@dash{}%
 \pst@cntm0
 \def\next##1 ##2\relax{%
   \expandafter\ifnum\psk@maxdashes>\pst@cntm\relax  % 04-08-07
     \edef\@tempa{##1}%
     \ifx\@tempa\@empty\else% gobble leading spaces
       \pssetlength\pst@dimc{##1}%
       \advance\pst@cntm by 1
       \edef\psk@dash{\psk@dash\space\pst@number\pst@dimc}%
     \fi%
     \edef\@tempa{##2}%
     \ifx\@tempa\@empty\else% detect end
       \ifx\@tempa\space\else% gobble trailing spaces
         \next##2\relax%
     \fi\fi%
   \else% 04-08-07
     \@pstrickserr{Number of dashes > \psk@maxdashes. Increasing 
        'maxdashes' might work.}\@ehpa% 04-08-07
   \fi% 04-08-07
 }%
 \expandafter\next#1 \relax}
\psset[pstricks]{dash=5pt 3pt 0pt 0pt}% black white black white 
%%------------------- end patch 15 HV 2004-05-15 -------------
\define@boolkey[psset]{pstricks}[ps]{dashadjust}[true]{}
\psset[pstricks]{dashadjust}
\def\tx@DashLine{DashLine }
%
\def\psls@dashed{
  \ifPst@coloreddashed \psls@solid grestore gsave \pst@usecolor\psdashcolor \tx@setlinejoin \fi
  \psk@linecap\space setlinecap 
  \ifpsdashadjust
    [ \psk@dash ] \pst@linetype\space \tx@DashLine
  \else
    [ \psk@dash ] 0 setdash stroke
  \fi}
%% End patch TN; Date (YY-MM-DD): 04-07-17; 2nd part
%
\define@key[psset]{pstricks}{dotsep}[3pt]{\pst@getlength{#1}\psk@dotsep}
\psset[pstricks]{dotsep=3pt}
\def\tx@DotLine{DotLine }
\def\psls@dotted{
  \ifpsdashadjust
    \psk@dotsep \pst@linetype\space \tx@DotLine
  \else
    [ 0 \psk@dotsep CLW add ] 0 setdash 1 setlinecap stroke
  \fi
}
%
\define@key[psset]{pstricks}{linestyle}[solid]{%
  \@ifundefined{psls@#1}%
    {\@pstrickserr{Line style `#1' not defined}\@eha}%
    {\def\pslinestyle{#1}}}
\psset[pstricks]{linestyle=solid}
%
\define@key[psset]{pstricks}{linecap}[0]{%
  \def\psk@linecap{0}%
  \ifnum#1>-1
    \ifnum#1<3
      \pst@getint{#1}\psk@linecap%
  \fi\fi}
\psset{linecap=0}
%------------------------- Transparency modes ----------------------------
\pst@def{setTransparency}< \psk@opacityalpha .setopacityalpha >
\pst@def{setStrokeTransparency}< \psk@strokeopacityalpha .setopacityalpha >
\pst@def{setBlendmode}<
    \ifcase\psk@blendmode
      /Normal \or
      /Compatible \or
      /Screen \or
      /Multiply \or
      /HardLight \or
      /Darken \or
      /Ligten \or
      /Difference
    \else
      /Normal 
    \fi
    .setblendmode \psk@shapealpha .setshapealpha >
%
%--------------------------------- hv 2007-09-09 begin ---------------------
% transparency needs a run through latex -> dvips -> ps2pdf14(!) 
%
\def\e@fill@inverse{oefill}
\define@key[psset]{pstricks}{fillcolor}[white]{%
  \ifx\psk@fillstylename\e@fill@inverse
    \pst@getcolor{#1}\psk@oefillcolor
    \pst@getcolor{white}\psfillcolor
  \else \pst@getcolor{white}\psk@oefillcolor
        \pst@getcolor{#1}\psfillcolor
  \fi}

\psset[pstricks]{fillcolor=white}
\define@key[psset]{pstricks}{strokeopacity}[1]{\pst@checknum{#1}\psk@strokeopacityalpha }% for lines
\psset[pstricks]{strokeopacity=1}
\define@key[psset]{pstricks}{opacity}[1]{\pst@checknum{#1}\psk@opacityalpha }% for filled areas 
\psset[pstricks]{opacity=1}
\define@key[psset]{pstricks}{shapealpha}[0.6]{\pst@checknum{#1}\psk@shapealpha }
\psset[pstricks]{shapealpha=0.6}
\define@key[psset]{pstricks}{blendmode}[0]{\pst@getint{#1}\psk@blendmode }% must be one of 
% /Normal     0
% /Compatible 1
% /Screen     2
% /Multiply   3
% /HardLight  4
\psset[pstricks]{blendmode=0}
\define@key[psset]{pstricks}{fsAngle}[137.50775]{\pst@getangle{#1}\pst@fsAngle }
\define@key[psset]{pstricks}{fsOrigin}[(0,0)]{%
  \pst@@getcoor{#1}\edef\pst@fsOrigin{\pst@coor T }}
\psset[pstricks]{fsOrigin={0,0},fsAngle=137.50775}
%
\def\tx@LineFill{LineFill }
\def\tx@DotFill{DotFill }
\def\tx@PenroseFill{PenroseFill }
\def\tx@PenroseFillA{PenroseFillA }
\def\tx@TruchetFill{TruchetFill }
%
\def\psfs@none{}
\def\psfs@solid{\pst@fill{\pst@usecolor\psfillcolor \tx@setTransparency fill }}
\def\psfs@eofill{\pst@fill{\pst@usecolor\psfillcolor \tx@setTransparency eofill}}
\def\psfs@oefill{\pst@fill{\pst@usecolor\psk@oefillcolor  \tx@setTransparency fill } \psfs@eofill }
\def\psfs@shape{\pst@fill{\pst@usecolor\psfillcolor \tx@setBlendmode fill }}
\def\psfs@spiral{\pst@fill{\pst@fsOrigin \pst@usecolor\psfillcolor clip newpath
    0 .1 500 { dup dup sqrt 4 div 0 360 arc fill \pst@fsAngle rotate } for }}
%
\define@key[psset]{pstricks}{hatchwidth}[0.8pt]{\pst@getlength{#1}\psk@hatchwidth}
\psset[pstricks]{hatchwidth=.8pt}
\define@key[psset]{pstricks}{hatchsep}[4pt]{\pst@getlength{#1}\psk@hatchsep}
\psset[pstricks]{hatchsep=4pt}
\define@key[psset]{pstricks}{hatchcolor}[black]{\pst@getcolor{#1}\pshatchcolor}
\psset[pstricks]{hatchcolor=black}
\define@key[psset]{pstricks}{hatchangle}[45]{\pst@getangle{#1}\psk@hatchangle}
\psset[pstricks]{hatchangle=45}
\define@key[psset]{pstricks}{hatchsepinc}[0pt]{\pst@getlength{#1}\psk@hatchsepinc}
\define@key[psset]{pstricks}{hatchwidthinc}[0pt]{\pst@getlength{#1}\psk@hatchwidthinc}
\psset[pstricks]{hatchwidthinc=0pt,hatchsepinc=0pt}
%
\def\pst@linefill#1{
  /clipType { \ifx\relax#1\relax clip \else#1\fi} def 
  \psk@hatchangle rotate
  \psk@hatchwidth SLW
  \pst@usecolor\pshatchcolor
  \psk@hatchsep 
  \psk@hatchsepinc
  \psk@hatchwidthinc
  \tx@LineFill }
%
\def\psfs@vlines{\pst@fill{\pst@linefill{}}}
\def\psfs@eovlines{\pst@fill{\pst@linefill{eoclip}}}
\@namedef{psfs@vlines*}{\psfs@solid \psfs@vlines}
\@namedef{psfs@eovlines*}{\psfs@eofill \psfs@eovlines}
\def\psfs@hlines{\pst@fill{90 rotate \pst@linefill{}}}
\def\psfs@eohlines{\pst@fill{90 rotate \pst@linefill{eoclip}}}
\@namedef{psfs@hlines*}{\psfs@solid \psfs@hlines}
\@namedef{psfs@eohlines*}{\psfs@eofill \psfs@eohlines}
\def\psfs@crosshatch{\psfs@vlines \psfs@hlines}
\@namedef{psfs@crosshatch*}{\psfs@solid \psfs@vlines \psfs@hlines}
\@namedef{psfs@eocrosshatch*}{\psfs@eofill \psfs@eovlines \psfs@eohlines}
%
\define@key[psset]{pstricks}{psscale}[1]{%
  \def\psk@@psscale{#1}%   for use with \psscalebox
  \pst@checknum{#1}\psk@psscale}
\psset[pstricks]{psscale=1}
%
\def\pst@dotFill[#1]{%
  /clipType { \ifx\relax#1\relax clip \else #1 \fi } def 
  gsave
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
%  /DotLineColor { \pst@usecolor\pslinecolor } def
  \psk@hatchsep 
  \psk@hatchwidth
  \tx@DotFill }

\def\psfs@dots{\pst@fill{ /SolidDot false def \pst@dotFill[] }}
\def\psfs@eodots{\pst@fill{ /SolidDot false def \pst@dotFill[eoclip] }}
\@namedef{psfs@dots*}{\pst@fill{ /SolidDot true def \pst@dotFill[] }}
\@namedef{psfs@eodots*}{\pst@fill{ /SolidDot true def \pst@dotFill[eoclip] }}
%
\def\pst@penroseFill{%
%  gsave					% restore in PenroseFill
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
  \psk@psscale 
  \tx@PenroseFill }
\def\psfs@penrose{\pst@fill\pst@penroseFill}
\@namedef{psfs@penrose*}{\psfs@solid \psfs@penrose}
%
\def\pst@penroseFillA{%
%  gsave					% restore in PenroseFillA
  \pst@number\pslinewidth SLW
%  \pst@usecolor\pshatchcolor
%  on stack: scaling factor, border color, kite color, dart color
%  dup dup scale
%  /border_colour ED % 
%  /kite_colour ED %
%  /dart_colour 
  { \pst@usecolor\ps@dartcolor }
  { \pst@usecolor\ps@kitecolor }
  { \pst@usecolor\pshatchcolor }
  \psk@psscale 
  \tx@PenroseFillA }
\def\psfs@penroseA{\pst@fill\pst@penroseFillA}
\@namedef{psfs@penroseA*}{\psfs@solid \psfs@penroseA}
%
\def\pst@truchetFill{%
  gsave					% restore in PenroseFill
  \pst@number\pslinewidth SLW
  \pst@usecolor\pshatchcolor
  \psk@psscale 
  \tx@TruchetFill }
\def\psfs@truchet{ \pst@fill\pst@truchetFill }
\@namedef{psfs@truchet*}{\psfs@solid \psfs@truchet}
%
\define@key[psset]{pstricks}{fillstyle}[none]{%
  \def\psk@fillstylename{#1}%  needed for inverse eofill
  \edef\pst@tempg{#1}\def\pst@temph{none}%
  \ifx\pst@tempg\pst@temph
     \let\psk@fillstyle\relax
  \else
    \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{\expandafter\noexpand\csname psfs@#1\endcsname}}%
  \fi%
}
\define@key[psset]{pstricks}{addfillstyle}[]{%
  \@ifundefined{psfs@#1}%
    {\@pstrickserr{Undefined fill style: `#1'}\@eha}%
    {\edef\psk@fillstyle{%
      \expandafter\noexpand\psk@fillstyle
      \expandafter\noexpand\csname psfs@#1\endcsname}%
    }}
\psset[pstricks]{fillstyle=none}
%
%--------------------------- continous linewidth -------------------
\newdimen\psk@startLW
\newdimen\psk@endLW
\define@key[psset]{pstricks}{startLW}[\pslinewidth]{\pssetlength{\psk@startLW}{#1}}%
\define@key[psset]{pstricks}{endLW}[\pslinewidth]{\pssetlength{\psk@endLW}{#1}}%
\define@key[psset]{pstricks}{startWL}[380]{\pst@getint{#1}\psk@startWL}%
\define@key[psset]{pstricks}{endWL}[780]{\pst@getint{#1}\psk@endWL}%
\define@boolkey[psset]{pstricks}[Pst@]{variableLW}[true]{}
\define@boolkey[psset]{pstricks}[Pst@]{variableColor}[true]{}
\define@key[psset]{pstricks}{setflat}[0.1]{\pst@checknum{#1}\psk@setflat}%
\psset[pstricks]{startLW=\pslinewidth,endLW=\pslinewidth,variableColor=false,
  variableLW=false,startWL=380,endWL=780,setflat=0.1}
%
\def\pst@flattenpath{
  /Coors [] def         % the array of all points
  /lambda \psk@startWL\space def
  %
  /add2Values { Coors aload length 2 add array astore /Coors exch def } def
  /add6Values { Coors aload length 6 add array astore /Coors exch def } def
%
  \psk@setflat\space setflat   % the value for the line snippets
  flattenpath            % flatten the existing path into line segments
%
  { add2Values }         % what to do with moveto
  { add2Values }         % what to do with lineto 
  { add6Values }         % what to do with curveto (not needed here) 
  { }                    % what to do with closepath
  pathforall             % do it for the existing path
%
  \pst@number\psk@startLW setlinewidth
  \tx@setlinejoin
  \psk@linecap\space setlinecap
  Coors aload length 2 sub 2 div cvi /N0 exch def % set number of points
  /NN 0 def
  /N N0 def
  { N 3 gt { N 3 sub /N ED }{ N 1 sub /N ED } ifelse 
    NN 1 add /NN ED
    N 0 eq { exit } if
  } loop
  /dLW \pst@number\psk@endLW \pst@number\psk@startLW sub NN div def          % the step for the linewidth
  \ifPst@variableColor
    /dColor \psk@endWL\space \psk@startWL\space sub NN div def
    lambda dColor add dup /lambda ED 
    tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
  \else
    \pst@usecolor\pslinecolor
  \fi
  moveto                 % move to the first one
  /N N0 def
  {
    N 3 gt {  
%    CP 6 2 roll
    \psk@curvature\space /c ED /b ED /a ED
    /ArrowA {} def
    /ArrowB {} def
    BOC NC EOC %    curveto 
    N 3 sub /N ED }{ lineto N 1 sub /N ED } ifelse
    currentlinewidth dLW add setlinewidth % increase line width
    \ifPst@variableColor
      lambda dColor add dup /lambda ED 
      tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
    \else
      \pst@usecolor\pslinecolor
    \fi
    CP /Y ED /X ED       % put coors of current point on the stack
%    0.4 .setopacityalpha 
    stroke               % draw the line segment
    N 0 eq { exit }{ X Y moveto } ifelse
  } loop
%  N {                    % repeat for the other N coords
%    lineto               % line to next point
%    currentlinewidth dLW add setlinewidth % increase line width
%    lambda dColor add dup /lambda ED 
%    tx@addDict begin wavelengthToRGB Red Green Blue end setrgbcolor
%    currentpoint         % put coors of current point on the stack
%    0.4 .setopacityalpha 
%    stroke               % draw the line segment
%    moveto
%  } repeat
}

%
%--------------------------- A R R O W S ---------------------------
%
\def\psk@arrowA{}
\def\psk@arrowB{}
\def\pst@arrowtable{,-,<->,<<->>,>-<,>>-<<,(-),[-],)-(,]-[,|>-<|,<D-D>,D>-<D,<D<D-D>D>} % hv --1.16
\edef\pst@arrowtable{\pst@arrowtable,|<*->|*,|<->|}
\begingroup
  \catcode`\<=13
  \catcode`\>=13
  \catcode`\|=13
  \gdef\pst@activearrows{\def<{\string<}\def>{\string>}\def|{\string|}}
\endgroup
\def\tx@BeginArrow{BeginArrow }
\def\tx@EndArrow{EndArrow }
%
\def\tx@Arrow{ \tx@setStrokeTransparency Arrow }% hv 2008-01-13
\def\tx@ArrowD{ \tx@setStrokeTransparency ArrowD }% hv 2008-01-13
%
\@namedef{psas@<|}{ 
    \psk@tbarsize\space \tx@Tbar
    0 CLW 2 div T
    newpath
    true 
    \psk@arrowinset 
    \psk@arrowlength 
    \psk@arrowsize 
    \tx@Arrow 
}
% ]-[ arrow
\def\tx@BracketOut{BracketOut }
\@namedef{psas@[}{%
  /BracketOut {%
  CLW mul add dup CLW sub 2 div
%/x ED mul CLW add
  /x ED mul neg
  /y ED
  /z CLW 2 div def
  x neg y moveto
  x neg CLW 2 div L x CLW 2 div L x y L stroke 0 CLW moveto } def
  \psk@bracketlength\space \psk@tbarsize\space \tx@BracketOut
}
% )-( arrow
\def\tx@RoundBracketOut{ \tx@setStrokeTransparency RoundBracketOut }% hv 2008-01-13
\@namedef{psas@(}{%
  /RoundBracketOut {%
    CLW mul add dup 2 div
%/x ED mul
    /x ED mul neg
    /y ED
    /mtrx CM def
    0 CLW
    2 div T x y mul 0 ne { x y scale } if
    1 1 moveto
    .85 .5 .35 0 0 0 curveto
    -.35 0 -.85 .5 -1 1 curveto
    mtrx setmatrix stroke 0 CLW moveto } def
  \psk@rbracketlength\space \psk@tbarsize\space \tx@RoundBracketOut
}
% end of new definitions of the missing arrows ---- hv 1.12
\@namedef{psas@>}{ false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow }
\@namedef{psas@>>}{%
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  0 h T gsave newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP grestore CP newpath moveto 2 copy 
  CLW \pst@arrowscale\space div SLW % set the original line width  
  L stroke moveto
}
\@namedef{psas@<}{true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow}
\@namedef{psas@<<}{
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
  CP newpath moveto 0 a neg 
  gsave
  CLW \pst@arrowscale\space div SLW % set the original line width  
  L stroke 
  grestore
  0 h neg T
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@D>}{ false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD }%	hv 20071211
\@namedef{psas@D>D>}{ %	hv 20071211
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  0 h Inset sub T gsave newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  CP grestore moveto 
}
\@namedef{psas@<D}{ %	hv 20071211
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
}
\@namedef{psas@<D<D}{ %	hv 20071211
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
  CP newpath moveto 0 a neg L stroke 0 h neg T
  true \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@ArrowD
}
\define@key[psset]{pstricks}{tbarsize}[2pt 5]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@tbarsize{\pst@number\pst@dimg \pst@tempg}}
\psset[pstricks]{tbarsize=2pt 5}
%
\def\tx@Tbar{Tbar }
\@namedef{psas@|}{\psk@tbarsize \tx@Tbar}
\@namedef{psas@|*}{0 CLW -2 div T \psk@tbarsize \tx@Tbar}
\@namedef{psas@>|}{%
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
\@namedef{psas@>|*}{%
  0 CLW -2 div T
  \psk@tbarsize \tx@Tbar
  0 CLW 2 div T
  newpath
  false \psk@arrowinset \psk@arrowlength \psk@arrowsize \tx@Arrow
}
%
\define@key[psset]{pstricks}{bracketlength}[0.15]{\pst@checknum{#1}\psk@bracketlength}
\psset[pstricks]{bracketlength=.15}
\def\tx@Bracket{Bracket }
\@namedef{psas@]}{\psk@bracketlength \psk@tbarsize \tx@Bracket}
\define@key[psset]{pstricks}{rbracketlength}[0.15]{\pst@checknum{#1}\psk@rbracketlength}
\psset[pstricks]{rbracketlength=.15}
\def\tx@RoundBracket{RoundBracket }
\@namedef{psas@)}{\psk@rbracketlength \psk@tbarsize \tx@RoundBracket}
%
\def\psas@c{1 \psas@@c}
\def\psas@cc{0 CLW 2 div T 1 \psas@@c}
\def\psas@C{2 \psas@@c}
\def\psas@@c{%
  setlinecap
  0 0 moveto
  0 0.1 L % changed value from 0.5 to 0.1
  stroke
  0 0 moveto }
%
\def\psas@{}
%
\define@key[psset]{pstricks}{arrowLW}{\pst@getlength{#1}\psk@arrowLW}
\psset[pstricks]{arrowLW=0}
% arrowLW as LineWidth for the circled line ends
%
\def\psas@o{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {\pst@usecolor\psfillcolor true} false \psk@dotsize \tx@EndDot }
\def\psas@oo{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {\pst@usecolor\psfillcolor true} true \psk@dotsize \tx@EndDot }
\@namedef{psas@*}{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {false} false \psk@dotsize \tx@EndDot }
\@namedef{psas@**}{\psk@arrowLW\space dup 0 eq { pop }{ SLW } ifelse
  {false} true \psk@dotsize \tx@EndDot }
%
\define@key[psset]{pstricks}{arrows}[-]{%
  \begingroup
    \pst@activearrows
    \xdef\pst@tempg{#1}%
  \endgroup
  \expandafter\psset@@arrows\pst@tempg\@empty-\@empty\@nil
  \if@pst\else\@pstrickserr{Bad arrows specification: #1}\@ehpa\fi}
\def\psset@@arrows#1-#2\@empty#3\@nil{%
  \@psttrue
  \def\ps@next##1,#1-##2,##3\@nil{\def\pst@tempg{##2}}%
  \expandafter\ps@next\pst@arrowtable,#1-#1,\@nil
  \@ifundefined{psas@\pst@tempg}{\@pstfalse\def\psk@arrowA{}}{\let\psk@arrowA\pst@tempg}%
  \@ifundefined{psas@#2}{\@pstfalse\def\psk@arrowB{}}{\def\psk@arrowB{#2}}}
\psset[pstricks]{arrows=-}
%
\define@key[psset]{pstricks}{arrowscale}[1]{%                                   hv --1.12
  \pst@getscale{#1}\psk@arrowscale
  \pst@@arrowscale@i#1 \@nil}%           hv --1.12
\def\pst@@arrowscale@i#1 #2\@nil{\edef\pst@arrowscale{#1}}% hv --1.12
\psset[pstricks]{arrowscale=1}
%
\define@key[psset]{pstricks}{arrowsize}[1.5pt 2]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil
  \edef\psk@arrowsize{\pst@number\pst@dimg \pst@tempg}%
}
\psset[pstricks]{arrowsize=1.5pt 2}
\define@key[psset]{pstricks}{arrowlength}[1.4]{\pst@checknum{#1}\psk@arrowlength}
\psset[pstricks]{arrowlength=1.4}
\define@key[psset]{pstricks}{arrowinset}[0.4]{\pst@checknum{#1}\psk@arrowinset}%
\psset[pstricks]{arrowinset=0.4}
%
\def\tx@SD{ \tx@setTransparency SD }
\def\tx@EndDot{EndDot }
%
\def\pst@par{}
\def\addto@par#1{%
  \ifx\pst@par\@empty
    \def\pst@par{#1}%
  \else
    \expandafter\def\expandafter\pst@par\expandafter{\pst@par,#1}%
  \fi%
}
\def\addbefore@par#1{%
  \ifx\pst@par\@empty
    \def\pst@par{#1}%
  \else
    \toks@{#1}%
    \pst@toks\expandafter{\pst@par}%
    \edef\pst@par{\the\toks@,\the\pst@toks}%
  \fi%
}
\def\use@par{%
  \ifx\pst@par\@empty\else%
    \expandafter\@psset\pst@par,\@nil%
    \def\pst@par{}%
  \fi}
\def\use@keep@par{%			same as \use@par, but keeps the values
  \ifx\pst@par\@empty\else
    \expandafter\@psset\pst@par,\@nil
%    \def\pst@par{}%
  \fi}
%
\def\pst@object#1{%
  \def\pst@par{}%
  \pst@ifstar{%
    \@ifnextchar[{\pst@@object{#1}}{\@nameuse{#1@i}}}%
}
\def\pst@@object#1[#2]{%
  \def\pst@par{#2}%
  \@ifnextchar+{\@nameuse{#1@i}}{\@nameuse{#1@i}}%
}
\def\newpsobject#1#2#3{%
\@ifundefined{#2@i}%
{\@pstrickserr{Graphics object `#2' not defined}\@eha}{%
\@namedef{#1}{\pst@object{#1}}%
\@namedef{#1@i}{\addbefore@par{#3}\@nameuse{#2@i}}}%
\ignorespaces}
%
\def\pst@getarrows#1{\@ifnextchar({#1}{\pst@@getarrows{#1}}}
% ------------------------- hv 1.10 beg ------------------------
%\def\pst@@getarrows#1#2{\addto@par{arrows=#2}#1}
\def\pst@@getarrows#1#2{%
  \def\pst@tempa{#2}% prevent empty arrow arguments, to allow \psline{}(...)(...)
  \ifx\pst@tempa\@empty\addto@par{arrows=-}\else\addto@par{arrows=#2}\fi#1}
% ------------------------- hv 1.10 end ------------------------
%
\def\begin@ClosedObj{%
  \leavevmode%
  \pst@killglue%
  \begingroup%
  \use@par%
  \solid@star%
  \ifpsdoubleline\pst@setdoublesep\fi%
  \pst@addarrowdef% DG addition
  \init@pscode}
%
\def\end@ClosedObj{%
  \ifpsshadow \pst@closedshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifshowpoints
% DG modification begin - Mar. 4, 1995
%\addto@pscode{Points aload length 2 div cvi /N ED \psdots@iii}%
  \pst@OpenShowPoints
% DG modification end
  \fi
  \use@pscode
  \endgroup
  \ignorespaces%
}
\def\begin@OpenObj{%
  \begin@ClosedObj%
  \let\pst@linetype\pst@arrowtype%
  \pst@addarrowdef%
}
\def\begin@AltOpenObj{%
  \begin@ClosedObj
  \def\pst@repeatarrowsflag{\z@}%
  \def\pst@linetype{0}}
%
\def\end@OpenObj{%
  \ifpsshadow \pst@openshadow \fi
  \ifdim\psk@border\p@>\z@ \pst@addborder \fi
  \psk@fillstyle
  \pst@stroke
  \ifpsdoubleline \pst@doublestroke \fi
  \ifnum\pst@repeatarrowsflag>\z@ \pst@repeatarrows \fi
  \ifshowpoints \pst@OpenShowPoints \fi
  \use@pscode
  \endgroup
  \ignorespaces}
%
\def\begin@SpecialObj{%
  \leavevmode
  \pst@killglue
  \begingroup
  \use@par
  \init@pscode}
%
\def\end@SpecialObj{%
  \use@pscode
  \endgroup
  \ignorespaces}
%
\def\pst@code{}%
\def\init@pscode{%
  \addto@pscode{%
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor}%
}
\def\addto@pscode#1{\xdef\pst@code{\pst@code#1\space}}
\def\use@pscode{%
  \pstverb{
    \pst@dict
    \tx@STP
    \pst@newpath
    \psk@origin
    \psk@swapaxes
    \pst@code
    end
  }%
  \gdef\pst@code{}%
}
\def\use@psCode{%
  \pstVerb{
    \pst@dict
    \tx@STP
    \pst@newpath
    \psk@origin
    \psk@swapaxes
    \pst@code
    end
  }%
  \gdef\pst@code{}%
}
\def\pst@newpath{newpath }
%
\def\pst@@killglue{\unskip\ifdim\lastskip>\z@\expandafter\pst@@killglue\fi}
\def\KillGlue{\let\pst@killglue\pst@@killglue}
\def\DontKillGlue{\let\pst@killglue\relax}
\DontKillGlue
%
\def\solid@star{%
  \if@star
    \pslinewidth=\z@
    \psdoublelinefalse
    \def\pslinestyle{none}%
    \def\psk@fillstyle{\psfs@solid}%
    \let\psfillcolor\pslinecolor
  \fi}
%
\def\pst@setdoublesep{%
\pst@getlength\psdoublesep\psdoublesep
\pslinewidth=2\pslinewidth
\advance\pslinewidth\psdoublesep\p@
\let\pst@setdoublesep\relax}
\def\tx@Shadow{Shadow }
\def\pst@closedshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    gsave fill grestore
    stroke
    grestore
    gsave
    \pst@usecolor\psfillcolor
    gsave fill grestore
    stroke
    grestore}}
%
\def\pst@openshadow{%
  \addto@pscode{%
    gsave
    \psk@shadowsize \psk@shadowangle \tx@PtoC
    \tx@Shadow
    \pst@usecolor\psshadowcolor
    \ifx\psk@fillstyle\relax\else
      gsave fill grestore
    \fi
    stroke}%
  \pst@repeatarrows%
  \addto@pscode{grestore}%
  \ifx\psk@fillstyle\relax\else
    \addto@pscode{%
      gsave
      \pst@usecolor\psfillcolor
      gsave fill grestore
      stroke
      grestore}%
  \fi}
%
\def\pst@addborder{%
  \addto@pscode{%
    gsave
    \psk@border 2 mul
    CLW add SLW
    \pst@usecolor\psbordercolor
    stroke
    grestore}}
%
\def\pst@stroke{%
  \ifx\pslinestyle\@none\else
    \addto@pscode{%
      gsave
      \pst@number\pslinewidth SLW
      \pst@usecolor\pslinecolor
      \tx@setStrokeTransparency % hv 2008-01-13
      \@nameuse{psls@\pslinestyle}
      grestore}%
  \fi}
%
\def\pst@fill#1{\addto@pscode{gsave #1 grestore}}%
%
\def\pst@doublestroke{%
    \addto@pscode{%
      gsave
      \psdoublesep SLW
      \pst@usecolor\psdoublecolor
      stroke
      grestore
}}
%
\def\pst@arrowtype{%
  \ifx\psk@arrowB\@empty 0 \else -2 \fi
  \ifx\psk@arrowA\@empty 0 \else -1 \fi
  add }
%
\def\pst@addarrowdef{%
  \addto@pscode{%
    /ArrowA {
      \ifx\psk@arrowA\@empty
        \pst@oplineto
      \else
        \pst@arrowdef{A}
        moveto
      \fi
    } def
    /ArrowB { \ifx\psk@arrowB\@empty \else \pst@arrowdef{B} \fi } def
}}
%
\def\pst@arrowdef#1{%
  \ifnum\pst@repeatarrowsflag>\z@
    /Arrow#1c [ 6 2 roll ] cvx def Arrow#1c
  \fi
  \tx@BeginArrow 
  \psk@arrowscale
  \@nameuse{psas@\@nameuse{psk@arrow#1}}
  \tx@EndArrow
}
%
\def\pst@repeatarrows{%
  \addto@pscode{%
    gsave
    \ifx\psk@arrowA\@empty\else ArrowAc ArrowA pop pop \fi
    \ifx\psk@arrowB\@empty\else ArrowBc ArrowB pop pop pop pop \fi
    grestore
}}
%
\def\pst@OpenShowPoints{%
  \addto@pscode{%
    gsave
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    newpath
    Points aload length 2 div 2 sub cvi /N ED
    N 0 ge
      { \ifx\psk@arrowA\@empty Dot \else pop pop \fi 
        N { Dot } repeat 
	\ifx\psk@arrowB\@empty Dot \else pop pop \fi }
      { N 2 mul { pop } repeat } ifelse
    grestore
}}
%
\newif\ifPst@custom\Pst@customfalse
\define@boolkey[psset]{pstricks}[Pst@]{noCurrentPoint}[true]{}
\psset[pstricks]{noCurrentPoint=false}
%
%
\def\pscustom{\pst@object{pscustom}}
\long\def\pscustom@i#1{%
  \begin@SpecialObj%
  \solid@star%
  \let\pst@ifcustom\iftrue%
  \Pst@customtrue%
  \let\begin@ClosedObj\begin@CustomObj%
  \let\end@ClosedObj\endgroup%
  \def\begin@OpenObj{\begin@CustomObj\pst@addarrowdef}%
  \let\end@OpenObj\endgroup%
  \let\begin@AltOpenObj\begin@CustomObj%
  \def\begin@SpecialObj{%
    \begingroup%
    \pst@misplaced{special graphics object}%
    \def\addto@pscode####1{}%
    \let\end@SpecialObj\endgroup}%
  \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
  \def\psclip##1{\pst@misplaced\psclip}%
  \def\pst@repeatarrowsflag{\z@}%
  \let\pst@setrepeatarrowsflag\relax%
  \showpointsfalse%
  \def\pst@linetype{\pslinetype}%
  \def\psk@liftpen{\z@}%
%  \psset{liftpen=0}%
  \def\pst@cp{/currentpoint load stopped pop }%
  \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \def\pst@optcp##1##2{\ifnum##1=\z@\def##2{/currentpoint load stopped { 0 0 } if }\fi}%
  \let\caddto@pscode\addto@pscode%
  \def\cuse@par##1{{\use@par##1}}%
  \the\pst@customdefs%
  \setbox\pst@hbox=\hbox{#1}%
  \psk@fillstyle%
  \pst@stroke%
  \end@SpecialObj%
}
%
\def\begin@CustomObj{%
  \begingroup%
  \use@par%
  \addto@pscode{
    \pst@number\pslinewidth SLW
    \pst@usecolor\pslinecolor
  }%
}
\def\pst@oplineto{moveto }
\def\pst@cp{}
\def\pst@optcp#1#2{}
\define@key[psset]{pstricks}{liftpen}[0]{%
  \ifPst@custom%
  \ifcase#1\relax%
    \def\psk@liftpen{\z@}%
    \def\pst@cp{/currentpoint load stopped pop }%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or%
    \def\psk@liftpen{1}%
    \def\pst@cp{}%
    \def\pst@oplineto{/lineto load stopped { moveto } if }%
  \or%
    \def\psk@liftpen{2}%
    \def\pst@cp{}%
    \def\pst@oplineto{moveto }%
  \fi\fi%
}
\psset[pstricks]{liftpen=0}
\def\psk@liftpen{-1}
%
\define@key[psset]{pstricks}{linetype}[2]{%
  \pst@getint{#1}\pslinetype
  \ifnum\pst@cntg<-3
    \@pstrickserr{linetype must be greater than -3}\@ehpa
    \def\pslinetype{2}%
  \fi}
\psset[pstricks]{linetype=2}% otherwise there is a problem when using e.g.
%                     \psaxes[axesstyle=frame,linestyle=dashed]{->}(3,-2)
%
\def\caddto@pscode#1{%
    \@pstrickserr{Command can only be used in \string\pscustom}\@ehpa}
\let\cuse@par\caddto@pscode
%
\def\tx@MSave{%
     /msavematrx
         [ tx@Dict /msavematrx known % does msavematrix exists?
             { msavematrx aload pop } if
             CM % matrix currentmatrix
         ]
     def
%----------------- hv begin 2004-05-07 ------------- patch 15
    msavematrx
%----------------- hv end 2004-05-07 ------------- patch 15
}
\def\tx@MRestore{% a typo in pstricks with msavematrx
     tx@Dict /msavematrx known { length 0 gt } { false } ifelse
         { msavematrx aload pop setmatrix } if
}
%
\newtoks\pst@customdefs
\pst@customdefs{%
  \def\newpath{\addto@pscode{newpath}}%
  \def\reversepath{\addto@pscode{ reversepath }}%                      20131209  hv
  \def\moveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor moveto}}%
  \def\rmoveto(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor rmoveto}}%
  \def\closepath{\addto@pscode{closepath}}%
  \def\gsave{\begingroup\addto@pscode{gsave}}%
  \def\grestore{\endgroup\addto@pscode{grestore}}%
  \def\translate(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor translate}}%
  \def\rotate#1{\pst@@getangle{#1}\addto@pscode{\pst@angle rotate}}%
  \def\scale#1{\pst@getscale{#1}\pst@tempg\addto@pscode{\pst@tempg}}%
  \def\msave{\addto@pscode{\tx@MSave}}%
  \def\mrestore{\addto@pscode{\tx@MRestore}}%
  \def\swapaxes{\addto@pscode{-90 rotate -1 1 scale}}%
  \def\stroke{\def\pst@par{}\pst@object{stroke}}%
  \def\fill{\def\pst@par{}\pst@object{fill}}%
  \def\openshadow{\def\pst@par{}\pst@object{openshadow}}%
  \def\closedshadow{\def\pst@par{}\pst@object{closedshadow}}%
  \def\movepath(#1){\pst@@getcoor{#1}\addto@pscode{\pst@coor \tx@Shadow}}%
  \def\lineto{\pst@onecoor{lineto}}%
  \def\rlineto{\pst@onecoor{rlineto}}%
  \def\curveto{\pst@threecoor{curveto}}%
  \def\rcurveto{\pst@threecoor{rcurveto}}%
  \def\code#1{\addto@pscode{#1}}%
  \def\coor(#1){\pst@@getcoor{#1}\addto@pscode\pst@coor\@ifnextchar({\coor}{}}%
  \def\rcoor{\pst@getcoors{}{}}%
  \def\dim#1{\pssetlength\pst@dimg{#1}\addto@pscode{\pst@number\pst@dimg}}%
  \def\setcolor#1{%
    \@ifundefined{\string\color@#1}{}{\addto@pscode{\pst@usecolor{#1}}}}%  hv 1.14  2005-12-17
  \def\arrows#1{{\psset[pstricks]{arrows=#1}\pst@addarrowdef}}%
  \let\file\pst@rawfile%
} % END \pst@customdefs
%
\def\closedshadow@i{\cuse@par\pst@closedshadow}
\def\openshadow@i{\cuse@par\pst@openshadow}
\def\stroke@i{\cuse@par\pst@stroke}%
\def\fill@i{\cuse@par\psk@fillstyle}%
\def\pst@onecoor#1(#2){%
\pst@@getcoor{#2}%
\addto@pscode{\pst@coor #1}}
\def\pst@threecoor#1(#2)#3(#4)#5(#6){%
  \begingroup
    \pst@getcoor{#2}\pst@tempa
    \pst@getcoor{#4}\pst@tempb
% DG/SR modification begin - Aug.  4, 1999 - Patch 11
%\pst@getcoor{#6}\pst@tembc
    \pst@getcoor{#6}\pst@tempc
% DG/SR modification end
    \addto@pscode{\pst@tempa \pst@tempb \pst@tempc #1}%
  \endgroup}
%
\def\pst@rawfile#1{%
  \begingroup
  \def\do##1{\catcode`##1=12\relax}"
  \dospecials
  \catcode`\%=14
  \pst@@rawfile{#1}%
  \endgroup}
%
\def\pst@@rawfile#1{%
  \immediate\openin1 #1
  \ifeof1
    \@pstrickserr{File `#1' not found}\@ehpa
  \else
    \immediate\read1 to \pst@tempg
    \loop
      \ifeof1 \@pstfalse\else\@psttrue\fi
      \if@pst
      \addto@pscode\pst@tempg
      \immediate\read1 to \pst@tempg
    \repeat
  \fi
  \immediate\closein1\relax}
%
\def\tx@NArray{NArray }
\def\tx@Line{Line }
\def\tx@Arcto{Arcto }
\def\tx@CheckClosed{CheckClosed }
\def\tx@Polygon{Polygon }
\define@key[psset]{pstricks}{gangle}[0]{\pst@getangle{#1}\psk@gangle}
\define@boolkey[psset]{pstricks}[Pst@]{trueAngle}[true]{}
\psset[pstricks]{trueAngle=false,gangle=0}
%
\def\tx@Diamond{Diamond }
\def\psdiamond{\def\pst@par{}\pst@object{psdiamond}}
\def\psdiamond@i(#1){\@ifnextchar({\psdiamond@ii(#1)}{\psdiamond@ii(0,0)(#1)}}
\def\psdiamond@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@getcoor{#2}\pst@tempb
  \addto@pscode{%
    \psline@iii
    pop
    \psk@dimen
    \pst@tempb
    \psk@gangle
    \pst@tempa
    \tx@Diamond
  }%
  \def\pst@linetype{4}%
  \end@ClosedObj}
%
\def\tx@Triangle{Triangle }
\def\pstriangle{\def\pst@par{}\pst@object{pstriangle}}
\def\pstriangle@i(#1){\@ifnextchar({\pstriangle@ii(#1)}{\pstriangle@ii(0,0)(#1)}}
\def\pstriangle@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa%	the center of the baseline
  \pst@getcoor{#2}\pst@tempb%	the height of the triangle
  \addto@pscode{%
    \psline@iii
    pop			    %	no showpoints option
    \psk@dimen		    %	outer/inner/middle
    \pst@tempb
    \psk@gangle		    %	rotating angle
    \pst@tempa
    \tx@Triangle
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj}
%
\def\tx@CCA{CCA }
\def\tx@CCA{CCA }
\def\tx@CC{CC }
\def\tx@IC{IC }
\def\tx@BOC{BOC }
\def\tx@NC{NC }
\def\tx@EOC{EOC }
\def\tx@BAC{BAC }
\def\tx@NAC{NAC }
\def\tx@EAC{EAC }
\def\tx@OpenCurve{OpenCurve }
\def\tx@AltCurve{AltCurve }
\def\tx@ClosedCurve{ClosedCurve }
%
\define@key[psset]{pstricks}{curvature}[1 0.1 0]{%
  \edef\pst@tempg{#1 }%
  \expandafter\psset@@curvature\pst@tempg * * * \@nil}
\def\psset@@curvature#1 #2 #3 #4\@nil{%
  \pst@checknum{#1}\pst@tempg
  \pst@checknum{#2}\pst@temph
  \pst@checknum{#3}\pst@tempi
  \edef\psk@curvature{\pst@tempg \pst@temph \pst@tempi}}
%
\psset[pstricks]{curvature=1 .1 0}
%
\def\pscurve{\pst@object{pscurve}}
\def\pscurve@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\pscurve@ii%
    }%
}
\def\pscurve@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi		% current point
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol OpenSymbolCurve \else \tx@OpenCurve \fi
    \ifPst@variableLW \pst@flattenpath \fi
  }%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj%
}
\def\psecurve{\pst@object{psecurve}}
\def\psecurve@i{\pst@getarrows{\begin@OpenObj\pst@getcoors[\psecurve@ii}}
\def\psecurve@ii{%
  \addto@pscode{
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol AltOpenSymbolCurve \else \tx@AltCurve \fi
  }%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj}
%
\def\psccurve{\pst@object{psccurve}}
\def\psccurve@i{\begin@ClosedObj\pst@getcoors[\psccurve@ii}
\def\psccurve@ii{%
  \addto@pscode{%
    \psk@curvature\space /c ED /b ED /a ED
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol ClosedSymbolCurve \else \tx@ClosedCurve \fi
  }%
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@ClosedObj}
%
\def\pscspline{\pst@object{pscspline}}%  Christoph Bersch
\def\pscspline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\pscspline@ii
  }%
}
\def\tx@Spline{Spline }
\def\pscspline@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi
    \tx@setlinejoin
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol 
      \psls@symbol OpenSymbolSpline
    \else
      \tx@Spline
    \fi
  }%      
  \end@OpenObj
}
%
\define@key[psset]{pstricks}{dotsize}[2pt 2]{%
  \pst@expandafter\pst@getdimnum{#1} 0 {} {}\@nil%
  \edef\psk@@dotsize{\pst@number\pst@dimg}%
  \let\psk@@@dotsize\pst@tempg%
  \edef\psk@dotsize{ /DS \psk@@dotsize \psk@@@dotsize CLW mul add 2 div def }}
\psset[pstricks]{dotsize=2pt 2}
%
\define@key[psset]{pstricks}{dotscale}[1]{%
  \pst@getscale{#1}\psk@dotscale
  \ifx\psk@dotscale\@empty
    \def\psk@xdotscale{1 }%
    \def\psk@ydotscale{1 }%
  \else
    \let\psk@xdotscale\pst@tempg
    \let\psk@ydotscale\pst@temph
  \fi}
%
\def\pst@Getangle#1#2{%
  \pst@getangle{#1}\pst@tempg
  \def\pst@temph{0. }%
  \ifx\pst@tempg\pst@temph\def#2{}\else\edef#2{\pst@tempg\space rotate }\fi}
%
\define@key[psset]{pstricks}{dotangle}[0]{%
  \pst@getangle{#1}\psk@@dotangle
  \ifdim\psk@@dotangle\p@=\z@
    \let\psk@dotangle\@empty
  \else
    \edef\psk@dotangle{\psk@@dotangle rotate }%
  \fi}
\psset[pstricks]{dotangle=0}
%
\def\pst@getdotsize{%
\pst@dimg=\psk@@@dotsize\pslinewidth
\advance\pst@dimg\psk@@dotsize\p@
\pst@dimh=\psk@ydotscale\pst@dimg
\pst@dimg=\psk@xdotscale\pst@dimg
\divide\pst@dimh 2
\divide\pst@dimg 2\relax}
%
\psset[pstricks]{dotscale=1}
%
\def\psdot{\pst@object{psdot}}
\def\psdot@i{\@ifnextchar({\psdot@ii}{\psdot@ii(\z@,\z@)}}
\def\psdot@ii(#1){%
  \begin@SpecialObj%
% hv modification 1.13 2005-11-28 
  \solid@star%
% hv modification end 
  \pst@@getcoor{#1}%
  \addto@pscode{
    \psk@dotsize
    \@nameuse{psds@\psk@dotstyle}
    \tx@setStrokeTransparency
    \pst@coor Dot}%
  \end@SpecialObj}
%
\def\psdots{\pst@object{psdots}}
\def\psdots@i{%
  \begin@SpecialObj%
  \pst@getcoors[\psdots@ii}
\def\psdots@ii{%
  \addto@pscode{ false \tx@NArray \psdots@iii }%
  \end@SpecialObj}
\def\psdots@iii{%
  \psk@dotsize
  \@nameuse{psds@\psk@dotstyle}
  \tx@setStrokeTransparency
  newpath
  n { transform floor .5 add exch floor .5 add exch itransform Dot  } repeat }
%
% DG: dead code (to suppress until \psset[pstricks]{dotstyle) ? - Aug. 4, 1997
\def\tx@SQ{SQ }
\def\tx@ST{ST }
\def\tx@SP{SP }
%
\def\pst@gdot#1{ /Dot { gsave T \psk@dotangle \psk@dotscale #1 grestore } def }
%
\@namedef{psds@*}{\pst@gdot{ 0 0 DS \tx@SD }}
\@namedef{psds@o}{%
  /r2 DS CLW sub def
  \pst@gdot{ 0 0 DS \tx@SD \pst@usecolor\psfillcolor SLW 0 0 r2 \tx@SD }}
\@namedef{psds@square*}{ /r1 DS .886 mul def \pst@gdot{r1 \tx@SQ }}
\@namedef{psds@square}{%
  /r1 DS .886 mul def /r2 r1 CLW sub def
  \pst@gdot{r1 \tx@SQ \pst@usecolor\psfillcolor r2 \tx@SQ}}
\@namedef{psds@triangle*}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST}}
\@namedef{psds@triangle}{%
  /y1 DS .778 mul neg def /x1 y1 1.732 mul neg def
  /y2 y1 CLW add def /x2 y2 1.732 mul neg def
  \pst@gdot{x1 y1 \tx@ST \pst@usecolor\psfillcolor x2 y2 \tx@ST}}
\@namedef{psds@pentagon*}{%
  /r1 DS 1.149 mul def
  \pst@gdot{r1 \tx@SP}}
\@namedef{psds@pentagon}{%
  DS .93 mul dup 1.236 mul /r1 ED CLW sub 1.236 mul /r2 ED
  \pst@gdot{r1 \tx@SP \pst@usecolor\psfillcolor r2 \tx@SP}}
\@namedef{psds@+}{%
  /DS DS 1.253 mul def
  \pst@gdot{DS 0 moveto DS neg 0 L stroke 0 DS moveto 0 DS neg L stroke}}
\@namedef{psds@|}{%
  \psk@tbarsize CLW mul add 2 div /DS ED
  \pst@gdot{0 DS moveto 0 DS neg L stroke}}
% DG: end dead code?
%
\define@key[psset]{pstricks}{dotstyle}[*]{%
  \@ifundefined{psds@#1}%
    {\@pstrickserr{Dot style `#1' not defined}\@eha}%
    {\edef\psk@dotstyle{#1}}}
\psset[pstricks]{dotstyle=*}
%
\def\tx@FontDot{FontDot }
\def\newpsfontdot#1[#2]#3#4{%
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
% DG/SR modification begin - Dec. 12, 1999 - Patch 14
%/Dot { moveto #4 show } bind def }}
    /Dot { moveto gsave \psk@dotscale #4 show grestore } bind def 
}}
% DG/SR modification end
\def\newpsfontdotH#1[#2]#3#4#5{%	for filled objects
  \@namedef{psds@#1}{%
    /#3 \psk@@dotangle [#2] \tx@FontDot
    /Dot {
      moveto
%      \iftrue
% DG/SR modification begin - Dec. 23, 1999 - Patch 14
%gsave \pst@usecolor\psfillcolor #5 show grestore
%\fi
%#4 show
      gsave \psk@dotscale \pst@usecolor\psfillcolor #5 show grestore % fill first
%      \fi					
      gsave \psk@dotscale #4 show grestore	% show the unfilled one
% DG/SR modification end
    } bind def 
}}
%
\pstheader{pst-dots.pro}
\newpsfontdot{*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{o}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{Bo}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
\newpsfontdotH{triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{Btriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{triangle*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{Bsquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{square*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdotH{pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{Bpentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{pentagon*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
% DG/SR modification begin - Mar. 18, 1997 and Dec. 16, 1999 - Patch 14
%\newpsfontdot{diamond*}[1.9 0.0 0.0 1.9 -0.4598 -0.70775]{Symbol}{<E0>}
%\newpsfontdot{diamond}[2.3 0.0 0.0 2.3 -0.8533 -0.5336]{Symbol}{<A8>}
% D.G. modification begin - Jan. 17, 2000
\newpsfontdotH{diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{Bdiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{diamond*}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
% DG/SR modification end
\newpsfontdot{oplus}[1.44928 0.0 0.0 1.44928 -0.562319 -0.478261]{Symbol}{<C5>}
\newpsfontdot{otimes}[1.44928 0.0 0.0 1.44928 -0.562319 -0.475362]{Symbol}{<C4>}
\newpsfontdot{x}[1.8 0.0 0.0 1.8 -0.495 -0.4788]{Symbol}{<B4>}
\newpsfontdot{+}[2.3 0.0 0.0 2.3 -0.6486 -0.5819]{Times-Roman}{<2B>}
\newpsfontdot{asterisk}[2.43309 0.0 0.0 2.43309 -0.609489 -1.14477]{Times-Roman}{<2A>}
\newpsfontdot{B+}[2.3 0.0 0.0 2.3 -0.6555 -0.5819]{Times-Bold}{<2B>}
\newpsfontdot{Basterisk}[2.29358 0.0 0.0 2.29358 -0.576835 -1.08486]{Times-Bold}{<2A>}
\newpsfontdot{|}[1.98413 0.0 0.0 1.38 -0.258929 -0.5]{Helvetica}{(|)}
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.258929 -0.712302]{Helvetica}{(|)}
% DG/SR modification end
\newpsfontdot{B|}[1.98413 0.0 0.0 1.38 -0.277778 -0.5]{Helvetica-Bold}{(|)}%
% DG/SR modification begin - Oct. 27, 1997 - Patch 7
%[1.98413 0.0 0.0 1.98413 -0.277778 -0.78302]{Helvetica-Bold}{(|)}

% DG/SR modification end
\iffalse
\newpsfontdot{*}[2.77778 0.0 0.0 2.77778 -0.638889 -0.813889]{Symbol}{<B7>}
\newpsfontdot{o}[3.33333 0.0 0.0 3.33333 -0.666667 -1.78167]{Symbol}{<B0>}
\newpsfontdot{Bo}[4.69484 0.0 0.0 4.69484 -0.78169 -2.97418]{Times-Bold}{<CA>}
\fi
% Etienne Riga
\newpsfontdot{Asterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(k)}
\newpsfontdot{BoldAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(K)}
\newpsfontdotH{SolidAsterisk}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(J)}{(b)}
%
\newpsfontdotH{Pentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(p)}{(q)}
\newpsfontdotH{BoldPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(P)}{(q)}
\newpsfontdot{SolidPentagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(q)}
\newpsfontdotH{Hexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(h)}{(G)}
\newpsfontdotH{BoldHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(H)}{(G)}
\newpsfontdot{SolidHexagon}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(G)}
\newpsfontdotH{Octogon}[1 0 0 1 0 0]{PSTricksDotFont}{(f)}{(g)}
\newpsfontdotH{BoldOctogon}[1 0 0 1 0 0]{PSTricksDotFont}{(F)}{(g)}
\newpsfontdot{SolidOctogon}[1 0 0 1 0 0]{PSTricksDotFont}{(g)}
%
\newpsfontdot{Bullet}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(b)}
\newpsfontdotH{Circle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(c)}{(b)}
\newpsfontdotH{BoldCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(C)}{(b)}
%\newpsfontdot{SolidCircle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Triangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(t)}{(u)}
\newpsfontdotH{BoldTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(T)}{(u)}
\newpsfontdot{SolidTriangle}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(u)}
\newpsfontdotH{Square}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(s)}{(r)}
\newpsfontdotH{BoldSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(S)}{(r)}
\newpsfontdot{SolidSquare}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(r)}
\newpsfontdot{Add}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(a)}
\newpsfontdot{BoldAdd}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(A)}
\newpsfontdot{Mul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(x)}
\newpsfontdot{BoldMul}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(X)}
\newpsfontdotH{Oplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(m)}{(b)}
\newpsfontdotH{BoldOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(M)}{(b)}
\newpsfontdotH{SolidOplus}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(e)}{(b)}
\newpsfontdotH{Otimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(n)}{(b)}
\newpsfontdotH{BoldOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(N)}{(b)}
\newpsfontdotH{SolidOtimes}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(E)}{(b)}
\newpsfontdot{Bar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(i)}
\newpsfontdot{BoldBar}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(I)}
\newpsfontdotH{Diamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(d)}{(l)}
\newpsfontdotH{BoldDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(D)}{(l)}
\newpsfontdot{SolidDiamond}[1.0 0.0 0.0 1.0 0.0 0.0]{PSTricksDotFont}{(l)}
%
\newdimen\pslinearc
\define@key[psset]{pstricks}{linearc}[0pt]{\pssetlength\pslinearc{#1}}
\psset[pstricks]{linearc=0pt}
%
\def\psline{\pst@object{psline}}
\def\psline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psline@ii%
  }%
}
\def\psline@ii{%
  \ifx\pslinestyle\psls@@symbol\addto@pscode{ \psls@symbol SymbolLine }%
  \else%
    \addto@pscode{
      \ifPst@noCurrentPoint\else\pst@cp\fi 	  % current point?
      \psline@iii % arc and lineto type
      \tx@Line	  % .pro function
    }%
  \fi%
  \end@OpenObj%
}
\def\psline@iii{
  \ifdim\pslinearc>\z@
    /r \pst@number\pslinearc def
    /Lineto { \tx@Arcto } def
  \else
    /Lineto /lineto load def
  \fi
  \tx@setlinejoin 			% hv 2007-10-13
  \ifshowpoints true \else false \fi
}
%
\def\pst@isnum#1{\pst@isnum@i\zap@space#1 \@empty\@nil}%
\def\pst@isnum@i#1\@nil{%
  \if!\ifnum9<1#1!\else_\fi%
      \expandafter\@firstoftwo%
  \else%
      \expandafter\@secondoftwo%
  \fi}
%
\def\psset@@symbol#1#2#3#4\@nil{%
  \ifx\relax#4\relax\def\psk@symbol{(#1)}%
  \else%
    \pst@isnum{#1#2#3}{%
      \pst@cnta='#1#2#3\relax%
      \ifnum\pst@cnta>'377\relax%
        \@pstrickserr{Number too large!}\@ehpb%
      \else%
        \def\psk@symbol{(\@backslashchar#1#2#3)}%
      \fi%
}{\@pstrickserr{Not a number!}\@ehpb}%
  \fi}
%
\define@key[psset]{pstricks}{symbol}[a]{\expandafter\psset@@symbol#1!!\@nil}
\psset[pstricks]{symbol=a}
%
\newdimen\pst@symbolStep
\define@key[psset]{pstricks}{symbolStep}[20pt]{\pst@expandafter\pst@@symbolStep#1\@nil}
\def\pst@@symbolStep#1#2\@nil{\if-#1\pssetlength\pst@symbolStep{-#2pt}\else\pssetlength\pst@symbolStep{#1#2}\fi}
\psset[pstricks]{symbolStep=20pt}

\newdimen\pst@symbolWidth
\newdimen\pst@symbolLinewidth
\define@key[psset]{pstricks}{symbolWidth}[10pt]{\pssetlength\pst@symbolWidth{#1}}
\define@key[psset]{pstricks}{symbolLinewidth}[0.5pt]{\pssetlength\pst@symbolLinewidth{#1}}
\psset[pstricks]{symbolWidth=10pt,symbolLinewidth=0.5pt}

\define@key[psset]{pstricks}{symbolFont}[Dingbats]{\def\psk@symbolFont{/#1 }}
\psset[pstricks]{symbolFont=Dingbats}
\define@boolkey[psset]{pstricks}[Pst@]{rotateSymbol}[true]{}
\psset[pstricks]{rotateSymbol=false}
\define@key[psset]{pstricks}{startAngle}[0]{\pst@getangle{#1}\psk@startAngle}
\define@key[psset]{pstricks}{tickAngle}[0]{\pst@getangle{#1}\psk@tickAngle}
\psset[pstricks]{startAngle=0,tickAngle=0}
\define@boolkey[psset]{pstricks}[Pst@]{curveticks}[true]{}
\psset[pstricks]{curveticks=false}

%
\def\psls@symbol{
  /Symbol \psk@symbol def
  /SymbolWidth \pst@number\pst@symbolWidth def
  /SymbolLinewidth \pst@number\pst@symbolLinewidth def
  /SymStep \pst@number\pst@symbolStep def
  \psk@symbolFont findfont %0. [1.0 0.0 0.0 1.0 0.0 0.0]
  \pst@number\pst@symbolWidth scalefont %dup 
  setfont 
  /rotateSymbol \ifPst@rotateSymbol true \else false \fi def
  /tickAngle \psk@tickAngle\space def
  /startAngle \psk@startAngle\space def
  /CorrAngle \ifx\psk@rot\@empty 0 \else \psk@rot \fi def
  /curveticks \ifPst@curveticks true \else false \fi def
  \pst@number\pslinewidth SLW
}
\def\psls@@symbol{symbol}
%
\def\psPline{\def\pst@par{}\pst@object{psPline}}% perpendicular to another line B-C
\def\psPline@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psPline@ii}%   \pst@coors on stack
}
\def\psPline@ii{%
  \addto@pscode{ % [ pC pB pA  is on stack
    /yA ED /xA ED
    /yB ED /xB ED
    yB sub exch xB sub div /mBC ED		% the slope
    /mA 1 mBC neg div def			% orthogonal
    /xS yA yB sub mBC xB mul add mA xA mul sub mBC mA sub div def
    /yS mBC xS xB sub mul yB add def
    xS yS xA yA 
    \ifPst@noCurrentPoint\else\pst@cp\fi 	% current point
    \psline@iii % arc and lineto type
    \tx@Line	% .pro function
  }%
  \end@OpenObj%
  \ignorespaces%
}
%
\def\qline(#1)(#2){%
  \def\pst@par{}%
  \begin@SpecialObj
  \def\pst@linetype{0}%
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{%
    \pst@tempa moveto \pst@coor L
    \@nameuse{psls@\pslinestyle}%
  }%
  \end@SpecialObj}
%
\def\pspolygon{\pst@object{pspolygon}}
\def\pspolygon@i{%
  \begin@ClosedObj%
  \def\pst@cp{}%
  \pst@getcoors[\pspolygon@ii%
}
\def\pspolygon@ii{%
  \ifx\pslinestyle\psls@@symbol\addto@pscode{ \psls@symbol SymbolPolygon }%
  \else                        \addto@pscode{\psline@iii \tx@Polygon}%
  \fi%
  \def\pst@linetype{1}%
  \end@ClosedObj}
%
\define@key[psset]{pstricks}{framearc}[0]{\pst@checknum{#1}\psk@framearc}
\psset[pstricks]{framearc=0}
%
\define@key[psset]{pstricks}{cornersize}[relative]{\pst@expandafter\psset@@cornersize{#1}\@nil}
\def\psset@@cornersize#1#2\@nil{%
  \if #1a\relax
    \def\psk@cornersize{\pst@number\pslinearc false }%
  \else\def\psk@cornersize{\psk@framearc true }%
  \fi}
\psset[pstricks]{cornersize=relative}
%
\def\tx@Rect{Rect }
\def\tx@OvalFrame{OvalFrame }
\def\tx@Frame{Frame }
%
\define@key[psset]{pstricks}{dimen}[outer]{\pst@expandafter\psset@@dimen{#1}\@nil}
\def\psset@@dimen#1#2\@nil{%
  \if #1o\relax%	outer
    \def\psk@dimen{.5 }%
  \else
    \if #1m\relax%	middle
      \def\psk@dimen{0 }%
    \else
      \if #1i\relax%	inner
        \def\psk@dimen{-.5 }%
  \fi\fi\fi}
\psset[pstricks]{dimen=outer}
%
\def\psframe{\pst@object{psframe}}
\def\psframe@i(#1){%
  \@ifnextchar({\psframe@ii(#1)}{\psframe@ii(0,0)(#1)}}
\def\psframe@ii(#1)(#2){%
  \begin@ClosedObj%
    \pst@getcoor{#1}\pst@tempa%
    \pst@@getcoor{#2}%
    \addto@pscode{ \psk@cornersize \pst@tempa \pst@coor \psk@dimen \tx@Frame }%
    \def\pst@linetype{2}%
    \showpointsfalse%
  \end@ClosedObj%
}
%
\def\psTextFrame{\pst@object{psTextFrame}}
\def\psTextFrame@i(#1)(#2)#3{%
  \addbefore@par{ref=c}%	to prevent an empty value
  \leavevmode%
  \pst@killglue
  \begingroup
  \use@par
  \ifx\psk@yref\relax \def\psk@yref{0}\fi% no Baseline possible
  \SpecialCoor
  \pst@getcoor{#1}\pst@tempA
  \pst@getcoor{#2}\pst@tempB
  \if@star\psframe*(#1)(#2)\else\psframe(#1)(#2)\fi
  \rput(! \pst@tempA \pst@tempB % x1 y1 x2 y2
    exch 4 -1 roll 		% y1 y2 x2 x1
    dup /x1 ED			% y1 y2 x2 x1
    sub /dx ED			% y1 y2 
    exch dup /y1 ED 		% y2 y1
    sub /dy ED	
    x1 dx \psk@xref\space mul add \pst@number\psxunit div 
    y1 dy \psk@yref\space mul add \pst@number\psyunit div ){#3}
  \endgroup
  \ignorespaces}
%
\def\tx@BezierNArray{ BezierNArray }
\def\tx@OpenBezier{ OpenBezier }
\def\tx@ClosedBezier{ ClosedBezier }
\def\tx@BezierShowPoints{ BezierShowPoints }
\def\tx@BezierCurve{ BezierCurve }
\def\pst@BezierType{2 }	% the default
%
\def\psbezier{\pst@object{psbezier}}
\def\psbezier@i{%
  \pst@getarrows{%
    \begin@OpenObj
      \pst@getcoors[\psbezier@ii%
  }%
}
\def\psbezier@ii{%
  \addto@pscode{
    \ifPst@noCurrentPoint\else\pst@cp\fi
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol OpenSymbolBezier 
    \else 
      \tx@OpenBezier 
      \ifshowpoints \tx@BezierShowPoints \fi
    \fi
  }%
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@OpenObj}
%
\def\pscbezier{\def\pst@par{}\pst@object{pscbezier}}
\def\pscbezier@i{%
  \begin@ClosedObj
  \pst@getcoors[\pscbezier@ii}
%
\def\pscbezier@ii{%
  \addto@pscode{%
    \ifshowpoints true \else false \fi
    \ifx\pslinestyle\psls@@symbol \psls@symbol ClosedSymbolBezier 
    \else 
      \tx@ClosedBezier
      \ifshowpoints \tx@BezierShowPoints \fi
    \fi}%
%  \chardef\pst@linetype=1
  \def\pst@linetype{1}%
  \ifx\pslinestyle\psls@@symbol\def\pslinestyle{none}\fi%
  \end@ClosedObj}
%
\iffalse
\define@key[psset]{pstricks}{epsilon}[0.005]{\pst@checknum{#1}\psk@epsilon}
\psset[pstricks]{epsilon=0.005}		% 200 steps for one curve
%
\def\psBezier#1{%		% allowed order is 1 ... 9
  \ifnum#1>0 \ifnum#1<10 \def\pst@BezierType{#1 }\fi\fi%
  \def\pst@par{}\pst@object{psBezier}}
\def\psBezier@i{%
  \pst@getarrows{%
    \begin@OpenObj
    \pst@getcoors[\psBezier@ii%
}}
\def\psBezier@ii{%
  \addto@pscode{%
    \psk@epsilon	    	% step for Bezier T=0,0+epsilon,0+i*epsilon,...,1
    \pst@BezierType 		% type of the Bezier curve 2,3,4,... 
    \tx@BezierCurve
    \ifshowpoints \tx@BezierShowPoints \fi
  }%
  \end@OpenObj}
\fi
%
\define@key[psset]{pstricks}{pType}[0]{\pst@cntg=#1\relax\edef\psk@pType{\the\pst@cntg}}
\psset[pstricks]{pType=0}
\def\tx@Parab{Parab }%	 given by 1 point and the min/max
\def\tx@Parabo{Parab1 }% given by 2 points for y-a=(x-b)^2
%
\def\psparabola{\pst@object{psparabola}}%  2009-05-19 (hv)
\def\psparabola@i{\pst@getarrows\psparabola@ii}
\def\psparabola@ii#1(#2)#3(#4){%  #2 P #4 SP
  \begin@OpenObj
  \pst@getcoor{#2}\pst@tempa
  \pst@@getcoor{#4}%
  \addto@pscode{\pst@tempa \pst@coor 
    \ifcase\psk@pType
      \tx@Parab \or
      \tx@Parabo
    \fi}%
  \end@OpenObj}
\let\parabola\psparabola% compatibility  (hv)
%
%
\define@key[psset]{pstricks}{gridwidth}[0.8pt]{\pst@getlength{#1}\psk@gridwidth}
\psset[pstricks]{gridwidth=.8pt}
\define@key[psset]{pstricks}{griddots}[0]{%
  \pst@cntg=#1\relax
  \edef\psk@griddots{\the\pst@cntg}}
\psset[pstricks]{griddots=0}
\define@key[psset]{pstricks}{gridcolor}[black]{\pst@getcolor{#1}\psgridcolor}
\psset[pstricks]{gridcolor=black}
\define@key[psset]{pstricks}{subgridwidth}[0.4pt]{\pst@getlength{#1}\psk@subgridwidth}
\psset[pstricks]{subgridwidth=0.4pt}
\define@key[psset]{pstricks}{subgridcolor}[gray]{\pst@getcolor{#1}\pssubgridcolor}
\psset[pstricks]{subgridcolor=gray}
\define@key[psset]{pstricks}{subgriddots}[0]{%
  \pst@cntg=#1\relax\edef\psk@subgriddots{\the\pst@cntg}}
\psset[pstricks]{subgriddots=0}
\define@key[psset]{pstricks}{subgriddiv}[5]{%
  \pst@cntg=#1\relax\edef\psk@subgriddiv{\the\pst@cntg}}
\psset[pstricks]{subgriddiv=5}
%
\define@key[psset]{pstricks}{gridfont}[Helvetica]{\def\psk@gridfont{/#1 }}%   hv 2007-11-13
\psset[pstricks]{gridfont=Helvetica}
%
\define@key[psset]{pstricks}{gridlabels}[10pt]{\pst@getlength{#1}\psk@gridlabels}
\psset[pstricks]{gridlabels=10pt}
\define@key[psset]{pstricks}{gridlabelcolor}[black]{\pst@getcolor{#1}\psgridlabelcolor}
\psset[pstricks]{gridlabelcolor=black}

\def\tx@Grid{Grid }

\def\psgrid{\pst@object{psgrid}}
\def\psgrid@i{\@ifnextchar({\psgrid@ii}{\expandafter\psgrid@iv\pic@coor}}
\def\psgrid@ii(#1){\@ifnextchar({\psgrid@iii(#1)}{\psgrid@iv(0,0)(0,0)(#1)}}
\def\psgrid@iii(#1)(#2){\@ifnextchar({\psgrid@iv(#1)(#2)}{\psgrid@iv(#1)(#1)(#2)}}
\def\psgrid@iv(#1)(#2)(#3){%
  \begin@SpecialObj%
    \pst@getcoor{#1}\pst@tempA%  hv 1.11
    \pst@getcoor{#2}\pst@tempB%  hv 1.11
    \pst@@getcoor{#3}%
    \ifnum\psk@subgriddiv>1\relax
      \addto@pscode{
        gsave
        \tx@setStrokeTransparency
        \psk@subgridwidth SLW 
        \pst@usecolor\pssubgridcolor
        \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
%        \pst@number\psxunit \pst@number\psyunit        % hv 1.11
        \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
        \psk@subgriddiv\space \psk@subgriddots\space
        {} 0 
        \psk@gridfont findfont 0 scalefont setfont      % hv 1.16
	\tx@Grid 
	grestore
      }%
    \fi%
    \addto@pscode{
      gsave
      \tx@setStrokeTransparency
      \psk@gridwidth SLW 
      \pst@usecolor\psgridcolor
      \pst@tempB \pst@coor \pst@tempA                 % hv 1.11
      \pst@number\psxunit abs \pst@number\psyunit abs % hv 1.11
%      \pst@number\psxunit \pst@number\psyunit        % hv 1.11
      1 \psk@griddots\space { \pst@usecolor\psgridlabelcolor }
      \psk@gridlabels 
      \psk@gridfont findfont \psk@gridlabels scalefont setfont  % hv 1.16
       \tx@Grid 
      grestore
    }%
  \end@SpecialObj}
%
\newif\ifpsmathbox
\psmathboxtrue
\def\pst@mathflag{\z@}
\newtoks\everypsbox
\let\pst@thisbox\relax
%
\long\def\pst@makenotverbbox#1#2{%
  \edef\pst@mathflag{%
  \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else\z@\fi\else\z@\fi}%
  \setbox\pst@hbox=\hbox{%
    \ifcase\pst@mathflag\or$\m@th\textstyle\or$\m@th\displaystyle\fi%
    {\pst@thisbox\the\everypsbox#2}%
    \ifnum\pst@mathflag>\z@$\fi%                                     $
  }%
  #1}
%
\def\pst@makeverbbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{\ifpsmathbox\ifmmode\ifinner1\else2\fi\else\z@\fi\else\z@\fi}%
  \afterassignment\pst@beginbox%
  \setbox\pst@hbox\hbox%
}
\def\pst@beginbox{%
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi%
  \bgroup\aftergroup\pst@endbox%
  \pst@thisbox%
  \the\everypsbox%
}
\def\pst@endbox{%
  \ifnum\pst@mathflag>\z@\relax$\fi%                      $
  \egroup%
  \pst@afterbox%
}
\def\pst@makebox{\pst@@makebox}
\def\psverbboxtrue{\def\pst@@makebox{\pst@makeverbbox}}
\def\psverbboxfalse{\def\pst@@makebox{\pst@makenotverbbox}}
\psverbboxfalse
\def\pst@longbox{%
  \def\pst@makebox{%
    \gdef\pst@makebox{\pst@@makebox}%
    \pst@makelongbox%
  }%
}
\def\pst@makelongbox#1{%
  \def\pst@afterbox{#1}%
  \edef\pst@mathflag{%
    \ifpsmathbox\ifmmode\ifinner 1\else 2\fi\else \z@\fi\else \z@\fi%
  }%
  \setbox\pst@hbox\hbox\bgroup
  \aftergroup\pst@afterbox
  \ifcase\pst@mathflag\or$\m@th\or$\m@th\displaystyle\fi
  \begingroup
  \pst@thisbox
  \the\everypsbox%
}
\def\pst@endlongbox{%
  \endgroup
  \ifnum\pst@mathflag>\z@$\fi		%$
  \egroup%
}
\def\pslongbox#1#2{%
  \@namedef{#1}{\pst@longbox#2}%
  \@namedef{end#1}{\pst@endlongbox}}
%
\newdimen\psframesep
\define@key[psset]{pstricks}{framesep}[3pt]{\pssetlength\psframesep{#1}}
\psset[pstricks]{framesep=3pt}
%
\define@boolkey[psset]{pstricks}[ps]{boxsep}[true]{}
\psset[pstricks]{boxsep}
%
\def\pst@useboxpar{%
  \use@par%
  \if@star%
    \let\pslinecolor\psfillcolor%
    \solid@star%
    \let\solid@star\relax
  \fi%
  \ifpsdoubleline \pst@setdoublesep \fi}
%
\def\psframebox{\def\pst@par{}\pst@object{psframebox}}
\def\psframebox@i{\pst@makebox\psframebox@ii}
\def\psframebox@ii{%
  \begingroup
  \pst@useboxpar
  \pst@dima=\pslinewidth
  \advance\pst@dima by \psframesep
  \pst@dimc=\wd\pst@hbox\advance\pst@dimc by \pst@dima
  \pst@dimb=\dp\pst@hbox\advance\pst@dimb by \pst@dima
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd by \pst@dima
  \setbox\pst@hbox=\hbox{%
    \ifpsboxsep\kern\pst@dima\fi
    \begin@ClosedObj
    \addto@pscode{%
      \psk@cornersize % arcradius boolean
      \pst@number\pst@dima neg
      \pst@number\pst@dimb neg
      \pst@number\pst@dimc
      \pst@number\pst@dimd
      .5
      \tx@Frame%
    }%
    \def\pst@linetype{2}%
    \showpointsfalse
    \end@ClosedObj
    \box\pst@hbox
    \ifpsboxsep\kern\pst@dima\fi%
  }%
  \ifpsboxsep\dp\pst@hbox=\pst@dimb\ht\pst@hbox=\pst@dimd\fi
  \leavevmode\box\pst@hbox
  \endgroup}
%
\def\psdblframebox{\def\pst@par{}\pst@object{psdblframebox}}
\def\psdblframebox@i{\addto@par{doubleline=true}\psframebox@i}
%
\define@key[psset]{pstricks}{clipcommand}[clip]{\def\pst@clipcommand{#1 }}
\psset[pstricks]{clipcommand=clip}% alternative is eoclip
%
\def\psclip{\@ifnextchar[\psclip@i{\psclip@i[]}}%
\def\psclip@i[#1]#2{%
  \leavevmode%
  \begingroup%
    \ifx\relax#1\relax\else\psset{#1}\fi%
    \begin@psclip%
      \begingroup%
        \def\use@pscode{%
          \pstVerb{
            \pst@dict
            /mtrxc CM def
            CP CP T
            \tx@STV
            \psk@origin
            \psk@swapaxes
            newpath
            \pst@code
            \pst@clipcommand
            newpath
            mtrxc setmatrix
            moveto
            0 setgray
            end
	  }%
          \gdef\pst@code{}}%
  \def\@multips(##1)(##2)##3##4{\pst@misplaced\multips}%
  \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
  \hbox to\z@{#2}%
  \endgroup%
  \def\endpsclip{%
    \end@psclip%
    \endgroup}%
  \ignorespaces}
%
\def\endpsclip{\pst@misplaced\endpsclip}
\let\begin@psclip\relax
\def\end@psclip{\pstVerb{currentpoint initclip moveto}}
%
\def\AltClipMode{%
  \def\end@psclip{\pstVerb{\pst@grestore}}%
  \def\begin@psclip{\pstVerb{gsave}}}
  \def\clipbox{\@ifnextchar[{\clipbox@}{\clipbox@[\z@]}}
% DG modification begin - Apr. 3, 1997
% From paulus@immd5.informatik.uni-erlangen.de (Dietrich Paulus)
%\def\clipbox@[#1]{\pst@makebox\clipbox@@{#1}}
\def\clipbox@[#1]{\pst@makebox{\clipbox@@{#1}}}
% DG modification end
\def\clipbox@@#1{%
  \pssetlength\pst@dimg{#1}%
  \leavevmode\hbox{%
  \begin@psclip%
  \pst@Verb{
    CM \tx@STV CP T newpath
    /a \pst@number\pst@dimg def
    /w \pst@number{\wd\pst@hbox}a add def
    /d \pst@number{\dp\pst@hbox}a add neg def
    /h \pst@number{\ht\pst@hbox}a add def
    a neg d moveto
    a neg h L
    w h L
    w d L
    closepath
    \pst@clipcommand
    newpath
    0 0 moveto
    setmatrix}%
  \unhbox\pst@hbox%
  \end@psclip}}
%
\def\psshadowbox{\def\pst@par{}\pst@object{psshadowbox}}
\def\psshadowbox@i{\pst@makebox\psshadowbox@ii}
\def\psshadowbox@ii{%
\begingroup
\pst@useboxpar
\psshadowtrue
\psboxseptrue
\def\psk@shadowangle{-45 }%
\setbox\pst@hbox=\hbox{\psframebox@ii}%
\pst@dimh=\psk@shadowsize\p@
\pst@dimh=.7071\pst@dimh
\pst@dimg=\dp\pst@hbox
\advance\pst@dimg\pst@dimh
\dp\pst@hbox=\pst@dimg
\pst@dimg=\wd\pst@hbox
\advance\pst@dimg\pst@dimh
\wd\pst@hbox=\pst@dimg
\leavevmode
\box\pst@hbox
\endgroup}
%
\def\pscirclebox{\pst@object{pscirclebox}}
\def\pscirclebox@i{\pst@makebox\pscirclebox@ii}
\def\pscirclebox@ii{%
\begingroup%
\pst@useboxpar%
\setbox\pst@hbox=\hbox{%
\pst@nodehook%
\pscirclebox@iii%
\box\pst@hbox}%
\ifpsboxsep\pscirclebox@sep\fi%
\leavevmode%
\box\pst@hbox%
\endgroup}
%
\def\pscirclebox@iii{%
  \if@star%
    \pslinewidth\z@%
    \pstverb{\pst@dict \tx@STP \pst@usecolor\psfillcolor
             newpath \pscirclebox@iv \tx@SD end}%
  \else%
    \begin@ClosedObj%
    \def\pst@linetype{4}\showpointsfalse%
    \addto@pscode{ \pscirclebox@iv\space CLW 2 div add 0 360 arc closepath}%
    \end@ClosedObj%
  \fi}
%
\def\pscirclebox@iv{
  \pst@number{\wd\pst@hbox} 2 div
  \pst@number{\ht\pst@hbox} \pst@number{\dp\pst@hbox} add 2 div
  2 copy \pst@number{\dp\pst@hbox} sub 4 2 roll
  \tx@Pyth \pst@number\psframesep add }
%
\def\pscirclebox@sep{%
  \pst@dimn=\ht\pst@hbox%			% the height of the box
  \advance\pst@dimn by \dp\pst@hbox%		% the depth  of the box added to \pst@dimn
  \divide\pst@dimn by 2%			% \pst@dimn/2
  \pst@dimm=0.5\wd\pst@hbox%			% the half of the width
  \pst@Pyth\pst@dimm\pst@dimn\pst@dimo%		% the diameter
  \advance\pst@dimo by \pslinewidth%
  \advance\pst@dimo by \psframesep%
  \advance\pst@dimn by -\pst@dimo%
  \setbox\pst@hbox=\hbox to 2\pst@dimo{\hss\vbox{\kern-\pst@dimn\box\pst@hbox}\hss}%
  \advance\pst@dimn by -\dp\pst@hbox%
  \dp\pst@hbox=-\pst@dimn}
%  
\let\pst@nodehook\relax
%
\def\psCirclebox{\def\pst@par{}\pst@object{psCirclebox}}
\def\psCirclebox@i{\pst@makebox\psCirclebox@ii}
\def\psCirclebox@ii{%
  \begingroup
  \pst@useboxpar
  \pst@dima=\ht\pst@hbox
  \advance\pst@dima\dp\pst@hbox
  \divide\pst@dima\tw@
  \pssetlength\pst@dimb\psk@radius
  \setbox\pst@hbox=\hbox{%
    \pst@nodehook
    \pscircle(.5\wd\pst@hbox,\pst@dima){\pst@dimb}%
    \box\pst@hbox}%
  \ifpsboxsep \psCirclebox@sep \fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\psCirclebox@sep{%
  \pst@dimc=\pst@dimb
  \advance\pst@dimb-\pst@dima
  \advance\pst@dima\pst@dimc
  \setbox\pst@hbox=\hbox to\tw@\pst@dimc{%
    \hss\vrule width \z@ depth \pst@dimb height \pst@dima
    \box\pst@hbox\hss}}
%
\def\psovalbox{\def\pst@par{}\pst@object{psovalbox}}
\def\psovalbox@i{\pst@makebox{\psovalbox@ii}}
\def\psovalbox@ii{%
  \begingroup
  \pst@useboxpar
  \psovalbox@iii
  \ifpsboxsep\psovalbox@sep\fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\psovalbox@iii{%
  \psovalbox@iv
  \setbox\pst@hbox=\hbox{%
    \begin@ClosedObj
    \addto@pscode{%
      0 360
      \pst@number\pst@dimc CLW 2 div sub
      \pst@number\pst@dimd CLW 2 div sub
      \pst@number\pst@dima
      \pst@number\pst@dimb
      \tx@Ellipse
      closepath }%
    \def\pst@linetype{2}%
    \end@ClosedObj
    \unhbox\pst@hbox}}
%
\def\psovalbox@iv{%
  \pst@dimc=\pslinewidth\advance\pst@dimc\psframesep
  \pst@dimd=\ht\pst@hbox\advance\pst@dimd\dp\pst@hbox
  \pst@dima=.5\wd\pst@hbox
  \pst@dimb=.5\pst@dimd\advance\pst@dimb-\dp\pst@hbox
  \pst@dimd=.707\pst@dimd
  \advance\pst@dimd\pst@dimc
  \advance\pst@dimc.707\wd\pst@hbox}
%
\def\psovalbox@sep{%
  \setbox\pst@hbox\hbox to 2\pst@dimc{\hss\unhbox\pst@hbox\hss}%
  \pst@dimg=\pst@dimd
  \advance\pst@dimg-\pst@dimb
  \dp\pst@hbox=\pst@dimg
  \advance\pst@dimd\pst@dimb
  \ht\pst@hbox=\pst@dimd}
%
\def\psdiabox{\def\pst@par{}\pst@object{psdiabox}}
\def\psdiabox@i{\pst@makebox{\psdiabox@ii}}
\def\psdiabox@ii{%
\begingroup
\pst@useboxpar
\psdiabox@iii
\ifpsboxsep\psdiabox@sep\fi
\leavevmode
\box\pst@hbox
\endgroup}
\def\psdiabox@iv{%
\pst@dimg=.707\pslinewidth
\advance\pst@dimg.707\psframesep
\pst@dima=\wd\pst@hbox
\divide\pst@dima 2
\pst@dimc=\pst@dima
\advance\pst@dimc\pst@dimg
\pst@dimd=\ht\pst@hbox
\advance\pst@dimd\dp\pst@hbox
\divide\pst@dimd 2
\pst@dimb=\pst@dimd
\advance\pst@dimb-\dp\pst@hbox
\advance\pst@dimd\pst@dimg}
\def\psdiabox@iii{%
\psdiabox@iv
\setbox\pst@hbox=\hbox{%
\begin@ClosedObj
\addto@pscode{%
\psline@iii
pop
.5
\pst@number\pst@dimc 2 mul \pst@number\pst@dimd 2 mul
0
\pst@number\pst@dima \pst@number\pst@dimb
\tx@Diamond}%
\def\pst@linetype{4}%
\end@ClosedObj
\box\pst@hbox}}
\def\psdiabox@sep{%
\setbox\pst@hbox\hbox to 4\pst@dimc{\hss\unhbox\pst@hbox\hss}%
\multiply\pst@dimd 2
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\advance\pst@dimd-2\pst@dimb
\dp\pst@hbox\pst@dimd}
%
\define@key[psset]{pstricks}{trimode}[U]{\pst@expandafter\psset@@trimode{#1}\@empty\@empty\@nil}
\def\psset@@trimode#1#2#3\@nil{%
  \let\pst@tempg#1\relax
  \ifx\pst@tempg*
    \let\psk@@trimode\@empty
    \let\pst@tempg#2\relax
  \else
    \let\psk@@trimode\relax
  \fi
  \edef\psk@trimode{%
    \ifx R\pst@tempg 1 % Right
    \else
      \ifx D\pst@tempg 2 % Down
      \else
        \ifx L\pst@tempg 3 % Left
        \else 
          \ifx l\pst@tempg 4 % |_
          \else
            \ifx r\pst@tempg 5 % _|
            \else 0 \fi     % Up
          \fi
        \fi
      \fi
    \fi}%
}
\psset[pstricks]{trimode=U}
%
\def\pstribox{\pst@object{pstribox}}
\def\pstribox@i{\pst@makebox{\pstribox@ii}}
\def\pstribox@ii{%
  \begingroup
  \pst@useboxpar
  \pstribox@iii
  \ifpsboxsep\pstribox@sep\fi
  \leavevmode
  \box\pst@hbox
  \endgroup}
%
\def\pstribox@iii{%
  \pstribox@iv
  \setbox\pst@hbox=\hbox{%
    \begin@ClosedObj
    \addto@pscode{
      \psline@iii
      pop
      0.5
      \pst@number\pst@dimc % Width
      \pst@number\pst@dimd % Height
      \ifcase\psk@trimode  
             \or  %% 0
        exch \or  %% 1
             \or  %% 2
        exch \or  %% 3
             \or  %% 4
             \or  %% 5
      \fi
      \psk@trimode -90 mul
      \pst@number\pst@dima % x coor for text
      \pst@number\pst@dimb % y coor for text
      \tx@Triangle}%
    \def\pst@linetype{2}%
    \end@ClosedObj
    \box\pst@hbox}%
}
%
\def\pstribox@iv{%
  \pst@dimh=\pslinewidth
  \advance\pst@dimh\psframesep
  \pst@dimg=\ht\pst@hbox
  \advance\pst@dimg-\dp\pst@hbox         % totalheight
  \divide\pst@dimg 2                     % 0.5 totalheight
  \edef\pst@tempa{\number\pst@dimg sp}%  % For use by nodes.
  \ifodd\psk@trimode                     % 
    \pst@dimb\pst@dimg
  \else
    \pst@dima=\wd\pst@hbox
    \divide\pst@dima 2
  \fi
  \ifcase\psk@trimode
    \pst@dimb=-\dp\pst@hbox
    \advance\pst@dimb-\pst@dimh
  \or\pst@dima=-\pst@dimh
  \or\pst@dimb=\ht\pst@hbox
     \advance\pst@dimb\pst@dimh
  \or\pst@dima=\wd\pst@hbox
     \advance\pst@dima\pst@dimh
  \fi
  \pst@dimd=\dp\pst@hbox
  \advance\pst@dimd\ht\pst@hbox
  \ifx\psk@@trimode\relax% no star for trimode=
    \pst@dimc=\wd\pst@hbox
    \advance\pst@dimc\ifodd\psk@trimode 1.447\else 1.789\fi\pst@dimh
    \multiply\pst@dimc 2
    \advance\pst@dimd\ifodd\psk@trimode 1.789\else 1.447\fi\pst@dimh
    \multiply\pst@dimd 2
  \else% trimode=R*,L*,U*,D*
    \ifodd\psk@trimode
      \advance\pst@dimd 1.1547\wd\pst@hbox
      \advance\pst@dimd 3.4641\pst@dimh
      \pst@dimc=.866\pst@dimd
    \else
      \advance\pst@dimd .866\wd\pst@hbox %.866=(sqrt(3)/2)
      \advance\pst@dimd 3\pst@dimh 
      \pst@dimc=1.1547\pst@dimd % 1.1547=(2/sqrt(3))
    \fi
  \fi}
%
\def\pstribox@sep{%
\ifodd\psk@trimode
\advance\pst@dimb.5\pst@dimd
\ht\pst@hbox=\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox=\pst@dimd
\else
\setbox\pst@hbox\hbox to \pst@dimc{\hss\unhbox\pst@hbox\hss}%
\global\pst@dimg=.5\pst@dimc
\fi
\ifcase\psk@trimode
\dp\pst@hbox-\pst@dimb
\advance\pst@dimd\pst@dimb
\ht\pst@hbox\pst@dimd
\or
\pst@dimg=.5\wd\pst@hbox
\global\advance\pst@dimg-\pst@dima
\setbox\pst@hbox\hbox to \pst@dimc{\kern-\pst@dima\box\pst@hbox\hss}%
\or
\ht\pst@hbox\pst@dimb
\advance\pst@dimd-\pst@dimb
\dp\pst@hbox\pst@dimd
\or
\pst@dimg=\pst@dimc
\advance\pst@dimg-\pst@dima
\global\advance\pst@dimg.5\wd\pst@hbox
\setbox\pst@hbox\hbox to \pst@dimc{%
\hss\box\pst@hbox\kern\psframesep\kern\pslinewidth}%
\fi}
%
\define@key[psset]{pstricks}{arcsepA}[0]{\pst@getlength{#1}\psk@arcsepA}
\define@key[psset]{pstricks}{arcsepB}[0]{\pst@getlength{#1}\psk@arcsepB}
\define@key[psset]{pstricks}{arcsep}[0]{%
  \pst@getlength{#1}\psk@arcsepA\let\psk@arcsepB\psk@arcsepA}
\psset[pstricks]{arcsep=0}
\def\tx@ArcArrow{ArcArrow }
%
\def\psarc{\pst@object{psarc}}
\def\psarc@i{\@ifnextchar({\psarc@iii}{\psarc@ii}}
\def\psarc@ii#1{\addto@par{arrows=#1}\@ifnextchar(\psarc@iii{\psarc@iii(0,0)}}
\def\psarc@iii(#1)#2#3#4{%
  \begin@OpenObj%
    \pst@getangle{#3}\pst@tempa%
    \pst@getangle{#4}\pst@tempb%
    \ifx\pst@tempa\pst@tempb\else%
      \pst@@getcoor{#1}%
      \pssetlength\pst@dima{#2}%
      \addto@pscode{\psarc@iv \psarc@v
        \ifPst@variableLW \pst@flattenpath \fi
      }%
      \gdef\psarc@type{0}%
      \showpointsfalse%
    \fi%
  \end@OpenObj%
}
\def\psarc@iv{%
  \pst@coor /y ED /x ED
  /r \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dima \fi def
  /c 57.2957 r \tx@Div def
  /angleA
    \pst@tempa
    \psk@arcsepA c mul 2 div
    \ifcase\psarc@type add \or sub \fi
  def
  /angleB
    \pst@tempb
    \psk@arcsepB c mul 2 div
    \ifcase\psarc@type sub \or add \fi
  def
  \ifshowpoints\psarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      r angleA \tx@PtoC
      y add exch x add exch moveto
    \fi
  \fi}
% hv ---- 1.10 2005-05-05 ----------------------> hv begin
\def\psarc@v{%
  /angleAtoB angleB angleA gt { true }{ false } ifelse def
  x y r
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    r 0 gt \pslbrace
    { \ifcase\psarc@type add \or sub \fi } \psrbrace\pslbrace
    { \ifcase\psarc@type sub \or add \fi } \psrbrace ifelse
%    { \ifcase\psarc@type add \or sub \fi }
    \tx@ArcArrow
%    dup AngleA gt AngleAtoB exor { neg } fi
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    r 0 gt \pslbrace
      { \ifcase\psarc@type sub \or add \fi } \psrbrace\pslbrace
      { \ifcase\psarc@type add \or sub \fi } \psrbrace ifelse
%      { \ifcase\psarc@type sub \or add \fi }
    \tx@ArcArrow
    dup angleA gt angleAtoB xor { pop angleA } if
  \fi
\ifcase\psarc@type arc \or arcn \fi}
% hv ----- 1.10 2005-05-05 ------------------------> end
%
\def\psarc@type{0}
\def\psarc@showpoints{%
  gsave
  newpath
  x y moveto
  x y r \pst@tempa \pst@tempb
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash stroke
  grestore }
\def\psarcn{\def\pst@par{}\pst@object{psarcn}}
\def\psarcn@i{\def\psarc@type{1}\psarc@i}
%
\def\psarcAB{\pst@object{psarcAB}}%		hv 2008-11-26
\def\psarcAB@i{%
  \addbefore@par{psscale=1}% be sure, that it is defined
  \pst@getarrows{%
    \begin@OpenObj%
      \pst@getcoors{}\psarcAB@ii%
    }%
}
\def\psarcAB@ii{%
  \addto@pscode{
  /y ED /x ED /yA ED /xA ED /yB ED /xB ED 
  /r xB yB x y Pyth2 \psk@psscale\space mul def
  /c 57.2957 r \tx@Div def
  /angleA
    yA y sub xA x sub atan
    \psk@arcsepA c mul 2 div
    \ifcase\psarc@type add \else sub \fi
  def
  /angleB
    yB y sub xB x sub atan
    \psk@arcsepB c mul 2 div
    \ifcase\psarc@type sub \else add \fi 
  def
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      r angleA \tx@PtoC
      y add exch x add exch moveto
    \fi
  \fi
  \psarc@v }%
  \gdef\psarc@type{0}%
  \showpointsfalse%
  \end@OpenObj%
}
\def\psarcnAB{\def\pst@par{}\pst@object{psarcnAB}}
\def\psarcnAB@i{\def\psarc@type{1}\psarcAB@i}
%
%------------------ tvz/DG/hv (2004-05-10) begin -------------------%%
% from Denis Giroux: http://www.tug.org/pipermail/pstricks/2001/000507.html
%
% I - Definition of \psellipticwedge, a generalization of \pswedge for wedges
%     of ellipses (from the code of \pswedge and \psellipse)
%
\def\psellipticwedge{\def\pst@par{}\pst@object{psellipticwedge}}
\def\psellipticwedge@i(#1){%
  \@ifnextchar({\psellipticwedge@ii(#1)}{\psellipticwedge@ii(0,0)(#1)}}
\def\psellipticwedge@ii(#1)(#2)#3#4{%
  \begin@ClosedObj
    \pst@getangle{#3}\pst@tempa
    \pst@getangle{#4}\pst@tempb
    \pst@getcoor{#1}\pst@tempc
    \pst@@getcoor{#2}%
    \def\pst@linetype{1}%
    \addto@pscode{%
      \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
      \pst@tempa \pst@tempb
      \pst@coor
      \pst@tempc moveto
      \ifdim\psk@dimen\p@=\z@\else
        \psk@dimen CLW mul dup 3 1 roll
        sub 3 1 roll sub exch
      \fi
      \pst@tempc
      \tx@Ellipse
      closepath
    }%
  \showpointsfalse
  \end@ClosedObj%
}
%
% Code mainly from "pstricks.tex'' 0.94 beta (TvZ)
%
\def\psellipticarcn{\def\pst@par{}\pst@object{psellipticarcn}}
\def\psellipticarcn@i{\let\if@psarcn\iftrue\psellipticarc@ii}
%
\def\psellipticarc{\def\pst@par{}\pst@object{psellipticarc}}
\def\psellipticarc@i{\let\if@psarcn\iffalse\psellipticarc@ii}
\define@boolkey[psset]{pstricks}[Pst@]{correctAngle}[true]{}
\psset{correctAngle}

\let\if@psarcn\iffalse

\def\psellipticarc@ii{\pst@getarrows\psellipticarc@iii}
\def\psellipticarc@iii(#1){%
  \@ifnextchar({\psellipticarc@iv(#1)}{\psellipticarc@iv(0,0)(#1)}}
\def\psellipticarc@iv(#1)(#2)#3#4{%
%  \addbefore@par{correctAngle=false}
  \begin@OpenObj%
  \pst@getcoor{#1}\pst@tempa%	origin
  \pst@getcoor{#2}\pst@tempb%	a b
  \pst@getangle{#3}\pst@tempc%	start angle
  \pst@getangle{#4}\pst@tempd% 	end angle
  \addto@pscode{ 
    \psellipticarc@definearg \psellipticarc@draw
    \ifPst@variableLW \pst@flattenpath \fi 
  }%
  \ifshowpoints
    \addto@pscode{
      gsave
      xOrig yOrig T % set origin to ellipse origin
      \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
      rx ry scale   % now we draw a circle :-)
      1 \pst@tempc  % start angle
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempc } 
         { rx abs ry abs sub cvi 0 eq { \pst@tempc }{ rx ry
           \tx@UserCoor exch \pst@tempc tan mul exch atan 
            \pst@tempc 180 div 0.5 add floor 
            180 mul sub } ifelse } ifelse
      \fi
      PtoC moveto 
      0 0 lineto 
      1 \pst@tempd % end angle
      \ifPst@correctAngle
       cvi 90 mod 0 eq { \pst@tempd } 
         { rx ry \tx@UserCoor exch \pst@tempd tan mul exch atan 
            \pst@tempd 180 div .5 add floor 180 mul sub } ifelse 
      \fi
      PtoC lineto
   %  \ifcase\psarc@type arc \or arcn \fi
      CLW 2 div SLW 
      [ 1 1 \tx@UserCoor ] 0 setdash 
      stroke
      grestore 
    }
  \showpointsfalse%
  \fi
  \end@OpenObj%
}
\def\psellipticarc@definearg{%
%  \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
  \pst@tempa /yOrig ED /xOrig ED  % Origin
  \pst@tempb                      % radii. Now adjust:
  \ifdim\psk@dimen\p@=\z@\else
    \psk@dimen CLW mul dup 3 1 roll
    sub 3 1 roll sub exch
  \fi
  /ry ED /rx ED		% a b
  /angleA
    /d { \if@psarcn sub \else add \fi } def
%    \pst@tempc 
% the angle in the parameter equation is not proportional to the real angle!
% phi=atan(b*tan(angle)/a)+floor(angle/180+0.5)*180
   \pst@tempc 
   \ifPst@correctAngle 
     cvi 90 mod 0 eq { \pst@tempc } 
       { rx ry \tx@UserCoor exch \pst@tempc tan mul exch atan 
          \pst@tempc 180 div .5 add floor 180 mul sub } ifelse 
    \fi
    \psk@arcsepA 2 div
    ArcAdjust
  def
  /angleB
    /d { \if@psarcn add \else sub \fi } def
%    \pst@tempd 
  \pst@tempd 
  \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempd } 
       { rx ry \tx@UserCoor exch \pst@tempd tan mul exch atan 
          \pst@tempd 180 div .5 add floor 180 mul sub } ifelse 
  \fi
  \psk@arcsepB 2 div ArcAdjust  def
%  \ifshowpoints\psellipticarc@showpoints\fi
  \ifx\psk@arrowA\@empty
    \ifnum\psk@liftpen=2
      angleA cos rx mul xOrig add
      angleA sin ry mul yOrig add
      moveto
    \fi%
  \fi%
}
\def\psellipticarc@draw{%
  0 0 1
  angleA
  \ifx\psk@arrowA\@empty\else
    { ArrowA CP }
    { \if@psarcn sub \else add \fi }
    EllipticArcArrow
  \fi
  angleB
  \ifx\psk@arrowB\@empty\else
    { ArrowB }
    { \if@psarcn add \else sub \fi }
    EllipticArcArrow
  \fi
  /mtrx CM def
  xOrig yOrig T
  \ifx\psk@rot\@empty \else \psk@rot\space rotate \fi
  rx ry scale
  0 0 moveto 
  exch dup dup               % end start start start
  cos exch sin moveto        % end start
  exch                       % start end 
%  \if@star 0 0 moveto \fi	% for filling
  \if@psarcn arcn \else arc \fi
%  \if@star 0 0 moveto \fi
  mtrx setmatrix%
}
\def\psellipticarc@showpoints{%
  gsave
  /mtrx CM def
  xOrig yOrig T
  rx ry scale
  0 0 moveto
  0 0 1 
  \pst@tempc % start angle
  \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempc } 
       { rx abs ry abs sub cvi 0 eq { \pst@tempc }{ rx ry
         \tx@UserCoor exch \pst@tempc tan mul exch atan 
          \pst@tempc 180 div 0.5 add floor 
          180 mul sub } ifelse } ifelse
    \fi
  \pst@tempd % end angle
   \ifPst@correctAngle
     cvi 90 mod 0 eq { \pst@tempd } 
       { rx abs ry abs sub cvi 0 eq { \pst@tempd } { rx ry 
         \tx@UserCoor exch \pst@tempd tan mul exch atan 
          \pst@tempd 180 div 0.5 add floor 
          180 mul sub } ifelse } ifelse
    \fi
  \ifcase\psarc@type arc \or arcn \fi
  closepath
  mtrx setmatrix
  CLW 2 div SLW
  [ \psk@dash\space ] 0 setdash 
  stroke
  grestore %
}
\def\pscircle{\def\pst@par{}\pst@object{pscircle}}
\def\pscircle@i{\@ifnextchar({\pscircle@do}{\pscircle@do(0,0)}}
\def\pscircle@do(#1)#2{%
  \if@star{\use@par\qdisk(#1){#2}}%   	qdisk does not allow
  \else%				to use opacity option
    \begin@ClosedObj
    \pst@@getcoor{#1}%
    \pssetlength\pst@dimc{#2}%
    \def\pst@linetype{4}%
    \addto@pscode{
      \pst@coor 2 copy moveto
      \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimc \fi      
      \psk@dimen CLW mul sub
      dup 0 rmoveto
      0 360 arc
      \ifPst@variableLW \pst@flattenpath \fi
      closepath
    }%
    \showpointsfalse
    \end@ClosedObj
  \fi
  \ignorespaces}
%
\def\pscircleOA{\def\pst@par{}\pst@object{pscircleOA}}%	hv 2008-04-14
\def\pscircleOA@i(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempA
  \pst@@getcoor{#2}%
  \def\pst@linetype{4}%
  \addto@pscode{
    \pst@tempA			% x0 y0
    2 copy			% xO yO xO yO 
    \pst@coor			% xO yO xO yO xA yA 
    Pyth2			% xO yO radius
    \psk@dimen CLW mul sub
    \if@star \tx@SD \else
      0 360 arc
      closepath 
    \fi }%
  \showpointsfalse
  \end@ClosedObj
  \ignorespaces}
%
\def\qdisk(#1)#2{%
  \def\pst@par{}%
  \begin@SpecialObj
  \pst@@getcoor{#1}%
  \pssetlength\pst@dimg{#2}%
  \addto@pscode{ 
    \pst@coor 
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimg \fi
%    \pst@number\pst@dimg 
    \tx@SD }%
  \end@SpecialObj}
%
\define@key[psset]{pstricks}{radius}[0.25cm]{\pst@@getlength{#1}\psk@radius}
\psset[pstricks]{radius=.25cm}
%
\def\psCircle{\pst@object{psCircle}}% same as \pscircle, but uses \psk@radius
\def\psCircle@i{\@ifnextchar({\psCircle@ii}{\psCircle@ii(0,0)}}
\def\psCircle@ii(#1){\pscircle@do(#1){\psk@radius}}
%
\def\psRing{\def\pst@par{}\pst@object{psRing}}%% hv 20130405
\def\psRing@i{\@ifnextchar({\psRing@ii}{\psRing@ii(0,0)}}
\def\psRing@ii(#1){%
  \pst@@getcoor{#1}%
  \@ifnextchar[{\psRing@iii}{\psRing@iii[0,360]}}
\def\psRing@iii[#1,#2]#3#4{%   origin, inner radius, outer radius
  \begin@ClosedObj
  \pssetlength\pst@dimc{#3}%
  \pssetlength\pst@dimd{#4}%
  \pst@getangle{#1}\pst@tempa
  \pst@getangle{#2}\pst@tempb
  \def\pst@linetype{4}%
  \addto@pscode{
    \pst@coor translate 
    \pst@number\pst@dimc \psk@dimen CLW mul sub /InnerRadius ED
    \pst@number\pst@dimd \psk@dimen CLW mul sub /OuterRadius ED
    InnerRadius 0 moveto newpath
    0 0 InnerRadius \pst@tempa\space \pst@tempb\space arc 
    OuterRadius \pst@tempb\space PtoC 
    \pst@tempb\space \pst@tempa\space sub abs 360 eq { moveto }{ lineto } ifelse % whole circle or not??
    0 0 OuterRadius \pst@tempb\space \pst@tempa\space arcn 
    closepath
  }%
  \showpointsfalse
  \end@ClosedObj
  \ignorespaces}
%
\def\pswedge{\def\pst@par{}\pst@object{pswedge}}
\def\pswedge@i{\@ifnextchar({\pswedge@ii}{\pswedge@ii(0,0)}}
\def\pswedge@ii(#1)#2#3#4{%
  \begin@ClosedObj%
  \pssetlength\pst@dimc{#2}%
  \pst@getangle{#3}\pst@tempa%
  \pst@getangle{#4}\pst@tempb%
  \pst@@getcoor{#1}%
  \def\pst@linetype{1}%
  \addto@pscode{
    \ifx\psk@rot\@empty 0 \else \psk@rot \fi rotate
    \pst@coor
    2 copy
    moveto
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pst@dimc \fi
%    \pst@number\pst@dimc 
    \psk@dimen CLW mul sub % Adjusted radius
    \pst@tempa \pst@tempb
    arc
    closepath}%
  \showpointsfalse%
  \end@ClosedObj%
}
\def\tx@Ellipse{ \ifx\psk@rot\@empty 0 \else \psk@rot \fi Ellipse }
%
\def\psellipse{\def\pst@par{}\pst@object{psellipse}}
\def\psellipse@i(#1){\@ifnextchar({\psellipse@ii(#1)}{\psellipse@ii(0,0)(#1)}}
\def\psellipse@ii(#1)(#2){%
  \begin@ClosedObj
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \addto@pscode{
    0 360
    \pst@coor 
    \ifdim\psk@dimen\p@=\z@\else
      \psk@dimen CLW mul
      dup 4 -1 roll sub neg 3 1 roll sub
    \fi
    \pst@tempa 
    \tx@Ellipse
    \ifPst@variableLW \pst@flattenpath \fi
    closepath
  }%
  \def\pst@linetype{2}%
  \end@ClosedObj%
}
\def\multips{\@ifnextchar({\def\pst@par{}\multips@ii}{\multips@i}}
\def\multips@i#1{\def\pst@par{rot=#1}\multips@ii}
\def\multips@ii(#1){\@ifnextchar({\multips@iii(#1)}{\multips@iii(\z@,\z@)(#1)}}
\long\def\multips@iii(#1)(#2)#3#4{%
  \begingroup
%----------------- hv 1.10 ------------------
  \pst@killglue
%----------------- hv 1.10 ------------------
  \use@par
  \pst@getcoor{#1}\pst@tempa
  \pst@@getcoor{#2}%
  \pst@cnta=#3\relax
  \init@pscode
  \addto@pscode{%
    \pst@tempa T \the\pst@cnta\space \pslbrace
    gsave \ifx\psk@rot\@empty\else\psk@rot rotate \fi}%
  \hbox to\z@{%
    \def\init@pscode{%
      \addto@pscode{%
        gsave
        \pst@number\pslinewidth SLW
        \pst@usecolor\pslinecolor}}%
    \def\use@pscode{\addto@pscode{grestore}}%
    \def\psclip##1{\pst@misplaced\psclip}%
    \def\nc@object##1##2##3##4{\pst@misplaced{node connection}}%
    #4%
  }%
  \addto@pscode{grestore \pst@coor T \psrbrace repeat}%
  \leavevmode
  \use@pscode
  \endgroup
  \ignorespaces}
\def\psscalebox#1{\pst@makebox{\ps@scalebox{#1}}}
\def\ps@scalebox#1{%
  \begingroup%
  \pst@getscale{#1}\pst@tempa%
  \let\pst@tempc\pst@tempg%
  \let\pst@tempd\pst@temph%
  \ps@@scalebox%
  \endgroup}
\def\ps@@scalebox{%
  \leavevmode%
  \hbox{%
    \ifdim\pst@tempd\p@<\z@%
      \pst@dimg=\pst@tempd\ht\pst@hbox%
      \pst@dimh=\pst@tempd\dp\pst@hbox%
      \dp\pst@hbox=-\pst@dimg%
      \ht\pst@hbox=-\pst@dimh%
    \else%
      \ht\pst@hbox=\pst@tempd\ht\pst@hbox%
      \dp\pst@hbox=\pst@tempd\dp\pst@hbox%
    \fi%
    \pst@dima=\pst@tempc\wd\pst@hbox%
    \ifdim\pst@dima<\z@\kern-\pst@dima\fi%
    \pst@Verb{CP CP translate \pst@tempa \tx@NET}%
    \hbox to \z@{\box\pst@hbox\hss}%
    \pst@Verb{
      CP CP translate
      1 \pst@tempc div 1 \pst@tempd div scale
      \tx@NET}%
    \ifdim\pst@dima>\z@\kern\pst@dima\fi%
  }%
}
\pslongbox{Scalebox}{\psscalebox}
%
\def\psscaleboxto(#1,#2){\pst@makebox{\ps@scaleboxto(#1,#2)}}
\def\ps@scaleboxto(#1,#2){%
  \begingroup
  \pssetlength\pst@dima{#1}%
  \pssetlength\pst@dimb{#2}%
  \ifdim\pst@dima=\z@\else
    \pst@divide{\pst@dima}{\wd\pst@hbox}\pst@tempc
    \edef\pst@tempc{\pst@tempc\space}%
  \fi
  \ifdim\pst@dimb=\z@
    \ifdim\pst@dima=\z@
      \@pstrickserr{%
        \string\psscaleboxto\space dimensions cannot both be zero}\@ehpa
      \def\pst@tempa{}%
      \def\pst@tempc{1 }%
      \def\pst@tempd{1 }% 
    \else
      \let\pst@tempd\pst@tempc
    \fi
  \else
    \pst@dimc=\ht\pst@hbox
    \advance\pst@dimc\dp\pst@hbox
    \pst@divide{\pst@dimb}{\pst@dimc}\pst@tempd
    \edef\pst@tempd{\pst@tempd\space}%
    \ifdim\pst@dima=\z@ \let\pst@tempc\pst@tempd \fi
  \fi
  \edef\pst@tempa{\pst@tempc \pst@tempd scale }%
  \ps@@scalebox
  \endgroup}
\pslongbox{Scaleboxto}{\psscaleboxto}
%
\def\tx@Rot{Rot }
\def\psrotateleft{\pst@makebox{\ps@rotateleft\pst@hbox}}
\def\ps@rotateleft#1{%
\leavevmode\hbox{\hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
\pst@Verb{90 \tx@Rot}
\vbox to \z@{\vss\hbox to \z@{\box#1\hss}\vskip\z@}%
\pst@Verb{-90 \tx@Rot}}}}
\def\psrotateright{\pst@makebox{\ps@rotateright\pst@hbox}}
\def\ps@rotateright#1{%
% ----------- hv begin 2004-05-07 ----------- patch 15
%    \hbox{%
  \leavevmode\hbox{%
% ----------- hv end 2004-05-07 ----------- patch 15
  \hskip\ht#1\hskip\dp#1\vbox{\vskip\wd#1%
  \pst@Verb{-90 \tx@Rot}
  \vbox to \z@{\hbox to \z@{\hss\box#1}\vss}%
  \pst@Verb{90 \tx@Rot}}}}
\def\psrotatedown{\pst@makebox{\ps@rotatedown\pst@hbox}}
\def\ps@rotatedown#1{%
\hbox{\hskip\wd#1\vbox{\vskip\ht#1\vskip\dp#1%
\pst@Verb{180 \tx@Rot}%
\vbox to \z@{\hbox to \z@{\box#1\hss}\vss}%
\pst@Verb{-180 \tx@Rot}}}}
\pslongbox{Rotateleft}{\psrotateleft}
\pslongbox{Rotateright}{\psrotateright}
\pslongbox{Rotatedown}{\psrotatedown}
% ----------- hv begin 2004-09-23 ----------- 1.11
% compatibility stuff 
\let\rotateleft\psrotateleft
\let\rotateright\psrotateright
\let\rotatedown\psrotatedown
% ----------- hv end 2005-09-23 ----------- 1.11
\def\pst@starbox{%
\setbox\pst@hbox\hbox{\psframebox*[boxsep=false]{\unhbox\pst@hbox}}}
\def\pst@@makesmall#1{%
\setbox#1=\hbox to\z@{\hss\vbox to \z@{\vss\box#1\vss}\hss}}
\def\pst@@@makesmall#1{%
\pst@dimh=\psk@xref\wd#1%
\ifx\psk@yref\relax
\pst@dimg=\dp#1%
\else
\pst@dimg=\psk@yref\ht#1%
\advance\pst@dimg\psk@yref\dp#1%
\fi
\setbox#1=\hbox to\z@{%
\kern-\pst@dimh\vbox to\z@{\vss\box#1\kern-\pst@dimg}\hss}}
%
\define@key[psset]{pstricks}{ref}[c]{\pst@expandafter\psset@@ref{#1}\@empty,,\@nil}
\def\psset@@ref#1#2,#3,#4\@nil{%
  \def\psk@xref{.5}%
  \def\psk@yref{.5}%
  \let\pst@makesmall\pst@@@makesmall
  \ifx\@empty#3\@empty
    \@nameuse{getref@#1}%
    \@nameuse{getref@#2}%
  \else
    \pst@checknum{#1#2}\psk@xref
    \pst@checknum{#3}\psk@yref
  \fi}
%
\def\getref@c{\let\pst@makesmall\pst@@makesmall}
\def\getref@t{\def\psk@yref{1}}
\def\getref@b{\def\psk@yref{0}}
\def\getref@B{\let\psk@yref\relax}
\def\getref@l{\def\psk@xref{0}}
\def\getref@r{\def\psk@xref{1}}
\psset[pstricks]{ref=c}
%
\def\pst@rotlist{ mark RAngle /ps@a ED cleartomark ps@a neg }
\def\pst@rottable{%
@0=%
@U=%
@L=90 %
@D=180 %
@R=-90 %
@N=\pst@rotlist
@W=\pst@rotlist 90 add %
@S=\pst@rotlist 180 add %
@E=\pst@rotlist 90 sub }
%
\define@key[psset]{pstricks}{rot}[0]{%
  \pst@expandafter{\@ifnextchar*{\psset@@@rot}{\psset@@rot}}{#1}\@nil}
\def\psset@@rot#1\@nil{%
  \def\next##1@#1=##2@##3\@nil{%
    \ifx##2\relax\pst@getangle{#1}\psk@rot \else\def\psk@rot{##2}\fi%
    \pst@Verb{ gsave  STV CP T /ps@rot \ifx\psk@rot\@empty 0 \else \psk@rot \fi def grestore }% (MJS)
  }%
  \expandafter\next\pst@rottable @#1=\relax @\@nil}
%
\def\psset@@@rot#1#2\@nil{%
  \psset@@rot#2\@nil%
  \edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\space ps@rot add \fi}%
  \pst@Verb{ gsave  STV CP T /ps@rot \ifx\psk@rot\@empty 0 \else \psk@rot \fi def grestore }}% (MJS)
%
%\def\psset@@rot#1\@nil{%
%\def\ps@next##1@#1=##2@##3\@nil{%
%\ifx\relax##2\pst@getangle{#1}\psk@rot\else\def\psk@rot{##2}\fi}%
%\expandafter\ps@next\pst@rottable @#1=\relax @\@nil}
%
%\def\psset@@@rot#1#2\@nil{%
%\psset@@rot#2\@nil
%\edef\psk@rot{\pst@rotlist \ifx\psk@rot\@empty\else\psk@rot add \fi}}
\psset[pstricks]{rot=0}
%
\def\tx@RotBegin{RotBegin }
\def\tx@RotEnd{RotEnd }
\def\pst@rotate#1#2{%
  \ifx#1\@empty\else
  \setbox#2=\hbox{\pst@Verb{#1 \tx@RotBegin}\box#2\pst@Verb{\tx@RotEnd}}%
  \fi%
}
\def\psput@cartesian#1{%
  \hbox to \z@{\kern\pst@dimg{\vbox to \z@{\vss\box#1\vskip\pst@dimh}\hss}}%
}
\def\psput@special#1{%
  \hbox{%
    \pst@Verb{{ \pst@coor } \tx@PutCoor \tx@PutBegin }%
    \box#1%
    \pst@Verb{ \tx@PutEnd }%
  }%
}
\def\tx@PutCoor{PutCoor }
\def\tx@PutBegin{PutBegin }
\def\tx@PutEnd{PutEnd }
\def\rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\rput@i}{\rput@ii}}}
\def\rput@i[#1]{\addto@par{ref={#1}}\rput@ii}
\def\rput@ii{\@ifnextchar({\rput@iv}{\rput@iii}}
\def\rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\rput@iv}{\rput@iv(\z@,\z@)}}
\def\rput@iv(#1){\pst@killglue\pst@makebox{\rput@v{#1}}}
\def\rput@v#1{%
  \begingroup%
    \use@par%
    \if@star\pst@starbox\fi%
    \pst@makesmall\pst@hbox%
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox%
    \psput@{#1}\pst@hbox%
  \endgroup%
  \ignorespaces}
%
\def\multirput{%
  \def\pst@par{}%
  \pst@ifstar{\@ifnextchar[{\multirput@i}{\multirput@ii}}}
\def\multirput@i[#1]{\addto@par{ref={#1}}\multirput@ii}
\def\multirput@ii{\@ifnextchar({\multirput@iv}{\multirput@iii}}
\def\multirput@iii#1{\addto@par{rot={#1}}\multirput@iv}
\def\multirput@iv(#1){%
  \@ifnextchar({\multirput@v(#1)}{\multirput@v(\z@,\z@)(#1)}}
\def\multirput@v(#1,#2)(#3,#4)#5{%
  \pst@makebox{\multirput@vi(#1,#2)(#3,#4){#5}}}
\def\multirput@vi(#1,#2)(#3,#4)#5{%
  \pst@killglue%
  \global\psLoopIndex=\@ne\relax
  \begingroup
    \use@par
    \if@star\pst@starbox\fi
    \pst@makesmall\pst@hbox
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox
    \pssetxlength\pst@dima{#1}%
    \pssetylength\pst@dimb{#2}%
    \pssetxlength\pst@dimc{#3}%
    \pssetylength\pst@dimd{#4}%
    \pst@cntg=#5\relax
    \leavevmode
    \loop
      \vbox to \z@{%
        \vss
        \hbox to \z@{\kern\pst@dima\copy\pst@hbox\hss}%
        \vskip\pst@dimb%
      }%
      \ifnum\pst@cntg>\psLoopIndex
        \advance\pst@dima\pst@dimc
        \advance\pst@dimb\pst@dimd
        \global\advance\psLoopIndex by \@ne
    \repeat 
  \endgroup
  \ignorespaces%
}
%
\newif\if@fixedradius
\def\cput{\def\pst@par{}\pst@object{cput}}
\def\cput@i{\@fixedradiusfalse\cput@ii}
\def\cput@ii{\pst@killglue\@ifnextchar({\cput@iv}{\cput@iii}}
\def\cput@iii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\cput@iv}{\cput@iv(\z@,\z@)}%
}
\def\cput@iv(#1){\pst@makebox{\cput@v{#1}}}
  \def\cput@v#1{%
  \begingroup
    \use@par
    \setbox\pst@hbox=\hbox{%
      \psboxsepfalse
      \if@fixedradius\psCirclebox@ii\else\pscirclebox@ii\fi%
    }%
    \pst@@makesmall\pst@hbox
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%    \pst@rotate\psk@rot\pst@hbox
    \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces%
}
%
\def\Cput{\def\pst@par{}\pst@object{Cput}}
\def\Cput@i{\@fixedradiustrue\cput@ii}
\newdimen\pslabelsep
\define@key[psset]{pstricks}{labelsep}[5pt]{%
  \pssetlength\pslabelsep{#1}%
  \ifx\PSTplotLoaded\endinput% Set labels for pst-plot, if laoded
    \let\psxlabelsep\pslabelsep%
    \let\psylabelsep\pslabelsep%
  \fi}
\psset[pstricks]{labelsep=5pt}
%
\define@key[psset]{pstricks}{refangle}[0]{\pst@expandafter\psset@@refangle{#1}\@nil}
\def\psset@@refangle#1\@nil{%
  \def\next##1@#1=##2"##3@##4\@nil{%
    \ifx\relax##2%
      \pst@getangle{#1}\psk@refangle
      \def\psk@uputref{}%
    \else
      \def\psk@refangle{##2 }%
      \def\psk@uputref{##3}%
    \fi}%
  \expandafter\next\pst@refangletable @#1=\relax"@\@nil%
  \pst@Verb{ gsave STV CP T /ps@refangle \psk@refangle\space def grestore }%ADDED (MJS)
}
%
\def\pst@refangletable{%
@r=0"20%
@u=90"02%
@l=180"10%
@d=-90"01%
@ur=45"22%
@ul=135"12%
@dr=-135"21%
@dl=-45"11}
\psset[pstricks]{refangle=0}

% DG/SR modification begin - Mar. 24, 1999 - Patch 10
%\def\uput{\def\pst@par{}\@ifnextchar[{\uput@ii}{\uput@i}}
\def\uput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\uput@ii}{\uput@i}}} 
% DG/SR modification end
\def\uput@i#1{\addto@par{labelsep=#1}\uput@ii}
\def\uput@ii[#1]{%
  \addto@par{refangle={#1}}%
  \@ifnextchar({\uput@iv}{\uput@iii}}
\def\uput@iii#1{%
  \addto@par{rot={#1}}%
  \@ifnextchar({\uput@iv}{\uput@iv(\z@,\z@)}}
\def\uput@iv(#1){\pst@killglue\pst@makebox{\uput@v{#1}}}
\def\uput@v#1{%
  \begingroup%
  \use@par%
  \if@star\pst@starbox\fi%
  \pstCheckCoorType{#1}% needed for \uput@vii
  \uput@vi%
  \psput@{#1}\pst@hbox%
  \endgroup%
  \ignorespaces}
%
\def\uput@vi{%
  \ifx\psk@uputref\@empty\uput@vii\tx@UUput{}%
  \else%
    \ifx\psk@rot\@empty\expandafter\uput@viii\psk@uputref%
    \else\uput@vii\tx@UUput{}\fi%
  \fi}
% 
\def\uput@vii#1#2{%
  \edef\pst@coor{%
    \ifPst@SpecialLength \pst@SpecialLength \else \pst@number\pslabelsep \fi 
%    \pst@number\pslabelsep % \ifdim\pslabelsep<\z@  neg \fi
    #2
    \pst@number{\wd\pst@hbox}%
    \pst@number{\ht\pst@hbox}%
    \pst@number{\dp\pst@hbox}%
    \ifnum\pst@C@@rType=7
      ps@refangle % CHANGED (MJS) FROM \psk@refangle\space
      \ifx\psk@rot\@empty\else ps@rot\space sub \fi
    \else
      \psk@refangle\space 
      \ifx\psk@rot\@empty\else \psk@rot\space sub \fi
    \fi
    \tx@Uput #1}%
    %\show\pst@coor
  \setbox\pst@hbox=\hbox to\z@{\hss\vbox to\z@{\vss\box\pst@hbox\vss}\hss}%
  \setbox\pst@hbox=\psput@special\pst@hbox
  \ifnum\pst@C@@rType=7
    \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% CHANGED FROM \psk@rot (MJS)
  \else
    \ifx\psk@rot\@empty\else\pst@rotate{\psk@rot}\pst@hbox\fi% 
  \fi}
%
%
\def\uput@viii#1#2{%
  \ifnum#1>\z@\relax\ifnum#2>\z@\relax\pslabelsep=.707\pslabelsep\fi\fi%
  \setbox\pst@hbox=\vbox to\z@{%
    \ifnum#2=1\relax\vskip\pslabelsep\else\vss\fi%
    \hbox to\z@{%
      \ifnum#1=2\relax\hskip\pslabelsep \else\hss\fi%
      \box\pst@hbox%
      \ifnum#1=1\relax\hskip\pslabelsep\else\hss\fi}%
    \ifnum#2=2\relax\vskip\pslabelsep\else\vss\fi}}
%
\def\tx@Uput{Uput }
\def\tx@UUput{UUput }
%
\def\Rput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\Rput@ii}{\Rput@i}}}
\def\Rput@i#1{\addto@par{labelsep=#1}\Rput@ii}
\def\Rput@ii[#1]{\addto@par{ref={#1}}\@ifnextchar({\Rput@iv}{\Rput@iii}}
\def\Rput@iii#1{\addto@par{rot={#1}}\@ifnextchar({\Rput@iv}{\Rput@iv(\z@,\z@)}}
\def\Rput@iv(#1){\pst@killglue\pst@makebox{\Rput@v{#1}}}
\def\Rput@v#1{%
  \begingroup
  \use@par
  \if@star\pst@starbox\fi
  \Rput@vi
  \pst@makesmall\pst@hbox
  \ifx\psk@rot\@empty\else\pst@rotate{ps@rot }\pst@hbox\fi% (MJS)
%  \pst@rotate\psk@rot\pst@hbox
  \psput@{#1}\pst@hbox
  \endgroup
  \ignorespaces}
%
\def\Rput@vi{%
  \pst@dimg=\dp\pst@hbox
  \advance\pst@dimg\pslabelsep
  \dp\pst@hbox=\pst@dimg
  \pst@dimg=\ht\pst@hbox
  \advance\pst@dimg\pslabelsep
  \ht\pst@hbox=\pst@dimg
  \setbox\pst@hbox\hbox{\kern\pslabelsep\box\pst@hbox\kern\pslabelsep}}%
%
\def\oldpsput{\def\pst@par{}\pst@ifstar{\@ifnextchar[{\oldpsput@i}{\oldpsput@ii}}}
\def\oldpsput@i[#1]{\addto@par{ref={#1}}\oldpsput@ii}
\def\oldpsput@ii{\@ifnextchar<{\oldpsput@iii}{\oldpsput@iv}}
\def\oldpsput@iii<#1>{\rput@iii{#1}}
\def\OldPsput{\let\psput\oldpsput}
\def\NewPsput{\let\psput\rput}
%
% -----------  hv 20120219 -------------------
\newpsstyle{gridstyle}{subgriddiv=0,gridcolor=lightgray,griddots=10,gridlabels=8pt}
%\define@boolkey[psset]{pstricks}[]{showgrid}[true]{}
\newif\ifshowgrid
\newdimen\sh@wgridXunit
\newdimen\sh@wgridYunit
\define@key[psset]{pstricks}{showgrid}[b]{\expandafter\pst@@showgrid#1!!\@nil}
\def\pst@@showgrid#1#2#3\@nil{%                            hv 20130403
  \def\showgridp@s{0}%
  \ifx#1b\showgridtrue\else%                               bottom
    \ifx#1f\showgridfalse\else%
      \ifx#1t%
        \ifx#2r\showgridtrue\else%  			   true->bottom
               \showgridtrue\def\showgridp@s{1}\fi%        top
  \fi\fi\fi%
  \ifnum\showgridp@s>0
    \sh@wgridXunit=\psxunit%
    \sh@wgridYunit=\psyunit%
  \fi%
}
\psset[pstricks]{showgrid=false}
\define@boolkey[psset]{pstricks}[Pst@]{pgffunctions}[true]{}
\psset[pstricks]{pgffunctions=false}
%
\newdimen\pst@shift
\newif\ifPst@shift@star
\define@key[psset]{pstricks}{shift}[0]{%
  \ifx#1*
    \global\Pst@shift@startrue
    \pst@shift=\p@
  \else
    \global\Pst@shift@starfalse
    \pssetlength\pst@dimg{#1}
    \global\pst@shift\pst@dimg%   only the outer pspicture env can have a shift
  \fi}
\psset[pstricks]{shift=0}
%
%------------------------------- pspicture ------------------------------
%
\def\pspicture{\begingroup\pst@ifstar\pst@picture}
\def\pst@picture{\@ifnextchar[{\pst@@picture}{\pst@@picture[]}}
\def\pst@@picture[#1]{\@ifnextchar({\pst@@picture@i[#1]}{\pst@@picture@i[#1](10,10)}}%
\def\pst@@picture@i[#1]#2(#3,#4){\@ifnextchar(%   ignore anything between [] and ()
  {\pst@@@picture[#1](#3,#4)}%
  {\pst@@@picture[#1](0,0)(#3,#4)}}
%
\def\pst@@@picture[#1](#2,#3)(#4,#5){%
  \pssetxlength\pst@dima{#2}%
  \pssetylength\pst@dimb{#3}%
  \pssetxlength\pst@dimc{#4}%
  \pssetylength\pst@dimd{#5}%
  \ifdim\pst@dima>\pst@dimc%
    \pst@dimg=\pst@dima%
    \pst@dima=\pst@dimc%
    \pst@dimc=\pst@dimg%
  \fi%
  \ifdim\pst@dimb>\pst@dimd%
    \pst@dimg=\pst@dimb%
    \pst@dimb=\pst@dimd%
    \pst@dimd=\pst@dimg%
  \fi%
  \setbox\pst@hbox=\hbox\bgroup%
  \begingroup\KillGlue%
  \@ifundefined{@latexerr}{}{\let\unitlength\psunit}%
  \edef\pic@coor{(#2,#3)(#2,#3)(#4,#5)}%
% ----------- 1.10/12 beg hv -------------------
  \psset{showgrid=false}%                % for nested pspicture environemnets
  \def\pst@tempA{#1}%
  \ifx\pst@tempA\@empty\else\psset{#1}\fi% sets the shift and grid option
  \ifshowgrid\ifnum\showgridp@s=0\psgrid[style=gridstyle]\fi\fi%
% ----------- 1.10/12 end hv -------------------
  \ignorespaces%			% 2008-12-07
  \ifPst@pgffunctions\pstVerb{ pgffunctions } \fi % hv 2013-04-17
}
\def\pic@coor{(0,0)(0,0)(10,10)}
%\newdimen\pst@shift
\def\endpspicture{%
  \ifshowgrid\ifnum\showgridp@s>0
    \psgrid[xunit=\sh@wgridXunit,yunit=\sh@wgridYunit,style=gridstyle]\fi\fi%
  \pst@killglue
%  \global\pst@shift=\pst@shift% in fact of the following endgroup
  \endgroup
  \egroup
  \ifdim\wd\pst@hbox=\z@\else
    %\@pstrickserr{Extraneous space in the pspicture environment}%
    %{Type \space <return> \space to proceed.}%
  \fi
  \ht\pst@hbox=\pst@dimd
  \dp\pst@hbox=-\pst@dimb
  \setbox\pst@hbox=\hbox{%
    \kern-\pst@dima
% Orig version ----------
%\ifx\pst@tempa\@empty\else
%\advance\pst@dimd-\pst@dimb
%\pst@dimd=\pst@tempa\pst@dimd
%\advance\pst@dimd\pst@dimb
%\lower\pst@dimd
%\fi
%----- end Orig
    \ifPst@shift@star%\typeout{==pstricks== old behaviour of the shift option}%     shift=*
      \advance\pst@dimd-\pst@dimb
      \pst@dimd=0.5\pst@dimd
    \else\pst@dimd-\pst@shift\fi
    \advance\pst@dimd\pst@dimb
    \lower\pst@dimd%
    \box\pst@hbox%
    \kern\pst@dimc}%
  \if@star\setbox\pst@hbox=\hbox{\clipbox@@\z@}\fi%
  \leavevmode\box\pst@hbox%
  \endgroup%
  \psset[pstricks]{shift=0}% reset value
}
%
\@namedef{pspicture*}{\pspicture*}
\@namedef{endpspicture*}{\endpspicture}
%
\ifx\pstcustomize\relax \input pstricks.con \fi
\catcode`\@=\PstAtCode\relax
%
\endinput
%%
%% END: pstricks.tex

